Towards Better Approximation of Graph Crossing Number

Graph Crossing Number is a fundamental problem with various applications. In this problem, the goal is to draw an input graph $G$ in the plane so as to minimize the number of crossings between the images of its edges. Despite extensive work, non-trivial approximation algorithms are only known for bounded-degree graphs. Even for this special case, the best current algorithm achieves a $\tilde O(\sqrt n)$-approximation, while the best current negative result is APX-hardness. All current approximation algorithms for the problem build on the same paradigm: compute a set $E'$ of edges (called a \emph{planarizing set}) such that $G\setminus E'$ is planar; compute a planar drawing of $G\setminus E'$; then add the drawings of the edges of $E'$ to the resulting drawing. Unfortunately, there are examples of graphs, in which any implementation of this method must incur $\Omega (\text{OPT}^2)$ crossings, where $\text{OPT}$ is the value of the optimal solution. This barrier seems to doom the only known approach to designing approximation algorithms for the problem, and to prevent it from yielding a better than $O(\sqrt n)$-approximation. In this paper we propose a new paradigm that allows us to overcome this barrier. We show an algorithm that, given a bounded-degree graph $G$ and a planarizing set $E'$ of its edges, computes another set $E''$ with $E'\subseteq E''$, such that $|E''|$ is relatively small, and there exists a near-optimal drawing of $G$ in which only edges of $E''$ participate in crossings. This allows us to reduce the Crossing Number problem to \emph{Crossing Number with Rotation System} -- a variant in which the ordering of the edges incident to every vertex is fixed as part of input. We show a randomized algorithm for this new problem, that allows us to obtain an $O(n^{1/2-\epsilon})$-approximation for Crossing Number on bounded-degree graphs, for some constant $\epsilon>0$.

==> RS_decomposition.tex <==

%\subsubsection{Graph Decomposition using Sparse Cuts}
%For a graph $G=(V(G),E(G))$ and an integer $\alpha$, we denote by $V_{\alpha}(G)\subseteq V(G)$ the subset of vertices with degree at least $\alpha$ in $G$, namely $V_{\alpha}(G)=\set{v\mid \deg_G(v)\ge \alpha}$. 
In this section we prove the following lemma.
\begin{lemma}
\label{lem:deco_wrt_high-deg_nodes}
There is an efficient algorithm, that, given a graph $G$ with $|E(G)|=\tilde{O}(\cro)$ and a parameter $\alpha=o(\cro)$, computes a subset $\hat{E}\subseteq E(G)$ of at most $\tilde O(|E(G)|\cdot \cro^{-\eps})$ edges, such that, in each connected component $C$ of the remaining graph $G\setminus \hat{E}$, for every pair $v,v'$ of vertices in that have degree at least $\alpha$ in $C$, there are $(\min\set{\deg_C(v),\deg_C(v')})/\cro^{\eps}$ edge-disjoint paths connecting them in $C$. Moreover, the number of connected components in $G\setminus \hat{E}$ is at most $O(|E(G)|/\alpha)$.
\end{lemma}


We now describe the algorithm. We say that a vertex $v$ is a \emph{high-degree} vertex in a subgraph $G'\subseteq G$, iff $\deg_{G'}(v)\ge \alpha$.
Throughout the algorithm, we maintain (i) a set $\tilde{E}$ of edges in $E(G)$, that is initialized to be $\emptyset$; and (ii) a collection $\cset$ of mutually node-disjoint subgraphs of $G$, that is initialized to be $\set{G}$. The algorithm proceeds in iterations.
%and continues to be executed iff there exists a subgraph $C\in \cset$ and a pair $v,v'$ of vertices in $V_{\alpha}(C)$ in $C$, such that the min-cut of $C$ separating $v$ and $v'$ contains no more than  $\alpha/\cro^{\eps}$ edges.
In an iteration, the algorithm computes, for each cluster $C\in \cset$, and for each pair of high-degree vertices in $C$, the minimum edge cut of $C$ separating them.
If for each cluster $C\in \cset$ and for each pair of high-degree vertices in $C$, the min-cut of $C$ separating them contains at least $\alpha/\cro^{\eps}$ edges, then the algorithm is terminated and output the current edge set $\tilde E$. Otherwise, we arbitrarily pick such a cluster $C\in \cset$ together with a pair $v,v'$ of high-degree vertices in $C$, such that the min-cut $(S,S')$ of $C$ separating $v$ and $v'$ contains no more than $(\min\set{\deg_C(v),\deg_C(v')})/\cro^{\eps}$ edges. We add all edges in this min-cut into $\tilde{E}$ and replace the cluster $C\in \cset$ by the clusters $C[S]$ and $C[S']$. This completes the description of an iteration, and also completes the description of the algorithm.

Denote by $\hat{E}$ the set $\tilde E$ at the end of the algorithm, and let $\hat\cset$ be the set of connected components of $G\setminus \hat{E}$.
It is clear that the number of high-degree nodes in $G$ is at most $O(|E(G)|/\alpha)$, and when the algorithm terminates, every connected component in $\hat\cset$ contains at least a vertex that is/was a high-degree vertex of $G$. Therefore, $|\hat{\cset}|=O(|E(G)|/\alpha)$.
On the other hand, it is clear from the algorithm that, for each $C\in \hat\cset$, and for every pair of high-degree vertices in $C$, there are $(\min\set{\deg_C(v),\deg_C(v')})/\cro^{\eps}$ edge-disjoint paths connecting them in $C$. Since in each iteration we add at least one edge to $\tilde E$, the algorithm terminates in polynomial time. 

It remains to bound the size of $\hat{E}$, which we do by a charging scheme as follows.
When in an iteration, we find a cut $(S,S')$ in $C$ (here we assume without loss of generality that $|E(S)|\le |E(S')|$) separating a pair $v,v'$ of high-degree vertices in $C$, we charge the edges in $E(S,S')$, the edges that is added into $\tilde E$ in this iteration, uniformly to the edges in $E(S)$.
Note that $|E(S)|\ge \alpha-O(\log n)\cdot \alpha/\cro^{\eps}=\alpha(1-o(1))$.
As a result, an edge is charged at most $O((\alpha/\cro^\eps)/\alpha)=O(\cro^{-\eps})$ every time.
Observe that each time an edge is charged, the size (the number of edges) of the cluster in $\cset$ that contains it shrinks by a constant factor. Therefore, each edge is charged at most $O(\log n)$ times. 
Therefore, the total charge throughout the algorithm is bounded by $|E(G)|\cdot O(\log n/\cro^{\eps})$, so the number of edges in $\hat{E}$ is $\tilde O(|E(G)|\cdot \cro^{-\eps})$.

%In the following steps, we will compute, for each cluster $C\in \hat{C}$, a drawing $\psi_C$. We will eventually combine all the drawings together and add back the edges in $\hat{E}$. From now on we focus on a specific cluster $C\in \hat\cset$.



==> RS_flipstatus.tex <==
\subsubsection{Refining The Rotation of High-Degree Vertices}
In this section we prove the following lemma.
\begin{lemma}
\label{lem:determine_flip_status}
There is an efficient randomized algorithm, that given
(i) a graph $G=(V,E)$ and a parameter $\alpha>\cro^{1/2+3\eps}$ such that, for each pair $v,v'$ of high-degree vertices, 
%(vertices that have degree at least $\alpha$ in $G$), 
there are $\alpha/\cro^{\eps}$ edge-disjoint paths connecting them in $G$; and
(ii) a rotation system $\Sigma$ on $G$, that contains, for each vertex $v\in V$, a semi-rotation $\set{\sigma_v,\sigma^f_v}$, such that $\optcro(G,\Sigma)=O(\cro)$;
computes, with probability $1-O(\cro^{-100})$, a rotation system $\tilde\Sigma$ that refines $\Sigma$, such that, for any drawing $\phi\in \Phi(G,\Sigma)$ with $\cro(\phi)=O(\cro)$, $\phi$ respects $\tilde\Sigma$ or $\tilde\Sigma^f$. In particular, $\tilde\Sigma$ contains, for each high-degree vertex $v\in V$, a rotation $\tilde{\sigma}_v\in \set{\sigma_v,\sigma^f_v}$. 
\end{lemma}

If $G$ does not contain any high-degree vertex, then we simply let $\tilde\Sigma=\Sigma$ and it is easy to verify that Lemma~\ref{lem:determine_flip_status} is true. If $G$ contains exactly one high-degree vertex $v$, then we simply let $\tilde{\Sigma}$ be obtained from $\Sigma$ by replacing the semi-rotation $\set{\sigma_v,\sigma^f_v}$ with any one rotation of them, and it is also easy to verify that Lemma~\ref{lem:determine_flip_status} is true.
From now on we consider the case where $G$ contains at least two high-degree vertices.

Let $v,v'$ be a pair of high-degree vertices of $G$.
First we compute a set of $\alpha/\cro^{\eps}$ in $G$ edge-disjoint paths connecting $v$ to $v'$, that we denote by $\pset$. We now apply Corollary~\ref{cor:finding_local_non_inf} to the set $\pset$ of paths. We let $\qset$ be the set of paths that we obtain, and let $\sigma$ be the cyclic order on the paths of $\qset$.
%We say that a path $Q\in \qset$ is \emph{bad} if it participates in at least $\cro^{1/2}$ crossings in $\phi$, namely $\cro_{\tphi'}(Q)\ge \cro^{1/2}$. Then the number of bad paths in $\qset$ is at most $\tilde O(\cro^{1/2})$. 
We let $\hat \qset\subseteq \qset$ be obtained by sampling each path from $\qset$ independently with probability $1/\cro^{1/2+\eps}$.
We use following observation.
\begin{observation}
With probability $1-O(n^{-100})$, the following is true for $\hat{\qset}$:
\begin{enumerate}
\item $|\hat \qset|%=\Omega(\alpha/(n^{2\eps}\cdot\cro^{1/2}))
		=\tilde\Omega(n^{\eps})$;
\item $\hat \qset$ contains no paths that participates in at least $\cro^{1/2}$ crossings in $\phi$; and
\item for each pair $\hat Q_1,\hat Q_2$ of paths in $\hat \qset$, such that $\sigma[\hat Q_1,\hat Q_2] \cap\hat{\qset}=\emptyset$, $|\sigma[\hat Q_1,\hat Q_2]|=\tilde\Omega(\cro^{1/2+\eps})$.
\end{enumerate}
\end{observation}
\begin{proof}
\end{proof}
\begin{corollary}
With probability $1-O(n^{-100})$, for each pair $\hat Q_1,\hat Q_2$ of paths in $\hat \qset$, $\cro_{\phi}(\hat Q_1,\hat Q_2)=0$.
\end{corollary}
%\begin{proof}\end{proof}

Therefore, if we fix the rotation of $v$, then the rotation of $v'$ is also fixed by the cyclic order $\sigma$ on the paths of $\hat{\qset}$.
%We remark that, even though the paths in $\hat\qset$ do not cross each other in $\phi$, a path in $\hat\qset$ may cross itself.
We now construct the rotation system $\tilde{E}$ as follows. First we arbitrarily pick a high-degree vertex $v\in V$, and fix the rotation $\tilde{\sigma}_v$ to be any rotation in the semi-rotation $\set{\sigma_v,\sigma^f_v}$.
Then, for every other high-degree vertex, we fix its rotation by the above process.
Now consider a drawing $\phi\in \Phi(G,\Sigma)$ with $\cro(\phi)=O(\cro)$. 
It is not hard to see that, if the cyclic ordering in which the image of edges in $\delta(v)$ enters the small disc around $\phi(v)$ is $\sigma_v$, then $\phi$ respects $\tilde{\Sigma}$, otherwise it respects $\tilde{\Sigma}^f$.


%Now since the flip status of $v$ is fixed, the induced flip status on the paths in $\hat\qset$ that enters $v$ is also fixed. Since all paths in $\hat{\qset}$ enters $v'$ and $|\hat\qset|\ge 3$, this also uniquely determines the flip status of $v'$.

==> RS_non_interfering.tex <==


\subsubsection{Obtaining Locally Non-Interfering Paths}

Let $G$ be a graph, let $P$ be a path in $G$, and let $v\in V(P)$ be a vertex of $P$. We denote by $P[v]$ the subpath of $P$ consisting of the edges in $P$ that are incident to $v$. Namely, if $P=(v_1,v_2,\ldots,v_k)$, then $P[v_1]=(v_1,v_2)$ and $P[v_k]=(v_{k-1},v_k)$, and for each $2\le i\le k-1$, $P[v_i]=(v_{i-1},v_i,v_{i+1})$.
For a set $\pset$ of paths in $G$ and a vertex $v$, we denote by $\pset_v\subseteq \pset$ the subset of paths that contain the node $v$, and we define $\pset[v]=\set{P[v]\mid P\in \pset_v}$, and define $G[\pset,v]$ be the subgraph of $G$ that contains all paths in $\pset[v]$. Therefore, $G[\pset,v]$ is a star graph with $v$ serving as the center of the star.
Given a rotation $\sigma_v$ on the edges of $\delta_G(v)$, we say that the set $\pset$ of paths is \emph{locally non-interfering at $v$ with respect to $\sigma_v$}, if the paths of $\pset[v]$ are non-interfering with respect to the unique planar drawing of $G[\pset,v]$ that respects $\sigma_v$.
%We consider a cluster $C\in \hat{\cset}$, and let $v,v'$ be two high-degree nodes in $C$ (assuming for now that it contains at least two high-degree nodes). Denote $d'=d/n^{\eps}=\Theta(n^{1/2-4\eps})$. From the last step, there are edge-disjoint paths $P_1,\ldots, P_{d'}$ in $C$ connecting $v$ to $v'$. Recall that we are also given a rotation system $\oset=\set{O_v\mid v\in V(\tG')}$ on $\tG'$. The following lemma shows that, given a set of edge-disjoint paths, we can efficiently transform it into a set of edge-disjoint paths that is locally non-interfering at all vertices of $\tG'$ with respect to their circular orderings in $\oset$.
We prove the following lemma.
\begin{lemma}
There exists an efficient algorithm, that, given a graph $G$, a rotation system $\Sigma$ on $G$ and a set $\pset$ of edge-disjoint paths connecting the same pair $v,v'$ of distinct vertices of $G$, computes another set $\pset'$ of edge-disjoint paths in $G$ connecting $v$ to $v'$, such that $E(\pset)=E(\pset')$, and $\pset'$ is locally non-interfering at all vertices of $G$ with respect to their rotations/semi-rotations in $\Sigma$.
\end{lemma}
\begin{proof}
\end{proof}

\begin{lemma}
\label{cor:finding_local_non_inf}
Given a graph $G$, a rotation system $\Sigma$ on $G$ and a set $\pset$ of edge-disjoint paths connecting the same pair $v,v'$ of distinct vertices of $G$, we can efficiently find (i) a set $\qset$ of $|\qset|=|\pset|$ edge-disjoint paths in $G$ connecting $v$ to $v'$ such that $E(\qset)=E(\pset)$; and (ii) a cyclic order $\sigma$ on the paths in $\qset$, such that, for any drawing $\phi\in \Phi(G,\Sigma)$ and any two paths $Q_1,Q_2\in \qset$, if $\cro_{\phi}(Q_1,Q_2)\ne 0$, then either for each $Q\in \sigma[Q_1,Q_2]$, we have $\cro_{\phi}(Q,Q_1\cup Q_2)\ne 0$, or for each each $Q\in \sigma[Q_2,Q_1]$, $\cro_{\phi}(Q,Q_1\cup Q_2)\ne 0$.
\end{lemma}


\paragraph{Regions.}
Let $G$ be a graph. Let $Q_1$ and $Q_2$ be two paths in $G$ connecting $v$ to $v'$.
Let $\Sigma$ be rotation system of $G$, such that $Q_1$ and $Q_2$ are locally non-interfering at all vertices of $G$ with respect to their rotation/semi-rotation in $\Sigma$. Let $\phi$ be a drawing respecting $\Sigma$ where $Q_1$ do not cross $Q_2$, and both $Q_1$ and $Q_2$ are non-blocking paths with respect to $\phi$.
We define the \emph{region} surrounded by the ordered pair $(Q_1, Q_2)$ as \znote{to do}, that we denote by $R_{\phi}(Q_1,Q_2)$. Please see Figure~\ref{fig:region} for an example.
\begin{figure}[h]
\label{fig:region}
\centering
\includegraphics[scale=0.4]{region}
%\subfigure[The left envelope is shown in purple, and the right envelope is shown in blue.]{\scalebox{0.3}{\includegraphics{left_right_paths}}}
\caption{An illustrations of region. $R_1$ is surrounded by the ordered pair $(P_1,P_2)$; $R_2$ is surrounded by the ordered pair $(P_2,P_3)$.} 
\end{figure}
The following observation is immediate.
\begin{observation}
Let $G$ be a graph and $\Sigma$ a rotation system on $G$. Let $\phi$ be a drawing of $G$. Let $Q$ and $Q'$ be two paths in $G$ connecting $v$ to $v'$ that are locally non-interfering at all vertices of $G$ with respect to their rotations/semi-rotations in $\Sigma$. If $\phi(Q)$ is a blocking curve, then $Q$ and $Q'$ cross in $\phi$.
\end{observation}








==> RS_prelim.tex <==

%\paragraph{Cyclic orders.} 
A \emph{cyclic order} $\sigma$ on a set $S=\set{s_1,\ldots,s_m}$ is an arrangement of the elements of $S$ on a cycle. 
%If the clockwise order of the elements in this arrangement is $s_1,s_2,\ldots,s_m,s_1$, then we write $s_1<_{\sigma} s_2<_{\sigma}\ldots<_{\sigma}s_m<_{\sigma}s_1$. 
If the element $s_k$ lies in the interior of the arc that starts at $s_i$ and goes clockwise to $s_j$, then we say that $s_k$ \emph{lies between $s_i$ and $s_j$} in the cyclic order $\sigma$. We denote by $\sigma[s_i,s_j]$ all elements of $S$ that lies between $s_i$ and $s_j$. Note that $s_i$ and $s_j$ do not belong to $\sigma[s_i,s_j]$.
%We define the \emph{inverse} (or \emph{flip}) $\sigma^{f}$ of $\sigma$ to be the cyclic order that the reverses the ordering of $\sigma$ of the elements of $S$ on the cycle. Clearly, $(\sigma^f)^f=\sigma$ and $s_k\in\sigma[s_i,s_j]$ iff $s_k\in\sigma^f[s_j,s_i]$.
Also note that, for each subset $S'\subseteq S$, any cyclic order $\sigma$ on $S$ naturally induces a cyclic order on $S'$.

%\paragraph{Rotations and rotation systems.}
Let $G=(V,E)$ be a graph and $v\in V$ be a vertex of $G$. 
A \emph{rotation} of $v$ is a cyclic order on $\delta(v)$.
%A \emph{semi-rotation} of $v$ is a set of two cyclic orders on $\delta_G(v)$, that are inverse of each other.
A \emph{rotation system} on graph $G$ is a set $\Sigma$ that contains, for each vertex $v\in V(G)$, a rotation $\sigma_v$ of $v$.
%For a rotation system $\Sigma$ on $G$, we defines its \emph{inverse} to be another rotation system $\Sigma^f$, that, for each vertex $v\in V$, if $\Sigma$ contains $\sigma_{v}$, then $\Sigma^f$ contains $\sigma^f_{v}$; if $\Sigma$ contains $\set{\sigma_{v},\sigma^f_{v}}$, then $\Sigma^f$ contains $\set{\sigma_{v},\sigma^f_{v}}$.
%For two rotation systems $\Sigma$ and $\tilde{\Sigma}$ on $G$, we say that $\tilde\Sigma$ \emph{refines} $\Sigma$ iff, for each vertex $v\in V$, one of the following two things happens: (i) $\tilde\Sigma$ contains a rotation $\tilde\sigma_{v}$ for $v$, and $\tilde\sigma_{v}\in \set{\sigma_{v},\sigma^f_{v}}$; or (ii) $\tilde\Sigma$ contains the semi-rotation $\set{\sigma_{v},\sigma^f_{v}}$ for $v$.
Let $\phi$ be a drawing of $G$.
We say that the drawing $\phi$ \emph{respects} the rotation system $\Sigma$ iff, for each vertex $v\in V(G)$, the image of the edges of $\delta(v)$ in $\phi$ enter the small disc around $\phi(v)$ in the same order as the rotation $\sigma_v$ (ignoring the orientation).
%or in the same order as a rotation $\sigma\in\set{\sigma_v, \sigma^f_v}$ of the semi-rotation of $v$. 
Given a rotation system $\Sigma$ on $G$, we denote by $\Phi(G,\Sigma)$ the set of drawings of $G$ that respects the rotation system $\Sigma$. 
%and denote $\optcro(G,\Sigma)=\min\set{\cro(\phi)\mid \phi\in \Phi(G,\Sigma)}$.
Note that, for a subgraph $G'\subseteq G$, the rotation system $\Sigma$ on $G$ naturally induces a rotation system $\Sigma'$ on $G'$. For a drawing $\phi\in \Phi(G',\Sigma')$, sometimes we also say that $\phi\in \Phi(G',\Sigma)$. We will use the following lemma, whose proof appears in Appendix~\ref{apd:proof_of_drawing_local_reodering}.
\begin{lemma}
\label{lem:drawing_local_reodering}
There is an efficient algorithm, that, given a graph $G=(V,E)$, a rotation system $\Sigma$ on $G$, and a drawing $\phi$ of $G$, computes a drawing $\phi'\in \Phi(G,\Sigma)$ such that $\cro(\phi')\le \cro(\phi)+\sum_{v\in V}\deg^2_G(v)$.
\end{lemma}

\iffalse
\begin{proof}
Given the input drawing $\phi$ of $G$,
we perform sequentially, for each vertex $v\in V$, a local adjustment step to the drawing, such that, after this step, the image of the edges of $\delta(v)$ in the current drawing enter $v$ in the same order as the rotation $\sigma_v$ of $v$ in $\Sigma$.
Therefore, after we perform the local adjustment steps for all vertices in $V$, the resulting drawing $\phi'$ respects the rotation system $\Sigma$.

It remains to describe a local adjustment step at $v$. If the image of the edges of $\delta(v)$ in the current drawing enter $v$ in the same order as the rotation $\sigma_v$, then we do nothing. Otherwise, we draw a small disc $D_v$ around $v$, and reorganize the ordering of image of the edges of $\delta(v)$ entring $v$ so that it coincides with $\sigma_v$, by letting each pair of edges in $\delta(v)$ cross at most once. Please see Figure~\ref{fig:loca_adjustment} for an illustration. It is clear that such a local adjustment step at $v$ introduce at most $\deg_G^2(v)$ new crossings. Therefore, the final drawing $\phi'$ contains at most $\cro(\phi)+\sum_{v\in V}\deg^2_G(v)$ crossings.
\begin{figure}[h]
\label{fig:loca_adjustment}
\centering
\subfigure[The local drawing at $v$ before the local adjustment.]{\scalebox{0.21}{\includegraphics{local_adjustment_1}}}
\hspace{0cm}
\subfigure[The rotation $\sigma_v$ of $v$ in $\Sigma$.]{\scalebox{0.21}{\includegraphics{local_adjustment_2}}}
\hspace{0cm}
\subfigure[The local drawing at $v$ after the local adjustment.]{\scalebox{0.21}{\includegraphics{local_adjustment_3}}}
\caption{An illustration of a local adjustment step.} 
\end{figure}
\end{proof}

\fi

\iffalse
\begin{figure}[h]
	\label{fig:region}
	\centering
	\includegraphics[scale=0.4]{region}
	%\subfigure[The left envelope is shown in purple, and the right envelope is shown in blue.]{\scalebox{0.3}{\includegraphics{left_right_paths}}}
	\caption{An illustrations of region. $R_1$ is surrounded by the ordered pair $(P_1,P_2)$; $R_2$ is surrounded by the ordered pair $(P_2,P_3)$.} 
\end{figure}

The following observation is immediate.
\begin{observation}
	Let $G$ be a graph and $\Sigma$ a rotation system on $G$. Let $\phi$ be a drawing of $G$. Let $Q$ and $Q'$ be two paths in $G$ connecting $v$ to $v'$ that are locally non-interfering at all vertices of $G$ with respect to their rotations/semi-rotations in $\Sigma$. If $\phi(Q)$ is a blocking curve, then $Q$ and $Q'$ cross in $\phi$.
\end{observation}

\fi



==> RS_recursion.tex <==

\paragraph{Recursion: Graph Decomposition via small cuts or bounding boxes.}
%Let $\alpha=\cro^{1-10\eps}$. We apply Lemma~\ref{lem:deco_wrt_high-deg_nodes} to $G'$ with parameter $\alpha$, and let $G''_1,\dots,G''_k$ be the graphs that we obtain. We now describe how to process one graph of $\set{G''_1,\dots,G''_k}$, and will process all other graphs in the same way. Consider the graph $G''_1$ and for brevity we rename it by $G''$. Note that if $G''$ does not contain a vertex of degree at least $\cro^{1-\eps}$, then we are in the recursion base case.
We now assume that there is at least one vertex $v\in V(G')$ with degree at least $\cro^{1-\eps}$ in $G'$, that we denote by $v$.
%We apply Lemma~\ref{lem:determine_flip_status} to $G''$, and let $\tilde\Sigma$ be the rotation system on $G''$ that we get.
We denote by $e_1,\ldots,e_r$ the edges incident to $v$ that are ordered according to the rotation $\sigma_v$ in $\Sigma$. 
Denote $E_1=\set{e_1,\ldots,e_{\floor{r/2}}}$ and $E_2=\set{e_{\floor{r/2}+1},\ldots,e_{r}}$. 
We first modify the graph $G'$, by replacing $v$ with two vertices, $v',v''$, where $v'$ is incident to all edges in $E_1$, and $v''$ is incident to all edges in $E_2$. Next, we compute the minimum edge-cut in $G'$ separating $v'$ from $v''$. Denote by $E'$ the set of edges in the cut. We distinguish between two cases, based on whether $|E'|$ is large or small.


\subsubsection{Case 1. $|E'|< \cro^{1-2\eps}$}
In this case, we let $G_1,G_2$ be the two subgraphs of $G'$ obtained by deleting the edges of $E'$ from it, with $v'\in G_1$ and $v''\in G_2$.
We then recurse on both $G_1$ and $G_2$. The sets of difficult edges and the associated drawings are defined in a natural way: for each $i\in \set{1,2}$, $\hat E(G_i)$ contains all edges of $\hat E(G')$ that lie in $G_i$, and the associated drawing $\phi'_{G_i}$ are simply the drawing of $G_i$ induced by $\phi'_{G'}$. %\snote{$\hat E(G')$ and $\phi'_{G'}$ are not defined yet}

Let $\psi_{G_1}$ ($\psi_{G_2}$, resp.) be the drawing of $G_1$ ($G_2$, resp.) that we obtain from the algorithm. We now describe how to produce a drawing $\psi_{G'}$ of $G'$ from $\psi_{G_1}$ and $\psi_{G_2}$.
%We go back to viewing $v$ as a single vertex of $G'$, so $V(G_1)\cap V(G_2)=\set{v}$. 
We first perform a stereographic projection from $v'$ to the drawing $\psi_{G_1}$, such that in the resulting drawing, which we denote by $\psi'_{G_1}$, the vertex $v'$ and its incident edges $e_1, e_{\lfloor r/2\rfloor}$ lie on the boundary of the outer face. Similarly, we obtain a new drawing $\psi'_{G_2}$ of $G_2$, where the vertex $v''$ and its incident edges $e_{\lfloor r/2\rfloor+1},e_r$ lie on the boundary of the outer face.
We now place the drawings $\psi'_{G_1}$ and $\psi'_{G_2}$ together by identifying the image of $v'$ in $\psi'_{G_1}$ and the image of $v''$ in $\psi'_{G_2}$, while guaranteeing that (i) the image of $G_1$ and $G_2$ intersect only at the image of $v=v'=v''$; and (ii) the cyclic ordering of the edges of $\set{e_1,\ldots,e_r}$ entering $v$ coincides with $\sigma_v$. We denote this drawing of $G_1\cup G_2$ by $\psi'$. We then add the edges of $E'$ back using the following lemma, whose proof is deferred to Appendix~\ref{apd:proof_of_add_back_discarded_edges}.
\begin{lemma}
\label{lem:add_back_discarded_edges}
Let $G=(V,E)$ be a graph, let $E'\subseteq E$ be a subset of its edges, let $\Sigma$ be a rotation system on $G$, and let $\phi'$ be any drawing of the subgraph $G\setminus E'$ that respects $\Sigma$.
% and every pair of edges in $E\setminus E'$ crosses at most once in $\phi'$. 
Then we can efficiently find a drawing $\phi$ of $G$ in the plane, such that (i) $\phi(G\setminus E')=\phi'$; (ii) $\phi$ respects $\Sigma$; and (iii) $\cro(\phi)\le \cro(\phi')+|E'|\cdot|E(G)|$.
\end{lemma}

We apply Lemma~\ref{lem:add_back_discarded_edges} to the graph $G'$, the edge set $E'$, the rotation system $\Sigma$ and the drawing $\psi'$ of $G'\setminus E'$.
Let $\psi_{G'}$ be the drawing of $G'$ that we obtain. From Lemma~\ref{lem:add_back_discarded_edges}, we get that
$$\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+\cro^{1-2\eps}\cdot |E(G')|.$$
We state the following immediate observation, that will be used for accounting in Section~\ref{subsec:accounting}.
\begin{observation}
\label{RS_obs:case_1}
In Case 1, $|E(G_1)|, |E(G_2)|\ge \cro^{1-\eps}/3$.
\end{observation}
\begin{proof}
Recall that the number of edges in $G'$ that are incident to $v'$ is at least $\cro^{1-\eps}/2$. Note that at most $\cro^{1-2\eps}$ of them belong to  $E'$, and the remaining of them lie in $G_1$. Therefore, $|E(G_1)|\ge \cro^{1-\eps}/3$. Similarly,
$|E(G_2)|\ge \cro^{1-\eps}/3$. 
\end{proof}



\subsubsection{Case 2. $|E'|\geq \cro^{1-2\eps}$}
In this case, we first compute a set $\tilde \pset$ of $\cro^{1-2\eps}$ edge-disjoint paths, that connect edges of $E_1$ to edges of $E_2$. 
Before we state the algorithm, we first introduce some new definitions.

\paragraph{Non-blocking curves, Envelopes and Regions.}
Let $\gamma$ be a curve in the plane, and denote by $x$ and $y$ the endpoints of $\gamma$. We say that $\gamma$ is \emph{non-blocking} iff there exists another curve $\gamma'$ in the plane connecting $x$ to $y$, that intersects $\gamma$ only at $x$ and $y$.
We view the curve $\gamma$ as directing from $x$ to $y$. We define the \emph{left envelope} (\emph{right envelope}, resp.) of a non-blocking curve $\gamma$ as the curve that starts from $x$ and ends at $y$, initially follows $\gamma$ immediately from the left (right, resp.) side of $\gamma$, and continues on the same side whenever encoutering a self-crossing of $\gamma$.
See Figure~\ref{fig:envelopes} for an example.
Let $P$ be a simple path in graph $G$ connecting $v$ to $v'$. Let $\phi$ be a drawing of $G$. 
%We say that $P$ is a \emph{non-blocking path with respect to $\phi$} iff $\phi(P)$ is a non-blocking curve. 
We will also refer to the \emph{left/right envelopes of $P$} as the left/right envelopes of the curve $\phi(P)$, if $\phi(P)$ is a non-blocking curve.
\begin{figure}[h]
	\label{fig:envelopes}
	\centering
	\subfigure[A non-blocking curve. The left envelope is shown in purple, and the right envelope is shown in blue.]{\scalebox{0.2}{\includegraphics{envelope}}}
	\hspace{0.5cm}
	\subfigure[A blocking curve connecting $x$ to $y$.]{\scalebox{0.18}{\includegraphics{blocking}}}
	\hspace{0.5cm}
	\subfigure[The region $R_1$ is surrounded by $(P_1,P_2)$, and the region $R_2$ is surrounded by $(P_2,P_3)$.]{\scalebox{0.22}{\includegraphics{region}}}
	\caption{An illustration of non-blocking curves and the region between non-blocking curves.} 
\end{figure}

Let $Q_1, Q_2$ be two paths originating from $v$ and terminating at $v'$.
%Let $\Sigma$ be rotation system of $G$, such that $Q_1$ and $Q_2$ are locally non-interfering at all vertices of $G$ with respect to their rotation/semi-rotation in $\Sigma$. 
Let $\phi$ be a drawing of $Q_1\cup Q_2$, such that $\phi(Q_1)$ and $\phi(Q_2)$ are both non-blocking curves.
We define the \emph{region} surrounded by the ordered pair $(Q_1, Q_2)$ as the set of all points in the plane, such that there exists a curve starting from the right envelope of $Q_1$, ending at the left envelope of $Q_2$, containing this point, and not intersecting the image of $Q_1$ and $Q_2$. 
We denote this region by $R_{\phi}(Q_1,Q_2)$. See Figure~\ref{fig:envelopes} for an illustration.

The remainder of the proof consists of three steps. In the first step, we pre-process the paths in $\tilde\pset$ to obtain a new set $\qset$ of paths that has some nice properties, which we will elaborate later. In the second step, we sample three paths from $\qset$ in a certain way, and show that, with high probability, the three paths do not cross each other in $\tphi$, and the number of edges whose image intersect the region surrounded by the first and the third path are small. In the third step, we use the region to decompose $G$ into smaller subgraphs and recurse on each of them. We now describe each of the steps in detail.


\subsubsection*{Step 1. Pre-processing the Path Set}
Let $\pset$ be a set of paths. We denote $E(\pset)=\bigcup_{P\in \pset}E(P)$.
Let $G$ be a graph and let $\phi$ be a drawing of $G$. We say a pair $G_1,G_2$ of disjoint subgraphs \emph{cross} in $\phi$, iff there is an edge $e_1\in G_1$ and another edge $e_2\in G_2$, such that the image of $e_1$ intersects the image of $e_2$ in $\phi$.
We use the following lemma, whose proof is deferred to Appendix~\ref{apd:proof_of_finding_local_non_inf}.

\begin{lemma}
	\label{cor:finding_local_non_inf}
	Given a graph $G$, a rotation system $\Sigma$ on $G$ and a set $\tilde\pset$ of edge-disjoint paths connecting the same pair $v,v'$ of distinct vertices of $G$, we can efficiently find (i) a set $\pset$ of $|\pset|=|\tilde\pset|$ edge-disjoint paths in $G$ connecting $v$ to $v'$ such that $E(\pset)\subseteq E(\tilde\pset)$; and (ii) a cyclic order $\sigma$ on the paths in $\pset$, such that, for any drawing $\phi\in \Phi(G,\Sigma)$ and any two paths $P_1,P_2\in \pset$, if $P_1$ and $P_2$ cross in $\phi$, then either every path in $\sigma[P_1,P_2]$ crosses $P_1\cup P_2$ in $\phi$, 
	or every path in $\sigma[P_2,P_1]$ crosses $P_1\cup P_2$ in $\phi$.
\end{lemma}
We apply Lemma~\ref{cor:finding_local_non_inf} to the set $\tilde \pset$ of paths connecting the edges of $E_1$ to the edges of $E_2$, and denote by $\pset$ the set of paths that we obtain. 
We say that a path in $\pset$ is \emph{long} if it contains at least $10\cro^{2\eps}$ edges. Therefore, the number of long paths in $\pset$ is at most $\cro^{1-2\eps}/10$.
%\snote{why? What happens if $\pset$ has more than $\cro$ edges?}.
Let $\beta=\cro^{1-2\eps}/100$. We say that a path in $\pset$ is \emph{marginal} if contains an edge from the set
$\set{e_1,\ldots, e_{\beta}}
\cup
\set{e_{\lfloor r/2 \rfloor-\beta},\ldots, e_{\lfloor r/2 \rfloor+\beta}}
\cup
\set{e_{r-\beta},\ldots,e_{r}}$.
Therefore, the number of marginal paths in $\pset$ is at most $\cro^{1-2\eps}/25$.
We discard all long paths and marginal paths from $\pset$, and let $\qset\subseteq\pset$ be the resulting set of paths, so $|\qset|\ge \cro^{1-2\eps}/3$. 
Recall that we also obtain a cyclic order on the paths of $\pset$. This cyclic order naturally induces a cyclic order  on the paths of $\qset$, that we denote by $\sigma$.

\iffalse
We now go back to viewing $v$ as a single vertex, but we still view the paths in $\qset$ as originating from some edge in $E_1$ and terminating at some edge in $E_2$.
For a pair $\hat Q_1, \hat Q_2$ of paths of $\qset$ that are locally non-interfering at $v$, with $\hat Q_1$ ($Q_2$, resp.) originating at $\hat e_1$ ($\hat e_2$, resp.)  and terminating at ($\hat e'_2$, resp.),
we say that the ordered pair $(\hat Q_1, \hat Q_2)$ \emph{well-separates} $v$ iff $|\tilde\sigma_v[\hat e'_1,\hat e_1]|=\Omega(\cro^{1-3\eps})$ and $|\tilde\sigma_v[\hat e_2,\hat e'_2]|=\Omega(\cro^{1-3\eps})$. Intuitively, if we delete all edges in $\tilde\sigma_v[\hat e_1,\hat e_2]$ and all edges in $\tilde\sigma_v[\hat e'_2,\hat e'_1]$, then the remaining edges in $\delta(v)$ is partitioned into two consecutive segments of at least $\Omega(\cro^{1-3\eps})$ paths each. Please see Figure~\ref{fig:separate} as an example.
\begin{figure}[h]
\label{fig:separate}
\centering
\includegraphics[scale=0.4]{left_right_paths}
\caption{An illustration of $Q$, $Q_L$ and $Q_R$.} 
\end{figure}\fi

\subsubsection*{Step 2. Constructing a $3$-Path Skeleton}
We choose a path $Q$ uniform at random from $\qset$.
Let $Q_R$ ($Q_L$, resp.) be the $(100\cro^{4\eps})$th path clockwise (anti-clockwise, resp.) from $Q$ in $\qset$ with respect to $\sigma$.
We denote $K=Q\cup Q_L\cup Q_R$, and call $K$ the \emph{skeleton} of $\qset$. We use the following claim.
\begin{claim}
\label{clm:skeleton}
With probability $1-O(\cro^{-2\eps})$, the following is true:
\begin{enumerate}
%\item\label{P1} the pair $(Q_L,Q_R)$ of paths well-separates $v$;
\item\label{P2} the skeleton $K$ participates in at most $\cro^{4\eps}$ crossings in $\tphi$; as a corollary, the paths in $K$ do not cross each other in $\tphi$, and their image are non-blocking curves in $\tphi$;
\item\label{P3} the number of edges that are incident to $(V(Q_L)\setminus V(Q_R))\cup (V(Q_R)\setminus V(Q_L))$ is at most $\cro^{1/2+8\eps}$.
\end{enumerate}
\end{claim}
\begin{proof}
We first prove property~\ref{P2}. Note that, the number of paths in $\qset$ that is crossed at least $\cro^{4\eps}/3$ times in $\tphi$ is at most $O(\cro^{1-4\eps})$. Therefore, the probability that one of $Q_L,Q,Q_R$ is crossed $\cro^{4\eps}/3$ times is at most $O(\cro^{-2\eps})$, and the probability that~\ref{P2} does not hold is $O(\cro^{-2\eps})$.
Assume now~\ref{P2} holds.
Note that, if a pair of paths from $K$ crosses in $\tphi$, from Lemma~\ref{cor:finding_local_non_inf}, at least $100\cro^{4\eps}$ paths from $\qset$ have to cross at least one of the paths in this pair. Therefore, at least one of the paths is crossed $50\cro^{4\eps}$ times in $\tphi$, this contradicts~\ref{P2}. 
On the other hand, if the image of a path in $K$ is a blocking curve, then it has to cross all paths in $\qset$ in $\tphi$, which makes it participate in at least $\Omega(\cro^{1-2\eps})$ crossings, again causing a contradiction to~\ref{P2}. Therefore, the image of paths in $K$ are non-blocking curves.


Now we prove property~\ref{P3}.
Denote $\qset=\set{Q_1,\ldots,Q_k}$. Let $r=200\cro^{4\eps}$.
We fix a vertex $u$ in the graph $G'$ that is not $v',v''$, and we will analyze the number of paths $Q_i$ in $\qset$ such that $u\in V(Q_i)\setminus V(Q_{i+r})$.

First we construct a sequence of indices as follows.
We say that an index $i$ is $u$-good if $u\in V(Q_i)\setminus V(Q_{i+r})$.
We find the smallest index $i_1\ge 1$ that is $u$-good. Then, for each $j>1$, assuming $i_1,\ldots,i_{j-1}$ are already defined, we let $i_j$ be the smallest $u$-good index that satisfies (i) $i_j\ge i_{j-1}+r$; and (ii) there exists $i_{j-1}< i^*< i_j$, such that $u\notin V(Q_{i^*})$. We continue this process to augment the sequence it cannot be augmented anymore. Let $I_u=(i_1,\ldots,i_{s})$ be the final sequence we get. We claim that $s\le  O(\cro^{1/2})$. To see why this is true, we assume the contrast that $s>30\cro^{1/2}$. For each $10\cro^{1/2}\le t\le 20\cro^{1/2}$, let $i^*_t$ be an index such that $i_t<i^*_t<i_{t+1}$ and $u\notin V(Q_{i^*_t})$. Note that the existence of such indices are guaranteed by our process of constructing the sequence $I_u$. Therefore, since each path in $\qset$ connects $v$ to $v'$, it is not hard to see that, each path in $\set{Q_{i^*_{t}}\mid 10\cro^{1/2}\le t\le 20\cro^{1/2}}$ will have to cross each path in $\set{Q_{i_{r}}\mid 1\le r\le 10\cro^{1/2}}$. This creates at least $100\cro$ crossings in $G'$, leading to a contradiction.
On the other hand, it is not hard to see that, the number of $u$-good indices in $\set{1,\ldots,k}$ is $O(s\cdot\cro^{4\eps})=O(\cro^{1/2+4\eps})$. Therefore, the probability that a random index $i$ is $u$-good is $O(\cro^{6\eps-1/2})$.

Now, for an edge $e=(u_1,u_2)$ where none of $u_1,u_2$ is $v$, for the edge to be incident to a vertex in $V(Q_i)\setminus V(Q_{i+r})$, $i$ has to be either $u_1$-good or $u_2$-good. Therefore, under the random choice of $i$, the probability that a specific edge is incident to a vertex in $V(Q_i)\setminus V(Q_{i+r})$ is at most $O(\cro^{6\eps-1/2})$. Therefore, the expected number of edges in $G'$ that are incident to a vertex in $V(Q_i)\setminus V(Q_{i+r})$, under a random choice of $i$, is at most $O(\cro^{1/2+6\eps})$. By Markov's bound, with probability $1-O(\cro^{-2\eps})$, this number is below $O(\cro^{1/2+8\eps})$.
\end{proof}

The next claim is crucial for further steps of the algorithm.
\begin{claim}
\label{clm:region_intersection}
With probability $1-O(\cro^{-2\eps})$, the number of edges in $G'$ whose image in $\tphi$ intersect the interior of the region $R_{\tphi}(Q_L,Q_R)$ 
is at most $O(\cro^{8\eps})$.
\end{claim}
\begin{proof}
Denote $\qset=\set{Q_1,\ldots,Q_k}$, where the paths are ordered with respect to $\sigma$. 
We first construct a graph $H$ as follows. The vertex set of $H$ is $\set{u_1,\ldots,u_k}$. There is an edge between the pair $u_i, u_j$ of vertices in $H$ iff (i) $|i-j|>\cro^{4\eps}$; and (ii) $Q_i$ and $Q_j$ crosses in $\tphi$.
We compute the maximum matching $M$ in $H$, and we claim that $|M|\le O(\cro^{1-4\eps})$. To see why this is true, on the one hand, from Lemma~\ref{cor:finding_local_non_inf}, if $(u_i,u_j)\in E(H)$, then at least one of $Q_i$ and $Q_j$ participates in at least $\cro^{4\eps}/2$ crossings in $\tphi$. On the other hand, the number of paths in $\qset$ that participate in at least $\cro^{4\eps}/2$ crossings is at most $O(\cro^{1-4\eps})$.
We denote by $U$ the set of endpoints of the edges in $M$, and define $\qset_U=\set{Q_i\mid u_i\in U}$. Therefore, we have  $|\qset_U|=O(\cro^{1-4\eps})$. We partition the paths in $\qset\setminus\qset_U$ into $\Omega(\cro^{1-8\eps})$ groups, where each group contains $\cro^{6\eps}$ consecutive paths with respect to $\sigma$, and there are $2\cro^{4\eps}$ paths between every consecutive pair of groups. %Note that this partition can be naturally extended to a partition of $\qset$. 
The paths that are the first path or the last path with respect to $\sigma$ of a group are called \emph{boundary} paths.
The following two observsations are immediate.
\begin{observation}
Boundary paths do not cross each other in $\tphi$.
\end{observation}
\begin{observation}
With probability $1-O(\cro^{-2\eps})$, the paths of $K$ are contained in the same group.
\end{observation}
Observe that, for each group in the partition, its boundary paths surround a region in the drawing $\tphi$. Let $\rset$ be the set of such regions, then the regions in $\rset$ are disjoint in their interior.
Note that, if an edge intersects with $t>1$ different regions, then it participates in at least $t$ crossings. Therefore, the total number of pairs of $(e,R)$ where $R$ is a region in $\rset$ and the edge $e$ intersect with the interior of region $R$ is at most $\cro$.
As a corollary of above two observations, with probability $1-O(\cro^{-2\eps})$, the number of edges whose image intersect the interior of the region $R_{\tphi}(Q_L,Q_R)$ is at most $O(\cro^{8\eps})$.
\end{proof}


\subsubsection*{Step 3. Graph Decomposition using the $3$-Path Skeleton}
If we go back to viewing $v$ as a single vertex, so $Q, Q_L, Q_R$ are actually directed cycles that contain the vertex $v$.
Denote by $\tilde e_L$ the out-edge of $v$ on $Q_L$, and by $\tilde e'_L$ the out-edge of $v$ on $Q'_L$. The edges $\tilde e_R$ and $\tilde e_R$ are defined similarly. 
Denote $E_L=\sigma_v[\tilde e'_{L}, \tilde e_{L}]$ and $E_R=\sigma_v[\tilde e_{R}, \tilde e'_{R}]$, so $|E_L|,|E_R| \ge \Omega(\cro^{1-2\eps})$.
Denote by $\tilde E$ the set of edges whose image in $\tphi$ intersect the interior of the region $R_{\tphi}(Q_L,Q_R)$. Note that the set $\tilde E$ is unknown to the algorithm.
We consider the following two cases.

\subsubsection*{Case 2.a. $V(Q_L)\cap V(Q_{R})=\set{v}$.}
Note that, if we delete all edges in $\tilde E$, the edges in $E'$ are separated from the edges in $E''$. Therefore, the min-cut in $G'$ separating $E'$ from $E''$ contains at most $O(\cro^{8\eps})$ edges.
We compute the min-cut in $G'$ separating $E'$ from $E''$, and let $(S,\bar S)$ be the cut we get. 
We denote $E^*=E_{G'}(S,\bar{S})$, so $|E^*|=O(\cro^{8\eps})$. We recurse on smaller graphs $G_1=G'[S]$ and $G_2=G'[\bar{S}]$, with respect to the induced rotation systems on them, respectively.
The set $\hat E(G_1)$ of difficult edges is simply defined to be $\hat{E}(G')\cap E(G_1)$, and the drawing $\phi'_{G_1}$ is defined to be the drawing of $G_1$ induced by $\phi'_{G'}$. The set $\hat{E}(G_2)$ and the drawing $\phi'_{G_2}$ are defined similarly.

Let $\psi_{G_1}$ ($\psi_{G_2}$, resp.) be the drawing of $G_1$ ($G_2$, resp.) that we obtain from the algorithm. We now describe how to produce a drawing $\psi_{G'}$ of $G'$ from $\psi_{G_1}$ and $\psi_{G_2}$. We do the same as in Case 1.
Specifically, we first perform a stereographic projection from $v$ to the drawings $\psi_{G_1}$ and $\psi_{G_2}$, and then place the drawings $\psi'_{G_1}$ and $\psi'_{G_2}$ together by identifying the image of $v$ in both drawings, while guaranteeing that (i) the image of $G_1$ and $G_2$ intersect only at $v$; and (ii) the cyclic ordering of the edges of $\set{e_1,\ldots,e_r}$ entering $v$ coincides with $\sigma_v$. We denote this drawing of $G_1\cup G_2$ by $\psi'$.
We then add the edges of $E^*$ back to the drawing $\psi'$ by applying Lemma~\ref{lem:add_back_discarded_edges} to the graph $G'$, the edge set $E^*$, the rotation system $\Sigma$ and the drawing $\psi'$ of $G'\setminus (E^*)$.
Let $\psi_{G'}$ be the drawing of $G'$ that we obtain. From Lemma~\ref{lem:add_back_discarded_edges}, we get that $\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+O(\cro^{8\eps}\cdot |E(G')|)$.
We state the following immediate observation, that will be used for accounting in Section~\ref{subsec:accounting}.
\begin{observation}
\label{RS_obs:case_2.1}
In Case 2.1, $|E(G_1)|, |E(G_2)|\ge \Omega(\cro^{1-2\eps})$.
\end{observation}



\subsubsection*{Case 2.b. $V(Q_L)\cap V(Q_{R})\ne \set{v}$.}
In this case we define the set $E^*$ to be the union of (i) all edges incident to vertices of $V(Q_L)\setminus V(Q_{R})$ and all edges incident to vertices of $V(Q_R)\setminus V(Q_{L})$; 
and (ii) all edges incident to vertices in $V(Q_L)\cap V(Q_R)$ whose degree is at most $\cro^{1-6\eps}$ in $G'$.
Recall that there are at most $\cro^{1/2+8\eps}$ edges of the first type.
On the other hand, since the paths $Q_L, Q_R$ are short, there are at most $O(\cro^{2\eps})\cdot \cro^{1-6\eps}\le O(\cro^{1-3\eps})$ edges of the second type. Therefore, $|E^*|=O(\cro^{1-3\eps})$ as $\eps\le 1/22$.
Let $\tilde V$ be the set of the remaining nodes of $V(Q_L)\cap V(Q_R)$, which we will call \emph{significant} nodes. Recall that we view the simple paths $Q_L$ and $Q_R$ as originating from an edge of $E_1$ and terminating at an edge of $E_2$. We prove the following observation.
\begin{claim}
\label{clm:left_right_envelope}
With probability $1-O(\cro^{-2\eps})$, all significant vertices appear on both the left and the right envelopes of the image of $Q_L$, and also both the left and the right envelopes of the image of $Q_R$ in $\tphi$.
\end{claim}
\begin{proof}
We say that a vertex $u$ is a \emph{high-degree} node iff its degree in $G'$ is at least $\cro^{1-6\eps}$, so each significant node is a high-degree node, and the number of high-degree nodes is $O(\cro^{7\eps})$.
For each high-degree node $u$, we denote by $\qset_u$ the set of paths in $\qset$ that contains $u$, and call the leftmost $100\cro^{2\eps}$ paths and the rightmost $100\cro^{2\eps}$ paths in $\qset_u$ \emph{bad paths}. Therefore, the number of bad paths in $\qset$ is at most $O(\cro^{9\eps})$.
We prove the following observation.
\begin{observation}
If both $Q_L$ and $Q_R$ are not bad paths, then all significant nodes appear on both the left and the right envelopes of the image of $Q_L$, and also both the left and the right envelopes of the image of $Q_R$ in $\tphi$.
\end{observation}
\begin{proof}
Assume the contrast that there is a significant node $u$, such that $u$ does not appear on the left envelope of $Q_L$, then at most $O(\cro^{2\eps})$ of $\qset$ to the left of $Q_L$ may contains the vertex of $u$. This is because each such path will has to cross $Q_L$, and $Q_L$ is crossed $O(\cro^{2\eps})$ times. Therefore, $Q_L$ has to be a bad path, causing a contradiction.
\end{proof}

From the above observation, and the fact that $\eps\le 1/13$, the probability that one of $Q_L$ and $Q_R$ is a bad path is at most $O(\cro^{9\eps}/\cro^{1-2\eps})\le O(\cro^{-2\eps})$. The claim then follows.
\end{proof}
\begin{corollary}
All significant vertices appear on both the left and the right envelopes of the image of $Q$ in $\tphi$, and the orders of appearance of them are the same on $Q_L$, $Q_R$ and $Q$.
\end{corollary}

In the remainder of this step, we use the skeleton $K$ to decompose the graph $G'$.
For each significant node $u$, we denote by $e^L_{in}(u)$ its in-edge on the path $Q_L$, denote by $e^L_{out}(u)$ its out-edge on the path $Q_L$, and denote $E_L(u)=\sigma_u[e^L_{out}(u),e^L_{in}(u)]$. 
Similarly, we denote by $e^R_{in}(u)$ its in-edge on the path $Q_R$, denote by $e^R_{out}(u)$ its out-edge on the path $Q_R$, and denote $E_R(u)=\sigma_u[e^R_{in}(u),e^R_{out}(u)]$. See Figure~\ref{fig:boundary_contract} for an illustration. 

We now delete from $G'$ all edges of $E^*$ and the edge of the paths in $K$ (but keep their vertices), and denote by $G''$ the remaining graph. Recall that $\tilde V$ is the set of significant nodes. Note that, if we further delete all edges in $\tilde E$, then the edges in $\tilde E_1=E_L\cup \left(\bigcup_{u\in \tilde V}E_L(u)\right)$ are separated from the edges in $\tilde E_2=E_R\cup \left(\bigcup_{u\in \tilde V}E_R(u)\right)$. We compute the minimum edge-cut in $G''$ separating the edges of $\tilde E_1$ from the edges of $\tilde E_2$, and denote by $(S,\bar{S})$ the cut we get, where $S$ contains all edges in $E_1$, so $E_{G'}(S,\bar{S})\le |E^*|+|E(K)|=O(\cro^{1-3\eps})$. Denote $G'_1=G''[S]\cup Q_L$ and $G'_2=G''[\bar S]\cup Q_R$. We perform a \emph{skeleton-contraction} step to the graphs $G'_1$ and $G'_2$ as follows.
We contract the paths on $Q_L$ in $G'_1$ into a single node, that we denote by $v_L$, and denote by $G_1$ the resulting graph, so now the set of edges incident to $v_L$ in $G_1$ is $\tilde E_1$. Note that the rotation system $\Sigma$ on $G$ naturally induces a rotation for each node of $V(G_1)\setminus\set{v_L}$. We define the rotation of $v_L$ as the cyclic concatenation of the edges of $E_L(u_1), E_L(u_2),\ldots, E_L$, where $u_1,u_2,\ldots$ are the significant nodes that are ordered according to their appearance on $Q_L$. We denote by $\Sigma_1$ the rotation system on $G_1$ that we defined this way.
We perform a similar skeleton-contraction operation to $G'_2$ and obtain a new graph $G_2$. We also define the rotation system $\Sigma_2$ on $G_2$ similarly. See Figure~\ref{fig:boundary_contract} for an illustration.
Now we recurse on smaller graphs $G_1$ and $G_2$, with rotation systems $\Sigma_1$ and $\Sigma_2$, respectively.
\begin{figure}[h]
	\label{fig:boundary_contract}
	\centering
	\subfigure[The layout of $Q_L\cup Q_R$ and the edges incident to nodes in $\tilde V$.]{\scalebox{0.36}{\includegraphics{boundary_contract_1}}}
	%\hspace{0.2cm}
	\subfigure[The rotations on $v_L$ and $v_R$.]{\scalebox{0.30}{\includegraphics{boundary_contract_2}}}
	\caption{An illustration of the skeleton-contraction step.} 
\end{figure}

It remains to define the sets $\hat{E}(G_1)$, $\hat{E}(G_2)$ of difficult edges  for graphs $G_1$ and $G_2$, and the drawings $\phi'_{G_1}$ and $\phi'_{G_2}$ with the desired properties. We now define $\hat{E}(G_1)$ and $\phi'_{G_1}$, and $\hat{E}(G_2)$ and $\phi'_{G_2}$ are defined similarly.
Consider again the graph $G'_1$, the graph before we contracted $Q_L$ into a single vertex. Consider the drawing of $G'_1$ induced by the drawing $\phi'_{G'}$ of the current graph $G'$. If all vertices and edges of $G'_1$ are drawn inside the region in $\phi'_{G'}$ surrounded by the left envelope of $Q_L$, that we denote by $F$, then we simply contract the image of $Q_L$ into a single vertex, let the resulting drawing be $\phi'_{G_1}$ and set $\hat{E}(G_1)$ be  $(\hat{E}(G')\cap E(G_1))\cup (\tilde E\cap E(G_1))$.
Clearly, $\cro(\phi'_{G_1})\le \cro_{\phi'_{G'}}(G_1)$.  
Now we consider the case where some subset $X$ of vertices of $G'_1\setminus Q_L$ is drawn outside $F$. Let $Y=V(G'_1\setminus Q)\setminus X$. Notice that, if $e$ is an edge connecting a vertex $w$ of $Q_L$ to a vertex of $G'_1\setminus Q_L$, then as $e$ leaves $w$, it is drawn inside $F$, but later it may cross the boundary of $F$. Therefore, if we delete all edges in $E(X\cup V(Q_L),Y)$, then $X$ becomes disconnected from both $Y$ and $Q_L$. Moreover, every edge in $E(X\cup V(Q_L),Y)$ must cross intersect with the region $R_{\tphi}(Q_L,Q_R)$. Therefore, the number of edges in $E(X\cup V(Q),Y)$ is at most $O(\cro^{6\eps})$. 
So we simply move the drawing of $X$ to lie inside $F$, and then add the edges of $E(X\cup V(Q_L),Y)$ to the current drawing using Lemma~\ref{lem:add_back_discarded_edges}. The edges of $E(X\cup V(Q_L),Y)$ become difficult edges for $G_1$. Additionally, every edge $e\in \hat{E}(G')$ that was difficult to $G'$ remains difficult for $G_1$.
This gives us the desired drawing $\phi'_{G_1}$ of $G_1$. It is not hard to see that, if $e,e'$ is a pair of edges that cross in the drawing $\phi'_{G_1}$, the either $e,e'$ cross in the original drawing $\tphi$ of $\tG$, or at least one of them is a difficult edge.

Let $\psi_{G_1}$ ($\psi_{G_2}$, resp.) be the drawing of $G_1$ ($G_2$, resp.) that we obtain from the algorithm. We now describe how to produce a drawing $\psi_{G'}$ of $G'$ from $\psi_{G_1}$ and $\psi_{G_2}$. 
We first perform a stereographic projection from $v_L$ to the drawings $\psi_{G_1}$, so that after this projection the image of $v_L$ lies on the outer face. Then we uncontract $v_L$ back to the path $Q_L$ in the outer face, where for each $u\in \tilde V$, the edges incident to $u$ are $E_L(u)$. In this way we obtain a drawing of $G'_1$, that we denote by $\phi'_{G'_1}$.
We do the same to $G_2$ and obtain a drawing $\phi'_{G'_2}$ of $G'_1$.
Then we place the drawings $\psi'_{G'_1}$ and $\psi'_{G'_2}$ together by identifying the image of corresponding significant nodes in both drawings, while guaranteeing that (i) the image of $G_1$ and $G_2$ intersect only at $v$ and the significant nodes; and (ii) the cyclic ordering of the edges of $\set{e_1,\ldots,e_r}$ entering $v$ coincides with $\sigma_v$. We denote this drawing of $G'_1\cup G'_2$ by $\psi'$.
We then add the edges of $E^*$ back to the drawing $\psi'$ by applying Lemma~\ref{lem:add_back_discarded_edges} to the graph $G'$, the edge set $E^*$, the rotation system $\Sigma$ and the drawing $\psi'$ of $G'\setminus (E^*)$.
Let $\psi_{G'}$ be the drawing of $G'$ that we obtain. From Lemma~\ref{lem:add_back_discarded_edges}, we get that $\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+O(\cro^{1-3\eps}\cdot |E(G')|)$. This completes the description of the whole algorithm.

We state the following immediate observation, that will be used for accounting in Section~\ref{subsec:accounting}.
\begin{observation}
\label{RS_obs:case_2.2}
In Case 2.2, $|E(G_1)|, |E(G_2)|\ge \Omega(\cro^{1-2\eps})$.
\end{observation}
















==> acceptable-clusters-correct.tex <==
\section{High-Level Overview}
\label{sec:overview}

In this section we provide a high-level overview of the proofs of our main results, and state the main theorems from which the proof is inferred. 
As in previous work, we start by considering a special case where the input graph $G$ is $3$-connected. This special case seems to capture the main technical challenges of the whole problem, and the extension to non-$3$-connected graphs is relatively easy and follows the same framework as in previous work \cite{chuzhoy2011graph}.
We start by defining several central notions that our proof uses.


%\mynote{An explanation why the things are set up this way and not the way we discussed. Our plan was to define an acceptable cluster like this:  a type-1 acceptable cluster has $\poly\log n$ terminals. A type-2 acceptable cluster is $3$-connected, good (no path connecting terminals lying on different faces), and terminals are well-linked. To get a planarizing set $\hat E$ of edges so that in $H=G\setminus \hat E$ every cluster is acceptable, we would follow these 3 steps:
%(1) make all clusters good, under a suitable definition of good.
%(2) do a well-linked decomposition.
%(3) cut-off 2-cuts to get 3-connected components.
%However, the third step does not actually work. If we start cutting off 2-vertex cuts we may end up creating new 2-vertex cuts that weren't there before. So type-2 acceptable clusters need to be defined differently. We need to allow to add fake edges that will replace the 2-vertex cuts we cut off, and the cluster itself with the fake edges should be 3-connected. This motivates the setup in this section.}



%\subsection*{Special Case: Input Graph $G$ is $3$-Connected}
		


\subsection{Acceptable Clusters and Decomposition into Acceptable Clusters}
In this section we define acceptable clusters and decomposition into acceptable clusters. These definitions are central for all our results. 
Let $G$ be an input graph on $n$ vertices of maximum degree at most $\Delta$; we assume that $G$ is $3$-connected. Let $\hat E$ be any planarizing set of edges for $G$, and let $H=G\setminus \hat E$. Let $\Gamma\subseteq V(G)$ be the set of all vertices that serve as endpoints of edges in $\hat E$; we call the vertices of $\Gamma$ \emph{terminals}. We will define a set $A$ of \emph{fake edges} -- a collection of edges $(x,y)$, where $x,y\in \Gamma$. We note that the edges of $A$ do not necessarily lie in $H$ or in $G$; in fact we will use these edges in order to augment the graph $H$. 

We denote by $\cset=\cset(H\cup A)$ the set of all connected components of $H\cup A$, and we call them \emph{clusters}.  For every cluster $C\in \cset$, we denote by $\Gamma(C)=\Gamma\cap V(C)$ the set of terminals that lie in $C$. We also denote by $A_C=A\cap C$ the set of all fake edges that lie in $C$.

%Next, we define some desirable properties of these clusters. 


\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-1 acceptable cluster} iff:
	
	\begin{itemize}
		\item $A_C=\emptyset$; and
		\item  $|\Gamma(C)|\leq \mu$ for $\mu=512\Delta\alphasc(n)\log_{3/2} n=O(\Delta\log^{1.5}n)$  (recall that $\alphasc(n)=O(\sqrt{\log n})$ is the approximation factor of the algorithm $\algsc$ for the sparsest cut problem).
	\end{itemize}
\end{definition}




\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-2 acceptable cluster} if the following conditions hold:
	
	\begin{itemize}
		\item {\bf (3-Connectivity):} $C$ is a simple $3$-connected planar graph, or it is isomorphic to $K_3$. In particular, $C$ has a unique planar drawing, that is denoted by $\rho_{C}$. Let $\rho'_C$ be the drawing of $C\setminus A_C$ induced by $\rho_C$.
		
		\item {\bf (Bridge Consistency Property):} for every bridge $R\in \rset_{G}(C\setminus A_C)$, there is a face $F$ in the  drawing $\rho'_C$ of $C\setminus A_C$, such that the set $L(R)$ of vertices lie on the boundary of $F$; and
		%{\color{blue} Note that as $C$ is no longer $3$-connected, its boundary is not a simple cycle and here we consider the full boundary of it, i.e., all edges $e$ such that every point on the drawing $\rho'_C(e)$ is adjacent to $F$.}
		
		\item {\bf (Well-Linkedness of Terminals)} the set $\Gamma(C)$ of terminals is $\alpha$-well-linked in $C$, for $\alpha=\frac{1}{128\Delta \alphasc(n)\log_{3/2} n}=\Theta \left (\frac{1}{\Delta \log^{1.5}n}\right )$.
		%	\item if $Q$ is any path in $G$ whose endpoints lie in $C$, such that $Q$ is internally disjoint from $C$, then the endpoints of $Q$ are terminals that lie on the boundary of a single face of the drawing $\rho_{C\cup A}$.
	\end{itemize}
\end{definition}	


Let $\cset_1\subseteq \cset$ denote the set of all type-1 acceptable clusters.
For a fake edge $e=(x,y)\in A$, an \emph{embedding} of $e$ is a path $P(e)\subseteq G$ connecting $x$ to $y$. We will compute an embedding of all fake edges in $A$ that has additional useful properties that are summarized below.

\begin{definition}
	A \emph{legal embedding} of the set $A$ of fake edges is a collection $\pset(A)=\set{P(e)\mid e\in A}$ of paths in $G$, such that the following hold.
	\begin{itemize}
		\item For every edge $e=(x,y)\in A$, path $P(e)$ has endpoints $x$ and $y$, and moreover, there is a type-1 acceptable cluster $C(e)\in \cset_1$ such that $P(e)\setminus\set{x,y}$ is contained in $C(e)$;
		\item For any pair $e,e'\in A$ of distinct edges, $C(e)\neq C(e')$; and
		\item All paths in $\pset(A)$ are mutually internally disjoint.
	\end{itemize}
\end{definition}


		


%\subsection{Main Theorems}
%\label{subsec: main technical theorems}


Finally, we define a decomposition of a graph $G$ into acceptable clusters; this definition is central for the proof of our main result.

\begin{definition} 
	A \emph{decomposition of a graph $G$ into acceptable clusters} consists of:
	
	\begin{itemize}
		\item a planarizing set $\hat E\subseteq E(G)$ of edges of $G$;
		\item a set $A$ of fake edges (where the endpoints of each fake edge are terminals with respect to $\hat E$);
		\item a partition $(\cset_1,\cset_2)$ of all connected components of the resulting graph $(G\setminus \hat E)\cup A$ into two subsets, such that every cluster $C\in \cset_1$ is a type-1 acceptable cluster and every cluster $C\in \cset_2$ is a type-2 acceptable cluster; and
		\item a legal embedding $\pset(A)$ of all fake edges.
		\end{itemize}

We denote such a decomposition by $\dset=\left (\hat E,A,\cset_1,\cset_2,\pset(A)\right )$.
\end{definition}



\iffalse
The proof of Theorem~\ref{thm: main} is divided into two parts.
In the first part (Section~\ref{sec:thm1} and Section~\ref{sec:canonical drawing}), we will show the proof of Theorem~\ref{thm: main}, assuming that the input \bdg $G$ is $3$-connected. 
In the second part (Section~\ref{sec:non_3}), we will complete the proof of Theorem~\ref{thm: main} by showing how to handle non-$3$-connected graphs.
We now state the two main theorems of the first part.
\fi

Our first result is the following theorem, whose proof appears in Section \ref{sec:thm1}, that allows us to compute a decomposition of the input graph $G$ into acceptable clusters.

\begin{theorem}\label{thm: can find edge set w acceptable clusters}
There is an efficient randomized algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree at most $\Delta$ and a planarizing set $E'$ of edges for $G$, with high probability computes a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A)\right )$ of $G$ into acceptable clusters, such that $E'\subseteq  E''$ and $| E''|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$.
\end{theorem}





\subsection{Canonical Drawings}
In this subsection, we assume that we are given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree at most $\Delta$, and a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A)\right )$ of $G$ into acceptable clusters. Next, we define drawings of $G\cup A$ that are ``canonical'' with respect to the clusters in the decomposition. Intuitively, in each such drawing, we require that the edges of type-2 acceptable clusters (clusters in $\cset_2$) do not participate in any crossings, and the edges of type-1 acceptable cluster (clusters in $\cset_1$) only participate in a small number of crossings (more specifically, we will define a subset $E^*(C)$ of edges for each cluster $C\in \cset_1$ that are allowed to participate in crossings). We then show that any drawing of $G$ can be transformed into such a canonical drawing of $G\cup A$, while only slightly increasing the number of crossings. This is sufficient in order to complete the proof of Theorem \ref{thm: main}, by adding to $E''$ the set $\bigcup_{C\in \cset_1}E^*(C)$ of edges. However, in order to be able to reduce the problem to the Crossing Number with Rotation System, we need stronger properties. We will define, for every cluster $C\in \cset_1\cup \cset_2$, a fixed drawing $\psi(C)$, and we will require that in the final drawing of $G\cup A$, the induced drawing of each such cluster $C$ is precisely $\psi(C)$. Additionally, for each cluster $C\in \cset_1\cup \cset_2$, and for each bridge $R\in \rset_G(C)$, we will define a disc $D(R)$ in the drawing $\psi(C)$ of $C$, and we will require that all vertices and edges of $R$ are drawn inside $D(R)$ in the final drawing of $G$. This will allow us to fix the locations of the clusters with respect to each other (that is, for each pair $C,C'$ of clusters, we will identify a face $F$ in the drawing $\psi(C)$ of $C$, and a face $F'$ in the drawing $\psi(C')$ of $C'$, such that, in the final drawing $\phi$ of the graph $G\cup A$, cluster $C'$ is drawn inside the face $F$ (of the drawing of $C$ induced by $\phi$), and similarly cluster $C$ is drawn inside the face $F'$.

We now proceed to define the drawings $\psi(C)$ of the clusters $C\in \cset_1\cup \cset_2$, and canonical drawings of the graph $G\cup A$ with respect to these clusters.


\subsubsection{Type-2 Acceptable Clusters}
Consider any type-2 acceptable cluster $C\in \cset_2$. Recall that $C$ has a unique planar drawing, denoted by $\rho_C$, and, from the definition of type-2 acceptable clusters, we have the following additional property: for every bridge $R\in \rset_{G\cup A}(C)$, there is a face $F$ of the drawing $\rho_C$, such that the vertices of $L(R)$ lie on the boundary of $F$ (we note that face $F$ is not uniquely defined; we break ties arbitrarily). We denote by $D(R)$ the open disc whose boundary is the boundary of $F$ in the drawing $\rho_C$.
Notice that for bridges $R\neq R'$, the discs $D(R),D(R')$ may not be disjoint.

\begin{definition}
	Let $\phi$ be any drawing of the graph $G\cup A$. We say that the drawing $\phi$ is \emph{canonical} with respect to the type-$2$ cluster $C\in \cset_2$ iff:
	\begin{itemize}
		\item the drawing of $C\setminus A_C$ induced by $\phi$ is precisely $\rho'_C$;
	\item the edges of $C\setminus A_C$ do not participate in any crossings in $\phi$; and
	\item for every bridge $R\in \rset_{G}(C\setminus A)$, all vertices and edges of $R$ are drawn inside the disc $D(R)$ (that is defined with respect to the drawing $\rho'_C$ of $C\setminus A$).
	\end{itemize}
\end{definition}

\subsubsection{Type-1 Acceptable Clusters}
Consider a cluster $C\in \cset_1$. %Recall that, from the definition of type-1 acceptable clusters, we are guaranteed that $|\Gamma(C)|\leq \mu$. 
%
%
%
%In this subsection, we show that we can find a drawing of $C\cup X_G(C)$ with relatively few crossings, and we will exploit this fact in the proof of Theorem~\ref{thm: from acceptable clusters to drawing} when dealing with type-1 acceptable clusters.
For convenience, we denote $\cset_1=\set{C_1,\ldots,C_q}$. We fix an arbitrary optimal drawing $\phi^*$ of the graph $G$. For each $1\leq i\leq q$, we denote by $\chi_i$ the set of all crossings $(e,e')$ such that either $e$ or $e'$ (or both) are edges of $E(C_i)$.   
The following observation is immediate.

\begin{observation}\label{obs: sum of chis}
$\sum_{i=1}^q|\chi_i|\leq 2\cdot\cro(\phi^*)=2\cdot\optcro(G)$. 
\end{observation}


Consider now some cluster $C_i\in \cset_1$. Let $e_i\in A$ be the unique fake edge that is embedded into $C_i$; if no such edge exists, $e_i$ is undefined. We set $C_i'=C_i\cup \set{e_i}$. Let $e_i=(x_i,y_i)$. Recall that edge $e_i$ belongs to some type-2 acceptable cluster $C$, and so $C$ contains a path $P_i$ connecting $x_i$ to $y_i$. Therefore, there must be a bridge $R_i\in \rset_{G\cup A}C_i'$ that contains $P_i\setminus \set{x_i,y_i}$, with $x_i,y_i\in L(R_i)$. 

Recall that the extension $X_{G\cup A}(C_i')$ (that is defined in Section \ref{sec:prelim}) is a collection of trees $\set{T_R\mid R\in \rset_{G\cup A}(C_i')}$. %Moreover, from the definition of the extension, for every tree $T_R$, the number of vertices whose degree in $T_R$ is greater than $2$ is bounded by $|L(R)|\leq |\Gamma(C_i)|\leq \mu$.
We denote by $C^+_i$ the graph obtained by the union of $C'_i$ and all trees in $X_{G\cup A}(C_i')$, namely $C^+_i=C_i'\cup \left(\bigcup_{R\in \rset_{G\cup A}(C_i)}T_R\right )$.
For every tree $T_R\in X_{G\cup A}(C_i')$, we denote by $\tilde E(R)$ the set of all edges of $T_R$ that are incident to the vertices of $L(R)$.  We use the following theorem in order to fix a drawing of each type-$1$ acceptable cluster $C_i$.

\begin{theorem}\label{thm: drawing of cluster extension-type 1}
	There is an efficient algorithm that computes, for every cluster $C_i\in \cset_1$, a subset $E^*(C_i)$ of at most $O(|\chi_i|\cdot\poly(\mu \Delta \log n))$ edges of $C_i$, and a drawing $\psi_i$ of $C_i^+$ with $ O\!\left(|\chi_i|\cdot \poly(\mu\Delta\log n)\right)$ crossings, such that the images of the edges in $E(C_i)\setminus E^*(C_i)$ do not participate in crossings. Additionally, the algorithm computes, for every tree $T_R\in X_{G\cup A}(C_i')$, a closed disc $D_{T_R}$, such that:
	\begin{itemize}
		\item for every vertex and edge of $C_i'$, its image in $\psi_i$ is disjoint from the interior of $D_{T_R}$;
		\item all vertices and edges of $T_R\setminus \tilde E(R)$ are drawn in the interior of $D_{T_R}$; 
		\item for every edge of $\tilde E(R)$, its image intersects the boundary of the disc $D_{T_R}$ exactly once; 
		\item the discs in $\set{D_{T_R}}_{T_R\in X_{G\cup A}(C'_i)}$ are mutually disjoint; and
		\item the image of the edge $e_i$ has a non-empty intersection with the boundary of the disc $D_{T_{R_i}}$, and this intersection is a contiguous curve.
	\end{itemize}
\end{theorem}

\mynote{Note that in addition to many notational changes, the above theorem requires the drawing to include the fake edge $e_i$, and the bridges are defined w.r.t. $G\cup A$. The latter is not a problem because every fake edge is embedded into some type-1 cluster, so bridges w.r.t. $G\cup A$ are same as bridges w.r.t. $G$. The former is a bit of a problem because we need to add the drawing of $e_i$ to the drawing of $G$. Because $e_i$ is contained in some type-2 cluster $C$, we can embed it into a real path $P_i$ in graph $G$, that does not contain any fake edges. This real path must be contained in a single bridge $R$. So we can route this edge along the boundary of the disc $D(T_R)$. Notice also that the theorem now requires that the edges of $E(C_i)\setminus E^*(C_i)$ do not participate in any crossings; previous version required that they don't cross each other.}

Let $E^*=\bigcup_{C_i\in \cset_1}E^*(C_i)$. Then, from Observation \ref{obs: sum of chis}:

\[
|E^*|\leq \sum_{C_i\in \cset_1}O\!\left(|\chi_i|\cdot \poly(\mu\Delta\log n)\right)\leq O\left (\optcro(G) \poly(\Delta\log n)\right ).
\]

We denote, for each type-$1$ acceptable cluster $C_i\in \cset_1$, by $\rho_{C_i}$ the drawing of $C_i$ that is induced by the drawing $\psi_i$ of $C_i^+$ (note that this drawing excludes the edge $e_i$).

\begin{definition}
	Let $\phi$ be any drawing of the graph $G\cup A$, and let $C_i\in \cset_1$ be a type-$1$ acceptable cluster. We say that $\phi$ is a \emph{canonical drawing} with respect to $C_i$, iff:
	\begin{itemize}
		\item the drawing of $C_i$ induced by $\phi$ is precisely $\rho_{C_i}$ (and in particular, the only edges of $C_i$ that participate in crossings are the edges of $E^*(C_i)$); and
		\item for every bridge $R\in \rset_{G\cup A}(C'_i)$, all vertices and edges of $R$ are drawn inside the disc $D_{T_R}$ (that is defined with respect to the drawing $\rho_{C_i}$ of $C_i$).
	\end{itemize}
\end{definition}

\mynote{need to decide between $D(R)$ and $D_{T_R}$, and also open/closed disc. There is a difference in definitions for type-1 and type-2 clusters: for type-2 clusters the boundary of the disc contains the vertices of $L(R)$, for type-1 it doesn't. Should make consistent.}



\subsubsection{Obtaining a Canonical Drawing}

%Recall that we are given a partition $(\cset_1,\cset_2)$ of all connected components of $H$ into type-1 and type-2 acceptable clusters, respectively. 
%\mynote{we need to be careful in that the boundary of $F$ may not be $2$-connected. We need to write this more carefully.}
%For a type-1 acceptable cluster $C\in \cset_1$, we denote by $\rho'_C$ the drawing of $C$ that is induced by the drawing of corresponding graph $C^+$ given by Corollary \ref{cor: drawing of cluster extension-type 1}. Recall that for every tree $T_R\in X_G(C)$, there is a disc $D_{T_R}$, such that, in the drawing of $C^+$ given by Corollary~\ref{cor: drawing of cluster extension-type 1}, $T_R\setminus \tilde E(R)$ is drawn inside the disc $D_{T_R}$ and graph $C$ is drawn outside $D_{T_R}$.


Our next result shows that there exists a near-optimal drawing of the graph $G$ that is canonical with respect to all clusters.


\begin{theorem}\label{thm: canonical drawing}
There is an efficient algorithm, that, given an $n$-vertex graph $G$ of maximum vertex degree at most $\Delta$, an arbitrary drawing $\phi$ of $G$, a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A))\right )$,  and, for each cluster $C\in \cset_1\cup \cset_2$, a drawing $\rho'_C$ of $C\setminus A_C$ as defined above, together with the set $\set{D_{T_R}}_{R\in X_G(C)}$ of discs, computes a drawing $\phi'$ of $G$ with $O(\cro(\phi)\cdot\poly(\Delta \log n))$ crossings, such that $\phi'$ is canonical with respect to every cluster $C\in \cset_1\cup \cset_2$. \mynote{to check: do we need $G$ to be $3$-connected in the proof?}
\end{theorem}


The proof of Theorem \ref{thm: canonical drawing} appears in Section \ref{sec:canonical drawing}.

\subsection{Completing the Proof of Theorem \ref{thm: main} for $3$-Connected Graphs}
Notice that the proof of Theorem \ref{thm: canonical drawing} concludes the proof of Theorem \ref{thm: main} for the special case where $G$ is a $3$-connected graph. Indeed, given a $3$-connected graph $G$, we use Theorem  \ref{thm: can find edge set w acceptable clusters} to compute a decomposition  $\dset=\left ( E'',\cset_1,\cset_2,A, \pset(C)\right )$ of $G$ into acceptable clusters, such that $E'\subseteq  E''$ and $| E''|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$. Next, we apply Theorem \ref{thm: drawing of cluster extension-type 1} to each type-1 cluster $C_i\in \cset_1$, to obtain the set $E^*(C_i)$ of edges, the drawing $\psi_i$ of $C_i$, and the discs $D_{T_R}$ for all trees $T_R\in X_G(C_i)$. Let $E^*=\bigcup_{C_i\in \cset_1}E^*(C_i)$, so $|E^*|\leq O\left (\optcro(G) \poly(\Delta\log n)\right )$, as observed above. The final outcome of the algorithm is the set $E''\cup E^*$ of edges. 
Observe that  $|E''\cup E^*|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$. Moreover, by using Theorem \ref{thm: canonical drawing} with the optimal drawing $\phi^*$ of $G$, we conclude that there exists a drawing $\phi'$ of $G\cup A$ with $O(\optcro(G)\cdot\poly(\Delta \log n))$ crossings, that is canonical with respect to all clusters in $\cset_1\cup \cset_2$. In particular, the only edges that may participate in crossings in $\phi'$ are edges of $E''\cup E^*$. By deleting the images of the fake edges from this drawing, we obtain the desired drawing of $G$.
%This concludes the proof of \ref{thm: main} for the special case where $G$ is a $3$-connected graph.


\iffalse
\begin{theorem}\label{thm: canonical drawing}
	There is an efficient algorithm, that, given an $n$-vertex graph $G$, a planarizing set $E''$ of its edges, a partition $(\cset_1,\cset_2)$ of all the connected components of the resulting graph $H=G\setminus E''$ into two subsets, a legal set $A_C$ of fake edges for each component $C\in \cset_2$, together with an embedding $\pset(A_C)$ of the edges in $A_C$ into $G$, such that (i) each cluster $C\in \cset_1$ is a type-1 acceptable cluster;
	(ii) For each cluster $C\in \cset_2$, $(C,A_C)$ is a type-2 acceptable cluster; and
	(iii) all paths in set $\bigcup_{C\in \cset_2}\pset(A_C)$ are mutually internally disjoint, together with an optimal drawing $\phi$ of $G$, computes a drawing $\phi'$ of $G$ with $O(\optcro(G)\cdot\poly(\Delta \log n))$ crossings, such that $\phi'$ is canonical with respect to every cluster $C\in \cset_1\cup \cset_2$.
\end{theorem}
\fi



\iffalse
We claim that the proof of Theorem~\ref{thm: canonical drawing} will conclude the proof of Theorem~\ref{thm: from acceptable clusters to drawing}. In fact, we simply set $E'''=E''\cup(\bigcup_{C_i\in \cset_1}E^*_i)$. Since $\sum_{C_i\in \cset_1}|E^*_i|=O(\optcro(G)\cdot \poly(\mu\Delta\log n))$, we get that $|E'''|=O(\optcro(G)+|E''|)\poly(\mu\Delta\log n)$. From the definition of canonical drawing and the definition of $E^*_i$, the drawing $\phi'$ obtained from Theorem~\ref{thm: canonical drawing} is in $\Phi_{E'''}(G)$.





\begin{theorem}\label{thm: from acceptable clusters to drawing}
There is an efficient randomized algorithm, that, given a $3$-connected graph with maximum vertex degree $\Delta$, and a decomposition $\dset=\left (E'',\cset_1,\cset_2,\bigcup_{C\in \cset_2}A_C,\bigcup_{C\in \cset_2}\pset(A_C)\right )$ of $G$ into acceptable clusters, computes a planarizing edge set $E'''\subseteq E(G)$, such that 
\begin{itemize}
\item $E''\subseteq E'''$;
\item $|E'''|\leq O((|E'|+\optcro(G))\cdot\poly(\Delta\log n))$; and
\item there is a drawing of $G$ in $\Phi_{E'''}(G)$ with at most $O(\optcro(G)\cdot\poly(\Delta\log n))$ crossings.
\end{itemize}
%$E''\subseteq E'''$ and $|E'''|\leq O(|E''|+\cro(G))\poly(\Delta\log n)$, and there is a drawing of $G$ in $\Phi_{E'''}(G)$ with at most $O(\optcro(G)\cdot\poly(\Delta\log n))$ crossings.
\end{theorem}
		
	\fi	
		

\subsection{Extensions to General Graphs}
In Section \ref{sec:non_3} we show how to extend the above proof of Theorem \ref{thm: main}  to general graphs, that are not necessarily $3$-connected. The extension builds on techniques that were introduced in \cite{chuzhoy2011graph}, combining them with Lemma \ref{lem:block_endpoints_routing}, that allows us to embed all fake edges of a given block decomposition into the input graph $G$, with low congestion. Additionally, in Section \ref{sec:non_3}, we prove the following theorem, that will be useful for our approximation algorithm.


\begin{theorem}
\label{thm:main_non_3}
Assume that there exists an efficient (possibly randomized) algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree $\Delta$, and a planarizing set $E'$ of its edges, computes a drawing of $G$ with at most $f(n,\Delta)\cdot(\optcro(G)+|E'|)$ crossings, for any function $f$ that is monotone increasing in both $n$ and $\Delta$. Then there exists an efficient (possibly randomized) algorithm that, given a (not necessarily 3-connected) graph $\hat{G}$ on $n$ vertices with maximum vertex degree $\Delta$,  and a planarizing set $\hat{E}'$ of its edges, computes a drawing of $\hat G$ with $O\left( f(n,\Delta)(\optcro(\hat G)+|\hat E'|)\cdot \poly(\Delta\log n)\right)$ crossings.
\end{theorem}


\subsection{Reduction to Crossing Number with Rotation System}

==> acceptable-clusters-corrupted.tex <==
\section{High-Level Overview}
\label{sec:overview}

In this section we provide a high-level overview of the proofs of our main results, and state the main theorems from which the proof is inferred. 
As in previous work, we start by considering a special case where the input graph $G$ is $3$-connected. This special case seems to capture the main technical challenges of the whole problem, and the extension to non-$3$-connected graphs is relatively easy and follows the same framework as in previous work \cite{chuzhoy2011graph}.
We start by defining several central notions that our proof uses.


%\mynote{An explanation why the things are set up this way and not the way we discussed. Our plan was to define an acceptable cluster like this:  a type-1 acceptable cluster has $\poly\log n$ terminals. A type-2 acceptable cluster is $3$-connected, good (no path connecting terminals lying on different faces), and terminals are well-linked. To get a planarizing set $\hat E$ of edges so that in $H=G\setminus \hat E$ every cluster is acceptable, we would follow these 3 steps:
%(1) make all clusters good, under a suitable definition of good.
%(2) do a well-linked decomposition.
%(3) cut-off 2-cuts to get 3-connected components.
%However, the third step does not actually work. If we start cutting off 2-vertex cuts we may end up creating new 2-vertex cuts that weren't there before. So type-2 acceptable clusters need to be defined differently. We need to allow to add fake edges that will replace the 2-vertex cuts we cut off, and the cluster itself with the fake edges should be 3-connected. This motivates the setup in this section.}



%\subsection*{Special Case: Input Graph $G$ is $3$-Connected}
		


\subsection{Acceptable Clusters and Decomposition into Acceptable Clusters}
In this section we define acceptable clusters and decomposition into acceptable clusters. These definitions are central for all our results. 
Let $G$ be an input graph on $n$ vertices of maximum degree at most $\Delta$; we assume that $G$ is $3$-connected. Let $\hat E$ be any planarizing set of edges for $G$, and let $H=G\setminus \hat E$. Let $\Gamma\subseteq V(G)$ be the set of all vertices that serve as endpoints of edges in $\hat E$; we call the vertices of $\Gamma$ \emph{terminals}. We will define a set $A$ of \emph{fake edges} -- a collection of edges $(x,y)$, where $x,y\in \Gamma$. We note that the edges of $A$ do not necessarily lie in $H$ or in $G$; in fact we will use these edges in order to augment the graph $H$. 

We denote by $\cset=\cset(H\cup A)$ the set of all connected components of $H\cup A$, and we call them \emph{clusters}.  For every cluster $C\in \cset$, we denote by $\Gamma(C)=\Gamma\cap V(C)$ the set of terminals that lie in $C$. We also denote by $A_C=A\cap C$ the set of all fake edges that lie in $C$.

%Next, we define some desirable properties of these clusters. 


\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-1 acceptable cluster} iff:
	
	\begin{itemize}
		\item $A_C=\emptyset$; and
		\item  $|\Gamma(C)|\leq \mu$ for $\mu=512\Delta\alphasc(n)\log_{3/2} n=O(\Delta\log^{1.5}n)$  (recall that $\alphasc(n)=O(\sqrt{\log n})$ is the approximation factor of the algorithm $\algsc$ for the sparsest cut problem).
	\end{itemize}
\end{definition}




\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-2 acceptable cluster} if the following conditions hold:
	
	\begin{itemize}
		\item {\bf (3-Connectivity):} $C$ is a simple $3$-connected planar graph, or it is isomorphic to $K_3$. In particular, $C$ has a unique planar drawing, that is denoted by $\rho_{C}$.
		
		\item {\bf (Bridge Consistency Property):} for every bridge $R\in \rset_{G\cup A}(C)$, there is a face $F$ in the drawing $\rho_C$, such that the set $L(R)$ of vertices lie on the boundary of $F$; and
		%{\color{blue} Note that as $C$ is no longer $3$-connected, its boundary is not a simple cycle and here we consider the full boundary of it, i.e., all edges $e$ such that every point on the drawing $\rho'_C(e)$ is adjacent to $F$.}
		
		\item {\bf (Well-Linkedness of Terminals)} the set $\Gamma(C)$ of terminals is $\alpha$-well-linked in $C$, for $\alpha=\frac{1}{128\Delta \alphasc(n)\log_{3/2} n}=\Theta \left (\frac{1}{\Delta \log^{1.5}n}\right )$.
		%	\item if $Q$ is any path in $G$ whose endpoints lie in $C$, such that $Q$ is internally disjoint from $C$, then the endpoints of $Q$ are terminals that lie on the boundary of a single face of the drawing $\rho_{C\cup A}$.
	\end{itemize}
\end{definition}	


Let $\cset_1\subseteq \cset$ denote the set of all type-1 acceptable clusters.
For a fake edge $e=(x,y)\in A$, an \emph{embedding} of $e$ is a path $P(e)\subseteq G$ connecting $x$ to $y$. We will compute an embedding of all fake edges in $A$ that has additional useful properties that are summarized below.

\begin{definition}
	A \emph{legal embedding} of the set $A$ of fake edges is a collection $\pset(A)=\set{P(e)\mid e\in A}$ of paths in $G$, such that the following hold.
	\begin{itemize}
		\item For every edge $e=(x,y)\in A$, path $P(e)$ has endpoints $x$ and $y$, and moreover, there is a type-1 acceptable cluster $C(e)\in \cset_1$ such that $P(e)\setminus\set{x,y}$ is contained in $C(e)$;
		\item For any pair $e,e'\in A$ of distinct edges, $C(e)\neq C(e')$; and
		\item All paths in $\pset(A)$ are mutually internally disjoint.
	\end{itemize}
\end{definition}


		


%\subsection{Main Theorems}
%\label{subsec: main technical theorems}


Finally, we define a decomposition of a graph $G$ into acceptable clusters; this definition is central for the proof of our main result.

\begin{definition} 
	A \emph{decomposition of a graph $G$ into acceptable clusters} consists of:
	
	\begin{itemize}
		\item a planarizing set $\hat E\subseteq E(G)$ of edges of $G$;
		\item a set $A$ of fake edges (where the endpoints of each fake edge are terminals with respect to $\hat E$);
		\item a partition $(\cset_1,\cset_2)$ of all connected components of the resulting graph $(G\setminus \hat E)\cup A$ into two subsets, such that every cluster $C\in \cset_1$ is a type-1 acceptable cluster and every cluster $C\in \cset_2$ is a type-2 acceptable cluster; and
		\item a legal embedding $\pset(A)$ of all fake edges.
		\end{itemize}

We denote such a decomposition by $\dset=\left (\hat E,A,\cset_1,\cset_2,\pset(A)\right )$.
\end{definition}



\iffalse
The proof of Theorem~\ref{thm: main} is divided into two parts.
In the first part (Section~\ref{sec:thm1} and Section~\ref{sec:canonical drawing}), we will show the proof of Theorem~\ref{thm: main}, assuming that the input \bdg $G$ is $3$-connected. 
In the second part (Section~\ref{sec:non_3}), we will complete the proof of Theorem~\ref{thm: main} by showing how to handle non-$3$-connected graphs.
We now state the two main theorems of the first part.
\fi

Our first result is the following theorem, whose proof appears in Section \ref{sec:thm1}, that allows us to compute a decomposition of the input graph $G$ into acceptable clusters.

\begin{theorem}\label{thm: can find edge set w acceptable clusters}
There is an efficient randomized algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree at most $\Delta$ and a planarizing set $E'$ of edges for $G$, with high probability computes a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A)\right )$ of $G$ into acceptable clusters, such that $E'\subseteq  E''$ and $| E''|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$.
\end{theorem}





\subsection{Canonical Drawings}
In this subsection, we assume that we are given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree at most $\Delta$, and a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A)\right )$ of $G$ into acceptable clusters. Next, we define drawings of $G\cup A$ that are ``canonical'' with respect to the clusters in the decomposition. Intuitively, in each such drawing, we require that the edges of type-2 acceptable clusters (clusters in $\cset_2$) do not participate in any crossings, and the edges of type-1 acceptable cluster (clusters in $\cset_1$) only participate in a small number of crossings (more specifically, we will define a subset $E^*(C)$ of edges for each cluster $C\in \cset_1$ that are allowed to participate in crossings). We then show that any drawing of $G$ can be transformed into such a canonical drawing of $G\cup A$, while only slightly increasing the number of crossings. This is sufficient in order to complete the proof of Theorem \ref{thm: main}, by adding to $E''$ the set $\bigcup_{C\in \cset_1}E^*(C)$ of edges. However, in order to be able to reduce the problem to the Crossing Number with Rotation System, we need stronger properties. We will define, for every cluster $C\in \cset_1\cup \cset_2$, a fixed drawing $\psi(C)$, and we will require that in the final drawing of $G\cup A$, the induced drawing of each such cluster $C$ is precisely $\psi(C)$. Additionally, for each cluster $C\in \cset_1\cup \cset_2$, and for each bridge $R\in \rset_G(C)$, we will define a disc $D(R)$ in the drawing $\psi(C)$ of $C$, and we will require that all vertices and edges of $R$ are drawn inside $D(R)$ in the final drawing of $G$. This will allow us to fix the locations of the clusters with respect to each other (that is, for each pair $C,C'$ of clusters, we will identify a face $F$ in the drawing $\psi(C)$ of $C$, and a face $F'$ in the drawing $\psi(C')$ of $C'$, such that, in the final drawing $\phi$ of the graph $G\cup A$, cluster $C'$ is drawn inside the face $F$ (of the drawing of $C$ induced by $\phi$), and similarly cluster $C$ is drawn inside the face $F'$.

We now proceed to define the drawings $\psi(C)$ of the clusters $C\in \cset_1\cup \cset_2$, and canonical drawings of the graph $G\cup A$ with respect to these clusters.


\subsubsection{Type-2 Acceptable Clusters}
Consider any type-2 acceptable cluster $C\in \cset_2$. Recall that $C$ has a unique planar drawing, denoted by $\rho_C$, that we used in order to define a drawing $\rho'_C$ of $C\setminus A_C$. From the definition of type-2 acceptable clusters, we have the following additional property: for every bridge $R\in \rset_{G}(C\setminus A_C)$, there is a face $F$ of the drawing $\rho'_C$, such that the vertices of $L(R)$ lie on the boundary of $F$ (we note that face $F$ is not uniquely defined; we break ties arbitrarily). We denote by $D(R)$ the open disc whose boundary is the boundary of $F$ in the drawing $\rho'_C$.
Notice that for bridges $R\neq R'$, the discs $D(R),D(R')$ may not be disjoint.

\begin{definition}
	Let $\phi$ be any drawing of the graph $G\cup A$. We say that the drawing $\phi$ is \emph{canonical} with respect to the type-$2$ cluster $C\in \cset_2$ iff:
	\begin{itemize}
		\item the drawing of $C$ induced by $\phi$ is precisely $\rho_C$;
	\item the edges of $C$ do not participate in any crossings in $\phi$; and
	\item for every bridge $R\in \rset_{G\cup A}(C)$, all vertices and edges of $R$ are drawn inside the disc $D(R)$ (that is defined with respect to the drawing $\rho_C$ of $C$).
	\end{itemize}
\end{definition}

\subsubsection{Type-1 Acceptable Clusters}
Consider a cluster $C\in \cset_1$. %Recall that, from the definition of type-1 acceptable clusters, we are guaranteed that $|\Gamma(C)|\leq \mu$. 
%
%
%
%In this subsection, we show that we can find a drawing of $C\cup X_G(C)$ with relatively few crossings, and we will exploit this fact in the proof of Theorem~\ref{thm: from acceptable clusters to drawing} when dealing with type-1 acceptable clusters.
For convenience, we denote $\cset_1=\set{C_1,\ldots,C_q}$. We fix an arbitrary optimal drawing $\phi^*$ of the graph $G$. For each $1\leq i\leq q$, we denote by $\chi_i$ the set of all crossings $(e,e')$ such that either $e$ or $e'$ (or both) are edges of $E(C_i)$.   
The following observation is immediate.

\begin{observation}\label{obs: sum of chis}
$\sum_{i=1}^q|\chi_i|\leq 2\cdot\cro(\phi^*)=2\cdot\optcro(G)$. 
\end{observation}


Consider now some cluster $C_i\in \cset_1$. Let $e_i\in A$ be the unique fake edge that is embedded into $C_i$; if no such edge exists, $e_i$ is undefined. We set $C_i'=C_i\cup \set{e_i}$. Let $e_i=(x_i,y_i)$. Recall that edge $e_i$ belongs to some type-2 acceptable cluster $C$, and so $C$ contains a path $P_i$ connecting $x_i$ to $y_i$. Therefore, there must be a bridge $R_i\in \rset_{G\cup A}C_i'$ that contains $P_i\setminus \set{x_i,y_i}$, with $x_i,y_i\in L(R_i)$. 

Recall that the extension $X_{G\cup A}(C_i')$ (that is defined in Section \ref{sec:prelim}) is a collection of trees $\set{T_R\mid R\in \rset_{G\cup A}(C_i')}$. %Moreover, from the definition of the extension, for every tree $T_R$, the number of vertices whose degree in $T_R$ is greater than $2$ is bounded by $|L(R)|\leq |\Gamma(C_i)|\leq \mu$.
We denote by $C^+_i$ the graph obtained by the union of $C'_i$ and all trees in $X_{G\cup A}(C_i')$, namely $C^+_i=C_i'\cup \left(\bigcup_{R\in \rset_{G\cup A}(C_i)}T_R\right )$.
For every tree $T_R\in X_{G\cup A}(C_i')$, we denote by $\tilde E(R)$ the set of all edges of $T_R$ that are incident to the vertices of $L(R)$.  We use the following theorem in order to fix a drawing of each type-$1$ acceptable cluster $C_i$.

\begin{theorem}\label{thm: drawing of cluster extension-type 1}
	There is an efficient algorithm that computes, for every cluster $C_i\in \cset_1$, a subset $E^*(C_i)$ of at most $O(|\chi_i|\cdot\poly(\mu \Delta \log n))$ edges of $C_i$, and a drawing $\psi_i$ of $C_i^+$ with $ O\!\left(|\chi_i|\cdot \poly(\mu\Delta\log n)\right)$ crossings, such that the images of the edges in $E(C_i)\setminus E^*(C_i)$ do not participate in crossings. Additionally, the algorithm computes, for every tree $T_R\in X_{G\cup A}(C_i')$, a closed disc $D_{T_R}$, such that:
	\begin{itemize}
		\item for every vertex and edge of $C_i'$, its image in $\psi_i$ is disjoint from the interior of $D_{T_R}$;
		\item all vertices and edges of $T_R\setminus \tilde E(R)$ are drawn in the interior of $D_{T_R}$; 
		\item for every edge of $\tilde E(R)$, its image intersects the boundary of the disc $D_{T_R}$ exactly once; 
		\item the discs in $\set{D_{T_R}}_{T_R\in X_{G\cup A}(C'_i)}$ are mutually disjoint; and
		\item the image of the edge $e_i$ has a non-empty intersection with the boundary of the disc $D_{T_{R_i}}$, and this intersection is a contiguous curve.
	\end{itemize}
\end{theorem}

\mynote{Note that in addition to many notational changes, the above theorem requires the drawing to include the fake edge $e_i$, and the bridges are defined w.r.t. $G\cup A$. The latter is not a problem because every fake edge is embedded into some type-1 cluster, so bridges w.r.t. $G\cup A$ are same as bridges w.r.t. $G$. The former is a bit of a problem because we need to add the drawing of $e_i$ to the drawing of $G$. Because $e_i$ is contained in some type-2 cluster $C$, we can embed it into a real path $P_i$ in graph $G$, that does not contain any fake edges. This real path must be contained in a single bridge $R$. So we can route this edge along the boundary of the disc $D(T_R)$. Notice also that the theorem now requires that the edges of $E(C_i)\setminus E^*(C_i)$ do not participate in any crossings; previous version required that they don't cross each other.}

Let $E^*=\bigcup_{C_i\in \cset_1}E^*(C_i)$. Then, from Observation \ref{obs: sum of chis}:

\[
|E^*|\leq \sum_{C_i\in \cset_1}O\!\left(|\chi_i|\cdot \poly(\mu\Delta\log n)\right)\leq O\left (\optcro(G) \poly(\Delta\log n)\right ).
\]

We denote, for each type-$1$ acceptable cluster $C_i\in \cset_1$, by $\rho_{C_i}$ the drawing of $C_i$ that is induced by the drawing $\psi_i$ of $C_i^+$ (note that this drawing excludes the edge $e_i$).

\begin{definition}
	Let $\phi$ be any drawing of the graph $G\cup A$, and let $C_i\in \cset_1$ be a type-$1$ acceptable cluster. We say that $\phi$ is a \emph{canonical drawing} with respect to $C_i$, iff:
	\begin{itemize}
		\item the drawing of $C_i$ induced by $\phi$ is precisely $\rho_{C_i}$ (and in particular, the only edges of $C_i$ that participate in crossings are the edges of $E^*(C_i)$); and
		\item for every bridge $R\in \rset_{G\cup A}(C'_i)$, all vertices and edges of $R$ are drawn inside the disc $D_{T_R}$ (that is defined with respect to the drawing $\rho_{C_i}$ of $C_i$).
	\end{itemize}
\end{definition}

\mynote{need to decide between $D(R)$ and $D_{T_R}$, and also open/closed disc. There is a difference in definitions for type-1 and type-2 clusters: for type-2 clusters the boundary of the disc contains the vertices of $L(R)$, for type-1 it doesn't. Should make consistent.}



\subsubsection{Obtaining a Canonical Drawing}

%Recall that we are given a partition $(\cset_1,\cset_2)$ of all connected components of $H$ into type-1 and type-2 acceptable clusters, respectively. 
%\mynote{we need to be careful in that the boundary of $F$ may not be $2$-connected. We need to write this more carefully.}
%For a type-1 acceptable cluster $C\in \cset_1$, we denote by $\rho'_C$ the drawing of $C$ that is induced by the drawing of corresponding graph $C^+$ given by Corollary \ref{cor: drawing of cluster extension-type 1}. Recall that for every tree $T_R\in X_G(C)$, there is a disc $D_{T_R}$, such that, in the drawing of $C^+$ given by Corollary~\ref{cor: drawing of cluster extension-type 1}, $T_R\setminus \tilde E(R)$ is drawn inside the disc $D_{T_R}$ and graph $C$ is drawn outside $D_{T_R}$.


Our next result shows that there exists a near-optimal drawing of the graph $G$ that is canonical with respect to all clusters.


\begin{theorem}\label{thm: canonical drawing}
There is an efficient algorithm, that, given an $n$-vertex graph $G$ of maximum vertex degree at most $\Delta$, an arbitrary drawing $\phi$ of $G$, a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A))\right )$,  and, for each cluster $C\in \cset_1\cup \cset_2$, a drawing $\rho'_C$ as defined above, together with the set $\set{D_{T_R}}_{R\in X_G(C)}$ of discs, computes a drawing $\phi'$ of $G\cup A$ with $O(\cro(\phi)\cdot\poly(\Delta \log n))$ crossings, such that $\phi'$ is canonical with respect to every cluster $C\in \cset_1\cup \cset_2$. \mynote{to check: do we need $G$ to be $3$-connected in the proof?}
\end{theorem}


The proof of Theorem \ref{thm: canonical drawing} appears in Section \ref{sec:canonical drawing}.

\subsection{Completing the Proof of Theorem \ref{thm: main} for $3$-Connected Graphs}
Notice that the proof of Theorem \ref{thm: canonical drawing} concludes the proof of Theorem \ref{thm: main} for the special case where $G$ is a $3$-connected graph. Indeed, given a $3$-connected graph $G$, we use Theorem  \ref{thm: can find edge set w acceptable clusters} to compute a decomposition  $\dset=\left ( E'',\cset_1,\cset_2,A, \pset(C)\right )$ of $G$ into acceptable clusters, such that $E'\subseteq  E''$ and $| E''|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$. Next, we apply Theorem \ref{thm: drawing of cluster extension-type 1} to each type-1 cluster $C_i\in \cset_1$, to obtain the set $E^*(C_i)$ of edges, the drawing $\psi_i$ of $C_i$, and the discs $D_{T_R}$ for all trees $T_R\in X_G(C_i)$. Let $E^*=\bigcup_{C_i\in \cset_1}E^*(C_i)$, so $|E^*|\leq O\left (\optcro(G) \poly(\Delta\log n)\right )$, as observed above. The final outcome of the algorithm is the set $E''\cup E^*$ of edges. 
Observe that  $|E''\cup E^*|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$. Moreover, by using Theorem \ref{thm: canonical drawing} with the optimal drawing $\phi^*$ of $G$, we conclude that there exists a drawing $\phi'$ of $G\cup A$ with $O(\optcro(G)\cdot\poly(\Delta \log n))$ crossings, that is canonical with respect to all clusters in $\cset_1\cup \cset_2$. In particular, the only edges that may participate in crossings in $\phi'$ are edges of $E''\cup E^*$. By deleting the images of the fake edges from this drawing, we obtain the desired drawing of $G$.
%This concludes the proof of \ref{thm: main} for the special case where $G$ is a $3$-connected graph.


\iffalse
\begin{theorem}\label{thm: canonical drawing}
	There is an efficient algorithm, that, given an $n$-vertex graph $G$, a planarizing set $E''$ of its edges, a partition $(\cset_1,\cset_2)$ of all the connected components of the resulting graph $H=G\setminus E''$ into two subsets, a legal set $A_C$ of fake edges for each component $C\in \cset_2$, together with an embedding $\pset(A_C)$ of the edges in $A_C$ into $G$, such that (i) each cluster $C\in \cset_1$ is a type-1 acceptable cluster;
	(ii) For each cluster $C\in \cset_2$, $(C,A_C)$ is a type-2 acceptable cluster; and
	(iii) all paths in set $\bigcup_{C\in \cset_2}\pset(A_C)$ are mutually internally disjoint, together with an optimal drawing $\phi$ of $G$, computes a drawing $\phi'$ of $G$ with $O(\optcro(G)\cdot\poly(\Delta \log n))$ crossings, such that $\phi'$ is canonical with respect to every cluster $C\in \cset_1\cup \cset_2$.
\end{theorem}
\fi



\iffalse
We claim that the proof of Theorem~\ref{thm: canonical drawing} will conclude the proof of Theorem~\ref{thm: from acceptable clusters to drawing}. In fact, we simply set $E'''=E''\cup(\bigcup_{C_i\in \cset_1}E^*_i)$. Since $\sum_{C_i\in \cset_1}|E^*_i|=O(\optcro(G)\cdot \poly(\mu\Delta\log n))$, we get that $|E'''|=O(\optcro(G)+|E''|)\poly(\mu\Delta\log n)$. From the definition of canonical drawing and the definition of $E^*_i$, the drawing $\phi'$ obtained from Theorem~\ref{thm: canonical drawing} is in $\Phi_{E'''}(G)$.





\begin{theorem}\label{thm: from acceptable clusters to drawing}
There is an efficient randomized algorithm, that, given a $3$-connected graph with maximum vertex degree $\Delta$, and a decomposition $\dset=\left (E'',\cset_1,\cset_2,\bigcup_{C\in \cset_2}A_C,\bigcup_{C\in \cset_2}\pset(A_C)\right )$ of $G$ into acceptable clusters, computes a planarizing edge set $E'''\subseteq E(G)$, such that 
\begin{itemize}
\item $E''\subseteq E'''$;
\item $|E'''|\leq O((|E'|+\optcro(G))\cdot\poly(\Delta\log n))$; and
\item there is a drawing of $G$ in $\Phi_{E'''}(G)$ with at most $O(\optcro(G)\cdot\poly(\Delta\log n))$ crossings.
\end{itemize}
%$E''\subseteq E'''$ and $|E'''|\leq O(|E''|+\cro(G))\poly(\Delta\log n)$, and there is a drawing of $G$ in $\Phi_{E'''}(G)$ with at most $O(\optcro(G)\cdot\poly(\Delta\log n))$ crossings.
\end{theorem}
		
	\fi	
		

\subsection{Extensions to General Graphs}
In Section \ref{sec:non_3} we show how to extend the above proof of Theorem \ref{thm: main}  to general graphs, that are not necessarily $3$-connected. The extension builds on techniques that were introduced in \cite{chuzhoy2011graph}, combining them with Lemma \ref{lem:block_endpoints_routing}, that allows us to embed all fake edges of a given block decomposition into the input graph $G$, with low congestion. Additionally, in Section \ref{sec:non_3}, we prove the following theorem, that will be useful for our approximation algorithm.


\begin{theorem}
\label{thm:main_non_3}
Assume that there exists an efficient (possibly randomized) algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree $\Delta$, and a planarizing set $E'$ of its edges, computes a drawing of $G$ with at most $f(n,\Delta)\cdot(\optcro(G)+|E'|)$ crossings, for any function $f$ that is monotone increasing in both $n$ and $\Delta$. Then there exists an efficient (possibly randomized) algorithm that, given a (not necessarily 3-connected) graph $\hat{G}$ on $n$ vertices with maximum vertex degree $\Delta$,  and a planarizing set $\hat{E}'$ of its edges, computes a drawing of $\hat G$ with $O\left( f(n,\Delta)(\optcro(\hat G)+|\hat E'|)\cdot \poly(\Delta\log n)\right)$ crossings.
\end{theorem}


\subsection{Reduction to Crossing Number with Rotation System}

==> acceptable-clusters-with-fake.tex <==
\section{High-Level Overview}
\label{sec:overview}

In this section we provide a high-level overview of the proofs of our main results, and state the main theorems from which the proof is inferred. 
As in previous work, we start by considering a special case where the input graph $G$ is $3$-connected. This special case seems to capture the main technical challenges of the whole problem, and the extension to non-$3$-connected graphs is relatively easy and follows the same framework as in previous work \cite{chuzhoy2011graph}.
We start by defining several central notions that our proof uses.


%\mynote{An explanation why the things are set up this way and not the way we discussed. Our plan was to define an acceptable cluster like this:  a type-1 acceptable cluster has $\poly\log n$ terminals. A type-2 acceptable cluster is $3$-connected, good (no path connecting terminals lying on different faces), and terminals are well-linked. To get a planarizing set $\hat E$ of edges so that in $H=G\setminus \hat E$ every cluster is acceptable, we would follow these 3 steps:
%(1) make all clusters good, under a suitable definition of good.
%(2) do a well-linked decomposition.
%(3) cut-off 2-cuts to get 3-connected components.
%However, the third step does not actually work. If we start cutting off 2-vertex cuts we may end up creating new 2-vertex cuts that weren't there before. So type-2 acceptable clusters need to be defined differently. We need to allow to add fake edges that will replace the 2-vertex cuts we cut off, and the cluster itself with the fake edges should be 3-connected. This motivates the setup in this section.}



%\subsection*{Special Case: Input Graph $G$ is $3$-Connected}
		


\subsection{Acceptable Clusters and Decomposition into Acceptable Clusters}
In this section we define acceptable clusters and decomposition into acceptable clusters. These definitions are central for all our results. 
Let $G$ be an input graph on $n$ vertices of maximum degree at most $\Delta$; we assume that $G$ is $3$-connected. Let $\hat E$ be any planarizing set of edges for $G$, and let $H=G\setminus \hat E$. Let $\Gamma\subseteq V(G)$ be the set of all vertices that serve as endpoints of edges in $\hat E$; we call the vertices of $\Gamma$ \emph{terminals}. We will define a set $A$ of \emph{fake edges} -- a collection of edges $(x,y)$, where $x,y\in \Gamma$. We note that the edges of $A$ do not necessarily lie in $H$ or in $G$; in fact we will use these edges in order to augment the graph $H$. 

We denote by $\cset=\cset(H\cup A)$ the set of all connected components of $H\cup A$, and we call them \emph{clusters}.  For every cluster $C\in \cset$, we denote by $\Gamma(C)=\Gamma\cap V(C)$ the set of terminals that lie in $C$. We also denote by $A_C=A\cap C$ the set of all fake edges that lie in $C$.

%Next, we define some desirable properties of these clusters. 


\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-1 acceptable cluster} iff:
	
	\begin{itemize}
		\item $A_C=\emptyset$; and
		\item  $|\Gamma(C)|\leq \mu$ for $\mu=512\Delta\alphasc(n)\log_{3/2} n=O(\Delta\log^{1.5}n)$  (recall that $\alphasc(n)=O(\sqrt{\log n})$ is the approximation factor of the algorithm $\algsc$ for the sparsest cut problem).
	\end{itemize}
\end{definition}




\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-2 acceptable cluster} if the following conditions hold:
	
	\begin{itemize}
		\item {\bf (3-Connectivity):} $C$ is a simple $3$-connected planar graph, or it is isomorphic to $K_3$. In particular, $C$ has a unique planar drawing, that is denoted by $\rho_{C}$.
		
		\item {\bf (Bridge Consistency Property):} for every bridge $R\in \rset_{G\cup A}(C)$, there is a face $F$ in the drawing $\rho_C$, such that the set $L(R)$ of vertices lie on the boundary of $F$; and
		%{\color{blue} Note that as $C$ is no longer $3$-connected, its boundary is not a simple cycle and here we consider the full boundary of it, i.e., all edges $e$ such that every point on the drawing $\rho'_C(e)$ is adjacent to $F$.}
		
		\item {\bf (Well-Linkedness of Terminals)} the set $\Gamma(C)$ of terminals is $\alpha$-well-linked in $C$, for $\alpha=\frac{1}{128\Delta \alphasc(n)\log_{3/2} n}=\Theta \left (\frac{1}{\Delta \log^{1.5}n}\right )$.
		%	\item if $Q$ is any path in $G$ whose endpoints lie in $C$, such that $Q$ is internally disjoint from $C$, then the endpoints of $Q$ are terminals that lie on the boundary of a single face of the drawing $\rho_{C\cup A}$.
	\end{itemize}
\end{definition}	


Let $\cset_1\subseteq \cset$ denote the set of all type-1 acceptable clusters.
For a fake edge $e=(x,y)\in A$, an \emph{embedding} of $e$ is a path $P(e)\subseteq G$ connecting $x$ to $y$. We will compute an embedding of all fake edges in $A$ that has additional useful properties that are summarized below.

\begin{definition}
	A \emph{legal embedding} of the set $A$ of fake edges is a collection $\pset(A)=\set{P(e)\mid e\in A}$ of paths in $G$, such that the following hold.
	\begin{itemize}
		\item For every edge $e=(x,y)\in A$, path $P(e)$ has endpoints $x$ and $y$, and moreover, there is a type-1 acceptable cluster $C(e)\in \cset_1$ such that $P(e)\setminus\set{x,y}$ is contained in $C(e)$;
		\item For any pair $e,e'\in A$ of distinct edges, $C(e)\neq C(e')$; and
		\item All paths in $\pset(A)$ are mutually internally disjoint.
	\end{itemize}
\end{definition}


		


%\subsection{Main Theorems}
%\label{subsec: main technical theorems}


Finally, we define a decomposition of a graph $G$ into acceptable clusters; this definition is central for the proof of our main result.

\begin{definition} 
	A \emph{decomposition of a graph $G$ into acceptable clusters} consists of:
	
	\begin{itemize}
		\item a planarizing set $\hat E\subseteq E(G)$ of edges of $G$;
		\item a set $A$ of fake edges (where the endpoints of each fake edge are terminals with respect to $\hat E$);
		\item a partition $(\cset_1,\cset_2)$ of all connected components of the resulting graph $(G\setminus \hat E)\cup A$ into two subsets, such that every cluster $C\in \cset_1$ is a type-1 acceptable cluster and every cluster $C\in \cset_2$ is a type-2 acceptable cluster; and
		\item a legal embedding $\pset(A)$ of all fake edges.
		\end{itemize}

We denote such a decomposition by $\dset=\left (\hat E,A,\cset_1,\cset_2,\pset(A)\right )$.
\end{definition}



\iffalse
The proof of Theorem~\ref{thm: main} is divided into two parts.
In the first part (Section~\ref{sec:thm1} and Section~\ref{sec:canonical drawing}), we will show the proof of Theorem~\ref{thm: main}, assuming that the input \bdg $G$ is $3$-connected. 
In the second part (Section~\ref{sec:non_3}), we will complete the proof of Theorem~\ref{thm: main} by showing how to handle non-$3$-connected graphs.
We now state the two main theorems of the first part.
\fi

Our first result is the following theorem, whose proof appears in Section \ref{sec:thm1}, that allows us to compute a decomposition of the input graph $G$ into acceptable clusters.

\begin{theorem}\label{thm: can find edge set w acceptable clusters}
There is an efficient randomized algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree at most $\Delta$ and a planarizing set $E'$ of edges for $G$, with high probability computes a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A)\right )$ of $G$ into acceptable clusters, such that $E'\subseteq  E''$ and $| E''|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$.
\end{theorem}





\subsection{Canonical Drawings}
In this subsection, we assume that we are given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree at most $\Delta$, and a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A)\right )$ of $G$ into acceptable clusters. Next, we define drawings of $G\cup A$ that are ``canonical'' with respect to the clusters in the decomposition. Intuitively, in each such drawing, we require that the edges of type-2 acceptable clusters (clusters in $\cset_2$) do not participate in any crossings, and the edges of type-1 acceptable cluster (clusters in $\cset_1$) only participate in a small number of crossings (more specifically, we will define a subset $E^*(C)$ of edges for each cluster $C\in \cset_1$ that are allowed to participate in crossings). We then show that any drawing of $G$ can be transformed into such a canonical drawing of $G\cup A$, while only slightly increasing the number of crossings. This is sufficient in order to complete the proof of Theorem \ref{thm: main}, by adding to $E''$ the set $\bigcup_{C\in \cset_1}E^*(C)$ of edges. However, in order to be able to reduce the problem to the Crossing Number with Rotation System, we need stronger properties. We will define, for every cluster $C\in \cset_1\cup \cset_2$, a fixed drawing $\psi(C)$, and we will require that in the final drawing of $G\cup A$, the induced drawing of each such cluster $C$ is precisely $\psi(C)$. Additionally, for each cluster $C\in \cset_1\cup \cset_2$, and for each bridge $R\in \rset_G(C)$, we will define a disc $D(R)$ in the drawing $\psi(C)$ of $C$, and we will require that all vertices and edges of $R$ are drawn inside $D(R)$ in the final drawing of $G$. This will allow us to fix the locations of the clusters with respect to each other (that is, for each pair $C,C'$ of clusters, we will identify a face $F$ in the drawing $\psi(C)$ of $C$, and a face $F'$ in the drawing $\psi(C')$ of $C'$, such that, in the final drawing $\phi$ of the graph $G\cup A$, cluster $C'$ is drawn inside the face $F$ (of the drawing of $C$ induced by $\phi$), and similarly cluster $C$ is drawn inside the face $F'$.

We now proceed to define the drawings $\psi(C)$ of the clusters $C\in \cset_1\cup \cset_2$, and canonical drawings of the graph $G\cup A$ with respect to these clusters.


\subsubsection{Type-2 Acceptable Clusters}
Consider any type-2 acceptable cluster $C\in \cset_2$. Recall that $C$ has a unique planar drawing, denoted by $\rho_C$, and, from the definition of type-2 acceptable clusters, we have the following additional property: for every bridge $R\in \rset_{G\cup A}(C)$, there is a face $F$ of the drawing $\rho_C$, such that the vertices of $L(R)$ lie on the boundary of $F$ (we note that face $F$ is not uniquely defined; we break ties arbitrarily). We denote by $D(R)$ the open disc whose boundary is the boundary of $F$ in the drawing $\rho_C$.
Notice that for bridges $R\neq R'$, the discs $D(R),D(R')$ may not be disjoint.

\begin{definition}
	Let $\phi$ be any drawing of the graph $G\cup A$. We say that the drawing $\phi$ is \emph{canonical} with respect to the type-$2$ cluster $C\in \cset_2$ iff:
	\begin{itemize}
		\item the drawing of $C$ induced by $\phi$ is precisely $\rho_C$;
	\item the edges of $C$ do not participate in any crossings in $\phi$; and
	\item for every bridge $R\in \rset_{G\cup A}(C)$, all vertices and edges of $R$ are drawn inside the disc $D(R)$ (that is defined with respect to the drawing $\rho_C$ of $C$).
	\end{itemize}
\end{definition}

\subsubsection{Type-1 Acceptable Clusters}
Consider a cluster $C\in \cset_1$. %Recall that, from the definition of type-1 acceptable clusters, we are guaranteed that $|\Gamma(C)|\leq \mu$. 
%
%
%
%In this subsection, we show that we can find a drawing of $C\cup X_G(C)$ with relatively few crossings, and we will exploit this fact in the proof of Theorem~\ref{thm: from acceptable clusters to drawing} when dealing with type-1 acceptable clusters.
For convenience, we denote $\cset_1=\set{C_1,\ldots,C_q}$. We fix an arbitrary optimal drawing $\phi^*$ of the graph $G$. For each $1\leq i\leq q$, we denote by $\chi_i$ the set of all crossings $(e,e')$ such that either $e$ or $e'$ (or both) are edges of $E(C_i)$.   
The following observation is immediate.

\begin{observation}\label{obs: sum of chis}
$\sum_{i=1}^q|\chi_i|\leq 2\cdot\cro(\phi^*)=2\cdot\optcro(G)$. 
\end{observation}


Consider now some cluster $C_i\in \cset_1$. Let $e_i\in A$ be the unique fake edge that is embedded into $C_i$; if no such edge exists, $e_i$ is undefined. We set $C_i'=C_i\cup \set{e_i}$. Let $e_i=(x_i,y_i)$. Recall that edge $e_i$ belongs to some type-2 acceptable cluster $C$, and so $C$ contains a path $P_i$ connecting $x_i$ to $y_i$. Therefore, there must be a bridge $R_i\in \rset_{G\cup A}C_i'$ that contains $P_i\setminus \set{x_i,y_i}$, with $x_i,y_i\in L(R_i)$. 

Recall that the extension $X_{G\cup A}(C_i')$ (that is defined in Section \ref{sec:prelim}) is a collection of trees $\set{T_R\mid R\in \rset_{G\cup A}(C_i')}$. %Moreover, from the definition of the extension, for every tree $T_R$, the number of vertices whose degree in $T_R$ is greater than $2$ is bounded by $|L(R)|\leq |\Gamma(C_i)|\leq \mu$.
We denote by $C^+_i$ the graph obtained by the union of $C'_i$ and all trees in $X_{G\cup A}(C_i')$, namely $C^+_i=C_i'\cup \left(\bigcup_{R\in \rset_{G\cup A}(C_i)}T_R\right )$.
For every tree $T_R\in X_{G\cup A}(C_i')$, we denote by $\tilde E(R)$ the set of all edges of $T_R$ that are incident to the vertices of $L(R)$.  We use the following theorem in order to fix a drawing of each type-$1$ acceptable cluster $C_i$.

\begin{theorem}\label{thm: drawing of cluster extension-type 1}
	There is an efficient algorithm that computes, for every cluster $C_i\in \cset_1$, a subset $E^*(C_i)$ of at most $O(|\chi_i|\cdot\poly(\mu \Delta \log n))$ edges of $C_i$, and a drawing $\psi_i$ of $C_i^+$ with $ O\!\left(|\chi_i|\cdot \poly(\mu\Delta\log n)\right)$ crossings, such that the images of the edges in $E(C_i)\setminus E^*(C_i)$ do not participate in crossings. Additionally, the algorithm computes, for every tree $T_R\in X_{G\cup A}(C_i')$, a closed disc $D_{T_R}$, such that:
	\begin{itemize}
		\item for every vertex and edge of $C_i'$, its image in $\psi_i$ is disjoint from the interior of $D_{T_R}$;
		\item all vertices and edges of $T_R\setminus \tilde E(R)$ are drawn in the interior of $D_{T_R}$; 
		\item for every edge of $\tilde E(R)$, its image intersects the boundary of the disc $D_{T_R}$ exactly once; 
		\item the discs in $\set{D_{T_R}}_{T_R\in X_{G\cup A}(C'_i)}$ are mutually disjoint; and
		\item the image of the edge $e_i$ has a non-empty intersection with the boundary of the disc $D_{T_{R_i}}$, and this intersection is a contiguous curve.
	\end{itemize}
\end{theorem}

\mynote{Note that in addition to many notational changes, the above theorem requires the drawing to include the fake edge $e_i$, and the bridges are defined w.r.t. $G\cup A$. The latter is not a problem because every fake edge is embedded into some type-1 cluster, so bridges w.r.t. $G\cup A$ are same as bridges w.r.t. $G$. The former is a bit of a problem because we need to add the drawing of $e_i$ to the drawing of $G$. Because $e_i$ is contained in some type-2 cluster $C$, we can embed it into a real path $P_i$ in graph $G$, that does not contain any fake edges. This real path must be contained in a single bridge $R$. So we can route this edge along the boundary of the disc $D(T_R)$. Notice also that the theorem now requires that the edges of $E(C_i)\setminus E^*(C_i)$ do not participate in any crossings; previous version required that they don't cross each other.}

Let $E^*=\bigcup_{C_i\in \cset_1}E^*(C_i)$. Then, from Observation \ref{obs: sum of chis}:

\[
|E^*|\leq \sum_{C_i\in \cset_1}O\!\left(|\chi_i|\cdot \poly(\mu\Delta\log n)\right)\leq O\left (\optcro(G) \poly(\Delta\log n)\right ).
\]

We denote, for each type-$1$ acceptable cluster $C_i\in \cset_1$, by $\rho_{C_i}$ the drawing of $C_i$ that is induced by the drawing $\psi_i$ of $C_i^+$ (note that this drawing excludes the edge $e_i$).

\begin{definition}
	Let $\phi$ be any drawing of the graph $G\cup A$, and let $C_i\in \cset_1$ be a type-$1$ acceptable cluster. We say that $\phi$ is a \emph{canonical drawing} with respect to $C_i$, iff:
	\begin{itemize}
		\item the drawing of $C_i$ induced by $\phi$ is precisely $\rho_{C_i}$ (and in particular, the only edges of $C_i$ that participate in crossings are the edges of $E^*(C_i)$); and
		\item for every bridge $R\in \rset_{G\cup A}(C'_i)$, all vertices and edges of $R$ are drawn inside the disc $D_{T_R}$ (that is defined with respect to the drawing $\rho_{C_i}$ of $C_i$).
	\end{itemize}
\end{definition}

\mynote{need to decide between $D(R)$ and $D_{T_R}$, and also open/closed disc. There is a difference in definitions for type-1 and type-2 clusters: for type-2 clusters the boundary of the disc contains the vertices of $L(R)$, for type-1 it doesn't. Should make consistent.}



\subsubsection{Obtaining a Canonical Drawing}

%Recall that we are given a partition $(\cset_1,\cset_2)$ of all connected components of $H$ into type-1 and type-2 acceptable clusters, respectively. 
%\mynote{we need to be careful in that the boundary of $F$ may not be $2$-connected. We need to write this more carefully.}
%For a type-1 acceptable cluster $C\in \cset_1$, we denote by $\rho'_C$ the drawing of $C$ that is induced by the drawing of corresponding graph $C^+$ given by Corollary \ref{cor: drawing of cluster extension-type 1}. Recall that for every tree $T_R\in X_G(C)$, there is a disc $D_{T_R}$, such that, in the drawing of $C^+$ given by Corollary~\ref{cor: drawing of cluster extension-type 1}, $T_R\setminus \tilde E(R)$ is drawn inside the disc $D_{T_R}$ and graph $C$ is drawn outside $D_{T_R}$.


Our next result shows that there exists a near-optimal drawing of the graph $G$ that is canonical with respect to all clusters.


\begin{theorem}\label{thm: canonical drawing}
There is an efficient algorithm, that, given an $n$-vertex graph $G$ of maximum vertex degree at most $\Delta$, an arbitrary drawing $\phi$ of $G$, a decomposition  $\dset=\left ( E'',A,\cset_1,\cset_2,\pset(A))\right )$,  and, for each cluster $C\in \cset_1\cup \cset_2$, a drawing $\rho'_C$ as defined above, together with the set $\set{D_{T_R}}_{R\in X_G(C)}$ of discs, computes a drawing $\phi'$ of $G\cup A$ with $O(\cro(\phi)\cdot\poly(\Delta \log n))$ crossings, such that $\phi'$ is canonical with respect to every cluster $C\in \cset_1\cup \cset_2$. \mynote{to check: do we need $G$ to be $3$-connected in the proof?}
\end{theorem}


The proof of Theorem \ref{thm: canonical drawing} appears in Section \ref{sec:canonical drawing}.

\subsection{Completing the Proof of Theorem \ref{thm: main} for $3$-Connected Graphs}
Notice that the proof of Theorem \ref{thm: canonical drawing} concludes the proof of Theorem \ref{thm: main} for the special case where $G$ is a $3$-connected graph. Indeed, given a $3$-connected graph $G$, we use Theorem  \ref{thm: can find edge set w acceptable clusters} to compute a decomposition  $\dset=\left ( E'',\cset_1,\cset_2,A, \pset(C)\right )$ of $G$ into acceptable clusters, such that $E'\subseteq  E''$ and $| E''|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$. Next, we apply Theorem \ref{thm: drawing of cluster extension-type 1} to each type-1 cluster $C_i\in \cset_1$, to obtain the set $E^*(C_i)$ of edges, the drawing $\psi_i$ of $C_i$, and the discs $D_{T_R}$ for all trees $T_R\in X_G(C_i)$. Let $E^*=\bigcup_{C_i\in \cset_1}E^*(C_i)$, so $|E^*|\leq O\left (\optcro(G) \poly(\Delta\log n)\right )$, as observed above. The final outcome of the algorithm is the set $E''\cup E^*$ of edges. 
Observe that  $|E''\cup E^*|\leq O((| E'|+\optcro(G))\cdot\poly(\Delta\log n))$. Moreover, by using Theorem \ref{thm: canonical drawing} with the optimal drawing $\phi^*$ of $G$, we conclude that there exists a drawing $\phi'$ of $G\cup A$ with $O(\optcro(G)\cdot\poly(\Delta \log n))$ crossings, that is canonical with respect to all clusters in $\cset_1\cup \cset_2$. In particular, the only edges that may participate in crossings in $\phi'$ are edges of $E''\cup E^*$. By deleting the images of the fake edges from this drawing, we obtain the desired drawing of $G$.
%This concludes the proof of \ref{thm: main} for the special case where $G$ is a $3$-connected graph.


\iffalse
\begin{theorem}\label{thm: canonical drawing}
	There is an efficient algorithm, that, given an $n$-vertex graph $G$, a planarizing set $E''$ of its edges, a partition $(\cset_1,\cset_2)$ of all the connected components of the resulting graph $H=G\setminus E''$ into two subsets, a legal set $A_C$ of fake edges for each component $C\in \cset_2$, together with an embedding $\pset(A_C)$ of the edges in $A_C$ into $G$, such that (i) each cluster $C\in \cset_1$ is a type-1 acceptable cluster;
	(ii) For each cluster $C\in \cset_2$, $(C,A_C)$ is a type-2 acceptable cluster; and
	(iii) all paths in set $\bigcup_{C\in \cset_2}\pset(A_C)$ are mutually internally disjoint, together with an optimal drawing $\phi$ of $G$, computes a drawing $\phi'$ of $G$ with $O(\optcro(G)\cdot\poly(\Delta \log n))$ crossings, such that $\phi'$ is canonical with respect to every cluster $C\in \cset_1\cup \cset_2$.
\end{theorem}
\fi



\iffalse
We claim that the proof of Theorem~\ref{thm: canonical drawing} will conclude the proof of Theorem~\ref{thm: from acceptable clusters to drawing}. In fact, we simply set $E'''=E''\cup(\bigcup_{C_i\in \cset_1}E^*_i)$. Since $\sum_{C_i\in \cset_1}|E^*_i|=O(\optcro(G)\cdot \poly(\mu\Delta\log n))$, we get that $|E'''|=O(\optcro(G)+|E''|)\poly(\mu\Delta\log n)$. From the definition of canonical drawing and the definition of $E^*_i$, the drawing $\phi'$ obtained from Theorem~\ref{thm: canonical drawing} is in $\Phi_{E'''}(G)$.





\begin{theorem}\label{thm: from acceptable clusters to drawing}
There is an efficient randomized algorithm, that, given a $3$-connected graph with maximum vertex degree $\Delta$, and a decomposition $\dset=\left (E'',\cset_1,\cset_2,\bigcup_{C\in \cset_2}A_C,\bigcup_{C\in \cset_2}\pset(A_C)\right )$ of $G$ into acceptable clusters, computes a planarizing edge set $E'''\subseteq E(G)$, such that 
\begin{itemize}
\item $E''\subseteq E'''$;
\item $|E'''|\leq O((|E'|+\optcro(G))\cdot\poly(\Delta\log n))$; and
\item there is a drawing of $G$ in $\Phi_{E'''}(G)$ with at most $O(\optcro(G)\cdot\poly(\Delta\log n))$ crossings.
\end{itemize}
%$E''\subseteq E'''$ and $|E'''|\leq O(|E''|+\cro(G))\poly(\Delta\log n)$, and there is a drawing of $G$ in $\Phi_{E'''}(G)$ with at most $O(\optcro(G)\cdot\poly(\Delta\log n))$ crossings.
\end{theorem}
		
	\fi	
		

\subsection{Extensions to General Graphs}
In Section \ref{sec:non_3} we show how to extend the above proof of Theorem \ref{thm: main}  to general graphs, that are not necessarily $3$-connected. The extension builds on techniques that were introduced in \cite{chuzhoy2011graph}, combining them with Lemma \ref{lem:block_endpoints_routing}, that allows us to embed all fake edges of a given block decomposition into the input graph $G$, with low congestion. Additionally, in Section \ref{sec:non_3}, we prove the following theorem, that will be useful for our approximation algorithm.


\begin{theorem}
\label{thm:main_non_3}
Assume that there exists an efficient (possibly randomized) algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree $\Delta$, and a planarizing set $E'$ of its edges, computes a drawing of $G$ with at most $f(n,\Delta)\cdot(\optcro(G)+|E'|)$ crossings, for any function $f$ that is monotone increasing in both $n$ and $\Delta$. Then there exists an efficient (possibly randomized) algorithm that, given a (not necessarily 3-connected) graph $\hat{G}$ on $n$ vertices with maximum vertex degree $\Delta$,  and a planarizing set $\hat{E}'$ of its edges, computes a drawing of $\hat G$ with $O\left( f(n,\Delta)(\optcro(\hat G)+|\hat E'|)\cdot \poly(\Delta\log n)\right)$ crossings.
\end{theorem}


\subsection{Reduction to Crossing Number with Rotation System}

==> acceptable-clusters_backup.tex <==
\section{Proof Overview}

In this section we provide the high-level overview of the proof and state the main theorems from which the proof is inferred. We start by defining several central notions that our proof uses.



\mynote{An explanation why the things are set up this way and not the way we discussed. Our plan was to define an acceptable cluster like this:  a type-1 acceptable cluster has $\poly\log n$ terminals. A type-2 acceptable cluster is $3$-connected, good (no path connecting terminals lying on different faces), and terminals are well-linked. To get a planarizing set $\hat E$ of edges so that in $H=G\setminus \hat E$ every cluster is acceptable, we would follow these 3 steps:
(1) make all clusters good, under a suitable definition of good.
(2) do a well-linked decomposition.
(3) cut-off 2-cuts to get 3-connected components.
However, the third step does not actually work. If we start cutting off 2-vertex cuts we may end up creating new 2-vertex cuts that weren't there before. So type-2 acceptable clusters need to be defined differently. We need to allow to add fake edges that will replace the 2-vertex cuts we cut off, and the cluster itself with the fake edges should be 3-connected. This motivates the setup in this section.}


		
Let $G$ be an input graph, let $\hat E$ be any planarizing set of edges for $G$, and let $H=G\setminus \hat E$. We denote by $\cset=\cset(H)$ the set of all connected components of $H$, that we call \emph{clusters}. 
Recall that $\Gamma\subseteq V(G)$ is the set of all vertices that serve as endpoints of edges in $\hat E$; we call the vertices of $\Gamma$ \emph{terminals}. For every cluster $C\in \cset$, we denote by $\Gamma(C)=\Gamma\cap V(C)$ -- the set of terminals that lie in $C$.


Next, we define some desirable properties of these clusters. 

\begin{definition}
	We say that a cluster $C\in \cset$ is a \emph{type-1 acceptable cluster} iff $|\Gamma(C)|\leq \poly\log n$. \mynote{will need to specify the exact threshold later}
\end{definition}		

Consider now any cluster $C\in \cset$, and assume that it is not a type-1 acceptable cluster. We will sometimes need to augment such clusters by a set of \emph{fake} edges; the fake edges may or may not lie in $G$.

\begin{definition}
	Let $C\in \cset$ be a cluster, and let $A$ be any collection of fake edges (that is, $A$ is a collection of pairs $(u,v)$ of vertices $u,v\in V(C)$, where $u\neq v$). We say that $A$ is a \emph{legal set of fake edges for $C$} iff every fake edge $e=(u,v)$ connects a pair of terminals in $\Gamma(C)$. 
\end{definition}

Given a cluster $C\in \cset$, and a legal set $A$ of fake edges for $C$, an \emph{embedding} of the edges in $A$ is a collection of paths $\pset(A)=\set{P(e)\mid e\in A}$ in graph $G$, where for each edge $e=(u,v)\in A$, path $P(e)$ connects $u$ to $v$ in $G$, and the paths in $\pset(A)$ are internally disjoint from $C$.

\begin{definition}
	Let $C\in \cset$ be any cluster, and let $A$ be a legal  set of fake edges for $C$. We say that $(C,A)$ is a \emph{acceptable cluster of type-2} iff the following conditions hold:
	
	\begin{itemize}
		\item $C\cup A$ is a simple $3$-connected graph, or it is a $K_3$. In particular, $C\cup A$ has a unique planar drawing denoted by $\rho_{C\cup A}$. Note that this planar drawing induces a planar drawing of $C$, that we denote by $\rho'_C$;
		\item for every bridge $R\in \rset_G(C)$, there is a face $F$ in the drawing $\rho'_C$, such that the set $L(R)$ of vertices that are the legs of the bridge lie on the boundary of $F$ \mynote{since $C$ is no longer $3$-connected, the boundary is no longer a simple cycle, we count all stuff hanging from that cycle as part of boundary. Not sure if this needs additional explanation}; and
		\item the set $\Gamma(C)$ of terminals is $\alpha$-well-linked in $C$, for $\alpha=1/\poly\log n$; \mynote{need to set $\alpha$}
	%	\item if $Q$ is any path in $G$ whose endpoints lie in $C$, such that $Q$ is internally disjoint from $C$, then the endpoints of $Q$ are terminals that lie on the boundary of a single face of the drawing $\rho_{C\cup A}$.
	\end{itemize}
\end{definition}
		
		
		
		

\subsection{Main Theorems}
\label{subsec: main technical theorems}

The remainder of the proof consists of two main theorems.


\begin{theorem}\label{thm: can find edge set w acceptable clusters}
	There is an efficient algorithm, that, given a $3$-connected graph $G$ and a planarizing set $E'$ of edges for $G$, computes a set $E''$ of edges with $E'\subseteq E''$, a partition $(\cset_1,\cset_2)$ of all connected components of the resulting graph $H=G\setminus E''$ into two subsets, a legal set $A_C$ of fake edges for each component $C\in \cset_2$, together with an embedding $\pset(A_C)$ of the edges in $A_C$ into $G$, such that:
	
	\begin{itemize}
		\item Each cluster $C\in \cset_1$ is a type-1 acceptable cluster;
		\item For each cluster $C\in \cset_2$, $(C,A_C)$ is a type-2 acceptable cluster; and
		\item All paths in set $\bigcup_{C\in \cset_2}\pset(A_C)$ are mutually disjoint, and for all $C\in \cset_2$, the paths in $\pset(A_C)$ are internally disjoint from $C$.
	\end{itemize} 
\end{theorem}


\mynote{this theorem replaces Theorem \ref{thm:ideal_drawing}}
\begin{theorem}\label{thm: from acceptable clusters to drawing}
	Let $G$ be a $3$-connected graph and let $E''$ be a planarizing edge set for $G$. Assume further that we are given a partition $(\cset_1,\cset_2)$ of all connected components of the resulting graph $H=G\setminus E''$ into two subsets, a legal set $A_C$ of fake edges for each component $C\in \cset_2$, together with an embedding $\pset(A_C)$ of the edges in $A_C$ into $G$, such that (i) each cluster $C\in \cset_1$ is a type-1 acceptable cluster;
		(ii) For each cluster $C\in \cset_2$, $(C,A_C)$ is a type-2 acceptable cluster; and
		(iii) All paths in set $\bigcup_{C\in \cset_2}\pset(A_C)$ are mutually disjoint. Then there is a drawing of $G$ in $\Phi_{E''}(G)$ with at most $O(\cro(G)\poly\log n)$ crossings.
\end{theorem}
		
		
		




==> accounting.tex <==
\subsection{Bounding the number of crossings in $\psi_{\tG}$}
\label{subsec:accounting}

In this section we analyze the number of crossings in the drawing $\psi_{\tG}$ that we produce in the algorithm. 
We first summarize the algorithm and recall the key properties. 
We start with $\tG$ as the initial instance.
\begin{enumerate}
\item If the current instance $G'$ is in the recursion base case, that is, there is no vertex in $G'$ with degree above $\cro^{1-\eps}$, and we can efficiently compute a drawing $\psi_{G'}\in \Phi(G',\Sigma)$ such that $\cro(\psi_{G'})\le \tilde{O}(\optcro(G')+\cro^{1-\eps}\cdot|E(G')|)$.
\item If the current instance $G'$ is decomposed into sub-instances $G_1, G_2$ through Case 1, then we have $|E(G_1)|, |E(G_2)|\ge \cro^{1-\eps}/3$ (from Observation~\ref{RS_obs:case_1}). And given the drawings $\psi_{G_1}$ and $\psi_{G_2}$ of sub-instances $G_1$ and $G_2$, respectively, we can efficiently compute a drawing $\psi_{G'}\in \Phi(G',\Sigma)$ such that $\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+\cro^{1-2\eps}\cdot |E(G')|$.
\item If the current instance $G'$ is decomposed into sub-instances $G_1, G_2$ through Case 2, then with probability $O(\cro^{-\eps})$, we have $|E(G_1)|, |E(G_2)|\ge \Omega(\cro^{1-2\eps})$ (from Observation~\ref{RS_obs:case_2.1} and Observation~\ref{RS_obs:case_2.2}). And given the drawings $\psi_{G_1}$ and $\psi_{G_2}$ of sub-instances $G_1$ and $G_2$, respectively, we can efficiently compute a drawing $\psi_{G'}\in \Phi(G',\Sigma)$ such that $\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+O(\cro^{1-3\eps})\cdot |E(G')|$. Here we use that $\eps<1/8$.
%\item If the current instance $G'$ is decomposed into smaller sub-instances $G_1, G_2$ through Case 2.2, the with probability $O(\cro^{-\eps})$, we have $|E(G_1)|, |E(G_2)|\ge \Omega(\cro^{1-2\eps})$ (from Observation~\ref{RS_obs:case_2.2}). and given the drawings $\psi'_{G_1}$ and $\psi'_{G_2}$ of sub-instances $G_1$ and $G_2$, respectively, we can efficient compute a drawing $\psi'_{G'}\in \Phi(G',\Sigma)$ such that $\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+O(\cro^{1-3\eps})\cdot |E(G')|$.
\end{enumerate}
\begin{figure}[h]
	\label{fig:recursion}
	\centering
	\subfigure[An illustration of the recursion algorithm. The recursion bases are shown in red.]{\scalebox{0.3}{\includegraphics{recursion_illustration}}}
	\caption{An illustration of the skeleton-contraction step.} 
\end{figure}
See Figrue~\ref{fig:recursion} for an illustration of the whole algorithm. We call the tree in Figrue~\ref{fig:recursion} the \emph{decomposition tree} of the algorithm.
From the above summary, the only randomized part of the algorithm is instance-decomposition through Case 2. 
The algorithm fails happens if the events stated in the probabilistic arguments in Claim~\ref{clm:skeleton}, Claim~\ref{clm:region_intersection} and Claim~\ref{clm:left_right_envelope} do not hold.
Now we argue that the algorithm does not fail with probability above $0.99$.
From the above summary, it is clear the number of instance-decompositions through Case 2 is at most $O(\cro^{2\eps})$. On the other hand, the probability that the bad events happen in Claim~\ref{clm:skeleton}, Claim~\ref{clm:region_intersection} and Claim~\ref{clm:left_right_envelope} is $\cro^{-2\eps}$. Therefore, we can choose the constants wisely to make sure that the probability that the bad events never happen is above $0.99$.

We now proceed to bound the number of crossings in $\psi'_{\tG}$. 
We denote by $\gset$ the set of all base instances. For a non-base instance $G'$, we denote by $\gset_{G'}$ the set of subsequent base instances that is obtained from decomposing $G'$.
First, since each non-base instance contains at least $\Omega(\cro^{1-\eps})$ edges, there are at most $O(\cro^{\eps})$ many of them. Therefore, the level of the recursion is bounded by $O(\cro^{\eps})$. 
Recall that in Case 1, when $G'$ is decompose into $G_1$ and $G_2$, we do not create any new difficult edges, while in Case 2 we may create at most $\tilde O(\cro^{5\eps})$ new difficult edges. So the total number of difficult edges in all base graphs are at most $O(\cro^{6\eps})$. Therefore, if we denote by $\gset$ the set of all instances and denode by $\gset_b$ the set of all base instances, then $\sum_{G'\in \gset}\optcro(G')=\optcro(\tG)+O(\cro^{6\eps})\cdot |E(\tG)|$.

Now we bound the number of crossings in $\psi'_{\tG}$ via a charging scheme. We start from $\tG$ and follows the decomposition tree of the algorithm, we will charge the edges in the sub-instances for the number of crossings in the drawing produced by the algorithm. At the end, we will sum up all the charges and reach a bound on $\cro(\psi_{\tG})$.
We now describe the charging scheme. 
\begin{enumerate}
\item If the current instance $G'$ is a base-instance, then we charge $\cro^{1-\eps}$ to every edge in $G'$, and we call this \emph{type-0 charge}. Note that, once an edge is type-0 charged, then it will not be further charged anymore. Therefore, each edge is type-0 charged at most once.
\item If the current instance $G'$ is a decomposed into sub-instances $G_1, G_2$ through Case 1, then we charge a total of $\cro^{1-2\eps}\cdot|E(G')|$ uniformly to every edge in $G_1$ and $G_2$, and we call this \emph{type-1 charge}.
Therefore, each edge is charged $O(\cro^{1-2\eps})$ every time it is type-1 charged.
Note that, once an edge is type-1 charged, then the size of the instance that it belongs to decreases by at least $\cro^{1-3\eps}/3$. Therefore, an edge is type-1 charged at most $O(\cro^{\eps})$ times.
\item If the current instance $G'$ is a decomposed into sub-instances $G_1, G_2$ through Case 2, then we charge a total of $O(\cro^{1-3\eps}\cdot|E(G')|)$ uniformly to every edge in $G_1$ and $G_2$, and we call this \emph{type-2 charge}.
Therefore, each edge is charged $O(\cro^{1-3\eps})$ every time it is type-2 charged.
Note that, once an edge is type-2 charged, then the size of the instance that it belongs to decreases by at least $\Omega(\cro^{1-2\eps})$. Therefore, an edge is type-2 charged at most $O(\cro^{2\eps})$ times.
\end{enumerate}

It not hard to see that every edge is type-0 charged $O(\cro^{1-\eps})$ in total, is type-1 charged $O(\cro^{1-\eps})$ in total, and is type-2 charged $O(\cro^{1-\eps})$ in total. Therefore, each edge is charged $O(\cro^{1-\eps})$ in all types in total. On the other hand, from the charging scheme, it is clear that $\cro(\psi_{\tG})$ can be bounded by the sum of $\sum_{G'\in \gset}\optcro(G')$ and the total charge received by all edges. Since $\sum_{G'\in \gset}\optcro(G')=\optcro(\tG)+O(\cro^{6\eps})\cdot |E(\tG)|$, and the total charge received by all edges is $O(\cro^{1-\eps})\cdot |E(\tG)|$, we conclude that:
\[\cro(\psi_{\tG})\le \optcro(\tG)+O(\cro^{6\eps})\cdot |E(\tG)|+ O(\cro^{1-\eps})\cdot |E(\tG)|= \tilde{O}\left(\optcro(\tG)+ \optcro(\tG)^{1-\eps}\cdot |E(\tG)|\right).\] 
This completes the proof of Theorem~\ref{thm: main_rot}.













\iffalse
\begin{claim}
\label{clm:accounting}
For each instance $G'$, $\cro(\psi_{G'})\le \sum_{H\in \gset_{G'}}\optcro(H)+(a\cdot\cro^{1-\eps}+b\cdot d_{G'}\cdot\cro^{1-2\eps})\cdot|E(G')|$, where $a$ and $b$ are universal constants and $d_{G'}$ is number of non-base nodes in the subtree rooted at $G'$ of the recursion tree.
\end{claim}
Since $d(\tG)\le \cro^{1-\eps}$ this claim implies that:
\[
\begin{split}
\cro(\psi_{\tG}) & \le \sum_{G'\in \gset}\optcro(G')+O\left(\cro^{1-\eps}\right)\cdot|E(\tG)|\\
 & \le \optcro(\tG)+O(\cro^{6\eps})\cdot |E(\tG)|+O\left(\cro^{1-\eps}\right)\cdot|E(\tG)|\\
 & \le \tilde O\left( \optcro(\tG)+\optcro(\tG)^{1-\eps}\cdot|E(\tG)|\right),
\end{split}\]
and therefore completes the proof of Theorem~\ref{thm: main_rot}.

We now prove Claim~\ref{clm:accounting} by induction according to the recursion tree as shown in Figure~\ref{fig:recursion}.
The base case is where $G'$ is a base-instance. Recall that, in the recursion base case we compute a drawing $\psi_{G'}$ with $\optcro(G')+a\cdot\cro^{1-\eps}\cdot|E(G')|$. Therefore, the claim holds. Assume the claim holds for each child-instance of $G'$ in the recursion tree, consider now the instance $G'$. It is decomposed through Case 1 or Case 2. In either case, it is decomposed into $G_1$ and $G_2$, and we compute a drawing $\psi_{G'}$ such that
$\cro(\psi_{G'})\le \cro(\psi_{G_1})+\cro(\psi_{G_2})+b\cdot \cro^{1-2\eps}\cdot |E(G')|$. From the induction hypothesis, and since $\gset_{G'}=\gset_{G_1}\cup \gset_{G_2}$ and $d_{G'}=d_{G_1}+d_{G_2}+1$, we have
\[
\begin{split}
\cro(\psi_{G'}) & \le \cro(\psi_{G_1})+\cro(\psi_{G_2})+b\cdot\cro^{1-2\eps}\cdot |E(G')|\\
& \le
\sum_{H\in \gset_{G_1}}\optcro(H)+a\cdot\cro^{1-\eps}\cdot|E(G_1)|+b\cdot d_{G_1}\cdot\cro^{1-2\eps}\cdot |E(G_1)|\\ & +\sum_{H\in\gset_{G_2}}\optcro(H)+a\cdot\cro^{1-\eps}\cdot|E(G_2)|+b\cdot d_{G_2}\cdot\cro^{1-2\eps}\cdot |E(G_2)|+b\cdot\cro^{1-2\eps}\cdot |E(G')|\\
& \le
\sum_{H\in \gset_{G'}}\optcro(H)+(a\cdot\cro^{1-\eps}+b\cdot d_{G'}\cdot\cro^{1-2\eps})\cdot|E(G')|.
\end{split}
\]
This completes the proof of Claim~\ref{clm:accounting}, and therefore completes the proof of Theorem~\ref{thm: main_rot}.


\fi













==> apd_drawing_type_1.tex <==
\section{Proof of Corollary~\ref{cor: drawing of cluster extension-type 1}}
\label{apd:drawing of cluster extension-type 1}

In this section we provide the proof of  Corollary~\ref{cor: drawing of cluster extension-type 1}.

We fix the index $i$. For simplicity, we denote $C_i$ by $C$, $C_i^+$ by $C^+$, and $\chi_i$ by $\chi$.
The edge set $E^*$ is obtained by directly applying Lemma~\ref{lem: type 1 drawing}. To obtain a drawing $\psi'$ of $C^+$, we start with the drawing $\psi$ of $C^+$ given by Lemma~\ref{lem: type 1 drawing}. We will iteratively process each bridge $R\in \rset_{G}(C)$, and finally obtain a drawing $\phi'$ that satisfies all conditions of Corollary~\ref{cor: drawing of cluster extension-type 1}. 
	
We now describe the execution of an iteration in detail.
For a bridge $R\in \rset_{G}(C)$, we let $T\in X_{G}(C)$ be the corresponding tree in the extension of $C$. Recall that $T'$ is obtained from $T$ by suppressing all degree-$2$ nodes, we denote its root by $r_{T'}$, and let $D_{r_{T'}}$ be a small disc around the image of $r_{T'}$ in $\psi$. We then place a planar drawing of whole tree $T'$ into this disc in a planar drawing, so that the vertices of $L(R)$ lie on the boundary of this disc.
Finally, we connect the image of the vertices of $L(R)$ in $\psi$ to the to the new copy of the vertices of $L(R)$ on the boundary of $D_{r_{T'}}$. This is done by following the images of the paths in $T'$ connecting it leaves to its root in the original drawing. Note that this may increase the number of crossings by at most a $O(\mu)$ factor, so the number of crossings in $\psi'$ is still bounded by $O\!\left(\chi_i\cdot \poly(\mu\Delta\log n)\right)$.






==> apd_good_block.tex <==
\section{Proof of Lemma~\ref{lem: good clusters cant be killed}}
\label{apd:good_cluster_preserving}

In this section we provide the proof of Lemma~\ref{lem: good clusters cant be killed}.

Assume for contradiction that the lemma is false. %, so there must be some pseudo-block $B_1\in \bset_{H'}$ that is bad. 
	Let $R\in \rset_G(\tilde B_1')$ be a witness for $B_1$.
	%Let $B_2\in \bset_H$ be the corresponding block given by Lemma \ref{lem: block containment}.
	Consider the unique planar drawing $\rho_{\tilde B_2}$ of $\tilde B_2$. Since every vertex and every real edge of $\tilde B_1$ lies in $\tilde B_2$, this drawing naturally induces a drawing of $\tilde B_1'$. For convenience, we denote by $\rho'$ the drawing of $\tilde B_1'$ induced by $\rho_{\tilde B_2}$, and denote by $\rho''=\rho'_{\tilde B_1'}$ the drawing of $\tilde B_1'$ induced by $\rho_{\tilde B_1}$. We start with the following claim.
	
	\begin{claim}\label{claim: identical drawings}
		The drawings $\rho'$ and $\rho''$ of $\tilde B_1'$ are identical. %\snote{$\rho''$ is not defined}
	\end{claim}
	\begin{proof}
		Let $A$ be the set of all fake edges of $\tilde B_1$, so that $\tilde B_1'=\tilde B_1\setminus A$.
		Consider the drawing $\rho'$ of $\tilde B_1'$. We will show that we can augment this drawing by adding drawings of the edges in $A$, so that the resulting drawing remains planar. Note that, if this is true, then it follows that $\rho'=\rho''$. To see this, note that $\tilde B_1$ is $3$-connected, so it has a unique planar drawing, and therefore the resulting drawing of $\tilde B_1$ is identical to $\rho_{\tilde B_1}$. It is clear both $\rho'$ and $\rho''$ are obtained from the drawing $\rho_{\tilde B_1}$ of $\tilde B_1$ by deleting the images of the fake edges from it. Therefore, $\rho'=\rho''$.
		
		From now on, it is enough to show that we can augment the drawing $\rho'$ by adding the images of edges in $A$ to it, while preserving the planarity. Recall that Lemma \ref{lem: block containment} defines, for every fake edge $e=(u,v)\in A$, a path $P(e)$ in $\tilde B_2$ that connects $u$ to $v$, and is internally disjoint from $V(\tilde B_1)$. Moreover, if $e$ and $e'$ are distinct fake edges in $A$, then their corresponding paths $P(e)$ and $P(e')$ are internally disjoint. Recall that these paths are allowed to contain fake edges of $\tilde B_2$, and that if graph $\tilde B_1$ contains a real edge connecting the endpoints of $B_2$, then the resulting paths in $\set{P(e)\mid e\in A}$ do not contain an edge connecting the endpoints of $B_2$. Therefore, we can simply map every fake edge $e\in A$ to the curve corresonding to the concatenation of curves that the edges of $P(e)$ are mapped to in $\rho_{\tilde B_2}$. Since the drawing $\rho_{\tilde B_2}$ of $\tilde B_2$ is planar, we obtain a planar drawing of $\tilde B_1$.
	\end{proof}
	
	
	Let $\fset$ be the set of all faces in the drawing $\rho'=\rho''$. 
	For every vertex $v\in V(\tilde B_2)\setminus V(\tilde B_1)$, there is a unique face $F(v)\in \fset$, such that the image of vertex $v$ in $\rho_{\tilde B_2}$ lies in the interior of the face $F$.
	
	Recall that $T_R$ is the tree with smallest number of edges among all trees in $R$ whose leaves are precisely the vertices of $L(R)$. 
	Assume first that $V(T_R)\cap V(\tilde B_2)=L(R)$. In this case, there is some bridge $R'\in \rset_G(\tilde B_2')$ of $\tilde B_2'$ that contains the tree $T_R$, and so $L(R)\subseteq L(R')$. Since $B_2$ is a good block, there must be a face in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B'_2$ whose boundary contains all vertices of $L(R)$. Therefore, for some face $F\in \fset$, all vertices of $L(R)$ must lie on the boundary of $F$. 
	
	Assume now that there is some vertex $v\in V(T_R)\cap  V(\tilde B_2)$ that does not lie in $L(R)$. Let $F=F(v)$ be the face of $\fset$ in whose interior the image of $v$ in $\rho_{\tilde B_2}$ lies. We will show that all vertices of $L(R)$ must lie on the boundary of $F$, leading to a contradiction. Let $u$ be an arbitrary vertex of $L(R)$. It suffices to show that $u$ must lie on the boundary of the face $F$.
	
	Let $P\subseteq T_R$ be the unique path connecting $v$ to $u$ in $T_R$. Since the leaves of tree $T(R)$ are precisely the vertices of $L(R)$, except for $v$, every vertex $x$ of $P$ lies outside $V(\tilde B_1)$, and the image of $x$ in $\rho_{\tilde B_2}$ lies in the interior of some face in $\fset$. Let $u=v_1,v_2,\ldots,v_r=v$ be all vertices of $P$ that belong to $V(\tilde B_2)$, and assume that they appear on $P$ in this order. 
	It remains to prove the following observation.
	
	\begin{observation}
		For $1\leq i<r-1$, $F(v_i)=F(v_{i+1})$. Moreover, $v_r$ lies on the boundary of $F(v_{r-1})$.
	\end{observation}
	\begin{proof}
		Fix some $1\leq i\leq r-1$. Assume that the observation is false.
		Then there is some face $F'\in \fset$, such that $v_i$ lies in the interior of $F'$, but $v_{i+1}$ does not lie in the interior or on the boundary of $F'$ (the latter case is only relevant for $i=r-1$). Therefore, $v_i$ and $v_{i+1}$ cannot lie on the boundary of the same face in the drawing $\rho'_{\tilde B_2'}$. 
		
		Let $\sigma_i$ be the subpath of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge connecting $v_i$ and $v_{i+1}$, then it is a bridge in $\rset_G(\tilde B_2')$, and, since $B_2$ is a good block, the endpoints of $\sigma_i$ must lie on the boundary of a single face of the drawing $\rho'_{\tilde B_2'}$, a contradiction. Otherwise, let $\sigma'_i$ be obtained from $\sigma_i$ by deleting the two endpoints from it. Then there must be a bridge $R'\in \rset_G(\tilde B_2')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. But then there must be a face $F'$ of the drawing $\rho_{\tilde B_2}$ whose boundary contains $v_i$ and $v_{i+1}$, leading to a contradiction. 
		%	We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B_2'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B_1'\subseteq \tilde B_2'$, and from the way the drawing $\rho'_{\tilde B_1'}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B_1'}$ that contains $F_i$.	
\end{proof}


\iffalse
For each $1\leq i<r$, let $\sigma_i$ be the segment of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge connecting $v_i$ and $v_{i+1}$, then it is a bridge in $\rset_G(\tilde B_2')$, and, since $B_2$ is a good block, the endpoints of $\sigma_i$ must lie on the boundary of a single face of the drawing $\rho_{\tilde B_2}$. Otherwise, let $\sigma'_i$ be obtained from $\sigma$ by deleting the two endpoints from it. Then there must be a bridge $R'\in \rset_G(\tilde B_2')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. But then there must be a face $F'$ of the drawing $\rho_{\tilde B_2}$ whose boundary contains $v_i$ and $v_{i+1}$. 
We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B_2'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B_1'\subseteq \tilde B_2'$, and from the way the drawing $\rho'_{\tilde B_1'}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B_1'}$ that contains $F_i$. Since $v_1,\ldots,v_{r-1}$ do not belong to graph $\tilde B_1'$, we get that $F_1,F_2,\ldots,F_{r-1}$ must all be contained in the same face $F=F(v)$ of $\fset$, proving that $u$ must lie on the boundary of $F$.\fi



==> blocks.tex <==
\section{Blocks and Block Decompositions}

\mynote{should be moved to prelims}

We use the following definitions from \cite{chuzhoy2011graph}.

\begin{definition}
	Let $G=(V,E)$ be a $2$-connected graph. 
	A subgraph $B=(V',E')$ of $G$ is called a \emph{block} iff: 
	
	\begin{itemize}
		\item $V\setminus V'\neq\emptyset$ and $|V'|\geq 3$;
		\item There are two special vertices $u,v\in V'$, called \emph{block end-points} and denoted by $I(B)=(u,v)$, such that there are no edges from $V\setminus V'$ to $V'\setminus\set{u,v}$ in $G$. All other vertices of $B$ are called \emph{inner vertices}; 
		
		\item  $B$ is the subgraph of $G$ induced by $V'$, except that it {\bf does not} contain the edge $\{u,v\}$ even if it is present in $G$.
	\end{itemize}
\end{definition}

Notice that every $2$-separator $(u,v)$ of $G$ defines at least two internally disjoint blocks $B',B''$ with $I(B'),I(B'')=(u,v)$.

Let $\fset$ be a collection of sub-graphs of $G$. We say that $\fset$ is \emph{laminar} iff for every pair $H,H'\in \fset$ of subgraphs, either $H\cap H'=\emptyset$, or $H\subseteq H'$, or $H'\subseteq H$ hold. Given a laminar collection $\fset$ of subgraphs of $G$ with $G\in \fset$, we can associate a tree $\tset(\fset)$ with it, called a \emph{decomposition tree}, as follows. For every graph $H\in \fset$, there is a vertex $v(H)\in \tset$. The tree is rooted at the vertex $v(G)$. For every pair $H,H'\in \fset$ of subgraphs, such that $H\subsetneq H'$, and there is no other graph $H''\in \fset\setminus\set{H,H'}$ with $H\subsetneq H''\subsetneq H'$, there is an edge $(v(H),v(H'))$ in the tree, and $v(H')$ is the parent of $v(H)$ in $\tset$.


Assume now that we are given a laminar family of sub-graphs of $G$ with $G\in \fset$, and let $\tset=\tset(\fset)$ be the decomposition tree associated with $\fset$. Assume further that every graph  $B\in \fset\setminus\set{G}$ is a block. For each such graph $B\in \fset$,  we will denote by $\tilde{B}$ the graph obtained as follows. First, for each child $v(B')$ of $v(B)$ in $\tset(\fset)$, we delete all edges and vertices of $B'$ from $B$, except for the endpoints $I(B')$. We then add an artificial edge connecting the vertices of $I(B')$ to $B$.
The resulting graph, obtained after processing every child vertex of $B$, is denoted by $\tilde B$. Additionally, we denote by $\tilde{B}'$ the graph obtained from $\tilde{B}$ by adding an artificial edge connecting the endpoints of $B$ (if $B=G$ then $\tilde B'=\tilde B$). We note that the definitions of $\tilde B$ and $\tilde B'$ depend on the family $\fset$ so when using these definitions we will always fix some such family. We are now ready to define a block decomposition.


\begin{definition}
	Let $\fset$ be a laminar family of sub-graphs of $G$ with $G\in \fset$, and let $\tset=\tset(\fset)$ be the decomposition tree associated with $\fset$. We say that $\fset$ is a \emph{block decomposition} of $G$, iff:
	
	\begin{itemize}
		\item Every graph $B\in \fset\setminus\set{G}$ is a block;
		
		\item For each graph $B\in \fset$, graph $\tilde{B}'$ is $3$-connected (we use the convention that the triangle graph, $K_3$, is 3-connected); and
		\item If a block $B\in \fset$ has exactly one child $B'$ then $I(B) \neq I(B')$.
	\end{itemize} 
\end{definition}


The following theorem was shown in \cite{chuzhoy2011graph}.

\begin{theorem}[Theorem 12 in the arxiv version of \cite{chuzhoy2011graph}]\label{thm: block decomposition} 
	There is an efficient algorithm, that, given a $2$-connected graph $G=(V,E)$ with $|V|\geq 3$, computes a block decomposition $\fset$ of $G$, such that the following holds. 
	Every vertex $v\in V$ that participates in any $2$-separator $(u,v)$ of $G$ is either an endpoint of a block $B\in\cal F$, or $d_G(v) = 2$ and there is an edge $(u,v)\in E$, such that $u$ is an endpoint of a block $B\in\cal F$.
\end{theorem}



==> computing-acceptable-decomposition-backup.tex <==

		
		
\section{Proof of Theorem \ref{thm: can find edge set w acceptable clusters}}	
\subsection{Pseudo-Terminals, Good Blocks and Good Clusters}
\label{sec: good blocks and acceptable clusters}

Throughout this section, we assume that we are given some planarizing set $\hat E$ of edges for the input graph $G$, that is, $G\setminus \hat E$ is planar. We note that $\hat E$ is not necessarily the same as the original planarizing set $E'$, since, as the algorithm progresses, we may add edges to the planarizing set. The definitions in this section refer to any planarizing set $\hat E$ that may arise over the course of the algorithm.

Given a planarizing set $\hat E$ of edges for $G$, let $H=G\setminus \hat E$. We say that a vertex $v$ of $H$ is a \emph{terminal} iff it is incident to some edge in $\hat E$. 
Recall that we have defined a block decomposition of a graph $H$, as follows. First, we denoted by $\cset(H)$ the set of all connected components of $H$; we refer to the elements of $\cset(H)$ as \emph{clusters}. For each cluster $C\in \cset$, we have defined a collection $\zset(C)$ of super-blocks: maximal $2$-connected subgraphs of $C$, and we denoted by $\zset_H=\bigcup_{C\in \cset(H)}\zset(C)$. Lastly, for each superblock $Z\in \zset_H$, we let $\lset(Z)$ be the block decomposition of $Z$ given by Theorem \ref{thm: block decomposition}, and we denoted by $\bset(C)=\bigcup_{Z\in \zset(C)}\lset(Z)$ the resulting collection of pseudo-blocks for cluster $C$. Finally, the block decomposition of $H$ is  $\bset_H=\bigcup_{C\in \cset}\bset(C)$.
 
 
 
\paragraph{Pseudo-terminal.}
Consider some cluster $C\in \cset(H)$, some super-block $Z\in\zset(C)$, and let $\lset=\lset(Z)$ be the block decomposition of $Z$.
Let $B\in \lset(Z)$ be any pseudo-block in this decomposition.  

We start by defining a set $\hat T(B)$ of \emph{pseudo-terminals} for $B$, as follows. First, we add to $\hat T(B)$ all terminals lying in $B$, that is, the vertices of $T\cap V(B)$. 
Additionally, for every child vertex $v(B')$ of $v(B)$ in the tree $\tset(\lset)$, we add both endpoints of the block $B'$ to $\hat T(B)$. 
If $B$ is an actual block (that is, $v(B)$ is not the root vertex of the decomposition tree $\tset(\lset)$),  then we also add the endpoints of $B$ to $\hat T(B)$. 
This concludes the definition of the set $\hat T(B)$ of pseudo-terminals for $B$. Note that, in additional to actual terminals, the set $\hat T(B)$ of pseudo-terminals contains, for every graph $B'\in \nset(B)$, the endpoints of $B'$ (where for the complement $B^c$ of $B$, the endpoints are $I(B)$.

\paragraph{Contracted Graph $J^B$.}
Next, we need to define a contracted graph $J^B$ associated with $B$. 
In order to do so, we start with the graph $G$, and then contract some of its connected sub-graphs. Specifically, 
consider a graph $B'\in \nset(B)$, and let $(u',v')$ be its endpoints (if $B'=B^c$ then the endpoints are $I(B)$; otherwise, $B'$ is a child block of $B$ and its endpoints are defined as usual). Observe that $B'\setminus \set{v'}$ must be a connected graph, since the super-block $Z$ containing $B$ is $2$-connected. We contract all vertices of $B'\setminus\set{v'}$, obtaining a super-node, that we still denote by $u'$. Once all graphs $B'\in \nset(B)$ are processed, we obtain the final graph $J^B$. Observe that every super-node of $J^B$ corresponds to some pseudo-terminal of $\hat T(B)$ (but not every pseudo-terminal is necessarily a super-node). We will not distinguish between the supernode and the corresponding pseudo-terminal. It is immediate to verify that $V(\tilde B)\subseteq V(J^B)$. Moreover, $E(\tilde B)\subseteq E(J^B)$ (we do not distinguish between real and artificial edges of $\tilde B$ here). However, graph $J^B$ may contain some additional vertices (all vertices of $V(J^B)\setminus V(B)$ must lie in $V(G)\setminus V(Z)$, and additional edges (for each such edge, each of its endpoints is either a pseudo-terminal of $\hat T(B)$, or it lies in $V(G)\setminus V(Z)$.



\paragraph{Good Pseudo-Blocks.}
We are now ready to define good pseudo-blocks. Consider some pseudo-block $B\in \bset_H$, and consider the unique planar drawing $\rho_{\tilde B}$. If there is a path $P$ graph $J^B$ that is internally disjoint from $V(\tilde B)$, whose endpoints are pseudo-terminals of $\hat T(B)$ that do not lie on the boundary of the same face in $\rho_{\tilde B}$, then pseudo-block $B$ is \emph{bad}, and the path $P$ is called the \emph{witness path}. If pseudo-block $B$ is not bad then it is called \emph{good}.


\iffalse
Recall that we have defined a $3$-connected graph $\tilde B'$ associated with the graph $B$ (based on the block decomposition $\lset$). Recall that, from Observation \ref{obs: block in 2-connected graph is planar} $\tilde B'$ has a unique planar drawing, that we denote by $\rho_{\tilde B'}$. 

\begin{definition}
	Consider some pseudo-block $B\in \bset$. We say that $B$ is a \emph{bad pseudo-block} iff there are two pseudo-terminals $t,t'\in \hat \tset(B)$ that do not lie on the boundary of the same face in the drawing $\rho(\tilde B')$, and there is a path $P$ in $G$ connecting $t$ to $t'$, such that $P$ does not contain the vertices of $\tilde B'$ as inner vertices. A pseudo-block that is not bad is called \emph{good}.
	\end{definition}

\fi


\paragraph{Good Clusters.}
Finally, we define good clusters.

\begin{definition}
	We say that a cluster $C\in \cset$ is \emph{good} iff pseudo-block $B\in \bset(C)$ is good.
\end{definition}



Recall that we start with some planarizing set $E'$ of edges, and then, over the course of several steps, we add additional edges to set $E'$. Suppose that at some point we compute a planarizing set $\hat E$ of edges, such that in graph $G\setminus \hat E$, every cluster is good. As the algorithm progresses, and more edges are added to $\hat E$, we would like to claim that this property continues to be preserved. The following lemma allows us to do so.

\begin{lemma}\label{lem: good clusters cant be killed}
Suppose we are given two planarizing sets $\hat E,\hat E'$ of edges, with $\hat E\subseteq \hat E'$. Let $H=G\setminus\hat E$ and $H'=G\setminus \hat E'$, so that $H'\subseteq H$. Assume that every cluster in $\cset(H)$ is good. Then every cluster in $\cset(H')$ is good as well. 
\end{lemma}

\begin{proof}
	Assume for contradiction that the lemma is false, so there must be some pseudo-block $B'\in \bset_{H'}$ that is bad. Let $B\in \bset_H$ be the corresponding block given by Lemma \ref{lem: block containment}.
	We denote by $Z'\in \zset(H')$ the super-block containing $B'$, and we denote by $Q$ the witness path for $B'$.
	Let $(e_1,e_2,\ldots,e_r)$ be the sequence of edges on the path $Q$, and let $x=v_1,v_2,\ldots,v_{r+1}=y$ be the sequence of vertices of $Q$. Recall that every inner vertex of $Q$ must lie in $V(G)\setminus Z$, and hence each such vertex belongs to the graph $J^{B'}$ associated with $B'$ (and is not part of a super-node). However, $x$ may either be a regular vertex of $J^{B'}$, or it may be a super-node of $J^{B'}$; in the latter case, edge $(x,v_1)$ may not belong to $G$. In the former case, we denote $x'=x$, and in the latter case, we let $x'$ be the endpoint of $e_1$ that was contracted into the super-node $x$. We define vertex $y'$ for $y$ similarly, so that the path $Q'=(x',v_2,v_3,\ldots,v_r,y')$ is contained in $G$. Recall that $x',y'\in V(Z)$, and the remaining vertices of $Q'$ do not lie in $Z$.
	
	
	We start by defining, for every fake edge $e$ of $\tilde B'$, a path $P(e)$ in $G$. We may also define up to two new fake edges and their corresponding paths. Next, we construct a slight modification of the graph $\tilde B'$, that we denote by $R$. Intuitively, $R$ contains the graph $\tilde B'$ and the path $Q$ (though the precise definition of $R$ is somewhat more intricate).  Since block $B'$ is bad and $Q$ is its witness path, we will argue that graph $R$ is not planar. We will then reach a contradiction by showing a planar drawing of graph $R$, using the block $B$ of $\bset_H$ and the fact that is a good block.
	
\paragraph{Paths for fake edges.}	
Let $A$ be the set of all fake edges of $\tilde B$. Recall that each fake edge $e=(a,b)\in A$ is associated with a distinct graph $B(e)\in \nset(B)$, such that $I(B(e))=(a,b)$. We define, for each such fake edge $e=(a,b)$ a path $P(e)$ that is contained in the graph $B(e)$, and connects $a$ to $b$. We may also add up to two new fake edges to $A$. Recall that all such graphs $B(e)$ are contained in $Z$.

If $x\neq x'$ (so $x$ is a super-node), then let $B_1\in \nset(B)$ be the unique graph that contains $x'$, and let $a_1,b_1$ be the endpoints of $B_1$ (if $B_1$ is the complement of $B'$ in $Z'$, then $a_1,b_1$ are the endpoints of $B'$). 
Since graph $Z'$ is $2$-connected, there are two internally disjoint paths, connecting $x'$ to $a_1$ and $b_1$, respectively. By concatenating these paths, we obtain a new path $P_1$ connecting $a_1$ to $b_1$ in graph $B_1$, that contains the vertex $x'$. 
Notice that $e_1=(a_1,b_1)$ may not be an fake edge of $\tilde B'$ (because we do not allow parallel edges). 
If this is the case, then we add edge $e_1$ to $A$, and we set $P(e_1)=P_1$. If $e_1$ is an fake edge of $A$, but it is associated with a different graph (that is, $B(e_1)\neq B_1$), then we set $B(e_1)=B_1$.

If $y\neq y'$, then we define a graph $B_2\in \nset(B')$ containing $y'$, and a path $P_2$ that is contained in $B_2$ and connects the endpoints of $B_2$, that we denote by $a_2$ and $b_2$, similarly. As before, if $e_2=(a_2,b_2)$ does not lie in $A$, then we add it to $A$, and if it already belongs to $A$ but is associated with some graph  $B(e_2)\neq B_2$), then we set $B(e_2)=B_2$.
 
For every other fake edge $e=(a,b)\in A$, we consider the corresponding graph $B(e)\in \nset(B)$, and we let $P(e)$ be any path connecting $a$ to $b$ in $B(e)$. Let $\pset=\set{P(e)\mid e\in a}$ be the resulting set of paths.	

We need the following immediate observation.

\begin{observation}\label{obs: fake edges and their paths}
	The new set $A$ of fake edges does not contain parallel edges. Moreover, all paths in $\pset$ are internally disjoint from each other and from $V(\tilde B')$.
\end{observation}


\paragraph{Constructing the graph $R$.}	
 We are now ready to define the graph $R$. We start with $R=\tilde B'$. If $x\neq x'$, then we consider two cases. First, if edge $e_1$ (the fake edge corresponding to the graph $B_1\in \nset(B')$ containing $x'$) belongs to $\tilde B'$ as an fake edge, then we replace this edge with the path $P_1$. Otherwise (edge $e_1$ is not an fake edge of $\tilde B'$, so a real edge parallel to $e_1$ must belong to $\tilde B'$), we simply add path $P_1$ to $R$. Similarly, if $y\neq y'$, and edge $e_2$  belongs to $\tilde B'$ as an fake edge, then we replace this edge with the path $P_2$ in $R$. If $y\neq y'$, and  edge $e_2$ does not belong to $\tilde B'$ as an fake edge, then we add the path $P_2$ to $R$. Lastly, we add the path $Q'$ to $R$.  Notice that graph $R$ can be obtained from graph $\tilde B'$ using the following transformation: (i) insert up to $2$ parallel edges; (ii) subdivide some fake edges; and (iii) add the path $Q'$. Since we have assumed that block $B'$ is a bad block, and $Q$ is its witness path, it is easy to see that graph $R$ cannot be planar. We will reach a contradiction by showing a planar drawing of $R$.
 
 \paragraph{Planar Drawing of $R$.}
 Recall that $B\in \bset_H$ is the block corresponding to $B'$, that is given by Lemma \ref{lem: block containment}.
 Recall that $V(\tilde B')\subseteq V(\tilde B)$, and that every real edge of $\tilde B'$ belongs to $\tilde B$ as a real edge, except possibly for an edge connecting the endpoints of $B$. 
 Let $\rho=\rho_{\tilde B}$ be the unique planar drawing of $\tilde B$. We will modify this drawing $\rho$ in order to obtain a planar drawing of the graph $R$, reaching a contradiction. First, since every vertex of $\tilde B'$ lies in $\tilde B$, we map each such vertex to the image of itself in the drawing $\rho$. Next, for every real edge $e=(u,v)$ of $\tilde B'$, if $e$ does not connect the endpoints of $\tilde B$, then  $e\in \tilde B$, and we map this edge to the image of itself in $\rho$. Assume now that $e$ connects the endpoints of $\tilde B$. Then there is an fake edge $e'$ connecting the endpoints of $e$ in $\tilde B$. We draw $e$ next to the image of $e'$ (so edge $e$ is inserted into the drawing).
 
 Next, we consider the edges in $A$ one-by-one, and define the drawings of the corresponding paths in $\pset$.
 
 Consider some edge $e\in A$, whose endpoints are denoted by $u$ and $v$, and let $P=P(e)$ be its corresponding path in $\pset$. 
 We partition the path $P$ into segments $\sigma_1,\eta_1,\sigma_2,\eta_2,\ldots,\eta_{q-1},\sigma_q$, where for all $1\leq i\leq q$, $\sigma_i$ is contained in $\tilde B$ (so that all edges of $\sigma_i$ are real edges), and for all $1\leq i<q$, $\eta_i$ is internally disjoint from $V(\tilde B)$. It is possible that a segment $\sigma_i$ only consists of a single vertex of $\tilde B$. We refer to the segments $\sigma_i$ as \emph{$\sigma$-segments}, and we refer to the segments $\eta_i$ as \emph{$\eta$}-segments. We denote by $\Sigma$ the set of all $\sigma$-segments for all edges $e\in A$, and we denote by $\Lambda$ the set of all $\eta$-segments.
 
Since all paths in $\pset$ are internally disjoint, and set $A$ does not contain any parallel edges, we obtain the following observation:

\begin{observation}\label{obs: eta and sigma segments}
	If $\eta',\eta''\in \Lambda$ are two distinct segments, $u,v$ are the endpoints of $\eta$, and $u',v'$ are the endpoints of $\eta'$, then $\set{u,v}\neq \set{u',v'}$. 
\end{observation} 

Consider again the path $P=P(e)$ and its partition into segments  $\sigma_1,\eta_1,\sigma_2,\eta_2,\ldots,\eta_{q-1},\sigma_q$. 
We define a \emph{drawing} of the path $P$, using the drawing $\rho$ of $\tilde B$. First, every edge lying on a $\sigma$-segment is mapped to a the image of itself in $\rho$. Consider now some $\eta$-segment $\eta_i$, and let $u,v$ denote its endpoints. Then either there is an fake edge $(u,v)$ in $\tilde B$, in which case we draw $\eta_i$ along the image of this edge (or, equivalently, the image of the fake edge is subdivided by the inner vertices of $\eta_i$), or no such fake edge exists in $\tilde B$. In the latter case, edge $e\in A$ corresponding to the path $P(e)$ cannot be $e_1$ or $e_2$, since we have inserted fake edges corresponding to them. Therefore, there is a real edge $(u,v)$ in $\tilde B$, that prevented us from adding the fake edge to $\tilde B$. Moreover, there cannot be a real edge $(u,v)$ in $\tilde B'$ because the paths in $\pset$ are internally disjoint from $V(\tilde B')$, and an edge of $A$ may only be a parallel edge of a real edge in $\tilde B'$ if that edge is $e_1$ or $e_2$. Therefore, the image of the real edge $(u,v)$ in $\rho$ is not utilized by the drawings of the real edges in $\tilde B'$ that we have constructed. We then draw the path $\eta_i$ along the image of this edge.

So far, for every fake edge $e\in A$, we have defined a drawing of the corresponding path $P(e)$, by mapping $P(e)$ to some path $P'(e)$ in graph $\tilde B$, such that the paths in $\set{P'(e)\mid e\in A}$ are internally disjoint from each other, do not share edges from each other, are internally disjoint from $V(\tilde B)$, and do not contain real edges of $\tilde B'$. 

For each edge $e\in A$ that is different from $e_1$ and $e_2$, we draw the edge $e$ along the drawing of the path $P(e)$ that we have just defined (in other words, we have replaced the drawing of $P$ with the drawing of $e$). We do not alter the drawings of $P(e_1)$ and $P(e_2)$.

So far we have utilized the drawing $\rho$ of $\tilde B$ in order to define a planar drawing of the graph $R'$, that is obtained from the graph $R$ by discarding all inner vertices of $Q'$ from it. We denote this drawing of $R'$ by $\rho'$. It is now sufficient to prove the following claim. Recall that $x'$ and $y'$ are the endpoints of the path $Q'$.

\begin{claim}\label{claim: can draw Q}
There is a face $F$ in the drawing $\rho'$ whose boundary contains the vertices $x'$ and $y'$.
\end{claim}

Observe that using the above claim we can complete the drawing of planar drawing of the graph $R$, by completing the drawing of the path $Q'$ inside the face $F$. Therefore, in order to complete the proof of Lemma \ref{lem: good clusters cant be killed}, it is now enough to prove Claim \ref{claim: can draw Q}.

\begin{proofof}{Claim \ref{claim: can draw Q}}
Recall that all inner vertices of the path $Q'$ lie in $V(G)\setminus V(Z')$. In particular, $Q'$ is internally disjoint from all paths in $\pset$, and from $V(\tilde B')$. Let $Z$ denote the super-block of $H$ that contains the block $B$. We partition the path $Q'$ into segments $\alpha_1,\beta_1,\ldots,\beta_{q-1},\alpha_q$, where for all $1\leq i\leq q$, segment $\alpha_i$ (that we refer to as an $\alpha$-segment) is contained in $Z$, and for all $1\leq i<q$, segment $\beta_i$ (that we refer to as a $\beta$-segment) is internally disjoint from $Z$. For all $1\leq i\leq q$, we denote the endpoints of $\alpha_i$ by $s_i,t_i$, where $s_i$ lies closer to $x'$ than $t_i$, and $s_1=x'$. Consider now the graph $J^B$ that is associated with the block $B$. Notice that some vertices $s_i,t_i$ may belong to this graph, while some of these vertices may have been contracted into super-nodes. For each $1\leq i\leq q$, if $s_i\in V(J^B)$, then we denote $s'_i=s_i$; otherwise, we let $s'_i$ be the supernode into which $s_i$ was contracted. We define $t'_i\in V(J^B)$ similarly. 

Let $\fset$ be the set of all faces in the drawing $\rho'$ of $R'$. Notice that drawing $\rho'$ of $R'$ is obtained by starting from the drawing $\rho$ of $\tilde B$, and then deleting some edges and vertices (and also inserting at most one edge -- the edge connecting the endpoints of $B$). Therefore, for every face $F\in \fset$, its boundary defines a closed simple curve in $\rho$. If some vertex $v$ of $\tilde B$ lies in the interior of this curve (that is, the side that does not contain images of vertices of $R'$), then we will say that the image of $v$ lies in the interior of $F$.

\begin{observation}
	
	If $q=1$, then there is some face $F\in \fset$ with $s'_1,t'_1$ lying on its boundary. Otherwise, there are faces $F_1,F_2,\ldots,F_q\in \fset$, such that, if we consider the drawing $\rho$ of $\tilde B$:
	
	\begin{itemize}
		\item $s'_1$ lies on the  boundary of $F_1$ and $t'_1$ lies in the interior of $F_1$;
		\item $t'_q$ lies on the boundary of $F_q$ and $s'_q$ lies in the interior of $F_q$; and
		\item for all $1<i<q$, $s'_i$ and $t'_i$ lie in the interior of $F_i$.
	\end{itemize}
\end{observation}

\begin{proof}
	Fix some $1\leq i\leq q$, and consider the path $\alpha_i$. Recall that this path connects $s_i$ to $t_i$, and it is contained in $Z$. As before, we partition this path into $\sigma$-segments and $\eta$-segments. Idea: $\sigma$-segments don't intersect the drawing $\rho$, and $\eta$-segments can be replaced with fake edges as before. We then transform $\alpha_i$ into a path $\alpha'_i$ in $\tilde B$ that is internally disjoint from $\tilde B'$, so its drawing lies inside a single face of $\rho'$.
\end{proof}

\begin{observation}
	For all $1\leq i<q$, there is some face $F$ of the drawing $\rho$, such that $t'_i$ and $s'_{i+1}$ lie on the boundary of $F$.
\end{observation}
The observation follows from the fact that block $B$ is good.

To complete the proof, we can connect each $t'_i$ to $s'_{i+1}$ with a curve $\gamma_i$ that is internally disjoint from the drawing $\rho$. But that means that $t'_i$ and $s_{i+1}$ lie in the interior of same face of $\rho'$.
\end{proofof}
		
	

 
 
 
 
 
 
 
 \iffalse
 Moreover, if $A'$ is the set of all fake edges for $\tilde B'$, then there is a set $\pset'=\set{P'(e)\mid e\in A'}$ of paths in $\tilde B$ that are mutually internally disjoint, such that path $P'(e)$ has the same endpoints as the edge $e$, and is internally disjoint from $V(\tilde B')$. Consider now the unique planar drawing $\rho=\rho_{\tilde B}$ of block $\tilde B$. This drawing naturally induces a planar drawing of $\tilde B'$, where every vertex of $\tilde B'$ is mapped to its image in $\rho$, every real edge of $\tilde B'$ is also mapped to its image in $\rho$, and every fake edge $e\in A'$ is mapped to the image of the path $P(e)$. If $e=(u,v)$ is a real edge of $\tilde B'$ whose endpoints are the endpoints of the block $B$, then graph $\tilde B$ contains a fake edge $(u,v)$, and Lemma \ref{lem: block containment} guarantees that no path in $\pset$ contains this fake edge. Therefore, we can map the edge $e$ to the image of the fake edge $(u,v)$ in $\rho$. Therefore, the drawing $\rho$ of $\tilde B$ naturally induces a planar drawing $\rho'$ of $\tilde B'$. Since $\tilde B'$ has a unique planar drawing, $\rho'=\rho_{\tilde B'}$.
	
	Consider now a witness edge $e=(x,y)\in E(J^{B'})$ that certifies that $B'$ is a bad block. Let us consider first an easy case where $x$ and $y$ are not super-nodes of $J^{B'}$. In that case, the edge $(x,y)$ belongs to the original graph $G$, and $x,y$ are both vertices of $\tilde B'$. It then follows that $x,y$ are also vertices of $\tilde B$. Therefore, edge $(x,y)$ must also belong to graph $J^B$. If this edge lies in $\tilde B$, then its endpoints must lie on the boundary of the same face of the drawing $\rho$. Otherwise, since $B$ is a good block, $x$ and $y$ lie on the boundary of the same face of $\rho$. Since $\rho'$ is obtained from the drawing $\rho$ by deleting some edges and vertices from it, we get that $x$ and $y$ must lie on the boundary of the same face in drawing $\rho'$ as well, contradicting the fact that $e$ is a witness edge.
	
	So far we have considered the case where neither of $x,y$ is a super-node of $J^{B'}$. The case where at least one of these vertices is a super-node of $J^{B'}$ is more challenging, since in this case it is no longer necessarily true that edge $(x,y)$ belongs to $G$, so it is not as easy to argue that such an edge must lie in $J^B$. In order to handle this more difficult case, we need to define the paths in set $\pset$ more carefully.
	We assume w.l.o.g. that $x$ is a super-node, and $y$ is either a regular vertex or a super-node. 
	 Let $e'=(x',y')$ be the edge of $G$ that corresponds to the witness edge $e$ (so $x'$ was contracted into the super-node $x$, and, if $y$ is a super-node, then $y'$ was contracted into $y$; otherwise $y=y'$ must hold).
	 
	 
	We construct the set $\tilde \bset$ of blocks with respect to block $B'$ as before: for every child vertex $v(B'')$ of $v(B')$ in the corresponding partitioning tree, block $B''$ is added to $\tilde \bset$, and, if $v(B'')$ is not the root of the partitioning tree, then we add another block $B^*$, whose endpoints are the same as the endpoints of $B'$, and whose inner vertices are $V(Z')\setminus V(B')$, where $Z'\in \zset_{H'}$ is the super-block containing $B'$. Let $B_1\in \tilde \bset$ be the block containing the vertex $x$, and let $a_1,b_1$ be its two endpoints. Recall that graph $\tilde B'$ contains a fake edge $e_1=(a_1,b_1)$. Since graph $Z'$ is $2$-connected, there are two internally disjoint paths, connecting $x$ to $a_1$ and $b_1$, respectively. By concatenating these paths, we obtain a new path $P^*(e_1)$ connecting $a_1$ to $B_1$ in block $B_1$, that contains the vertex $x'$. If $y$ is a super-node that corresponds to some block $B_2\in \tilde \bset$, whose endpoints are $a_2,b_2$, then we denote by $e_2=(a_2,b_2)$ the corresponding fake edge, and we define the path $P^*(e_2)$ connecting $a_2$ to $b_2$ that contains $y'$ as before. 
	
	Recall that in the proof of Lemma \ref{lem: block containment}, in order to obtain the set $\set{P'(e')\mid e'\in A}$ of paths (where $A$ is the set of all fake edges of $\tilde B'$), we started from an arbitrary set $\set{P(e)\mid e\in A}$ of internally disjoint paths in graph $H'$, where path $P(e)$ connects the endpoints of the edge $e$. We modify this set of paths by replacing $P(e_1)$ with the new path $P^*(e_1)$, and, if $y$ is a supernode, we also replace path $P(e_2)$ with the new path $P^*(e_2)$. We then follow the proof of Lemma \ref{lem: block containment} to construct the set $\pset=\set{P'(e')\mid e'\in A}$ of paths exactly as before. Consider the path $P^*(e_1)$. Recall that the algorithm from Lemma \ref{lem: block containment} partitions it into segments $\sigma_1,\eta_1,\ldots,\sigma_r$, where the $\sigma$-segments are contained in $\tilde B$, while every $\eta$-segment corresponds to some block in set $\tilde \bset$ for $B$, and connects the endpoints of the corresponding block. \mynote{need to define $\nset(B)$}
	
	
	
\fi	
\end{proof}



The remainder of the proof of Theorem \ref{thm: can find edge set w acceptable clusters} consists of three steps. In the first step, we augment the initial planarizing set $E'$ of edges to a new set $E_1$, such that every cluster in graph $G\setminus E_1$ is good. In the second step, we augment the set $E_1$ of edges into a larger set $E_2$, such that every cluster $C$ of $G\setminus E_2$ is good, and moreover, the terminals in $T(C)$ are $\alpha$-well-linked in $C$. Lastly, in the third step, we complete the proof of Theorem   \ref{thm: can find edge set w acceptable clusters} by further augmenting the set $E_2$ of edges into the final set $E''$. We now describe each of the three steps in turn.



\iffalse

Finally, we are ready to define acceptable clusters.


\begin{definition}
	A cluster $C\in \cset$ is called \emph{acceptable} iff it is good, and additionally one of the following two properties hold:
	
	\begin{itemize}
		\item either $C$ is $3$-connected, and the vertices of $T\cap V(C)$ are $\alpha$-well-linked in $C$, for $\alpha=1/\poly\log n$ (in which case $C$ is a type-1 acceptable cluster); or
		
		\item $C$ contains at most $O(\Delta \poly\log n)$ terminals, where $\Delta$ is maximum vertex degree in $G$ (in which case $C$ is a type-2 acceptable cluster).
	\end{itemize}
\end{definition}


\fi





==> computing-acceptable-decomposition-old.tex <==

		
		
\section{Proof of Theorem~\ref{thm: can find edge set w acceptable clusters}}
\label{sec:thm1}
		
\subsection{Good Pseudo-Blocks}
\label{sec: good blocks and acceptable clusters}

Throughout this subsection, we assume that we are given some planarizing set $\hat E$ of edges for the input graph $G$, that is, $G\setminus \hat E$ is planar. We note that $\hat E$ is not necessarily the same as the original planarizing set $E'$, since, as the algorithm progresses, we may add edges to the planarizing set. The definitions in this subsection refer to any planarizing set $\hat E$ that may arise over the course of the algorithm.

Given a planarizing set $\hat E$ of edges for $G$, let $H=G\setminus \hat E$. Recall that we say that a vertex $v$ of $H$ is a \emph{terminal} iff it is incident to some edge in $\hat E$, and we denote the set of terminals by $\Gamma$.

Recall that we have defined a block decomposition of a graph $H$, as follows. First, we denoted by $\cset(H)$ the set of all connected components of $H$, and we refer to the elements of $\cset(H)$ as \emph{clusters}. For each cluster $C\in \cset$, we have defined a collection $\zset(C)$ of super-blocks (maximal $2$-connected subgraphs) of $C$, and we denoted $\zset(H)=\bigcup_{C\in \cset(H)}\zset(C)$. Lastly, for each superblock $Z\in \zset(H)$, we let $\lset(Z)$ be the block decomposition of $Z$ given by Theorem \ref{thm: block decomposition}, and we denoted by $\bset(C)=\bigcup_{Z\in \zset(C)}\lset(Z)$ the resulting collection of pseudo-blocks for cluster $C$. The final block decomposition of $H$ is  $\bset(H)=\bigcup_{C\in \cset}\bset(C)$, and the elements of $\bset(H)$ are called pseudo-blocks.
 
 
Consider some pseudo-block $B\in \bset(H)$, and let $\tilde B$ be the corresponding graph, that is either a $3$-connected graph, or it is isomorphic to $K_3$. 
Recall that $\tilde B$ has a unique planar drawing, that we denote by $\rho_{\tilde B}$. Let $\tilde B'\subseteq \tilde B$ be the graph obtained from $\tilde B$ by deleting all its fake edges. Note that $\tilde B'$ may be not $3$-connected. The drawing $\rho_{\tilde B}$ of $\tilde B$ naturally induces a drawing of $\tilde B'$, that we denote by $\rho'_{\tilde B'}$. %\snote{why dont we use the same $\rho_{\tilde B'}$? $\rho_{\tilde B'}$ is the same drawing as $\rho'_{\tilde B'}$ but for a sub-graph.}
Consider now the set $\rset_G(\tilde B')$ of all bridges for $\tilde B'$ in graph $G$. We say that $B$ is a \emph{good pseudo-block} iff for each such bridge $R\in \rset_G(\tilde B')$, there is a face $F$ in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$, whose boundary contains all vertices of $L(R)$. If $B$ is not a good pseudo-block, then it is called a \emph{bad pseudo-block}. Note that, if $B$ is a bad pseudo-block, then there is some bridge $R\in \rset_G(\tilde B')$, such that no face of $\rho'_{\tilde B'}$ contains all vertices of $L(R)$. We call such a bridge $R$ a \emph{witness} for $B$.

\iffalse
\paragraph{Good Clusters.}
Finally, we define good clusters.

\begin{definition}
	We say that a cluster $C\in \cset$ is \emph{good} iff pseudo-block $B\in \bset(C)$ is good.
\end{definition}
\fi



\iffalse
Our algorithm starts with some planarizing set $E'$ of edges, and then, over the course of several steps, gradually adds additional edges to set $E'$. Suppose that at some point we compute a planarizing set $\hat E$ of edges, such that, in the block decomposition given by Theorem~\ref{thm: block decomposition} of every cluster of $G\setminus \hat E$, all pseudo-blocks are good. As the algorithm progresses, and more edges are added to $\hat E$, we would like to claim that this property continues to be preserved. The following lemma allows us to do so. Its proof is deferred to Appendix~\ref{apd:good_cluster_preserving}.

\begin{lemma}\label{lem: good clusters cant be killed}
Suppose we are given two planarizing sets $\hat E,\hat E'$ of edges, with $\hat E\subseteq \hat E'$. Let $H=G\setminus\hat E$ and $H'=G\setminus \hat E'$, so that $H'\subseteq H$. Consider some pseudo-block $B_1\in \bset(H')$, and let $B_2\in \bset(H)$ be the corresponding block given by Lemma \ref{lem: block containment}. Assume further that $\tilde B_2$ does not contain a real edge connecting the endpoints of $B_1$. Then, if $B_2$ is a good pseudo-block, so is $B_1$. % Assume that every pseudo-block in $\bset_H$ is good. Then every pseudo-block in $\bset_{H'}$ is good as well. 
\end{lemma}
\fi



The remainder of the proof of Theorem \ref{thm: can find edge set w acceptable clusters} consists of two stages. In the first stage, we augment the initial planarizing set $E'$ of edges to a new edge set $E_1$, such that every pseudo-block in the resulting block decomposition of $G\setminus E_1$ is good. Then in the second stage we further augment $E_1$ in order to obtain the final edge set $E''$ and a decomposition of $G$ into acceptable clusters. We now describe each of the two stages in turn.

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
\subsection{Stage 1: Good Pseudo-Blocks}

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
The main result of this step is summarized in the following theorem.

\begin{theorem}\label{thm: getting good pseudoblocks}
	There is an efficient algorithm, that, given a $3$-connected graph $G$ with maximum vertex degree at most $\Delta$ and a planarizing set $E'$ of edges for $G$, computes a planarizing edge set $E_1$ with $E'\subseteq E_1$, such that $|E_1|\leq O(|E'|+\cro(G))\poly(\Delta\log n)$, and, moreover, if we denote $H=G\setminus E_1$, then every pseudo-block in the block decomposition $\bset(H)$ is a good pseudo-block.
\end{theorem}


The remainder of this subsection is devoted to proving Theorem \ref{thm: getting good pseudoblocks}. 
Throughout the proof, we denote $H=G\setminus E'$ and we denote by $\cset$ the set of its connected components. Recall that the set $\Gamma$ of terminals contains all vertices that are endpoints of the edges of $E'$. Our first step is to compute a block decomposition $\bset(H)$ of $H$. We denote by $\bset'\subseteq \bset(H)$ the set of all pseudo-blocks $B\in \bset(H)$ for which $\tilde B$ contains more than three vertices. Observe that, if $|V(\tilde B)|\leq 3$, then $\tilde B$ must be a good block.

We use Lemma \ref{lem:block_endpoints_routing} that defines, for each pseudo-block $B\in \bset'$, an embedding $\pset_{\tilde B}=\set{P_{\tilde B}(e)\mid e\in A_{\tilde B}}$ of the set $A_{\tilde B}$ of fake edges of $\tilde B$ into paths that are internally disjoint from $\tilde B$ and are mutually internally disjoint. Recall that all paths in set $\pset=\bigcup_{ B\in \bset'}\left(\pset_{\tilde B}\setminus \set{P_{\tilde B}(e^*_{\tilde B})} \right)$ cause edge-congestion at most $O(\log n)$, and $e^*_{\tilde B}$ is the fake parent-edge for $B$, that connects the endpoints of $B$ (it is possible that $e^*_{\tilde B}$ is undefined). \mynote{If the lemma statement remains non-constructive we should add "Our algorithm does not compute the embedding $\pset$ explicitly; we only use it for accounting purposes.". But it's better if it can be made constructive}.

Consider now some pseudo-block $B\in \bset'$. We define a new graph $\tilde B^*$ as follows: we start from graph $\tilde B'$ that is obtained from $\tilde B$ after deleting all fake edges from it. We then add to it all vertices and edges participating in the paths in $\pset_{\tilde B}$. 
Consider now some fixed optimal drawing $\phi^*$ of $G$. We define a set $\chi(B)$ of its crossings as follows. First, every crossing $(e,e')$ in $\phi^*$, where either $e$ or $e'$ is a real edge of $\tilde B$ is added to $\chi(B)$. Additionally, if $e,e'$ lie on two distinct paths of $\pset_{\tilde B}$ (that is, $e\in \pset_{\tilde B}(e_1)$, $e'\in \pset_{\tilde B}(e_2)$ and $e_1\neq e_2$ are two distinct fake edges of $\tilde B$), then we add $(e,e')$ to $\chi(B)$. 

We need the following simple claim.

\begin{claim}\label{claim: chi is small for each B}
	$\sum_{B\in \bset'}|\chi(B)|\leq O(\cro(G)\cdot \log n)$.
\end{claim}
\begin{proof}
	Consider any crossing $(e,e')$ in the optimal drawing $\phi^*$ of $G$. Recall that $e,e'$ may belong to $\chi(B)$ in one of two cases: either at least one of $e,e'$ is a real edge of $\tilde B$; or $e,e'$ they lie on two distinct paths in $\pset_{\tilde B}$. In particular, in the latter case, one of the two edges $e,e'$ must lie on a path $P_{\tilde B}(\hat e)$, where $\hat e\neq e^*_{\tilde B}$ (that is, $\hat e$ is not the fake parent-edge of $B$). Note that there may be at most one pseudo-block $B\in \bset'$ for which $e$ is a real edge, and the same is true for $e'$. Moreover, there are at most $O(\log n)$ pseudo-blocks $B\in \bset'$, such that edge $e$ lies on a path of $\pset_{\tilde B}\setminus \set{P_{\tilde B}(e^*_{\tilde B})}$, and the same holds for $e'$. Therefore, altogether, there are at most $O(\log n)$ pseudo-blocks $B\in \bset'$ with $(e,e')\in \chi(B)$.
\end{proof}


 Our algorithm processes each pseudo-block $B\in \bset'$ one-by-one, employing the following lemma.

\begin{lemma}\label{lem: process a block}
	There is an efficient algorithm, that, given a pseudo-block $B\in \bset'$, computes a subset $E^*(B)\subseteq E(\tilde B')$ of edges, such that, if $\rho''$ is the drawing of the graph $\tilde B'\setminus E^*(B)$ induced by the unique planar drawing $\rho_{\tilde B}$ of graph $\tilde B$, then for every bridge $R\in \rset_G(\tilde B')$, all vertices of $L(R)$ lie on the boundary of a single face of $\rho''$. Moreover, $|E^*(B)|\leq O((|\chi(B)|+|\Gamma\cap V(\tilde B))\cdot \poly(\Delta \log n ))$.
\end{lemma}

Notice that the lemma only considers bridges $R$ that are defined with respect to the original block $B$, that is, bridges of $\rset_G(\tilde B')$. Graph $\tilde B'\setminus E^*(B)$ may not even be connected, and its bridges may be defined differently.
We provide the proof of the lemma below, after we conclude the proof of Theorem \ref{thm: getting good pseudoblocks} using it.

\iffalse
%----------------------
%----------------------
Let $\tilde E$ be a set of edges that contains, for every block $B\in \bset(H)$, the edge connecting the endpoints of $B$, if such an edge is present in $H$. We need the following observation.

\begin{observation}\label{obs: few edges connecting endpoints}
	$|\tilde E|\leq O(|E'|)$.
	
\end{observation}
\begin{proof}
	Let $C$ be any connected component of $H$, and let $Z$ be any super-block in $\zset(C)$. Consider the block decomposition $\lset=\lset(Z)$ of $Z$, and let $\tau=\tau(\lset)$ be its corresponding block decomposition. 
\end{proof}
%------------------------
%-----------------------
\fi
%
%
We let the final set of edges be $E_1=\left (\bigcup_{B\in \bset(H)}E^*(B)\right )\cup E'$. Note that:

\[
\begin{split}
|E_1|&=|E'|+\sum_{B\in \bset'}|E^*(B)| \\  
&\leq |E'|+\sum_{B\in \bset'} O\left ((|\chi(B)|+|\Gamma\cap V(\tilde B))\cdot \poly(\Delta\cdot \log n)\right )\\ &\leq O((|E'|+\cro(G))\poly(\Delta\cdot \log n)),\end{split}\]

from Claim \ref{claim: chi is small for each B}.

Let $H'=G\setminus E_1$, and let $\bset(H')$ be a block decomposition of graph $H'$. It is now enough to prove that every pseudo-block in this decomposition is good. We do so in the next claim.

\begin{claim}\label{claim: every block is good}
	Every pseudo-block in $\bset(H')$ is good.
\end{claim}

\begin{proof}
Assume for contradiction that the claim is false. 
%, so there must be some pseudo-block $B_1\in \bset_{H'}$ that is bad. 
Let $B_1\in \bset(H')$ be a pseudo-block that is bad, and let $R\in \rset_G(\tilde B_1')$ be a bridge that is a witness for $B_1$. Notice that $|V(B_1)|>3$ must hold if $B_1$ is bad.
Let $B_2\in \bset(H)$ be the pseudo-block corresponding to $B_1$, given by Lemma \ref{lem: block containment}. 
Recall that $V(\tilde B_1)\subseteq V(\tilde B_2)$;
 every real edge of $\tilde B_1$ belongs to $\tilde B_2$ as a real edge, except (possibly) for the edge connecting the endpoints of $B_2$; 
 for every fake edge $e=(u,v)$ in $\tilde B_1$, there is a path $P(e)$ in $\tilde B_2$ (that may contain fake edges of $\tilde B_2$) that connects $u$ to $v$, and is internally disjoint from $V(\tilde B_1)$. Moreover, if $e$ and $e'$ are distinct fake edges of $\tilde B_1$, then their corresponding paths $P(e)$ and $P(e')$ are internally disjoint, and, if graph $\tilde B_1$ contains a real edge connecting the endpoints of $B_2$, then for every fake edge $e\in E(\tilde B_1)$, the path $P(e)$ does not contain the edge connecting the endpoints of $B_2$.

We denote the endpoints of $B_2$ by $(x,y)$. If edge $(x,y)$ belongs to $\tilde B_1'$, then we denote this edge by $e^*$; otherwise, edge $e^*$ is undefined. Note that in either case, graph $\tilde B_2$ must contain a fake edge $(x,y)$.


Consider the unique planar drawing $\rho_{\tilde B_2}$ of $\tilde B_2$. Since every vertex and every real edge of $\tilde B_1$ lies in $\tilde B_2$, this drawing naturally induces a drawing of $\tilde B_1'$ (if edge $e^*$ is present in $\tilde B_1'$, we draw it along the image of the fake edge $(x,y)$). We denote by $\rho'$ the drawing of $\tilde B_1'$ induced by $\rho_{\tilde B_2}$, and denote by $\rho''=\rho'_{\tilde B_1'}$ the drawing of $\tilde B_1'$ induced by $\rho_{\tilde B_1}$. 
We use the following claim.

\begin{claim}\label{claim: identical drawings}
	The drawings $\rho'$ and $\rho''$ of $\tilde B_1'$ are identical. %\snote{$\rho''$ is not defined}
\end{claim}
\begin{proof}
	Let $A$ be the set of all fake edges of $\tilde B_1$, so that $\tilde B_1'=\tilde B_1\setminus A$.
	Consider the drawing $\rho'$ of $\tilde B_1'$. We will show that we can augment this drawing by adding drawings of the edges in $A$, so that the resulting drawing remains planar. Note that, if this is true, then it follows that $\rho'=\rho''$. To see this, note that $\tilde B_1$ is $3$-connected, so it has a unique planar drawing, and therefore the resulting drawing of $\tilde B_1$ is identical to $\rho_{\tilde B_1}$. Since both $\rho'$ and $\rho''$ are obtained from the drawing $\rho_{\tilde B_1}$ of $\tilde B_1$ by deleting the images of the fake edges from it, $\rho'=\rho''$.
	
	From now on, it is enough to show that we can augment the drawing $\rho'$ by adding the images of edges in $A$ to it, while preserving the planarity. Recall that Lemma \ref{lem: block containment} defines, for every fake edge $e=(u,v)\in A$, a path $P(e)$ in $\tilde B_2$ that connects $u$ to $v$, and is internally disjoint from $V(\tilde B_1)$, such that, if $e$ and $e'$ are distinct fake edges in $A$, then their corresponding paths $P(e)$ and $P(e')$ are internally disjoint. Moreover, if edge $e^*$ is present in $\tilde B_1'$, then no path in $\pset=\set{P(e)\mid e\in A}$ may contain this edge. Recall that the paths in $\pset$ are allowed to contain fake edges of $\tilde B_2$. We simply draw every fake edge $e\in A$ along the curve $\gamma(e)$ corresonding to the drawing of the path $P(e)$, that is obtained by concatenating the images of the edges of $P(e)$ in $\rho_{\tilde B_2}$. Since the drawing $\rho_{\tilde B_2}$ of $\tilde B_2$ is planar, we obtain a planar drawing of $\tilde B_1$.
\end{proof}


Let $\fset$ be the set of all faces in the drawing $\rho'=\rho''$. Observe that Lemma \ref{lem: process a block} ensures that for every 
bridge $R'\in \rset_G(\tilde B_2')$, if $L(R')\cap V(\tilde B_1')\neq \emptyset$, then there is some face $F\in \fset$, such that all vertices of $L(R')\cap V(\tilde B_1')$ lie on the boundary of $F$ in the drawing $\rho'$.

For every vertex $v\in V(\tilde B_2)\setminus V(\tilde B_1)$, there is a unique face $F(v)\in \fset$, such that the image of vertex $v$ in $\rho_{\tilde B_2}$ lies in the interior of the face $F$.

Recall that $T_R\subseteq R$ is a tree whose leaves are precisely the vertices of $L(R)$. 
Assume first that $V(T_R)\cap V(\tilde B_2)=L(R)$. In this case, there is some bridge $R'\in \rset_G(\tilde B_2')$ of $\tilde B_2'$ that contains the tree $T_R$, and so $L(R)\subseteq L(R')$. However, from Lemma \ref{lem: process a block}, we are guaranteed that all vertices of $L(R')$ lie on the boundary of the same face in the drawing $\rho''$. %Since $B_2$ is a good block, there must be a face in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B'_2$ whose boundary contains all vertices of $L(R)$.

Assume now that there is some vertex $v\in V(T_R)\cap  V(\tilde B_2)$ that does not lie in $L(R)$. Let $F=F(v)$ be the face of $\fset$ in whose interior the image of $v$ in $\rho_{\tilde B_2}$ lies. We will show that all vertices of $L(R)$ must lie on the boundary of $F$, leading to a contradiction. Let $u$ be an arbitrary vertex of $L(R)$. It suffices to show that $u$ must lie on the boundary of the face $F$.

Let $P\subseteq T_R$ be the unique path connecting $v$ to $u$ in $T_R$. Since the leaves of tree $T_R$ are precisely the vertices of $L(R)$, except for $v$, every vertex $x$ of $P$ lies outside $V(\tilde B_1)$, and the image of $x$ in $\rho_{\tilde B_2}$ lies in the interior of some face in $\fset$. Let $u=v_1,v_2,\ldots,v_r=v$ be all vertices of $P$ that belong to $V(\tilde B_2)$, and assume that they appear on $P$ in this order. 
It remains to prove the following observation.

\begin{observation}
	For $1\leq i<r-1$, $F(v_i)=F(v_{i+1})$. Moreover, $v_r$ lies on the boundary of $F(v_{r-1})$.
\end{observation}
\begin{proof}
	Fix some $1\leq i\leq r-1$. Assume that the observation is false.
	Then there is some face $F'\in \fset$, such that $v_i$ lies in the interior of $F'$, but $v_{i+1}$ does not lie in the interior or on the boundary of $F'$ (the latter case is only relevant for $i=r-1$). Since the boundary of $F'$ separates $v_i$ from $v_{i+1}$, they  cannot lie on the boundary of the same face in the drawing $\rho'_{\tilde B_2'}$. 
	
	Let $\sigma_i$ be the subpath of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge connecting $v_i$ and $v_{i+1}$, then it is either a bridge in $\rset_G(\tilde B_2')$, or it is an edge of $\tilde B_2'$. In the former case, Lemma \ref{lem: process a block} ensures that the endpoints of $\sigma_i$  may not be separated by the boundary of a face of drawing $\rho'$. In the latter case, the same holds since the drawing $\rho'_{\tilde B_2'}$ is planar. In either case, we reach a contradiction. Otherwise, there must be a bridge $R'\in \rset_G(\tilde B_2')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. But then, from Lemma \ref{lem: process a block}, it is impossible that the boundary of a face in the drawing $\rho'$ separates the two vertices, a contradiction. 
	%	We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B_2'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B_1'\subseteq \tilde B_2'$, and from the way the drawing $\rho'_{\tilde B_1'}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B_1'}$ that contains $F_i$.	
\end{proof}	
\end{proof}

In order to complete the proof of Theorem \ref{thm: getting good pseudoblocks} it is now enough to prove Lemma \ref{lem: process a block}, which we do next.

%-------------------------------------------------------
%-------------------------------------------------------
%-------------------------------------------------------
\subsection{Proof of Lemma \ref{lem: process a block}}
%-------------------------------------------------------
%-------------------------------------------------------
%-------------------------------------------------------
%-------------------------------------------------------
	
Throughout the proof, we fix a pseudo-block $B\in \bset'$. Let $\rho=\rho_{\tilde B}$ be the unique planar drawing of $\tilde B$.   %, and $\rho'$ is the drawing of $\tilde B'$ that is induced by $\rho$. 
	For convenience, we denote by $\Gamma'$ the set of all terminals that belong to $\tilde B$. The set $\Gamma'$ of terminals remains fixed throughout the algorithm.
	
	Throughout the algorithm, we maintain a subgraph $J$ of $\tilde B$. Initially, we set $J=\tilde B'$ (recall that $\tilde B'$ is the graph obtained from $\tilde B$ by deleting all its fake edges), and over the course of the algorithm, we delete some edges from $J$, adding them to the set $E^*(B)$ of edges. We will always use $\rho'$ to denote the drawing of the current graph $J$ induced by the drawing $\rho$ of $\tilde B$. We note that graph $J$ may become disconnected over the course of the algorithm, but its drawing $\rho'$ is always fixed to be the drawing of $J$ induced by $\rho$.

Notice that a terminal in $\Gamma'$ may belong to the boundaries of two different faces in the drawing $\rho'$, which is somewhat inconvenient for us. As our first step, we add to $E^*(B)$ all edges that are incident to the terminals in $\Gamma'$, and we delete all such edges from $J$. Notice that each terminal now becomes an isolated vertex, but its drawing in $\rho'$ is fixed, as $\rho'$ is the unique drawing of the current graph $J$ induced by the drawing $\rho$ of $\tilde B$ (throughout this proof, we only refer to the vertices in the original set $\Gamma'$ as terminals). We are now guaranteed that every terminal $t\in \Gamma'$ lies on the (inner) boundary of exactly one face of the current drawing $\rho'$. Clearly,  $|E^*(B)|\leq \Delta\cdot |\Gamma'|$.


%--------------------
%--------------------
%--------------------
%--------------------
%--------------------
%--------------------

\iffalse
%--------------------
%--------------------
%--------------------

In our first step, we slightly modify the graph $\tilde B'$ to ensure that every terminal that lies in this graph has degree $1$. This will ensure that every terminal lies on an \emph{inner} boundary of some face of the drawing, and in particular there is a unique face of the drawing on whose boundary the terminal lies. As our algorithm progresses, we may add new edges to the set $E'$, and delete them from $\tilde B'$, creating new terminals. We will ensure that all such new terminals have degrees at most $1$ as well.

In order to achieve this, we construct a new graph $J$ from $\tilde B'$, as follows. We start with $J=\tilde B'$. Next, for every edge $e=(u,v)\in E(J)$, we subdivide the edge by two new vertices, replacing it with a path $(u,u_e,v_e,v)$. We denote the edges $(u,u_e),(u_e,v_e)$ and $(v_e,v)$ by $e_1,e_2$ and $e_3$, respectively. Each of these edges is referred to as a \emph{segment} of $e$, and edge $e_2$ is called the \emph{middle segment} of $e$. We will maintain a set $\hat E$ of edges that we gradually delete from $J$. Eventually, set $E^*(B)$ will contain every edge whose segment belongs to $\hat E$. At the beginning, $\hat E$ contains all edges (incident to the terminals of $\Gamma'$) that we have removed so far. Throughout the algorithm, the set $\Gamma'$ of terminals contains all vertices that are endpoints of edges in $E'\cup \hat E$.

Next, we consider the terminals $t\in \Gamma'$ one-by-one. We would like to ensure that the degree of each such terminal in $J$ is $1$. Consider any such terminal $t$, and assume that its degree in the current graph $J$ is greater than $1$. Let $(t,v)\in E(J)$ be any edge that is incident to $t$. We add this edge to $\hat E$ and delete it from $J$. Vertex $v$ now becomes a terminal, and its degree in $J$ is $1$, since $(e,z)$ must be a segment of some edge $e\in E(\tilde B')$ that was incident to $t$. Once we process all terminals that belonged to the original set $\Gamma'$, the cardinality of $\Gamma'$ increases by at most factor $\Delta$, and we are now guaranteed that every terminal in $\Gamma'$ has degree $1$ in $J$. In the remainder of the algorithm, whenever an edge $e\in E(J)$ is added to the set $\hat E$ of deleted edges, if $e$ is a segment of some edge $e'\in E(\tilde B')$, then we will ensure that $e$ is the middle segment of $e'$. This will ensure that all terminals that are added to $\Gamma'$ over the course of the algorithm have degree at most $1$. As the algorithm progresses, we denote by $\phi$ the drawing of $J$  that is induced by the drawing $\rho'$ of $\tilde B'$, and we denote by $\fset$ the set of its faces.
\fi


Throughout the algorithm, we denote by $\fset$ the set of all faces of the drawing $\rho'$ of the current graph $J$.
For every terminal $t\in \Gamma'$, there is a unique face $F(t)\in \fset$, such that $t$ lies on the (inner) boundary of $F(t)$. For a face $F\in \fset$, we denote by $\Gamma(F)\subseteq \Gamma'$ the set of all terminals $t$ with $F(t)=F$.

\paragraph{Bad Faces.} 
Throughout the algorithm, we denote by $\rset=\rset_{\tilde B'}(G)$ the set of all bridges for the graph $\tilde B'$ in $G$. 
For a bridge $R\in \rset$, let $\fset(R)=\set{F\in \fset\mid L(R)\cap \Gamma(F)\neq \emptyset}$ be the set of all faces in the drawing $\rho'$ of the current graph $J$, whose inner boundaries contain terminals of $L(R)$. We say that a bridge $R\in \rset$ is \emph{bad} for $J$ iff $|\fset(R)|>1$, or, equivalently, if not all vertices of $L(R)$ lie on the boundary of the same face of $\fset$. In such a case, we say that every face in $\fset(R)$ is a bad face, and for each face $F\in \fset(R)$, we say that bridge $R$ is \emph{responsible for $F$ being bad}. As the algorithm progresses and the graph $J$ changes, so does the set $\fset$ of the faces of the drawing $\rho'$ of $J$. The set $\rset$ of bridges does not change over the course of the algorithm, and the definitions of the sets $\fset(R)$ of faces for $R\in \rset$ and of bad faces are always with respect to the current graph $J$ and its drawing. 
The main subroutine that we use in our algorithm is summarized in the following lemma.

\begin{lemma}\label{lem: one step for bad faces}
	There is an efficient algorithm, that, given the current graph $J$ and its drawing $\rho'$, computes a subset $\hat E$ of at most $O(|\chi(B)|\cdot \Delta\log^2n)$ edges, such that, if $n_1$ denotes the number of bad faces in the drawing $\rho'$ of $J$, and $n_2$ is the number of bad faces in the drawing of $J\setminus \hat E$ induced by $\rho'$, then $n_2\leq n_1/2$.
\end{lemma}

It is now easy to complete the proof of Lemma \ref{lem: process a block} using Lemma \ref{lem: one step for bad faces}. As long as the  drawing $\rho'$ of the current graph $J$ contains bad faces (note that the number of bad faces is always either $0$ or at least $2$), we apply the algorithm from Lemma \ref{lem: one step for bad faces} to graph $J$ to compute a set $\hat E$ of edges, then update $J$ by deleting the edges of $\hat E$ from it, while also adding the edges of $\hat E$ to $E^*(B)$, and continue to the next iteration. Once the drawing $\rho'$ of the current graph $J$ contains no bad faces, the algorithm terminates. It is easy to see that the number of iterations in the algorithm is $O(\log n)$, and so, at the end of the algorithm, $|E^*(B)|\leq O\left ((|\chi(B)|+|\Gamma'|)\cdot \poly(\Delta\log n)\right )$.
Consider now the final graph $J$ obtained at the end of the algorithm. Since the drawing $\rho'$ of $J$ contains no bad faces, for every bridge $R\in \rset_{\tilde B'}(G)$, there is a single face of $\rho'$ whose boundary contains all vertices of $L(R)$ (we emphasize that the graph $J$ is no longer be connected, and the vertices of $L(R)$ are now isolated; but the drawing of each such vertex and the face to whose boundary it belongs are fixed by the original drawing $\rho_{\tilde B'}$ of $\tilde B'$). In order to complete the proof of Lemma \ref{lem: process a block}, it is now enough to prove Lemma \ref{lem: one step for bad faces}.

\begin{proofof}{Lemma \ref{lem: one step for bad faces}}
	Throughout the proof, we fix the drawing $\rho'$ of the current graph $J$.
Consider a pair $(F,F')$ of faces in $\fset$. Let $P$ be the shortest path connecting $F$ to $F'$ in the graph dual to the drawing $\rho'$ of $J$. This path defines a curve $\gamma(F,F')$, that starts at the interior of $F$, terminates at the interior of $F'$, and intersects the image of $J$ on edges only. Let $E(\gamma(F,F'))$ be the set of all edges whose images $\gamma(F,F')$ intersects. Equivalently, $\gamma(F,F')$ can be defined as a curve connecting a point in the interior of $F$ to a point in the interior of $F'$ that only intersects the image of $J$ at its edges, and among all such curves $\gamma$, it minimizes $|E(\gamma)|$. We define the distance between $F$ and $F'$ to be $\dist(F,F')=|E(\gamma(F,F'))|$. Equivalently, $\dist(F,F')$ is the minimum cardinality of a set $\tilde E\subseteq E(J)$ of edges, such that in the drawing of $J\setminus \tilde E$ induced by $\rho'$, the faces $F$ and $F'$ are merged into a single face.

Let $\fset'\subseteq \fset$ be the set of all bad faces. For each bad face $F\in \fset'$, let $\hat F\in \fset'$ be the face minimizing $\dist(F,\hat F)$. Let $\Pi=\set{(F,\hat F)\mid F\in \fset'}$ be the resulting set of pairs of bad faces; note that a bad face may participate in several such pairs. We define $\hat E=\bigcup_{F\in \fset'}E(\gamma(F,\hat F))$. In other words, set $\hat E$ contains, for every pair $(F,\hat F)\in \Pi$ of bad faces, the set $E(\gamma(F,\hat F))$ of edges -- the minimum-cardinality set of edges whose removal from $J$ results in a merge of these faces. Notice that, since a bad face may participate in several pairs in $\Pi$, it is possible that more than two faces may be merged into a single face. It is immediate to verify that, after the edges of $\hat E$ are removed from $J$, the number of bad faces decreases by at least factor 2 (recall that no new bad faces may be created, since the bad faces are only defined with respect to the original set $\rset_{\tilde B'}(G)$ of bridges). It now only remains to show that $|\hat E|\leq O(|\chi(B)|\cdot \Delta\log n)$. 
We do so in the next claim, whose proof completes the proof of Lemma \ref{lem: one step for bad faces}.

\begin{claim}
	$|\hat E|\leq O((|\Gamma'|+|\chi(B)|)\cdot \Delta\log n)$. 
\end{claim}

\begin{proof}

For each bad face $F\in \fset'$, we denote by $c(F)=\dist(F,\hat F)$. It is enough to show that $\sum_{F\in \fset'}c(F)\leq O(\chi(\tilde B')\cdot \Delta)$.
%Consider now some bad face $F\in \fset'$, and let $R\in \rset_{\tilde B'}(G)$ be the bad bridge that is responsible for $F$ being bad.
%We denote by $F'\in \fset'$ any face with a vertex of $L(R)$ lying on the boundary of $F'$, such that $F'\neq F$. We call $F'$ the \emph{twin face} of $F$.

\iffalse

Our proof uses the notion of $G$-normal curves:

\begin{definition} 
Suppose we are given a planar graph $\hat J$ together with its plane drawing, and any simple curve $\gamma$ in this drawing (that is, $\gamma$ does not intersect itself). We say that $\gamma$ is an \emph{$\hat J$-normal curve} iff it intersects the drawing of $\hat J$ in its vertices only. The \emph{length} of $\gamma$ is the number of vertices of $\hat J$ that lie on $\gamma$.
\end{definition}

We also use the following easy observation.

\begin{observation}\label{obs: long normal curve between bad vertices}
	Let $F\in \fset'$ be a bad face, and let $F'$ be its twin face. Consider the drawing $\rho'$ of $J$, and let $\gamma$ be a $J$-normal curve connecting a vertex that lies on the boundary of $F$ to a vertex that lies on the boundary of $F'$. Then the length of $\gamma$ is at least $c(F)/\Delta$.
\end{observation}
\begin{proof}
	Assume for contradiction that the claim is false. Let $U\subseteq V(J)$ be the set of all vertices of $J$ whose images lie on the curve $\gamma$.
	We can slightly modify the curve $\gamma$, obtaining a new curve $\gamma'$, that starts at a point in the interior of $F$, terminates at a point in the interior of $F'$, does not intersect images of vertices of $J$, and only intersects images of those edges of $J$ that are incident to the vertices of $U$. Therefore, curve $\gamma'$ intersects images of fewer than $c(F)$ edges of $J$, and so $\dist(F,F')<c(F)$, contradicting the definition of $c(F)$.
\end{proof}
\fi


\iffalse
We partition the set $\fset'$ of bad faces into $O(\log n)$ classes $\fset'_1,\ldots,\fset'_z$, for $z\leq O(\log n)$ as follows. For $1\leq i\leq z$, face $F\in \fset'$ lies in class $\fset'_i$ iff $2^i\leq c(F)<2^{i+1}$. Clearly, there must be an index $i^*$, such that $\sum_{F\in \fset'_i}c(F)\geq \sum_{F'\in \fset'}c(F')/O(\log n)$. We denote $\fset'_{i^*}=\fset^*$ and $c^*=2^{i^*}$. Therefore, for every bad face $F\in \fset^*$, $c^*\leq c(F)<2c^*$. 

Notice that we can assume that $c^*$ is greater than a large enough constant. This is since $|F^*|\geq |\Gamma'|$ must hold, as each bad face contains at least one terminal of $\Gamma'$ on its inner boundary, and so, if $c^*$ is bounded by a constant, we get that $\sum_{F'\in \fset'}c(F')\leq O(c^*\cdot |\fset^*|\cdot \log n)\leq O(|\Gamma'|\log n)$. We will assume from now on that $c^*$ is greater than some large constant, say $100$. It is now enough to prove the following claim.

\begin{claim}\label{claim: Fstar is large enough}
 $|\fset^*|\leq O(|\chi(B)|\Delta/c^*)$. 
\end{claim}

Indeed, if the claim is true, then:

\[\sum_{F'\in \fset'}c(F')\leq O(\log n)\cdot \sum_{F\in \fset^*}c(F)\leq O(|\fset^*|\cdot c^*\cdot \log n)\leq O(|\chi(B)|\Delta\log n).
\]


From now on we focus on the proof of \ref{claim: Fstar is large enough}. 
\fi

In the remainder of the proof, we will compute a large subset $\hat \fset\subseteq \fset'$ of bad faces, and associate, with each face $F\in \hat \fset$, a subset $\chi^F$ of $\Omega(c(F)/\Delta)$ crossings $\chi(B)$, such that for $F\neq F'$, $\chi^F\cap \chi^{F'}=\emptyset$. This will be used in order to show that $\sum_{F\in \fset'}c(F) \leq O((|\Gamma'|+|\chi(B)|)\cdot \Delta\log n)$.

More precisely, we start by constructing, for each  (but one) bad face $F\in \fset'$, a collection $\yset(F)$ of $\Omega(c(F)/\Delta)$ disjoint cycles in graph $J$. We will ensure that all cycles in $\bigcup_{F\in \fset'}\yset(F)$ are completely disjoint from each other. Moreover, the collections of cycles will have a nice structure that will allow us to organize all faces in $\fset'$ into a forest-like structure, which will in turn allow us to select a subset $\hat \fset\subseteq \fset'$ of faces with $\sum_{F\in \hat \fset}c(F)\geq \Omega(\sum_{F\in \fset'}c(F)/\log n)$, such that the faces in $\hat \fset$ correspond to vertices of degree $1$ and $2$ in the forest, and all values $c(F)$ of such faces are close to each other. For each face $F\in \hat \fset$, we will use the cycles in $\yset(F)$ in order to define a subgraph of graph $B^*$, that will in turn allow us to define the subset $\chi^F\subseteq \chi(B)$ of $\Omega(c(F)/\Delta)$ crossings in $\chi(B)$.

The remainder of the proof consists of three parts. In the first part, we define the collections $\yset(F)$ of cycles for the bad faces $F\in \fset'$. In the second part, we prove that the resulting collections of cycles are disjoint, and use their structure in order to organize the faces of $\fset'$ into a forest, selecting a large subset $\hat \fset\subseteq \fset'$ of faces. Lastly, in the third part, we associate a subgraph of $B^*$ with each face $F\in \hat \fset$, and use this subgraph in order to define the set $\chi^F\subseteq \chi(B)$ of crossings.


\paragraph{Part 1: Defining the families of cycles.}
Let $F^*\in \fset'$ be a face with minimum value $c(F^*)$, breaking ties arbitrarily. Note that $c(F^*)\leq \half \sum_{F\in \fset'}c(F)$. In the remainder of the proof, view $F^*$ as the outer face of the current drawing $\rho'$ of the graph $J$. We now define, for each face $F\in \fset'\setminus\set{F^*}$, a set $\yset(F)$ of cycles, in graph $J$, using the notion of \emph{tight concentric cycles}, that was used in \cite{chuzhoy2016improved}, and is defined next.
%For the remainder of the proof it may be convenient to think of $\rho'$ as a drawing of $J$ on the sphere instead of the plane.

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%\paragraph{Tight Concentric Cycles.}

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------



Suppose we are given a planar graph $\hat H$ and its drawing $\psi$ in the plane.
 Consider any simple cycle $Y$ in $\hat H$. We denote by $\gamma(Y)$ the curve that is the drawing of $Y$ in $\psi$ (so $\gamma(Y)$ is the concatenation of the images of the edges of $Y$ in $\phi$). We denote by $D(Y)$ the unique disc in the plane whose boundary is $\gamma(Y)$.


Assume now that we are given any vertex $v$ of $\hat H$. We define a cycle $\mincycle(\hat H,v)$ as follows. We let $\mincycle(\hat H,v)$ be the simple cycle $Y\subseteq \hat H$ with $v$ lying in the interior of the disc $D(Y)$ (so $v\not\in V(Y)$), for which $D(Y)$ is smallest inclusion-wise. 

\iffalse
\begin{definition}
	Given a planar graph $H$ drawn in the plane and a vertex $v \in V(H)$ that is not incident to the infinite face, $\mincycle(H, v)$ is the cycle $C$ in $H$, such that: (i) $v\in\dnot(C)$; and (ii) among all cycles satisfying (i), $C$ is the one for which $D(C)$ is minimal inclusion-wise. 
\end{definition}
\fi

It is easy to verify that, if graph $\hat H$ contains a cycle $Y$ with $v$ lying in the interior of $D(Y)$, then $\mincycle(\hat H,v)$ is uniquely defined. Indeed, consider the graph $\hat H \setminus v$, and the face $F$ in the drawing of $\hat H \setminus v$ where $v$ used to reside. Then the outer boundary of $F$ is a simple cycle $Y$, and $Y=\mincycle(\hat H, v)$.
 



\begin{definition}
	Suppose we are given a planar graph $\hat H$, an embedding $\psi$ of $\hat H$ in the plane, a simple cycle $Y$ in $\hat H$, and an integral parameter $r\geq 1$. A \emph{family of $r$ tight concentric cycles around $Y$} is a sequence $Z_1,Z_2,\ldots,Z_r$ of disjoint simple cycles in $\hat H$, with the following properties:
	
	\begin{itemize}
		\item $Y=Z_1$;
		
		\item $D(Z_1)\subsetneq D(Z_2)\subsetneq\cdots\subsetneq D(Z_r)$;  and \label{prop: disc}
		
		%\item if $\hat H'$ is the graph obtained from $\hat H$ by contracting all vertices lying in $D(C)$ into a super-node $a$, then $Z_1=\mincycle(\hat H',a)$; and
		
		\item for every $1< h\leq r$, if $\hat H'$ is the graph obtained from $\hat H$ by contracting all vertices lying in $D(Z_{h-1})$ into a super-node $a$, then $Z_h = \mincycle(\hat H', a)$.
	\end{itemize}
\end{definition}

Next, we need the notion of $\hat H$-normal curves.

\begin{definition} 
	Suppose we are given a planar graph $\hat H$ together with its plane drawing, and any simple curve $\gamma$ in this drawing (that is, $\gamma$ does not intersect itself). We say that $\gamma$ is a \emph{$\hat H$-normal curve} iff it intersects the drawing of $\hat H$ in its vertices only. The \emph{length} of $\gamma$ is the number of vertices of $\hat J$ that lie on $\gamma$.
\end{definition}

We need the following observation about tight concentric cycles, that was shown in \cite{chuzhoy2016improved}.

\begin{observation}\label{obs: curve for concentric cycles}
	Let $Z_1,Z_2,\ldots,Z_r$ be a sequence of tight concentric cycles around $Z_1$ in a plane graph $\hat H$. Then for every vertex $v_r\in V(Z_r)$, there is a vertex $v_1\in V(Z_1)$, and an $\hat H$-normal curve $\gamma(v_r,v_1)$ in $\psi$, connecting $v_r$ to $v_1$, such that for all $1\leq i\leq r$, $\gamma(v_r,v_1)$ intersects the image of cycle $Z_i$ on exactly one vertex, and $\gamma$ does not intersect the images of any other vertices of $\hat H$.
\end{observation}

\begin{proof}
	In order to prove the observation, it is enough to show that for all $1\leq i<r$, for any vertex $v_{i+1}\in V(Z_{i+1})$, there is a vertex $v_{i}\in V(Z_{i})$, and a curve $\gamma_{i+1}$ connecting $v_{i+1}$ to $v_{i}$, that intersects the image of $\hat H$ on its endpoints only.
	%Assume for contradiction that such a curve does not exist.
	
	Let $\hat H'$ be the graph obtained from $\hat H$, by deleting all vertices that lie in the interior of $D(Z_i)$, and all vertices that lie outside of $D(Z_{i+1})$. Let $\psi'$ be the drawing of $\hat H'$ induced by $\psi$. Let $\hat H''$ be the graph obtained from $\hat H'$ by contracting all vertices of $Z_i$ into a single super-node $a$, and let $\psi''$ be the resulting drawing. Recall that, if we consider the drawing of $\hat H''\setminus\set{a}$ induced by $\psi''$, then $Z_{i+1}$ is precisely the outer boundary of the face where $a$ used to reside. Therefore, there is a curve $\gamma$ in the drawing $\psi'$ of $\hat H'$, connecting $v_{i+1}$ to $a$, that only intersects the image of $\hat H'$ on its endpoints. It is now immediate to see that there must be a curve  $\gamma_{i+1}$ in the drawing $\psi'$ of $\hat H'$ (and hence in the drawing $\psi$ of $\hat H$), connecting $v_{i+1}$ to some vertex of $Z_i$, that intersects the image of $\hat H$ on its endpoints only.	
	% Let $F$ be a face in this drawing, such that $v_{i+1}$ lies on the boundary of $F$, and $F\subseteq D(Z_{i+1})$. Note that the boundary of $F$ may not contain a vertex of $Z_i$, since otherwise there must be a curve connecting $v_{i+1}$ to a vertex of $Z_i$ that intersects the image of $\hat H$ on its endpoint only. Since $v_{i+1}$ lies on the boundary of $F$, the outer boundary of $F$ intersects $Z_{i+1}$. Moreover, it is impossible that the outer 	
\end{proof}




We now consider any bad face $F\in \fset'\setminus\set{F^*}$, and define the family $\yset(F)$ of cycles for it. Let $Y$ be the cycle that serves as the boundary of $F$. We then let $\yset(F)=\set{Z_1(F),Z_2(F),\ldots,Z_{r_F}(F)}$ be a maximal collection of tight concentric cycles around $Y$ in the drawing $\rho'$ of graph $J$  (that is, $r$ is the maximum integer for which such a collection of cycles exists).
 
%Recall that we have defined a face $F'$ in the drawing $\rho'$ of $J$, that we called the twin face of $F$. We let $Y$ be the simple cycle that forms the outer boundary of $F$ and $Y'$ the simple cycle that forms the outer boundary of $F'$. \mynote{need to be careful that neither of them is the outer face.}


%We consider the graph $\tilde B'$ and the drawing $\psi$ of this graph that is induced by the unique drawing $\rho_{\tilde B}$ of $\tilde B$. Let $v$ be any vertex of $Y'$, and let $F^*$ be any face of $\psi$ that has $v$ on its boundary, such that cycle $Y'$ separates the interior of $F^*$ from all vertices of $Y$; it is easy to verify that such a face must exist. We will view the face $F^*$ as the outer face of the drawing $\psi$ of $\tilde B$. Next, we construct a maximal collection $Z_1,Z_2,\ldots,Z_r$ of tight concentric cycles around $Y$ such that $V(Y')\cap V(Z_r)=\emptyset$ (that is, $r$ is the maximum integer for which such a collection of cycles exists).

\begin{claim}\label{claim: many cycles}
	$r\geq c(F)/\Delta$.
\end{claim}
\begin{proof}
	Assume otherwise. 
		Consider the graph $J'$ that is obtained from $J$, after we contract all vertices whose image lies in $D(Z_r(F))$ into a super-node $a$. Since we could not further augment the collection of tight concentric cycles, $\mincycle(J',a)$ does not exist.
		
		Let $Y^*$ be the boundary of the outer face $F^*$. Assume first that some vertex $v\in V(Y^*)$ lies on the cycle $Z_r(F)$. Then, from Observation \ref{obs: curve for concentric cycles}, there is a curve $\gamma$ in the drawing $\rho'$ of $J$, that connects $v$ to some vertex $v'\in V(Y)$, that intersects graph $J$ at exactly $r< c(F)/\Delta$ vertices and no edges. Let $U$ be the set of all vertices of $J$ that $\gamma$ intersects. By slightly adjusting the curve $\gamma$, we can ensure that it originates at a point in the interior of face $F$, terminates at a point in the interior of face $F^*$, does not intersect any vertices of $J$, and only intersects edges of $J$ that are incident to the vertices of $U$. But then $\dist(F,F^*)<c(F)$, a contradiction.
		
		Therefore, we can now assume that no vertex of  $v\in V(Y^*)$ lies on the cycle $Z_r(F)$. But then, since $Y^*$ is a connected graph, and it serves as the boundary of the outer face in the drawing $\rho^*$, no vertex of $V(Y^*)$ may lie in the disc $D(Z_r(F))$, and the cycle $Y^*$ must be present in the graph $J'$, contradicting the fact that $\mincycle(J',a)$ does not exist.
\end{proof}

We discard from $\yset(F)$ all but the first $\floor {c(F)/(10\Delta)}$ cycles, so now $\yset(F)=\set{Z_1(F),Z_2(F),\ldots,Z_{q_F}(F)}$, where $q_F(F)=\floor{c(F)/(10\Delta)}$. For convenience, we denote the disc $D(Z_{q_F}(F))$ by $\dout(F)$.
	
\paragraph{Part 2: Selecting the Set $\hat \fset$ of Bad Faces.}
We start with the following claim, that was also shown in \cite{chuzhoy2016improved}:

\begin{claim}
	All cycles in $\bigcup_{F\in \fset'\setminus\set{F^*}}\yset(F)$ are mutually disjoint.
\end{claim}
\begin{proof}
	Assume otherwise. Then there are faces $F_1,F_2\in \fset'$, with $F_1\neq F_2$, and cycles $Y'\in \yset(F_1)$, $Y''\in \yset(F_2)$, such that $Y'\cap Y''\neq \emptyset$. We let $v$ be any vertex in $V(Y)\cap V(Y'')$. Assume that $Y'$ is the $i$th cycle in $\yset(F_1)$, and that it is the $j$th vertex in $\yset(F_2)$. Assume without loss of generality that $c(F)\leq c(F')$, so $i+j\leq c(F)/(5\Delta)$. Then from Observation \ref{obs: curve for concentric cycles}, there is a curve $\gamma_1$ in the drawing $\psi$ of $\tilde B'$ that connects $v'$ to some vertex of $Y(F_1)$, that intersects at most $i$ vertices of $\tilde B'$ and no edges, and similarly, there is a curve $\gamma_2$ in $\psi$, connecting $v'$ to some vertex of $Y(F_2)$, that intersects at most $j$ vertices of $\tilde B'$ and no edges. By letting $\gamma$ be a concatenation of $\gamma_1$ and $\gamma_2$, we conclude that there is a $J$-normal curve $\gamma$ in $\rho'$, of length at most $c(F)/(5\Delta)$ connecting the interior of face $F_1$ to the interior of face $F_2$. Let $U$ be the set of all vertices of $J$ that $\gamma$ intersects. We can then slightly adjust $\gamma$ so it still connects the interior of face $F_1$ to the interior of face $F_2$, but now it does not intersect any vertices of $J$, and only intersects edges of $J$ that are incident to the vertices of $U$. We get that $\dist(F_1,F_2)<c(F)$, contradicting the definition of $c(F)$.
\end{proof}


Consider now a pair $F_1,F_2\in \fset'\setminus \set{F^*}$ of bad faces. We say that $F_1$ \emph{captures $F_2$} iff the face $F_2$ is contained in the disc $\dout(F_1)$.

The following observation is immediate:

\begin{observation}
	For any bad faces $F_1,F_2,F_3\in \fset'\setminus F^*$:
	\begin{itemize}
\item If $F_1$ captures $F_2$ and $F_2$ captures $F_3$ then $F_1$ captures $F_2$.
\item If $F_1$ captures $F_2$, then $F_2$ does not capture $F_1$.
\item If $F_1$ captures $F_2$, then either $\dout(F_2)\subseteq D(Z_1(F_1))$, or there is some index $1\leq i<q_{F_1}$, such that $\dout(F_2)\subseteq D(Z_{i+1}(F_1))\setminus D(Z_i(F_1))$.
\end{itemize}
\end{observation}

(the last statement follows from the fact that the cycles in $\yset(F_1)$ and $\yset(F_2)$ may not intersect).


Consider now some face $F\in \fset'\setminus \set{F^*}$. We say that $F$ is an \emph{eligible face} iff there is another face $F'\neq F$ with $F'\in \fset'$, such that $F$ does not capture $F'$, and there is some bridge $R\in \rset_{\tilde B'}(G)$ with legs $t,t'\in L(R)$, such that $t$ lies in $F$ and $t'$ lies in $F'$. Let $F^*\subseteq  \fset'\setminus \set{F^*}$ be the set of all eligible faces.





We can now construct a directed graph $\hat G$, whose vertex set is $\fset{v(F)\mid F\in \fset'\setminus \set{F^*}}$, and there is an edge $(v(F),v(F'))$ iff $F'$ interferes with $F$, and there is no face $F''\in \fset'\setminus\set{F^*}$, such that $F''$ interferes with $F$ and $F'$ interferes with $F''$. It is immediate to verify that the resulting graph $\hat G$ is a forest.

Consider now any vertex $v(F)$ of $\hat G$. We say that $v(F)$ is an 


We now proceed to gradually define the set $\hat \fset$ of faces. In order to do so, we start by defining a subset  $\fset^*\subseteq \fset'\setminus \set{F^*}$ of faces, that we will later refine. 

\paragraph{Part 3: Bounding $c(F)$}
Consider again some bad face $F\in \fset'$. We denote $\yset(F)=\set{Z_1,Z_2,\ldots,Z_q}$, where $q=\Omega(c(F)/\Delta)$. We will prove that for all $1\leq i\leq \floor{q/3}$, at least one edge of $C_{3i}\cup C_{3i+1}\cup C_{3i+2}$ must participate in a crossing in any drawing of the graph $G$. This will prove that $\chi(\tilde B')\geq \Omega(\sum_{F\in \fset'}c(F)/\Delta)$ and will thus complete the proof of Lemma \ref{lem: one step for bad faces}. We use the following claim in order to show this.


\mynote{next claim is false. This whole argument is to be fixed}
\begin{claim}\label{claim: crossins in a 3-cycle graph}
	Let $H$ be any  graph, such that there are three disjoint simple cycles $Y_1,Y_2,Y_3$ in $H$, an edge $e^*$ connecting a vertex of $Y_1$ to a vertex of $Y_3$, and three disjoint paths $P_1,P_2,P_3$, such that each path $P_i$ originates at a vertex of $Y_1$, terminates at a vertex of $Y_3$, and contains at least one vertex of $Y_2$. 
	Assume further that $H\setminus\set{e^*}$ is planar.
	Then in any drawing of $H$ in the plane, at least one edge of $Y_1\cup Y_2\cup Y_3$ must participate in a crossing.
\end{claim}
\begin{proof}
	Assume otherwise, that is, we have a planar drawing $\phi$ of $H$, in which on edge of $Y_1\cup Y_2\cup Y_3$ participates in crossings. It will be convenient for us to view $\phi$ as a drawing of $H$ on the sphere.
	Consider the curve $\gamma(Y_2)$ corresponding to the drawing of $Y_2$ in $\phi$. This curve partitions the sphere into two discs $D_1,D_2$.
	 Since the image of $e^*$ does not cross images of edges of $Y_2$, both endpoints of $e^*$ lie in the interior of the same disc - assume w.l.o.g. that it is $D_1$. Since $Y_1$ is a connected graph, and the images of its edges do not cross the edges of $Y_2$, all vertices and edges of $Y_1$ must be drawn in the interior of $D_1$, and the same is true for $Y_3$.
\end{proof}



\end{proof}





\end{proofof}



%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
\iffalse
--------------------------------------

Old stuff

-------------------------------------



We use the following Lemma, whose proof is deferred to Appendix~\ref{apd:crossing_charged_to_consecutive_cycles}.
\begin{lemma}
	\label{lem:crossing_charged_to_consecutive_cycles}
	Let $H$ be a $3$-connected graph and $C_1,\ldots,C_{\ell}$ ($\ell>30$) be vertex-disjoint cycles in $G$, such that, for any $1\le x<y<z\le \ell$, there is no path in $H\setminus C_y$ connecting any vertex of $C_x$ to any vertex of $C_z$. Let $P$ be a path (which does not belong to $H$) that connects a vertex of $C_1$ to a vertex of $C_{\ell}$, then in any drawing of the graph $H\cup P$ on the plane, for each $1\le i\le \ell-2$, at least one cycle of $C_{i}, C_{i+1}, C_{i+2}$ is crossed.
\end{lemma}

\begin{corollary}
	\label{cor:local_crossing}
	Let $H$ be a graph and $C_1,\ldots,C_{\ell}$ ($\ell>30$) be vertex-disjoint cycles in $G$, such that, for any $1\le x<y<z\le \ell$, there is no path of $H\setminus C_y$ connecting any vertex of $C_x$ to any vertex of $C_z$. Let $P$ be a path (which does not belong to $H$) that connects a vertex of $C_1$ to a vertex of $C_{\ell}$, then in any drawing of the graph $H\cup P$ on the plane, the number of crossings that the cycles $C_1,\ldots,C_{\ell}$ participate in is at least $\ell/3$.
\end{corollary}


Let $\cset=\set{C_1,\ldots,C_r}$ be the connected components of $G\setminus \hat E$.
%It is clear that the sets $V(C_1),\ldots,V(C_r)$ is a partition of $V(G)$.
So the each of graphs $C_1,\ldots, C_r$ is a subgraph of $H$. 
Fix a planar drawing $\psi$ of $H$. 
For any cluster $S$ of $H$, we denote by $\psi_{S}$ the induced drawing of $\psi$ on $S$.
%let $\fset_i$ be the collection of faces in the drawing $\psi_{C_i}$. 
We say that a vertex $v\in T\cap V(C_i)$ is a \emph{bad terminal} if there exist another vertex $v'$, a pair of distinct faces $F, F'$ in the drawing $\psi_{C_i}$ and a path $P$, such that (i) $v\in V(F)\setminus V(F')$ and $v'\in V(F')\setminus V(F)$; (ii) the path $P$ consists of edges in $\hat{E}$ {\color{red}(is this what we want to say or we want to say the path consists of edges in $G\setminus C_i$?)}; and (iii) the path $P$ connects $v$ to $v'$.

For each component $C\in \cset$, we run a separate process on $C$ that gradually adds some edges of $E(C)$ into $\hat{E}$. Let $E_C\subseteq E(C)$ be the subset of edges that are added into $E$ {\color{red}($\hat{E}$?)}.
The goal is to ensure that the induced planar drawing of $\psi_{C}$ on $C\setminus E_C$ contains no bad terminals, and $\sum_{C\in \cset}|E_C|=\tilde{O}(|E'|+\cro(G))$.
%Then, for each $C\in \cset$, we add edges of $E_C$ into $\hat{E}$.

Now we fix a component $C\in \cset$. We denote $T(C)=T\cap V(C)$.
%and denote $\psi_C$ to be the induced drawing of $\psi$ on $C$.
We have $\sum_{C\in \cset}|T_C|=O(|E'|)$. 
Let $T^b\subseteq T(C)$ be the set of bad terminals of $C$.
For any sub-cluster $S$ of $C$, we denote by $T^b(S)$ the set of bad terminals in $T^b(S)$ {\color{red}($S$?)}.
Notice that, as the set $T$ changes, $T^b(S)$ also evolves.
Let $\fset_C$ be the set of faces in the drawing $\psi_C$ that contains some bad terminals. It is clear that $|\fset_C|=O(|T(C)|)$. 
%since each vertex lies on the boundary of at most $\Delta=O(1)$ faces.

We now describe the separate process on $C$ that gradually adds edges of $E(C)$ into $\hat{E}$.
The process proceeds in iterations. In the $i$th iteration, it takes as input a tuple $(S,T^b(S), \fset_S)$, where $S$ is a sub-cluster of $C$, $T^b(S)$ is the set of its bad terminals, and $\fset_S$ is a face cover of the vertices of $T^b(S)$ in the drawing $\psi_S$, computes a set $\tilde{E}_i$ of the edges of $S$, and outputs another tuple $(S',T^b(S'), \fset_{S'})$, where $S'=S\setminus \tilde{E}_i$ is a sub-cluster of $S$, $T^b(S')$ is the set of its bad terminals, and $\fset_{S'}$ is a face cover of vertices $T^b(S')$ in the drawing $\psi_{S'}$, such that $|\fset_{S'}|\le |\fset_{S}|/2$.  
The input of the first iteration is $(C,T^b, \fset_C)$.
Whenever in the output tuple $(S',T^b(S'), \fset_{S'})$ of some iteration, the set $T^b(S')=\emptyset$, we terminate the algorithm on $C$.
At the end, let $E_C$ be the union of the sets $\tilde E_i$ in all iterations of the process on $C$.

We now describe the $i$th iteration of the process on $C$.
Let $S^*$ be the dual graph of $S$ with respect to the planar drawing $\psi_S$. From the definition of a dual graph, for each face $F$ in the drawing $\psi_S$, there is a vertex $v_F\in V(S^*)$ in the dual graph $S^*$.
Define $\tilde V=\set{v_F\in V(S^*)\mid F\in\fset_S}$, so $\tilde{V}$ is a subset of $V(S^*)$.
For each $F\in \fset_S$, we perform a BFS in $S^*$ to compute a vertex 
$v^*\in \arg\min_{v\in \tilde{V}}\set{\dist_{S^*}(v,v_{F})}$, with tie breaking arbitrarily.
Let $N(F)\in \fset_S$ be the face of $\psi_S$ that $v^*$ corresponds to, and we also denote $d(F)=\dist_{S^*}(v^*,v_{F})$. We consider two cases.

\textbf{Case 1.} $d(F)\le 30$.
Let $\tilde{E}_i(F)$ be the set that we obtain by applying Lemma~\ref{lem:separating} to the cluster $S$ and its faces $F$ and $N(F)$. 
From Lemma~\ref{lem:separating}, $|\tilde{E}_i(F)|\le 30$.

\textbf{Case 2.} $d(F)> 30$.
Let $\tilde{E}_i(F)$ be the set that we obtain by applying Lemma~\ref{lem:separating} to the cluster $S$ and its faces $F$ and $N(F)$.
From Lemma~\ref{lem:separating}, $|\tilde{E}_i(F)|\le d(F)$.



We let the set $\tilde{E}_i$ be the union of $\tilde{E}_i(F)$ for all $F\in \fset_S$, namely $\tilde{E}_i=\cup_{F\in \fset_S}\tilde{E}_i(F)$. Then we add the edges of $\tilde{E}_i$ into $\hat{E}$ and update $T^b$ accordingly.
From Lemma~\ref{lem:separating}, each face $F$ of $\fset_S$ is merged with the face $N(F)$ after we take out the edges of $\tilde{E}_i$ from $S$. Therefore, we set $S'=S\setminus \tilde{E}_i$, set $T^b(S')=T^b\cap V(S')$, and let $\fset_{S'}$ be the faces in $\psi_{S'}$ that is formed by merging faces of $\fset_{S}$ in $\psi_{S}$. It is easy to see that $|\fset_{S'}|\le |\fset_{S}|/2$. The tuple $(S',T^b(S'), \fset_{S'})$ is our output.
This finishes the description of an iteration of the separate process on $C$, and also finishes the description of the separate process on $C$.

\begin{observation}
	\label{obs:number_of_iterations}
	The separate process on $C$ runs at most $O(\log |T_C|)=O(\log n)$ iterations.
\end{observation}

At the end of the process on $C$, we define $E_C$ to be the union of the sets $\tilde{E}_i$ from all iterations, namely the set of edges that are added into $\hat{E}$ in this process. From the process, it is easy to verify that the induced planar drawing of $\psi_{C}$ on $C\setminus E_C$ contains no bad terminals. It remains to show $\sum_{C\in \cset}|E_C|=\tilde{O}(|E'|+\cro(G))$.

\begin{proposition}
	\label{pro:C_share}
	For each $C\in \cset$, $|E_C|=O(\log n\cdot (|T_C|+\cro_{\phi}(C)))$.
\end{proposition}
\begin{proof}
	Recall that $|\fset_C|=O(|T_C|)$. For each $i>1$, let $(S,T^b(S),\fset_S)$ be the tuple output by the $(i-1)$th iteration of the process on $C$. From the process, 
	$|\fset_S|\le |\fset_C|=O(|T_C|)$.
	Therefore,
	$$\sum_{F\in \fset_S, d(F)\le 30}|\tilde{E}_i(F)|\le O(|T_C|).$$
	For each face $F\in\fset_S$ such that $d(F)>30$, let $L_1,\ldots, L_{d(F)/3}$ be tight concentric cycles \explain around $F$, and let $E_F$ be the set of edges in these cycles. On one hand, it is not hard to see that, for every pair $F, F'$ of faces in $\fset_S$, the edge sets $E_F$ and $E_{F'}$ are disjoint. Therefore, $\sum_{F\in \fset_S}\cro_{\phi}(E_F)\le O(\cro_\phi(S))=O(\cro_\phi(C))$.
	On the other hand, from Corollary~\ref{cor:local_crossing}, 
	$\cro_{\phi}(E_F)= \Omega(d(F))$. Combined together, we have
	\[\sum_{F\in \fset, d(F)>30}|\tilde{E}_i(F)|\le \sum_{F\in \fset, d(F)>30}d(F)=O(\cro_{\phi}(C)).\]
	From Observation~\ref{obs:number_of_iterations}, $|E_C|=\sum_{1\le i\le \log n}|\tilde{E}_i|=O(\log n\cdot (|T_C|+\cro_{\phi}(C)))$. This finishes the proof of Proposition~\ref{pro:C_share}.
\end{proof}

Since the clusters in $\cset$ are mutually vertex-disjoint, we have $\sum_{C\in \cset}\cro_{\phi}(C)=O(\cro(\phi))$. Recall that $\sum_{C\in \cset}|T_C|=O(|E'|)$. As a result,
$\sum_{C\in \cset}|E_C|=O(\log n\cdot(|E'|+\cro(\phi)))$.

For each $C\in\cset$, we denote $C'=C\setminus \hat{E}$.
So far, we have computed a set $\hat{E}$ of edges (and a subset $T\subseteq V(H)$ accordingly), such that, for each component $C'$ of $H\setminus \hat{E}$, in the planar drawing $\psi_{C'}$, there is no path consisting of only edges of $\hat{E}$ that connects two vertices from $T\cap V(C)$ that do not lie on the same face of $\psi_{C'}$. However, we are not yet guaranteed that, for each $C'$, $T\cap V(C')$ is $(1/\poly\log n)$-well-linked in $C'$. Therefore, we still need to perform, for each $C'$, another well-linked decomposition in $C'$ with respect to $T\cap V(C')$ using Lemma~\ref{lem:well_linked-decomposition}. We add into $\hat{E}$ all inter-cluster edges, update $T$ accordingly, and denote by $\cset''=\set{C''_1,C''_2\ldots,C''_t}$ the set of clusters we get. It suffices to show that each $C''\in\cset''$ contains no bad terminals. {\color{red}TODO~}

{\color{red}Comment: we are not yet guaranteed that each connected component is $3$-connected.}



\fi

%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------



%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
\subsection{Stage 2: Obtaining a Decomposition into Acceptable Clusters}

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------

In this subsection we complete the proof of Theorem \ref{thm: can find edge set w acceptable clusters}. We start with a $3$-connected graph $G$ with maximum vertex degree at most $\Delta$, and a planarizing set $E'$ of edges of $G$. We then use Theorem \ref{thm: getting good pseudoblocks} to compute a subset $E_1$ of edges of $G$, with $E'\subseteq E_1$, such that $|E_1|\leq O(|E'|+\cro(G))\poly(\Delta\log n)$.
Throughout the algorithm, we use a parameter \fbox{$\alpha'=8\Delta\alpha=\frac{1}{16 \alphasc(n)\log n}$} (recall that $\alpha=\frac{1}{128\Delta \alphasc(n)\log n}$ is the well-linkedness parameter from the definition of type-2 acceptable clusters).



The remainder of the algorithm is iterative. Throughout the algorithm, we maintain a set $\hat E$ of edges of $G$, initializing $\hat E=E_1$. Throughout the algorithm, we denote $\hH=G\setminus \hat E$, and we let $\hcset$ be the set of all connected components of $\hH$, that we refer to as \emph{clusters}. The set of vertices that serve as endpoints of the edges of $\hat E$ are called \emph{terminals} and the set of all such vertices is denoted by $\hGamma$.
We maintain a partition of $\hcset$ into two subsets: set $\cset^A$ of \emph{active} clusters, and set $\cset^I$ of \emph{inactive} clusters.
Set $\cset^I$ of inactive clusters is in turn partitioned into two subsets, $\cset_1^I$ and $\cset_2^I$. We will ensure that every cluster $C\in \cset_1^I$ is a type-1 acceptable cluster. For every cluster $C\in \cset_2^I$, we will maintain a set $A_C$ of fake edges, such that $C\cup A_C$ is a type-2 acceptable cluster, and we will maintain an embedding $\pset(A_C)$ of all fake edge in $A_C$ 
into $G$. If $e=(u,v)\in A_C$
is a fake edge of cluster $C\in \cset_2^I$, and $P(e)\in \pset(A_C)$ is its embedding, then we will ensure that $P(e)$ is internally disjoint from $C$, and moreover, all internal vertices of $P(e)$ lie in clusters of $\cset^I$. We will also ensure that all paths in $\bigcup_{C\in \cset_2^I}\pset(A_C)$ are internally disjoint.

\paragraph{Vertex Budgets.}
For the sake of accounting, we assign a budget $B(v)$ to every vertex $v\in V(G)$ (as the algorithm progresses, the budget $B(v)$ may change). The budget $B(v)$ is defined as follows. 
If $v$ is not a terminal, that is, $v\not\in \hG$, then $B(v)=0$. Assume now that $v\in \hG$, and 
let $C\in \hcset$ be the unique cluster containing $v$. If $C\in \cset^I$ (that is, $C$ is inactive), then $B(v)=1$. Otherwise, $B(v)=8\Delta\cdot \log_{3/2}(|\hGamma\cap C|)$. At the beginning of the algorithm, the total budget of all vertices is $\sum_{t\in \Gamma}B(t)\leq O(\Delta\cdot |\Gamma|\log n)\leq O(|E_1|\Delta \log n)$. We will ensure that over the course of the algorithm, the total budget of all vertices does not increase. Since the total budget of all vertices is at least $|\hGamma|$ throughout the algorithm, this will ensure that the total number of terminals at the end of the algorithm is bounded by $O(|E_1|\Delta\log n)$.

\paragraph{Initialization.}
At the beginning, we let $\hat E=E'$, and we let $\hcset$ be the set of all connected components of the resulting graph $\hH=G\setminus \hat E$. Every cluster in $\hcset$ is active, so $\cset^A=\hcset$ and $\cset^I=\emptyset$. The set $\hG$ of terminal contains all endpoints of edges in $\hE$. As long as $\cset^A\neq \emptyset$, we perform iterations, that we describe next.


\subsection*{Iteration Description}
We now describe a single iteration.
 Let $C\in \cset^A$ be any active cluster. First, if $|\hGamma\cap V(C)|\leq \mu$, then we add $C$ to set $\cset^I$ of inactive clusters, and we add it to set $\cset^I_1$; clearly, $C$ is a type-1 acceptable cluster. We then proceed to the next iteration. Note that the budgets of vertices may only decrease.

We assume from now on that $|\hGamma\cap V(C)|> \mu$, and we denote, for convenience, $\Gamma'=\hGamma\cap V(C)$. 
Next, we apply the algorithm $\algsc$ for computing the (approximate) sparsest cut to the graph $C$, with the set $\Gamma'$ of terminals. 
Let $(X,Y)$ denote the cut that the algorithm returns, and assume w.l.o.g. that $|X\cap \Gamma'|\leq |Y\cap \Gamma'|$. Denote $E^*=E_C(X,Y)$. Assume first that $|E^*|<\alpha'\cdot \alphasc(n) |X\cap \Gamma'|$. Then we add the edges of $E^*$ to the set $\hat E$, and delete them from $\hH$. We also remove cluster $C$ from $\cset^A$ and from $\cset$, and instead add all connected components of $C\setminus E^*$ to both sets. We then continue to the next iteration. Notice that we may have added new terminals to $\hGamma$ in this iteration: the endpoints of the edges in $E^*$. Let $\Gamma^*$ be the set of endpoints of these edges. The changes in the budgets of vertices are as follows. First, for every new terminal $t\in \Gamma^*$, the budget $B(t)$ may have grown from $0$ to $8\Delta\cdot \log_{3/2} |\Gamma'|$ (this is since the total number of terminals that lie in $X$ at the end of this iteration is at most $|\Gamma'|$ -- the number of terminals that originally lied in $C$, and the same is true for $Y$). Recall however that $|\Gamma^*|\leq 2|E^*|\leq 2 \alpha'\cdot \alphasc(n) |X\cap \Gamma'|$. Therefore, the total increase in the budget of the new terminals is at most $2 \alpha'\cdot \alphasc(n) |X\cap \Gamma'|\cdot 8\Delta\cdot \log_{3/2} n$.
Note that for terminals in $\Gamma'\cap Y$, their budgets can only decrease. Moreover, if we let $k$ be the total number of terminals that lie in $X$ at the end of the current iteration, then, since $|\Gamma'\cap X|\leq |\Gamma'\cap Y|$, and since the cut $(X,Y)$ is sufficiently sparse, we get that $k\leq 2|\Gamma'|/3$. Therefore, the budget of every terminal in $\Gamma'\cap X$ decreases by at least $8\Delta\cdot$, and the total decrease in the budget is therefore at least $|X\cap \Gamma'|\cdot 8\Delta\cdot$. Since \fbox{$\alpha'=\frac{1}{16\alphasc(n)\log_{3/2}n}$}, the total budget of all terminals does not increase.

From now on we assume that algorithm $\algsc$ returned a cut of sparsity at least $\alpha'\cdot \alphasc(n)$. Then we are guaranteed that with high probability, the set $\Gamma'$ of terminals is $\alpha'$-well-linked in $C$. We denote by $U$ the set of all $1$-separator vertices of $C$, that is, a vertex $v\in U$ iff graph $C\setminus v$ is not connected. 

The high-level plan for the remainder of the algorithm is the following. We will remove a small subset of edges from $C$, decomposing it into a collection of connected components, such that all but one of these components are type-1 acceptable clusters. For the remaining component, that we denote by $C^*$, we will define a set $A_{C^*}$ of fake edges, and their embedding into $C$, such that $C^*\cup A_{C^*}$ is a type-2 acceptable cluster. The remainder of the algorithm consists of three steps. In the first step, we compute the decomposition $\zset(C)$ of the cluster $C$ into super-blocks, and we identify a super-block $J^*\in \cset(C)$, such that, roughly speaking, every connected component of $C\setminus J^*$ contains less than $\mu/4$ terminals of $\Gamma'$. In the second step, we compute a block decomposition $\lset(J^*)$ of $J^*$, and identify a pseudo-block $B^*\in \lset(J^*)$, such that every connected component of $C\setminus B^*$ contains at most $\mu$ terminals. In the third and the final step, we select a subset of edges to delete from $C$, define the cluster $C^*$ and the set $A_{C^*}$ of fake edges together with their embedding $\pset(A_{C^*})$ (in fact we will ensure that $C^*\cup A_{C^*}=\tilde B^*$), and complete the iteration. We now describe each of the three steps in turn.

\paragraph{Step 1: selecting a super-block.}

Let $\zset(C)$ be the decomposition of cluster $C$ into super-blocks (maximal $2$-connected components). 
We can naturally associate a tree $T$ with this decomposition, as follows. The set $V(T)$ of vertices is the union of two subsets: set $U$ of separator vertices, and the set $U'=\set{v_J\mid J\in \zset(C)}$ of vertices, that we call \emph{super-nodes}, that represent the super-blocks of the decomposition. For every super-block $J\in \zset(C)$, and every separator vertex $u\in U$, such that $u\in V(J)$, we add the edge $(u,v_J)$ to the graph. It is easy to verify that graph $T$ is indeed a tree. Next, we define weights of vertices of $T$: for a separator vertex $u\in U$, the weight $w(u)$ is $1$ if $u\in \hGamma$, and it is $0$ otherwise. For a super-node $v_J$, the weight is the total number of terminals that lie in $J\setminus U$. For a sub-graph $T'\subseteq T$, the weight of $T'$ is $w(T')=\sum_{u\in V(T')}w(v)$. Clearly, $w(T)=|\Gamma'|$.
The current step is summarized in the following lemma.

\begin{lemma}\label{lemma: finding good super-block}
	There is a super-block $J^*\in \cset(C)$, such that the weight of every connected component of $T\setminus \set{v_{J^*}}$ is at most $\mu/4$.
\end{lemma}
\begin{proof}
	We root the tree $T$ at an arbitrary super-node $v_{J}$. Let $v_{J^*}$ be the lowest (that is, furthest from the root) vertex in the tree $T$, such that the sub-tree of $T$ rooted at $v_{J^*}$ has weight at least $\mu/16$. Consider now the connected components of $T\setminus \set{v_J}$. Let $T'$ be the connected component containing the root vertex (if such a component exists), and let $T_1,\ldots,T_q$ denote the remaining components, where component $T_i$ is the sub-tree of $T$ rooted at a child vertex $u_i$ of $v_J$ (that must be a separator vertex). 
	We need the following two observations.
	
	\begin{observation}\label{obs: few terminals in root component}
		$w(T')<\mu/4$.
	\end{observation}
\begin{proof}
	Assume otherwise. Consider a partition $(X,Y)$ of $V(C)$, that is defined as follows. Set $X$ contains, for every super-node $v_{J'}\in V(T')$, all vertices of $J'$, while set $Y$ contains all remaining vertices of $C$. Since $w(T')\geq \mu/4$, $|X\cap \Gamma'|\geq \mu/4$. Moreover, from the choice of $J^*$, $w(Y)\geq \mu/16$ must hold. Let $u'$ be the parent vertex of $v_{J^*}$ in the tree, that must be a separator vertex, and let $E^*$ be the set of all edges of $C$ that are incident to $u'$. Clearly, $E_C(X,Y)\subseteq E^*$, and so $|E_C(X,Y)|\leq \Delta$. On the other hand, since the set $\Gamma'$ of terminals is $\alpha'$-well-linked in $C$, $|E_C(X,Y)|\geq \alpha'\cdot \min\set{|X\cap \Gamma'|,|Y\cap \Gamma'|}\geq \alpha'\mu/16>\Delta$ (as $\mu=512\Delta \alphasc(n)\log n$, while $\alpha'=\frac{1}{16\alphasc(n)\log n}$), a contradiction.
\end{proof}


	
	\begin{observation}\label{obs: few terminals in child components}
		For all $1\leq i\leq q$, $w(T_i)\leq \mu/4$.
	\end{observation}
\begin{proof}
	Fix some $1\leq i\leq q$, and assume for contradiction that $w(T_i)>\mu/4$. Let $u$ be the child vertex of $v_{J^*}$ in $T$, that serves as the root of the tree $T_i$, and let $T'_1,\ldots,T'_z$ be the trees that are rooted at the child vertices of $u$. From the choice of $v_{J^*}$, for all $1\leq j\leq z$, $w(T'_j)<\mu/16$. Let $j'$ be the smallest index, such that $\sum_{j''=1}^{j'}w(T_{j''})>\mu/16$. Then $\sum_{j''=1}^{j'}w(T_{j''})<\mu/8$ must hold. We define a cut $(X,Y)$ in $C$ as follows. We let $X$ contain, for every super-node $v_J\in \bigcup_{j''=1}^{j'}V(T_{j''})$, all vertices of $J$, and we let $Y=V(C)\setminus X$. From the above discussion, $|X\cap \Gamma'|,|Y\cap \Gamma'|>\mu/16$. Let $E^*$ be the set of all edges that are incident to the vertex $u$. Then $E_C(X,Y)\subseteq E^*$, and we reach a contradiction exactly as in Observation \ref{obs: few terminals in root component}.
\end{proof}
\end{proof}

\paragraph{Step 2: selecting a pseudo-block.}
We root the tree $T$ at the vertex $v_{J^*}$, given by Lemma \ref{lemma: finding good super-block}, and we let $U^*=\set{u_1,\ldots,u_q}$ be set of the child vertices of $v_{J}^*$ in $T$. For each $1\leq i\leq q$, let $T_i$ be the sub-tree of $T$ rooted at $u_i$. 
Let $X_i\subseteq V(C)$ be the set of all vertices of $C$ associated with the tree $T_i$: set $X_i$ contains every separator vertex $u\in U\cap V(T_i)$, and for every super-node $v_J\in V(T_i)$, set $X_i$ contains all vertices of $J$.
Let $\Gamma_i\subseteq \Gamma'$ be the set of all terminals that contribute to $w(T_i)$, so $\Gamma_i=X_i\cap \Gamma'$. % that is, terminal $t$ belongs to $\Gamma_i$, if either $t$ is a separator vertex and belongs to $T_i$, or if there is a super-node $v_{J'}\in V(T_i)$ with $t\in J'$. 

Next, we compute a block decomposition $\lset(J^*)$ of the super-block $J^*$ corresponding to the super-node $v_{J^*}$. 
Consider now any block $B\subseteq J$ (block $B$ may not necessarily be a block of the decomposition). We say that $B$ \emph{owns} a terminal $t\in \Gamma'$ iff one of the following two happen: (i) $t$ is a vertex of $B$; or (ii) $t\in T_i$ for some $1\leq i\leq q$, and $u_i\in V(B)$. 
We use the following lemma in order to select the pseudo-block $B^*$.

\begin{lemma}\label{lemma: find the right block}
	There is a pseudo-block $B^*\in \lset(J)$ that owns at least $\mu/2$ terminals, such that every pseudo-block $B'\in \nset(B)$ owns at most $\mu/2$ terminals.
\end{lemma}
\begin{proof}
	We let $B^*$ be the lowest pseudo-block in the decomposition tree $\tau=\tau(\lset(J^*))$, that owns at least $\mu/2$ terminals (since the super-block $J^*$ owns at least $\mu$ terminals, such a pseudo-block exists). We now claim that every  pseudo-block $B'\in \nset(B)$ owns at most $\mu/2$ terminals. This is clearly true for every child block $B'$ of $B$, from the choice of $B$. It now remains to prove that block $B^c$ owns at most $\mu/2$ terminals. Assume otherwise. 
	
	Let $x,y$ be the endpoints of $B$. We define a partition $(X,Y)$ of $C$ as follows. Set $X$ contains all vertices of $B$. Additionally, for each $1\leq i\leq q$ with $u_i\in B$, we add all vertices of $X_i$ to $X$. We then set $Y=V(C)\setminus X$. Note that $X$ contains all terminals that $B$ owns, and $Y$ contains all terminals that $B^c$ owns, except, possibly, for $x$ and $y$. Therefore $|X\cap \Gamma'|,|Y\cap \Gamma'|\geq \mu/2-2\geq \mu/4$. However, $E_C(X,Y)\subseteq E^*$, so $|E_C(X,Y)|\leq \Delta<\alpha' \mu/4\leq \alpha'\cdot \min\set{|X\cap \Gamma'|,|Y\cap \Gamma'|}$, a contradiction (we have used the fact that $\mu=512\Delta \alphasc(n)\log n$ and $\alpha'=\frac{1}{16\alphasc(n)\log n}$).
\end{proof}



\paragraph{Step 3: defining the clusters.}
Consider the block $B^*\in \lset(J^*)$, given by Lemma \ref{lemma: find the right block}. We will gradually construct a cluster $C^*$ (roughly speaking, $C^*$ is obtained from $\tilde B^*$ by removing the fake edges from it), the set $A_{C^*}$ of fake edges (which roughly correspond to the fake edges of $\tilde B^*$), and an embedding of these edges. We will also add some additional edges to $\hat E$, and ensure that, once these edges are deleted from $C$, we obtain a collection of connected components, where all but one of the components are type-1 acceptable clusters, and the additional component is precisely $C^*$.
%We denote $\nset(B)=\set{B^C,\ldots,B_1,\ldots,B_r}$, where $B_1,\ldots,B_r$ are child blocks of $B$. For each $1\leq i\leq r$, we denote by $x_i,y_i$ the endpoints of the block $B_i$, and we denote the endpoints of $B$ by $(x,y)$. We process the blocks in 
In order to do so, we start by processing the blocks in $\nset(B)$ one-by-one. We now describe an iteration in which some block $B'\in \nset(B)$ is processed.

Let $(x',y')$ denote the endpoints of block $B'$. First, we add to $\hat E$ every edge of $B'$ that is incident to $x'$ or to $y'$. Let $E^*$ be the set of all such edges.
Consider now the connected components of the graph $C\setminus E^*$. Let $C'$ be the unique component containing the vertices of $\tilde B^*$, and let $\cset'$ be the set of all remaining components. Observe that every component of $\cset'$ only contains terminals that were owned by $B'$. The number of such terminals is at most $\mu/2$. Additionally, we have created at most $2\Delta$ terminals by removing the edges of $E'$. Overall, since \fbox{$\mu\geq 8\Delta$}, every connected component of $\cset'$ contains at most $\mu$ terminals. We then add all connected components of $\cset'$ to the set $\cset^I$ of inactive clusters and to the set $\cset^I_1$ of type-1 acceptable clusters, and replace $C$ with $C'$. Additionally, if the edge $(x',y')$ does not belong to the current cluster $C$, then we create a fake edge $e=(x',y')$ for the cluster $C$, that replaces $B'$, and we let $P(e)$ be any path connecting $x'$ to $y'$ in $B'$. 

Once every pseudo-block $B'\in \nset(B)$ is processed, we consider every vertex $u_i\in U^*$ that belongs to $B^*$, one-by-one. For each such vertex $u_i$, we add all edges that are incident to $u_i$, whose other endpoint lies in $X_i$, to the set $\hat E$. Let $E^*$ be the set of all these newly added edges. As before, we consider the set of all connected components of $C\setminus E^*$, denoting by $C'$ the unique component containing the vertices of $\tilde B^*$, and by $\cset'$ the set of all remaining components. For every component $\hat C\in \cset'$, $V(\hat C)\subseteq X_i$, and so $\hat C$ originally contained at most $\mu/2$ terminals. We may have created at most $\Delta$ new terminals -- the vertices that are incident to the edges of $E^*$, so the total number of terminals in each such component $\hat C$ is at most $\mu/2+\Delta\leq \mu$. We add every cluster $\hat C\in \cset'$ to sets $\cset^I$ and $\cset^I_1$.

Consider now the final cluster $C$ that we obtain after each block $B'\in \nset(B^*)$ and every vertex $u_i\in U^*\cap V(B^*)$ are processed. We have defined a set $\aset_C$ of fake edges for $C$, so that $C\cup A_C=\tilde B^*$. Therefore, $C\cup A_C$ is a simple $3$-connected graph, or it is a $K_3$. We have also defined an embedding $\pset(A_C)$ of the fake edges in $A_C$ via paths that are internally disjoint from $C$. We need to do one last step to ensure that $C\cup A_C$ is a type-2 acceptable cluster. Let $\bset$ be the block decomposition of the graph $H=G\setminus E_1$. Let $B\in \bset$ be the block with $V(\tilde B^*) \subseteq V(\tilde B)$ given by Lemma \ref{lem: block containment}. Recall that Theorem \ref{thm: getting good pseudoblocks} guarantees that $B$ is a good block. Let $(x,y)$ be the endpoints of block $B$. If the edge $(x,y)$ belongs to $C$, then we delete it from $C$, and add it to $A_C$ as a fake edge. The embedding of the new fake edge $e$ is $P(e)=(x,y)$.
We denote the final cluster $C$ that we obtain by $C^*$, and we denote its corresponding set of fake edges by $A=A_{C^*}$. We need the following lemma.

\begin{lemma}\label{lemma: resulting cluster is acceptable} $(C^*,A)$ is a type-2 acceptable cluster.
\end{lemma}

We provide the proof of Lemma \ref{lemma: resulting cluster is acceptable} in the following subsection, 
after we complete the proof of  Theorem \ref{thm: can find edge set w acceptable clusters} using it.

All that remains to show now is that the total budget of all vertices does not increase after cluster $C^*$ is processed. We do so next.


\paragraph{Accounting.}
It now remains to show that the total budget of all vertices does not increase. Let $\Gamma'$ be the set of all terminals that belonged to the cluster $C^*$ before we started processing it. Let $\tilde \Gamma$ be the set of all new terminals that were added over the course of processing $C^*$. We further partition $\tilde \Gamma$ into two subsets: set $\tilde \Gamma'$ contains all terminals lying in $V(C^*)$, and set $\tilde \Gamma''$ contains all remaining new terminals. Note that each terminal in $\tilde \Gamma''$ must be connected with an edge to some terminal in $\tilde \Gamma'$, so $|\tilde \Gamma''|\leq \Delta\cdot |\tilde \Gamma'|$.

Consider any new terminal $t\in \tilde \Gamma'$. 
Then either $t\in U^*\cap V(B^*)$, or there is some block $B'\in \nset(B^*)$, such that $t$ is the endpoint of this block. Therefore, the total number of new terminals in $\tilde \Gamma'$ is bounded by $|U^*\cap V(B^*)|+2|\nset(B^*)|$. However, since graph $G$ is $3$-connected, for every vertex $u_i\in U^*$, at least one vertex of $X_i\setminus\set{u_i}$ must be a terminal of $\Gamma'$ (since vertex $u_i$ is a $1$-separator for $X_i\setminus\set{u_i}$. Similarly, for every block $B'\in \nset(B^*)$ with endpoints $x',y'$, if no vertex of $U^*$ lies in $B'\setminus \set{x',y'}$, then some vertex of $V(B')\setminus \set{x',y'}$ must lie in $\Gamma'$. Otherwise, there must be some vertex $u_i\in U^*\cap  (V(B')\setminus \set{x',y'})$, such that some vertex of $X_i\setminus \set{u_i}\in \Gamma'$. Therefore, it is easy that $|\tilde \Gamma'|\leq 2|\Gamma'|$, and $|\tilde \Gamma|\leq (\Delta+1)\cdot |\tilde \Gamma'|\leq 4\Delta|\Gamma'|$.

When the iteration terminates, every vertex of $C^*$ lies in an inactive cluster, so every terminal in $\tilde \Gamma\cup \tilde \Gamma'$ has budget $1$, and the total budget of these vertices is therefore at most $5\Delta|\Gamma'|$. On the other hand, before the current iteration started, every terminal of $\Gamma'$ had budget $8\Delta\cdot \log_{3/2}|\Gamma'|\geq 8\Delta$. Therefore, the total budget of all vertices does not increase.

We conclude that the total budget of all vertices does not increase over the course of the algorithm, and so the number of terminals is always bounded by $O(|E_1|\Delta\log n)=O((|E'|+\cro(G))\cdot \poly(\Delta\log n))$. The algorithm terminates when there are no more active clusters. We are then guaranteed that every cluster $C\in \cset^I_1$ is a type-1 acceptable cluster. For every cluster $C\in \cset^I_2$, we have defined a set $A_C$ of fake edges and their embedding $\pset(A_C)$ into paths that are internally disjoint from $C$, such that $C\cup A_C$ is a type-2 acceptable cluster. Moreover, it is easy to verify from our algorithm that all paths in $\bigcup_{C\in \cset_2}\pset(A_C)$ are mutually internally disjoint. Therefore, in order to complete the proof of Theorem \ref{thm: can find edge set w acceptable clusters}, it is now sufficient to prove Lemma \ref{lemma: resulting cluster is acceptable}.


\subsection{Proof of Lemma \ref{lemma: resulting cluster is acceptable}}
In this subsection we complete the proof of Theorem \ref{thm: can find edge set w acceptable clusters}, by proving Lemma \ref{lemma: resulting cluster is acceptable}.
		First, it is immediate to verify that $C^*\cup A=\tilde B^*$. Therefore, $C^*\cup A$ is a simple $3$-connected graph, or it is a $K_3$.
		
		Second, we claim that the set $\hGamma \cap V(C^*)$ of terminals is $\alpha$-well-linked in $C^*\cup A$, in the following claim.

%-------------------------------
%-------------------------------
%-------------------------------		
\begin{claim}\label{claim: well linkedness of new terminals}
The set $\hGamma \cap V(C^*)$ of terminals is $\alpha$-well-linked in $C^*\cup A$.
\end{claim}
%-------------------------------
%-------------------------------
%-------------------------------

%-------------------------------
%-------------------------------
%-------------------------------	
\begin{proof}
For convenience, we denote by $\Gamma'$ the original set of terminals that belonged to cluster $C$, before cluster $C$ was processed, and we denote by $\Gamma''$ the set of all terminals that belong to $V(C^*)$, after cluster $C$ is processed. For convenience, we also denote $G'=C^*\cup A$.

Consider any partition $(X,Y)$ of $V(C^*)$. Denote $\Gamma_X=\Gamma''\cap X$, $\Gamma_Y=\Gamma''\cap Y$. %, and assume w.l.o.g. that $|\Gamma_X|\leq |\Gamma_Y|$. 
Our goal is to show that $|E_{G'}(X,Y)|\geq \alpha\cdot \min\set{|\Gamma_X|,|\Gamma_Y|}$.

Recall that, in addition to the terminals of $\Gamma'\cap V(C^*)$, the new set $\Gamma''$ of terminals also contains endpoints of all blocks in $\nset(B^*)$, and vertices $u_i\in U^*\cap V(C^*)$. We call such terminals \emph{new terminals} (a new terminal cannot belong to $\Gamma'$). Consider now any such new terminal $t$. We say that it is a \emph{type-1 new terminal} iff there is some block $B'\in \nset(B^*)$, such that $t$ is an endpoint of $B'$, and the other endpoint $t'$ of $B'$ lies in a different set in $\set{X,Y}$ than $t$ (so if $t\in X$, $t'\in Y$ and vice versa). We let $\Gamma^1_X\subseteq \Gamma_X,\Gamma^1_Y\subseteq \Gamma_Y$ be the sets of all type-1 new terminals lying in $X$ and $Y$, respectively. The remaining new terminals are called \emph{type-$2$ new terminals}, and we let $\Gamma^2_X=\Gamma_X\setminus \Gamma^1_X,\Gamma^2_Y=\Gamma_Y\setminus \Gamma^1_Y$ be the sets of type-2 terminals lying in $X$ and $Y$ respectively. Observe that a new terminal may be an endpoint of several blocks in $\nset(B^*)$, and it may be a vertex of $U^*$ (or both). Since the endpoints of every block in $\nset(B^*)$ are connected by a fake edge in $G'$, it is immediate to verify that:

\begin{equation}
|E_{G'}(X,Y)|\geq |\Gamma^1_X|\mbox{  and  } |E_{G'}(X,Y)|\geq |\Gamma^1_Y|. \label{eq: cut comparable to type 1 terminals}
\end{equation}

Next, we modify the cut $(X,Y)$ to obtain a cut $(X',Y')$ in graph $C$, and then use the well-linkedness of the terminals in $\Gamma'$ in graph $C$. We start with $X'=X$ and $Y'=Y$. Next, consider any block $B'\in \nset(B^*)$, and let $(x',y')$ be its endpoints. We define a set $J(B')$ of vertices as follows. First, we add the vertices of $V(B')\setminus \set{x',y'}$ to $J(B')$. Next, for every vertex $u_i\in U^*$ that lies in $V(B')\setminus\set{x',y'}$, we add the vertices of $X_i$ to $J(B')$. Note that the endpoints $x',y'$ of $B'$ are terminals in $\Gamma''$ but they may not have been terminals in $\Gamma'$. However, since we have assumed that graph $G$ is $3$-connected, set $J(B')\setminus \set{x',y'}$ must contain at least one terminal that belongs to $\Gamma'$. We denote this terminal by $t_{B'}$, and we will view this terminal as ``paying'' for $x'$ and $y'$ (if they are type-2 new terminals).

If both $x',y'\in X$, then we add all vertices of $J(B')$ to $X$, and otherwise we add them to $Y$. Notice that, if both $x',y'$ lie in the same set in $\set{X,Y}$, then we do not increase the number of edges in the cut $(X,Y)$. Moreover, we can think of replacing the new terminals $x',y'$ with a terminal $t_{B'}\in \Gamma'\setminus \Gamma''$. Assume now that $x'\in X$ and $y'\in Y$ (the other case is symmetric). In this case, we have increased the number of edges in the cut $(X,Y)$ by at most $\Delta$, by adding all edges that are incident to $x'$ to this cut. Note however that the edge $(x',y')$ already belonged to this cut (possibly as a fake edge), so we charge this increase in the cut size to this fake edge. Note also that $x',y'$ must be type-1 new terminals in this case.

Once every block $B'\in \nset(B^*)$ is processed, we perform one last modification to the cut: for every vertex $u_i\in V(C^*)$, if $u_i\in X$, then we add all vertices of $X_i$ to $X$, and otherwise we add them to $Y$. This step does not increase the number of edges in the cut $(X,Y)$. Observe that $u_i$ may be a new terminal, that does not belong to $\Gamma'$. However, since graph $G$ is $3$-connected, set $X_i$ must contain some terminal, that we denote by $t_i$, and we view this terminal as ``paying'' for the terminal $u_i$.

We now obtain a cut $(X',Y')$ in graph $C^*$. From the above discussion:

\begin{equation}
 |E_{C^*}(X',Y')|\leq \Delta\cdot |E_{G'}(X,Y)|.\label{eq: few new edges in cut}
 \end{equation}
 
 
  Consider now the terminals of $\Gamma_X$. Each terminal in $\Gamma_X\cap \Gamma'$ still belongs to $X'$. For each type-2 new terminal in $\Gamma_X$, we have added a terminal of $\Gamma'$ to $X'$ that pays for it, where each newly added terminal of $X'\cap \Gamma'$ pays for at most two terminals in $\Gamma_X$. Therefore, $|\Gamma_X\setminus \Gamma^1_X|\leq 2|\Gamma'\cap X'|$, and similarly $|\Gamma_Y\setminus \Gamma^1_Y|\leq 2|\Gamma'\cap Y'|$. Since the set $\Gamma'$ of terminals was $\alpha'$-well-linked in $C^*$, we get that:

\[|E_{C^*}(X',Y')|\geq \alpha'\cdot\min\set{|\Gamma'\cap X'|,|\Gamma'\cap Y'|}\geq \frac{\alpha'}{2}\cdot \min\set{|\Gamma_X\setminus \Gamma^1_X|,|\Gamma_Y\setminus \Gamma^1_Y|}.  \]

Combining this with Equation \ref{eq: few new edges in cut}, we get that:

\begin{equation}
 |E_{G'}(X,Y)| \geq \frac{\alpha'}{2\Delta}\cdot \min\set{|\Gamma_X\setminus \Gamma^1_X|,|\Gamma_Y\setminus \Gamma^1_Y|}.
 \end{equation}
 
Lastly, combining this with Equation \ref{eq: cut comparable to type 1 terminals}, we get that:

\[ |E_{G'}(X,Y)| \geq \frac{\alpha'}{4\Delta}\min\set{|\Gamma_X|,|\Gamma_Y|}\geq \alpha \min\set{|\Gamma_X|,|\Gamma_Y|}, \]

since \fbox{$\alpha'=8\Delta\alpha$}.
\end{proof}
%-------------------------------
%-------------------------------
%-------------------------------


Recall that graph $C^*\cup A$ is either a simple $3$-connected graph, or it is a $K_3$. Therefore, $C^*\cup A$ has a unique planar drawing, that we denote by $\rho$. This drawing induces a planar drawing of $C^*$, that we denote by $\rho'$. It now remains to prove the following claim, that will conclude the proof of Lemma \ref{lemma: resulting cluster is acceptable}.

\begin{claim}\label{claim: good cluster}
	For every bridge $R\in \rset_G(C^*)$, there is a face $F$ in the drawing $\rho'$, such that the set $L(R)$ of vertices lie on the boundary of $F$.
\end{claim}

\begin{proof}
	The proof of the claim is almost identical to the proof of Claim \ref{claim: every block is good}.
	Throughout the proof, we denote by $E_2$ the set $\hat E$ of edges obtained after cluster $C$ is processed. 

Let $H=G\setminus E_1$ and $H'=G\setminus E_2$, so that $H'\subseteq H$.
Recall that we have denoted by $\bset$ the set of all pseudo-blocks in the block decomposition of the graph $H$. 
Recall also that we have denoted by $B\in \bset(H)$  the pseudo-block corresponding to $B^*$, given by Lemma \ref{lem: block containment}, and by $(x,y)$ the endpoints of $B$. Therefore, $V(\tilde B^*)\subseteq V(\tilde B)$, every real edge of $\tilde B^*$ (except for possibly $(x,y)$) belongs to $\tilde B$ as a real edge, and for every fake edge $e\in E(\tilde B^*)$, there is a path $P(e)$ in $\tilde B$ connecting its endpoints, that is internally disjoint from $\tilde B^*$, such that all paths in $\qset=\set{P(e)\mid e\in A_{B^*}}$ are internally disjoint. Notice that the graph $\tilde B^*$ is precisely $C^*\cup A$, and $A_{B^*}\subseteq A$, while $A\setminus A_{B^*}$ may contain at most one edge -- the edge $(x,y)$. Therefore, $V(C^*)\subseteq V(\tilde B)$; every real edge of $C^*$ is a real edge of $\tilde B$, and set $\qset$ contains a routing of every edge of $A$, except possibly for the edge $(x,y)$.

	
	Assume for contradiction that the claim is false, and let $R\in \rset_G(C^*)$ be a bridge such that not all vertices of $L(R)$ lie on the boundary of a single face of the drawing $\rho'$ of $C^*$.
%	Let $R\in \rset_G(\tilde B^*)$ be a witness for $B^*$.
%Let $B\in \bset_H$ be the corresponding block given by Lemma \ref{lem: block containment}.

Consider the unique planar drawing $\rho_{\tilde B}$ of $\tilde B$. Since every vertex and every real edge of $C^*$ lie in $\tilde B$, this drawing naturally induces a drawing of $C^*$. For convenience, we denote by $\rho''$ the drawing of $C^*$ induced by $\rho_{\tilde B}$. We start with the following claim.

\begin{claim}\label{claim: identical drawings}
	The drawings $\rho'$ and $\rho''$ of $C^*$ are identical. %\snote{$\rho''$ is not defined}
\end{claim}
\begin{proof}
%	Let $A$ be the set of all fake edges of $\tilde B^*$, so that $\tilde B^*_z=\tilde B^*\setminus A$.
	Consider the drawing $\rho''$ of $C^*$. We will show that we can augment this drawing by adding drawings of the edges in $A$, so that the resulting drawing remains planar. Note that, if this is true, then it follows that $\rho'=\rho''$. Indeed, recall that $C^*\cup A=\tilde B^*$ is either a simple $3$-connected graph, or it is a $K_3$, and so it has a unique planar drawing. Therefore the resulting planar drawing of $\tilde B^*$ that we obtain from $\rho''$ is identical to $\rho_{\tilde B^*}$. Therefore, both $\rho'$ and $\rho''$ are obtained from the drawing $\rho_{\tilde B^*}$ of $\tilde B^*$ by deleting the images of the fake edges from $A$ from it, and so $\rho'=\rho''$.

	From now on, it is enough to show that we can augment the drawing $\rho''$ by adding the images of edges in $A$ to it, while preserving the planarity of the drawing. Recall that Lemma \ref{lem: block containment} defines, for every fake edge $e=(u,v)\in A\setminus \set{(x,y)}$, a path $P(e)$ in $\tilde B$ that connects $u$ to $v$, and is internally disjoint from $V(\tilde B^*)$. Moreover, if $e$ and $e'$ are distinct fake edges in $A$, then their corresponding paths $P(e)$ and $P(e')$ are internally disjoint. Recall that these paths are allowed to contain fake edges of $\tilde B$, and that, if graph $\tilde B^*$ contains a real edge connecting the endpoints of $B$, then the resulting paths in $\set{P(e)\mid e\in A\setminus\set{(x,y)}}$ do not contain an edge $(x,y)$. Therefore, we can simply map every fake edge $e\in A\setminus\set{(x,y)}$ to the curve $\gamma(P(e))$ that represents the drawing of the path $P(e)$ in $\rho_{\tilde B}$. Curve $\gamma(P(e))$ is obtained by concatenating the images of the edges of $P(e)$ in $\rho_{\tilde B}$. Since the drawing $\rho_{\tilde B}$ of $\tilde B$ is planar, we obtain a planar drawing of $\tilde B^*$. 
	
	Lastly, if edge $e^*(x,y)$ belongs to $\tilde B^*$ as a real edge, then it does not belong to $C^*$, but it lies in the set $A$ of fake edges. We need to add the image of this edge to our drawing. Recall that $(x,y)$ are the endpoints of the block $B$, and so the edge $e^*$ belongs to $B$ either as a real or a fake edge. Recall that in this case, Lemma \ref{lem: block containment} guarantees that the paths in $\set{P(e)\mid e\in A\setminus\set{e^*}}$ do not contain the edge $(x,y)$. Therefore, we can let $P(e^*)=(x,y)$, embedding the edge $e^*$ into the edge $(x,y)$ in $\tilde B$. We then draw the edge $e^*$ along the image of the edge $(x,y)$ in drawing $\rho_{\tilde B}$ of $\tilde B$.
\end{proof}


Let $\fset$ be the set of all faces of the drawing $\rho'=\rho''$. 
For every vertex $v\in V(\tilde B)\setminus V(C^*)$, there is a unique face $F(v)\in \fset$, such that the image of vertex $v$ in $\rho_{\tilde B}$ lies in the interior of the face $F$.


\mynote{should we define $T_R$ here? Do we need it to have smallest number of edges, or is it enough that it is some tree spanning $L(R)$? (note that $R$ is no longer a bridge of a block, it's a bridge of $C^*$).}
Recall that $T_R$ is the tree with smallest number of edges among all trees in $R$ whose leaves are precisely the vertices of $L(R)$. 
Assume first that $V(T_R)\cap V(\tilde B)=L(R)$. In this case, there is some bridge $R'\in \rset_G(\tilde B')$ of $\tilde B'$ that contains the tree $T_R$, and so $L(R)\subseteq L(R')$. Since $B$ is a good block, there must be a face in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$ whose boundary contains all vertices of $L(R)$. Therefore, for some face $F\in \fset$, all vertices of $L(R)$ must lie on the boundary of $F$. 

Assume now that there is some vertex $v\in V(T_R)\cap  V(\tilde B)$ that does not lie in $L(R)$. Let $F=F(v)$ be the face of $\fset$ in whose interior the image of $v$ in $\rho_{\tilde B}$ lies (recall that $v\not\in V(C^*)$, so it may not lie on a boundary of a face in $\fset$). We will show that all vertices of $L(R)$ must lie on the boundary of $F$, leading to a contradiction. Let $u$ be an arbitrary vertex of $L(R)$. It suffices to show that $u$ must lie on the boundary of the face $F$.

Let $P\subseteq T_R$ be the unique path connecting $v$ to $u$ in $T_R$. Since the leaves of tree $T_R$ are precisely the vertices of $L(R)$, except for $v$, every vertex $x$ of $P$ lies outside $V(C^*)$, and the image of $x$ in $\rho_{\tilde B}$ lies in the interior of some face in $\fset$. Let $u=v_1,v_2,\ldots,v_r=v$ be all vertices of $P$ that belong to $V(\tilde B)$, and assume that they appear on $P$ in this order. 
It remains to prove the following observation.

\begin{observation}
	For $1\leq i<r-1$, $F(v_i)=F(v_{i+1})$. Moreover, $v_r$ lies on the boundary of $F(v_{r-1})$.
\end{observation}
\begin{proof}
	Fix some $1\leq i\leq r-1$. Assume that the observation is false.
	Then there is some face $F'\in \fset$, such that $v_i$ lies in the interior of $F'$, but $v_{i+1}$ does not lie in the interior or on the boundary of $F'$ (the latter case is only relevant for $i=r-1$). Since the boundary of $F'$ separates $v_i$ from $v_{i+1}$, these two vertices cannot lie on the boundary of the same face in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$. 
	
	Let $\sigma_i$ be the subpath of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge connecting $v_i$ and $v_{i+1}$, then it is a bridge in $\rset_G(\tilde B')$, and, since $B$ is a good block, the endpoints of $\sigma_i$ must lie on the boundary of a single face of the drawing $\rho'_{\tilde B'}$, a contradiction. Otherwise, let $\sigma'_i$ be obtained from $\sigma_i$ by deleting the two endpoints from it. Then there must be a bridge $R'\in \rset_G(\tilde B')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. But then there must be a face $F'$ of the drawing $\rho_{\tilde B}$ whose boundary contains $v_i$ and $v_{i+1}$, leading to a contradiction. 
	%	We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B^*_z\subseteq \tilde B'$, and from the way the drawing $\rho'_{\tilde B^*_z}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B^*_z}$ that contains $F_i$.	
\end{proof}







\end{proof}





\iffalse

Finally, we are ready to define acceptable clusters.


\begin{definition}
	A cluster $C\in \cset$ is called \emph{acceptable} iff it is good, and additionally one of the following two properties hold:
	
	\begin{itemize}
		\item either $C$ is $3$-connected, and the vertices of $T\cap V(C)$ are $\alpha$-well-linked in $C$, for $\alpha=1/\poly\log n$ (in which case $C$ is a type-1 acceptable cluster); or
		
		\item $C$ contains at most $O(\Delta \poly\log n)$ terminals, where $\Delta$ is maximum vertex degree in $G$ (in which case $C$ is a type-2 acceptable cluster).
	\end{itemize}
\end{definition}


\fi





==> computing-acceptable-decomposition.tex <==

		
		
\section{Computing a Decomposition into Acceptable Clusters: Proof of Theorem~\ref{thm: can find edge set w acceptable clusters}}
\label{sec:thm1}

\iffalse

A note for fixing things later.
	
	\begin{itemize}
\item The legs of a bridge $R\in \rset_G(\tilde B)$ for a block $B$ may not be terminals. They may be endpoints of the block.
\item For every block that either contains at least one terminal, or has more than 2 fake edges, we can isolate the endpoints of all fake edges (delete all edges incident to them in $G$). This way we can define the ``goodness'' property w.r.t. $\tilde B$ with the fake edges, as the fake edges will be eliminated.

\item For a block that contains no terminals and has 1 or 2 fake edges: if every bridge has all legs on same face we are OK as before (now the legs are the endpoints of the 2 fake edges). But if this is not the case, we need to argue that at least one edge of the block, or both fake edges participate in crossings. If we can show this, then we can again isolate the endpoints of the fake edges. But now every "terminal" lies on boundaries of 2 faces. So it's possible that every pair of terminals lies on the boundary of the same face, but for some bridge its legs don't lie on the boundary of the same face. We can't afford to delete edges incident to terminals unless we can show that some edge of the block participates in crossings.

\item However, we can take the block, and the tree $T_R$, which we can compress into a star, and claim that the resulting graph is not planar, so there must be a crossing. Our problem is when the only crossing is that in which the fake parent-edge participates. We could embed all parent-edges in case of long chains of blocks each of which has 1 child only, or we could turn this chain upside down so the parent-edge stop being parent-edge. (These blocks cannot be $K_3$'s because they are not good, each has 2 fake edges. Both can be embedded without going through each other. Alternatively, we can claim that the parent-block has a crossing in which a real edge participates, because the endpoints of the fake edge have 3 paths connecting them). 

\end{itemize}

\fi



This section is dedicated to the proof of Theorem \ref{thm: can find edge set w acceptable clusters}. 
\iffalse
The proof consists of two stages. In the first stage, we compute a subset $E_1$ of edges of $G$ with $E'\subseteq E_1$ and 
$|E_1|\leq O\left ( (|E'|+\optcro(G))\cdot \poly(\Delta\log n)\right )$. We will ensure that for every connected component $C$ of the resulting graph $G\setminus E_1$, either $C$ contains at most $\mu$ terminals (endpoints of edges of $E_1$) and therefore can be considered a type-1 acceptable cluster, or it has another nice property that is somewhat similar to the Bridge Consistency Property. In the second part of the proof, we augment the edges in $E_1$ to another set $E''$ of edges, and complete the construction of the decomposition. Intuitively, the first stage deals with the Bridge Consistency property, while the second stage ensures the Terminal Well-Linkedness and $3$-Connectivity properties of the type-2 acceptable clusters.
\fi
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
%-----------------------------
We start by introducing some notation and defining the notions of good pseudo-blocks, in the following subsection.
		
\subsection{Good Pseudo-Blocks}
\label{sec: good blocks and acceptable clusters}

Throughout this subsection, we assume that we are given some planarizing set $\hat E$ of edges for the input graph $G$, that is, $G\setminus \hat E$ is planar. We note that $\hat E$ is not necessarily the same as the original planarizing set $E'$, since, as the algorithm progresses, we may add edges to the planarizing set. The definitions in this subsection refer to any planarizing set $\hat E$ that may arise over the course of the algorithm.

Given a planarizing set $\hat E$ of edges for $G$, let $H=G\setminus \hat E$. Recall that we say that a vertex $v$ of $H$ is a \emph{terminal} iff it is incident to some edge in $\hat E$, and we denote the set of terminals by $\Gamma$.

Recall that we have defined a block decomposition of a graph $H$ as follows. We denoted by $\cset=\cset(H)$ the set of all connected components of $H$, and we refer to the elements of $\cset$ as \emph{clusters}. For each cluster $C\in \cset$, we have defined a collection $\zset(C)$ of super-blocks (maximal $2$-connected subgraphs) of $C$, and we denoted $\zset(H)=\bigcup_{C\in \cset}\zset(C)$. Lastly, for each superblock $Z\in \zset(H)$, we let $\lset(Z)$ be the block decomposition of $Z$ given by Theorem \ref{thm: block decomposition}, and we denoted by $\bset(C)=\bigcup_{Z\in \zset(C)}\lset(Z)$ the resulting collection of pseudo-blocks for cluster $C$. The final block decomposition of $H$ is defined to be $\bset(H)=\bigcup_{C\in \cset}\bset(C)$. %, and the elements of $\bset(H)$ are called pseudo-blocks.
 
 
Consider some pseudo-block $B\in \bset(H)$, and let $\tilde B$ be the corresponding graph that is either a $3$-connected graph or isomorphic to $K_3$. 
Recall that $\tilde B$ has a unique planar drawing, that we denote by $\rho_{\tilde B}$. Throughout this section, for any pseudo-block $B$, we denote by $\tilde B'\subseteq \tilde B$ the graph obtained from $\tilde B$ by deleting all its fake edges. Note that $\tilde B'$ may be not $3$-connected, and it may not even be connected. The drawing $\rho_{\tilde B}$ of $\tilde B$ naturally induces a drawing of $\tilde B'$, that we denote by $\rho'_{\tilde B'}$. %\snote{why dont we use the same $\rho_{\tilde B'}$? $\rho_{\tilde B'}$ is the same drawing as $\rho'_{\tilde B'}$ but for a sub-graph.}
Consider now the set $\rset_G(\tilde B')$ of all bridges for $\tilde B'$ in graph $G$. We say that $B$ is a \emph{good pseudo-block} iff for each such bridge $R\in \rset_G(\tilde B')$, there is a face $F$ in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$, whose boundary contains all vertices of $L(R)$. If $B$ is not a good pseudo-block, then it is called a \emph{bad pseudo-block}. Note that, if $B$ is a bad pseudo-block, then there is some bridge $R\in \rset_G(\tilde B')$, such that no face of $\rho'_{\tilde B'}$ contains all vertices of $L(R)$. We call such a bridge $R$ a \emph{witness} for $B$. We note that for each bridge $R\in \rset_G(\tilde B')$ and for every vertex $v\in L(R)$, either $v$ is a terminal of $\Gamma$; or it is an endpoint of a fake edge of $\tilde B$; or it is a separator vertex for the connected component $C$ of $H$ that contains $B$. %\znote{make it an observation?}

\iffalse
\paragraph{Good Clusters.}
Finally, we define good clusters.

\begin{definition}
	We say that a cluster $C\in \cset$ is \emph{good} iff pseudo-block $B\in \bset(C)$ is good.
\end{definition}
\fi



\iffalse
Our algorithm starts with some planarizing set $E'$ of edges, and then, over the course of several steps, gradually adds additional edges to set $E'$. Suppose that at some point we compute a planarizing set $\hat E$ of edges, such that, in the block decomposition given by Theorem~\ref{thm: block decomposition} of every cluster of $G\setminus \hat E$, all pseudo-blocks are good. As the algorithm progresses, and more edges are added to $\hat E$, we would like to claim that this property continues to be preserved. The following lemma allows us to do so. Its proof is deferred to Appendix~\ref{apd:good_cluster_preserving}.

\begin{lemma}\label{lem: good clusters cant be killed}
Suppose we are given two planarizing sets $\hat E,\hat E'$ of edges, with $\hat E\subseteq \hat E'$. Let $H=G\setminus\hat E$ and $H'=G\setminus \hat E'$, so that $H'\subseteq H$. Consider some pseudo-block $B_1\in \bset(H')$, and let $B_2\in \bset(H)$ be the corresponding block given by Lemma \ref{lem: block containment}. Assume further that $\tilde B_2$ does not contain a real edge connecting the endpoints of $B_1$. Then, if $B_2$ is a good pseudo-block, so is $B_1$. % Assume that every pseudo-block in $\bset_H$ is good. Then every pseudo-block in $\bset_{H'}$ is good as well. 
\end{lemma}
\fi



The remainder of the proof of Theorem \ref{thm: can find edge set w acceptable clusters} consists of two stages. In the first stage, we augment the initial planarizing set $E'$ of edges to a new edge set $E_1$, such that 
for every connected component $C$ of $G\setminus E_1$, either $C$ is a type-$1$ acceptable cluster, or every pseudo-block in the block decomposition of $C$ is good. In the second stage, we further augment $E_1$ in order to obtain the final edge set $E''$ and a decomposition of $G$ into acceptable clusters. We now describe each of the two stages in turn.

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------


%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
\subsection{Stage 1: Obtaining Type-1 Acceptable Clusters and Good Pseudo-Blocks}
\label{sec:stage1}

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------



The main result of this stage is summarized in the following theorem.

\begin{theorem}\label{thm: getting good pseudoblocks}
There is an efficient algorithm, that, given a $3$-connected $n$-vertex graph $G$ with maximum vertex degree $\Delta$ and a planarizing set $E'$ of edges for $G$, computes a planarizing edge set $E_1$ with $E'\subseteq E_1$, such that $|E_1|\leq O\left ( (|E'|+\optcro(G))\cdot \poly(\Delta\log n)\right )$, and, if we denote $H_1=G\setminus E_1$, and let $\Gamma_1$ be the set of all endpoints of edges in $E_1$, then for every connected component $C$ of $H_1$, either $|V(C)\cap \Gamma_1|\leq \mu$, or every pseudo-block in the block decomposition $\bset(C)$ of $C$ is a good pseudo-block.
\end{theorem}


The remainder of this subsection is dedicated to proving Theorem \ref{thm: getting good pseudoblocks}. 
%
%
%The goal of this stage is to compute a planarizing edge set $E_1$ with $E'\subseteq E_1$, such that $|E_1|\leq O\left ( (|E'|+\optcro(G))\cdot \poly(\Delta\log n)\right )$, and, if we denote $H=G\setminus E_1$, and by $\Gamma_1$ the set of all endpoints of edges in $E_1$, then for every connected component $C$ of $H$, either $|C\cap \Gamma_1|\leq \mu$, or $C$ has another nice property that is somewhat similar to bridge consistency property, and is defined below. 
We start with a high-level intuition in order to motivate the steps in this stage. Consider any pseudo-block $B\in \bset(H)$ in the block decomposition of the graph $H$. We would like to construct a small set $E^*(B)$ of edges of $\tilde B'$, such that, for every bridge $R\in \rset_G(\tilde B')$, all vertices of $L(R)$ lie on the boundary of a single face in the drawing of $\tilde B'\setminus E^*(B)$ induced by $\rho_{\tilde B}$. In general, we are able to find such an edge set $E^*(B)$, while ensuring that its size is small when compared with the following two quantities. The first quantity is the size of the vertex set $\Gamma'(B)$, that is defined to be the union of (i) all terminals in $\tilde B$; (ii) all endpoints of fake edges of $\tilde B$; and (iii) all separator vertices of $C$ that lie in $\tilde B$, where $C\in \cset$ is the component of $H$ that contains $B$. The second quantity is, informally, the number of crossings in which the edges of $\tilde B'$ participate in the optimal drawing $\phi^*$ of $G$ (we need a slightly more involved definition of the second quantity that we provide later).
We would like to augment $E'$ with the edges of $\bigcup_{B\in \bset(H)}E^*(B)$ to obtain the desired set $E_1$. 
Unfortunately, we cannot easily bound the size of $|E_1|$, as we cannot directly bound $\sum_{B\in \bset(H)}|\Gamma'(B)|$. For example, consider a situation where the decomposition tree $\tau_Z$ associated with some maximal $2$-connected subgraph $Z$ of $H$ contains a long induced path $P$. Then for every vertex $v(B)$ on path $P$, graph $\tilde B$ contains exactly two fake edges, one corresponding to its parent, and the other corresponding to its unique child. Note that, it is possible that many of the graphs $\tilde B$ with $v(B)\in P$ do not contain any terminals or separator vertices of the component of $H$ that contains $B$, so the graphs $\tilde B$ with $v(B)\in P$ may contain many fake edges that cannot be charged to the set $\Gamma$ of terminals. However, we can carefully decompose all such  paths $P$, such that, after we delete a small number of edges from the graph, we obtain a collection of type-1 acceptable clusters, and for each block $B$ with $v(B)\in P$, graph $\tilde B$ is contained in one of these clusters. Our proof proceeds as follows. First, we bound the cardinality of the set $U$ of separator vertices by comparing it to the size of $\Gamma$. 
%Then we ``mark'' some vertices $v(B)$ in the forest associated with the block decomposition $\bset(H)$ of $H$. We say that a block $B$ is marked if its corresponding vertex $v(B)$ is marked.
Then we mark some blocks $B$ in the block decomposition $\bset(H)$ of $H$. 
We will ensure that, on the one hand, we can bound the total cardinality of the sets $\Gamma'(B)$ for all marked blocks $B$, while on the other hand, in the forest associated with the block decomposition $\bset(H)$ of $H$, if we delete all vertices corresponding to the marked blocks in $\bset(H)$, we obtain a collection of paths, each of which can be partitioned into sub-paths that are used to define the type-1 acceptable clusters of $\cset_1'$. Let $\bset'$ denote the set of all marked blocks. For each block $B\in \bset'$, we define a collection $\chi(B)$ of crossings in the optimal drawing $\phi^*$ of $G$, such that $\sum_{B\in \bset'}|\chi(B)|$ can be suitably bounded. We then process each such block $B\in \bset'$ one by one, computing the edge set $E^*(B)$ of $\tilde B$, such that, 
for every bridge $R\in \rset_G(\tilde B')$, all vertices of $L(R)$ lie on the boundary of a single face in the drawing of $\tilde B'\setminus E^*(B)$ induced by $\rho_{\tilde B}$.  The cardinality of $E^*(B)$ will be suitably bounded by comparing it to $|\Gamma'(B)|+|\chi(B)|$. 

We now proceed with the formal proof. 
Throughout the proof, we denote $H=G\setminus E'$ and denote by $\cset$ the set of connected components of $H$ that we call clusters. Recall that the set $\Gamma$ of terminals contains all vertices that are endpoints of the edges of $E'$. 
For every cluster $C\in \cset$, we denote by $U(C)$ the set of all separator vertices of $C$; that is, vertex $v\in U(C)$ iff graph $C\setminus\set{v}$ is not connected. Let $U=\bigcup_{C\in \cset}U(C)$. We start by proving the following observation.

\begin{observation}\label{obs: few sep vertices}
	$|U|\leq O(|\Gamma|)$.
\end{observation}
\begin{proof}
	It suffices to show that, for every cluster $C\in \cset$, $|U(C)|\leq O(|\Gamma\cap V(C)|)$. From now on we fix a cluster $C\in \cset$. Let $\zset(C)$ be the decomposition of $C$ into super-blocks. 
	We can associate a graph $T$ with this decomposition as follows. The set $V(T)$ of vertices is defined to be the union of (i) the set $U(C)$ of separator vertices; and (ii) the set $U'=\set{v_Z\mid Z\in \zset(C)}$ of vertices, representing the super-blocks of the decomposition.
	%We call the vertices in $U'$ \emph{super-nodes}. 
	For every super-block $Z\in \zset(C)$ and every separator vertex $u\in U(C)$ such that $u\in V(Z)$, we add the edge $(u,v_Z)$ to the graph.
	For every pair of distinct separator vertices $u,u'\in U(C)$, such that $(u,u')\in E(C)$ and there is no super-block $Z\in \zset(C)$ that contains both $u$ and $u'$, we add the edge $(u,u')$ to the graph.
	It is easy to verify that graph $T$ is a tree. 
	
	Let $L\subseteq V(T)$ be the set of all leaves of $T$. Clearly, the set of edges in $T$ that are incident to a node with degree at least $3$, that we denote by $\hat E$, has size $O(|L|)$. Observe that $L\subseteq U'$, and moreover, if $v_Z\in L$ corresponds to the super-block $Z\in \zset(C)$, then there must be at least one terminal vertex in $\Gamma\cap V(Z)$ that does not belong to $U(C)$. This follows from the fact that $G$ is $3$-connected, and $|V(Z)\cap U(C)|=1$. Therefore, $|L|\le |\Gamma\cap V(C)|$.
	Similarly, let $U'_2\subseteq U'$ denote the set of vertices of $U'$ that has degree $2$ in $T$, then for each vertex $v_Z\in U'_2$, its corresponding block $Z$ must contain a terminal in $\Gamma\cap V(Z)$ that does not belong to $U(C)$. Therefore, $|U'_2|\le |\Gamma\cap V(C)|$.
	
	Observe that each vertex of $U(C)$ has degree at least $2$ in $T$. 
	Note that, if a vertex $u\in U(C)$ has degree $2$ in $T$, and both neighbors of $u$ also belong to $U(C)$, then $u$ has to be a terminal in $\Gamma\cap V(C)$.
	On the other hand, the number of vertices in $U(C)$ with degree $2$ in $G$ that has at least one neighbor in $U'$ is at most $O(|U'_2|+|\hat E|)$.
	Also observe that, the number of vertices of $U(C)$ that has degree at least $3$ is at most $|L|$. Altogether, $|U(C)|\le O(|\Gamma\cap V(C)|+|U'_2|+|\hat E|+|L|)\le O(|\Gamma\cap V(C)|)$. Summing over all clusters $C\in \cset$, we get that $|U|\le O(|\Gamma|)$.
	%Let $S_2\subseteq V(T)$ be the set of all nodes in $U'$ that have degree $2$ in $T$. Similarly, for every vertex $v_Z\in S_2$, there must be at least one terminal vertex of $\Gamma\cap V(Z)$ in the corresponding superblock $Z$ that does not belong to $U(C)$. Therefore, $|S_1|+|S_2|\leq |\Gamma\cap V(C)|$.
	%Let $T'$ be the tree obtained from $T$ by suppressing every vertex $u\in U(C)$ whose degree in $T$ is $2$. Then $T'$ is a tree, and $|V(T')|\leq O(|S_1|+|S_2|)\leq O(|\Gamma\cap V(C)|)$. Since for every vertex $u\in U(C)$ that has degree $2$ in $T$, both its endpoints are in $U'$, we get that $|V(T)|\leq |V(T')|+|E(T')|\leq O(|V(T')|)\leq O(|\Gamma\cap V(C)|)$. Therefore, $|U(C)|\leq O(|\Gamma\cap V(C)|)$.
\end{proof}
\iffalse
\begin{proof}
It suffices to show that, for every cluster $C\in \cset$, $|U(C)|\leq O(|\Gamma\cap V(C)|)$. From now on we fix a cluster $C\in \cset$. Let $\zset(C)$ be the decomposition of $C$ into super-blocks. 
We can associate a tree $T$ with this decomposition as follows. The set $V(T)$ of vertices is the union of two sets: the set $U(C)$ of separator vertices, and the set $U'=\set{v_Z\mid Z\in \zset(C)}$ of vertices, that represent the super-blocks of the decomposition.
%We call the vertices in $U'$ \emph{super-nodes}. 
For every super-block $Z\in \zset(C)$, and every separator vertex $u\in U(C)$, such that $u\in V(Z)$, we add the edge $(u,v_Z)$ to the graph. It is easy to verify that graph $T$ is indeed a tree. 

Let $S_1\subseteq V(T)$ be the set of all leaves of $T$. Clearly, $S_1\subseteq U'$. Moreover, if $v_Z\in S_1$ corresponds to the super-block $Z\in \zset(C)$, then there must be at least one terminal vertex in $\Gamma\cap V(Z)$ that does not belong to $U(C)$. This follows from the fact that $G$ is $3$-connected, and $|V(Z)\cap U(C)|=1$. 	
Let $S_2\subseteq V(T)$ be the set of all nodes in $U'$ that have degree $2$ in $T$. Similarly, for every vertex $v_Z\in S_2$, there must be at least one terminal vertex of $\Gamma\cap V(Z)$ in the corresponding superblock $Z$ that does not belong to $U(C)$. 
Therefore, $|S_1|+|S_2|\leq |\Gamma\cap V(C)|$.
	
Let $T'$ be the tree obtained from $T$ by suppressing every vertex $u\in U(C)$ whose degree in $T$ is $2$. Then $T'$ is a tree, and $|V(T')|\leq O(|S_1|+|S_2|)\leq O(|\Gamma\cap V(C)|)$.
Since for every vertex $u\in U(C)$ that has degree $2$ in $T$, both its endpoints are in $U'$, we get that $|V(T)|\leq |V(T')|+|E(T')|\leq O(|V(T')|)\leq O(|\Gamma\cap V(C)|)$. Therefore, $|U(C)|\leq O(|\Gamma\cap V(C)|)$.
\end{proof}
\fi


Let $C\in \cset$ be any cluster of $H$, and let  $\zset(C)$ be the set of all super-blocks of $C$. For each super-block $Z\in \zset(C)$, we let $\lset(Z)$ be the block decomposition of $Z$, given by Theorem \ref{thm: block decomposition}. Recall that this block decomposition is associated with a decomposition tree, that we denote for brevity by $\tau_Z$. As before, we denote by $\bset(C)=\bigcup_{Z\in \zset(C)}\lset(Z)$ and by $\bset(H)=\bigcup_{C\in \cset}\bset(C)$ the block decompositions of $C$ and $H$, respectively. Let $\tset$ be the forest that consists of the trees $\tau_Z$ for all $Z\in \bigcup_{C\in\cset}\zset(C)$. Recall that every vertex $v(B)\in \tset$ corresponds to a pseudo-block $B\in \bset(H)$ and vice versa.

Consider now some tree $\tau_Z\in \tset$. We \emph{mark} a vertex $v(B)$ of $\tau_Z$ iff, either vertex $v(B)$ has at least two children in the tree $\tau_Z$, or graph $\tilde B$ contains at least one vertex of $\Gamma\cup U$ that is not an endpoint of a fake edge of $\tilde B$. 
We denote by $\bset'\subseteq \bset(H)$ the set of all pseudo-blocks $B$ whose corresponding vertex $v(B)$ was marked. For each pseudo-block $B\in \bset'$, let $\Gamma'(B)$ be the set of vertices of $\tilde B$ that contains all terminals that lie in $\tilde B$, the vertices of $U$ that lie in $\tilde B$, and all endpoints of the fake edges that belong to $\tilde B$.
We need the following simple observation.

\begin{observation}\label{obs: bound gamma for marked blocks}
	$\sum_{B\in \bset'}|\Gamma'(B)|\leq O(\Delta\cdot|\Gamma|)$.
\end{observation}
\begin{proof}
Consider a pseudo-block $B\in \bset'$. We partition the set $\Gamma'(B)$ of vertices into three subsets: set $\Gamma'_1(B)$ contains all endpoints of fake edges of $\tilde B$; set $\Gamma'_2(B)$ contains all vertices of $\Gamma\setminus U$ that lie in $\tilde B$ and do not serve as endpoints of fake edges, and set $\Gamma'_3(B)$ contains all vertices of $U$ that lie in $\tilde B$ and do not serve as endpoints of fake edges.
	
Notice that the sets $\set{\Gamma'_2(B)}_{B\in \bset'}$ are mutually disjoint, since for any pair $B_1,B_2\in \bset(H)$ of pseudo-blocks in the decomposition, the only vertices of $\tilde B_1$ that may possibly lie in $\tilde B_2$ are vertices of $U$ and vertices that serve as endpoints of fake edges in $\tilde B_1$. 
 Therefore, $\sum_{B\in \bset'}|\Gamma'_2(B)|\leq |\Gamma|$. 

Notice that a vertex $u\in U$ may belong to at most $\Delta$ super-blocks in $\zset(H)$. For each super-block $Z\in \zset(H)$, there is at most one pseudo-block $B\in \lset(Z)$, such that $u$ belongs to $\tilde B$ but is not an endpoint of a fake edge of $\tilde B$. This is because for any pair $B_1,B_2$ of blocks of $\lset(Z)$, the only vertices of $\tB_1$ that may possibly lie in $\tB_2$ are endpoints of fake edges of $\tB_1$. Therefore, $\sum_{B\in \bset'}|\Gamma'_3(B)|\leq \Delta\cdot |U|\leq \Delta \cdot |\Gamma|$, from Observation~\ref{obs: few sep vertices}.
		
In order to bound $\sum_{B\in \bset'}|\Gamma'_1(B)|$,
we partition the set $\bset'$ of pseudo-blocks into two subsets: set $\bset'_1$ contains all pseudo-blocks $B$ such that $v(B)$ has at least two children in the forest $\tset$, and $\bset'_2$ contains all remaining pseudo-blocks.
Let $\bset^*\subseteq \bset(H)$ be the set of all pseudo-blocks whose corresponding vertex $v(B)$ has degree $1$ in $\tset$. Since the original graph $G$ is $3$-connected, and since for each pseudo-block $B\in \bset^*$, $\tilde B$ contains at most one fake edge, for each pseudo-block $B\in \bset^*$, the corresponding graph $\tilde B$ must contain a terminal $t\in \Gamma$ that is not one of its endpoints. 
If $t\not\in U$, then $B$ is the only pseudo-block in $\bset^*$ such that $t\in \tilde B$ and $t$ is not one of the endpoints of $B$. Otherwise, there are at most $\Delta$ such pseudo-blocks in $\bset^*$.
Therefore, $|\bset^*|\leq |\Gamma|+\Delta\cdot |U|\leq O(\Delta\cdot |\Gamma|)$. From the definition of the set $\bset'_1$, it is immediate that the total number of fake edges in all pseudo-blocks of $\bset'_1$ is at most $O(|\bset^*|)\leq O(\Delta\cdot|\Gamma|)$. Therefore, $\sum_{B\in \bset'_1}|\Gamma'_1(B)|\leq O(\Delta \cdot |\Gamma|)$.
Consider now a pseudo-block $B\in \bset'_2$. Then $\tilde B$ contains at most two fake edges and at least one vertex of $\Gamma\cup U$, that is not an endpoint of a fake edge. Therefore, for each pseudo-block $B\in \bset'_2$, $|\Gamma'_1(B)|\leq 4$, and $\sum_{B\in \bset'_2}|\Gamma'_1(B)|\leq 4\sum_{B\in \bset'_2}(|\Gamma'_2(B)|+|\Gamma'_3(B)|)\leq O(\Delta \cdot |\Gamma|)$. Altogether, we conclude that $\sum_{B\in \bset'}|\Gamma'(B)|\leq O(\Delta\cdot |\Gamma|)$.
\end{proof}

The final set $E_1$ of edges is set to be the union of $E'$ and four other edge sets, $\tilde E_1,\tilde E_2,\tilde E_3$ and $\tilde E_4$, that we define next.

%\vspace{-4mm}
\paragraph{Sets $\tilde E_1$ and $\tilde E_2$.}
%Set $\tilde E_1$ of edges is defined as follows. 
We let set $\tilde E_1$ contain, for every pseudo-block $B\in \bset'$ and for every fake edge $e=(x,y)$ of $\tilde B$, all edges of $G$ that are incident to $x$ or $y$. From Observation \ref{obs: bound gamma for marked blocks} and the definition of the set $\Gamma'(B)$, it is immediate that $|\tilde E_1|\leq O(\Delta^2\cdot |\Gamma|)$.
We let set $\tilde E_2$ contain all edges incident to vertices of $U$. From Observation \ref{obs: few sep vertices}, $|\tilde E_2|\leq O(\Delta \cdot |\Gamma|)$.

%\vspace{-4mm}
\paragraph{Set $\tilde E_3$.}
We now define the set $\tilde E_3$ of edges and identify a set $\cset_1'$ of connected components of $H\setminus (\tilde E_1\cup \tilde E_2\cup \tilde E_3)$, each of which contains at most $\mu$ vertices that serve as endpoints of edges in $E'\cup \tilde E_1\cup \tilde E_2\cup \tilde E_3$. %The components of $\cset_1'$ will eventually become type-1 acceptable clusters in the final decomposition, though we may create additional type-1 acceptable clusters.

Consider the graph obtained from the forest $\tset$ by deleting all marked vertices in it. It is easy to verify that the resulting graph is a collection of disjoint paths, that we denote by $\qset$. 
Observe that the total number of paths in $\qset$ is bounded by the total number of fake edges in graphs of $\set{\tilde B\mid B\in \bset'}$, so $|\qset|\leq O(\Delta\cdot |\Gamma|)$ from Observation \ref{obs: bound gamma for marked blocks}.
Next, we will process the paths in $\qset$ one-by-one.

Consider now a path $Q\in \qset$. Notice that, from the definition of marked vertices, for every vertex $v(B)\in Q$, graph $\tB$ may contain at most two fake edges and at most four vertices of $\Gamma\cup U$, and all such vertices must be endpoints of the fake edges of $\tB$. 
For any sub-path $Q'\subseteq Q$, we define the graph $H(Q')$ as the union of all graphs $\tilde B'$, for all pseudo-blocks $B\in \bset(H)$ with $v(B)\in V(Q')$ (recall that graph $\tilde B'$ is obtained from graph $\tilde B$ by removing all fake edges from it). The \emph{weight} $w(Q')$ of the path $Q'$ is defined to be the total number of vertices of $H(Q')$ that belong to $\Gamma\cup U$. We need the following simple observation.

\begin{observation}\label{obs: partition paths}
There is an efficient algorithm that computes, for every path $Q\in \qset$, a partition $\Sigma(Q)$ of $Q$ into disjoint sub-paths $Q_1,\ldots,Q_{z}$, such that for all $Q_i\in \Sigma(Q)$, $w(Q_i)\leq \mu/(2\Delta)$, and all but at most one path of $\Sigma(Q)$ have weight at least $\mu/(4\Delta)$.
\end{observation}
\begin{proof}
We start with $\Sigma(Q)=\emptyset$ and then iterate as  long as $w(Q)>\mu/(2\Delta)$. In an iteration, we let $Q'$ be the shortest sub-path of $Q$ that contains one endpoint of $Q$ and has weight at least $\mu/(4\Delta)$. Since for every pseudo-block $B$ with $v(B)\in Q$, $|(\Gamma\cup U)\cap V(\tilde B)|\leq 4$ and $\mu>16\Delta$, we get that $w(Q')\leq \mu/(2\Delta)$. We add $Q'$ to $\Sigma(Q)$, delete all vertices of $Q'$ from $Q$, and terminate the iteration. Once $w(Q)\leq \mu/(2\Delta)$ holds, we add the current path $Q$ to $\Sigma(Q)$ and terminate the algorithm. %\znote{maybe omit this proof?}
\end{proof}

Consider a sub-path $Q_i\in \Sigma(Q)$ and let $Q_i=(v(B_1),\ldots,v(B_x))$. We assume that $v(B_1)$ is an ancestor of $v(B_x)$ in the forest $\tset$, and we denote by $v(B_{x+1})$ the unique child of $v(B_x)$ in the forest, if it exists. We denote by $\eta(Q_i)$ the set that consists of the endpoints of $B_1$ and the endpoints of $B_{x+1}$ (if $B_{x+1}$ exists).
Note that the only vertices that $H(Q_i)$ may share with other graphs $H(Q_j)$ (for $i\neq j$) are the vertices of $\eta(Q_i)$. Moreover, for any path $Q'\neq Q$ in $\qset$ and any sub-path $Q'_j\in \Sigma(Q')$, the only vertices of $H(Q_i)$ that may possibly belong to $H(Q'_j)$ are the vertices of $\eta(Q_i)$ and $U\cap H(Q_i)$. On the other hand, note that a vertex $u\in U$ may belong to at most $\Delta$ super-blocks of $\zset(H)$. Therefore, for each $u\in U$, the number of graphs in $\set{H(Q_i)\mid Q\in \qset,Q_i\in \Sigma(Q)}$ such that $u\in V(H(Q_i))\setminus \eta(Q_i)$ is at most $\Delta$.
% endpoints of blocks $B_1$ and $B_{x+1}$. Therefore, if $w(Q_i)\geq \mu/(2\Delta)$, then there are at least $\mu/(2\Delta)-4\geq \mu/(4\Delta)$ vertices of $U\cup \Gamma$ that belong to $H(Q_i)$ but do not belong to any other graph $H(Q'_j)\neq H(Q_i)$. Recall that there is at most one path $Q_i\in \Sigma(Q)$ with $w(Q_i)<\mu/(2\Delta)$.
Denote $\Sigma=\bigcup_{Q\in \qset}\Sigma(Q)$ and $\eta=\bigcup_{Q_i\in \Sigma}\eta(Q_i)$. We let $\tilde E_3$ contain all edges of $G$ that are incident to the vertices of $\eta$.
The following observation bounds the cardinality of $\tilde E_3$.
\begin{observation}
\label{obs: third edge set small}
 $|\tilde E_3|\leq O(\Delta^2 \cdot |\Gamma|)$.
\end{observation}
\begin{proof}
Consider any path $Q\in \qset$ and the corresponding subset $\Sigma(Q)$ of its sub-paths. From Observation~\ref{obs: partition paths}, there is at most one path $Q_i\in \Sigma(Q)$ with $w(Q_i)<\mu/4$.
Denote $\Sigma'(Q)=\Sigma(Q)\setminus \set{Q_i}$ and $\Sigma'=\bigcup_{Q\in \qset}\Sigma'(Q)$. Observe that $|\Sigma\setminus \Sigma'|\leq |\qset|\leq O(\Delta \cdot|\Gamma|)$. We claim that $|\Sigma'|\leq O(\Delta\cdot |\Gamma|)$. Note that this implies Observation~\ref{obs: third edge set small}, since every path in $\Sigma$ contributes at most four vertices to set $\eta$, and the maximum vertex degree of a vertex in $\eta$ is at most $\Delta$.
	
It remains to show $|\Sigma'|\leq O(\Delta\cdot |\Gamma|)$.
Consider again some path $Q\in \qset$.	 
Each sub-path $Q_i\in\Sigma'(Q)$ has weight $w(Q_i)\geq \mu/(4\Delta)$. Since $\mu>16\Delta$ and $|\eta(Q_i)|\leq 4$, there are at least $\mu/(8\Delta)$ vertices of $H(Q_i)\setminus \eta(Q_i)$ that belong to $\Gamma\cup U$. Let $S(Q_i)$ be the set of all these vertices. Note that every terminal vertex $t\in \Gamma$ may belong to at most one set $S(Q_i)$ for all paths $Q_i\in \Sigma'$, and every vertex $u\in U$ may belong to at most $\Delta$ such sets. Therefore, $|\Sigma'|\leq \frac{|\Gamma|+\Delta |U|}{\mu/(8\Delta)}\leq O (\Delta\cdot |\Gamma|)$, since $\mu=\Theta(\Delta\cdot \log^{1.5}n)$.
\end{proof}

Consider now the graph $H'=H\setminus (\tilde E_1\cup \tilde E_2\cup \tilde E_3)$. 
From the definition of $\tilde E_1, \tilde E_2, \tilde E_3$, it is immediate that, for every path $Q_i\in \Sigma$,
$\out_G(V(H(Q_i)))\subseteq E'\cup \tilde E_1\cup \tilde E_2\cup \tilde E_3$. Therefore, for every connected component $C$ of $H'$, either $V(C)\subseteq V(H(Q_i))$, or $V(C)\cap V(H(Q_i))=\emptyset$. We let $\cset'_1$ contain all connected components $C$ of $H'$, such that $V(C)\subseteq V(H(Q_i))$ for some path $Q_i\in \Sigma$.
\begin{observation}
Each connected component $\cset'_1$ contains at most $\mu$ vertices that are endpoints of edges in $E'\cup \tilde E_1\cup \tilde E_2\cup \tilde E_3$.
\end{observation}
\begin{proof}
Let $C\in \cset'_1$ be any component, and let $Q_i\in \Sigma$ be the path such that $V(C)\subseteq V(H(Q_i))$. 
Let $S(Q_i)$ be the set of all vertices $v\in V(C)$, such that $v\in U\cup \Gamma\cup \eta(Q_i)$. From the construction of the path $Q_i$ and the definition of $w(Q_i)$, $|S(Q_i)|\leq w(Q_i)+4\leq \mu/(2\Delta)+4$. Notice that a vertex $v$ of $H(Q_i)$ may be an endpoint of an edge in $E'\cup \tilde E_1\cup \tilde E_2\cup \tilde E_3$ iff $v\in S(Q_i)$, or $v$ has a neighbor that lies in $S(Q_i)$. Therefore, the total number of vertices of $C$ that may be incident to edges of  $E'\cup \tilde E_1\cup \tilde E_2\cup \tilde E_3$ is at most $(\Delta+1)|S(Q_i)|\leq (\Delta+1)\cdot (\mu/(2\Delta)+4)\leq \mu$.
\end{proof}


\iffalse
Therefore, we can partition the path $Q$ into sub-paths $Q_1,\ldots,Q_z$, such that, if we denote, for all $1\leq j\leq z$, the set of all terminals lying in graphs in $\set{\tilde B\mid v(B)\in Q_j}$ by $\Gamma_j$, then $|\Gamma_j|\leq q/2$ must hold, and, moreover, if $z>1$, then for all $1\leq j\leq z$, $|\Gamma_j|\geq q/4$.  

 Consider now any resulting path $Q_j$, for $1\leq j\leq z$, and denote $Q_j=(v(B_1),\ldots,v(B_r))$. Let $x_1,y_1$ be the endpoints of $B_1$, and let $x_r,y_r$ be the endpoints of $B_r$. 
 Notice that there are at most four terminals in set $\Gamma_j$ that may be shared by other sets $\Gamma_j'\neq \Gamma_j$: the terminals in $\set{x_1,y_1,x_r,y_r}$; the remaining terminals of $\Gamma_j$ may not belong to any other set $\Gamma_j'$, and moreover, they may not belong to any graph $\tilde B$ whose corresponding vertex $v(B)\not\in Q_j$. Let $H_j$ be the graph obtained by the union of all graphs $\tilde B$ with $B\in V(Q_j)$, after we delete all fake edges. Notice that $H_j$ contains at most $q/2$ terminals.
 We add to $\tilde E_2$ all edges of $G$ that are incident to the vertices $x_1,y_1,x_r,y_r$. 
It is easy to verify that $|\tilde E_2|\leq \Delta\cdot \left(|\qset|+O(\Delta |\Gamma|/q)\right )=O(\Delta \cdot |\Gamma|)$. 
We let $\cset_1'$ contain all connected components $C$ of $H\setminus\set{\tilde E_1\cup \tilde E_2}$ such that for every block $B\in \bset'$, $C\cap \tilde B'=\emptyset$. From the above discussion, for every component $C\in \cset'_1$, the number of vertices of $C$ that are incident to the edges of $E'\cup \tilde E_1\cup \tilde E_2$ is at most $q$.
\fi

%Our first step is to compute a block decomposition $\bset(H)$ of $H$. 
%We denote by $\bset'\subseteq \bset(H)$ the set of all pseudo-blocks $B\in \bset(H)$ for which $\tilde B$ contains more than three vertices. Observe that, if $|V(\tilde B)|\leq 3$, then $\tilde B$ must be a good block.

%\vspace{-4mm}
\paragraph{Set $\tilde E_4$.}
We now define the set $\tilde E_4$ of edges. 
Let $\bset''\subseteq \bset'$ be the set of pseudo-blocks with $|V(\tilde B)|>3$. Note that all pseudo-blocks in $\bset'\setminus \bset''$ are good, since for each pseudo-block $B\in \bset'\setminus \bset''$, graph $\tilde B$ is isomorphic to $K_3$.
Recall that, for every pseudo-block $B\in \bset''$, $\tilde B'$ is the graph obtained from $\tilde B$ by deleting all its fake edges. %Note that the unique planar drawing $\rho_{\tilde B}$ of $B$ induces a drawing of $\tilde B'$, that we denote by $\rho'_{\tilde B'}$. 
We will define, for each pseudo-block $B\in \bset''$, 
a set $E^*(B)$ of edges of $\tilde B'$, that have the following useful property: for every bridge $R\in \rset_{G}(\tilde B')$, all vertices of $L(R)$ lie on the boundary of a single face in the drawing of $\tilde B'\setminus E^*(B)$ induced by $\rho_{\tilde B}$. %This property will allow us to establish the Bridge Consistency Property in the type-2 acceptable clusters in our final decomposition. 
%\znote{this sentence does not relate to $E^*(B)$}
We will then set $\tilde E_4=\bigcup_{B\in \bset''}E^*(B)$.

In order to bound $|\tilde E_4|$, we start by setting up an accounting scheme.
We use Lemma~\ref{lem:block_endpoints_routing} to compute, for each pseudo-block $B\in \bset''$, an embedding $\pset_{\tilde B}=\set{P_{\tilde B}(e)\mid e\in A_{\tilde B}}$ of the set $A_{\tilde B}$ of fake edges of $\tilde B$ into paths that are internally disjoint from $\tilde B$ and are mutually internally disjoint. Recall that all paths in $\pset=\bigcup_{ B\in \bset''}\left(\pset_{\tilde B}\setminus \set{P_{\tilde B}(e^*_{\tilde B})} \right)$ cause edge-congestion at most $O(\log n)$ in $G$, where $e^*_{\tilde B}$ is the fake parent-edge for $B$, that connects the endpoints of $B$ (it is possible that $e^*_{\tilde B}$ is undefined). %\mynote{If the lemma statement remains non-constructive we should add "Our algorithm does not compute the embedding $\pset$ explicitly; we only use it for accounting purposes.". But it's better if it can be made constructive}.

Consider now some pseudo-block $B\in \bset''$. 
%We define a new graph $\tilde B^*$ as follows. We start from graph $\tilde B'$, and then add to it all vertices and edges participating in the paths in $\pset_{\tilde B}$. 
Recall that $\phi^*$ is some fixed optimal drawing of $G$. The set $\chi(B)$ of its crossings is defined to be the union of (i) all crossings $(e,e')$ in $\phi^*$, such that either $e$ or $e'$ is a real edge of $\tilde B$; and (ii) all crossings $(e,e')$ in $\phi^*$, such that $e,e'$ lie on two distinct paths of $\pset_{\tilde B}$ (that is, $e\in \pset_{\tilde B}(e_1)$, $e'\in \pset_{\tilde B}(e_2)$ and $e_1\neq e_2$ are two distinct fake edges of $\tilde B$). 
We need the following simple observation.
\begin{observation}\label{claim: chi is small for each B}
$\sum_{B\in \bset''}|\chi(B)|\leq O(\optcro(G)\cdot \log n)$.
\end{observation}
\begin{proof}
Consider any crossing $(e,e')$ in the optimal drawing $\phi^*$ of $G$. Recall that $e,e'$ may belong to $\chi(B)$ in one of two cases: either at least one of $e,e'$ is a real edge of $\tilde B$; or $e,e'$ lie on two distinct paths in $\pset_{\tilde B}$. In particular, in the latter case, one of the two edges $e,e'$ must lie on a path $P_{\tilde B}(\hat e)$, where $\hat e\neq e^*_{\tilde B}$ (that is, $\hat e$ is not the fake parent-edge of $B$). Note that there may be at most one pseudo-block $B\in \bset''$ for which $e$ is a real edge, and the same is true for $e'$. Moreover, there are at most $O(\log n)$ pseudo-blocks $B\in \bset''$, such that edge $e$ lies on a path of $\pset_{\tilde B}\setminus \set{P_{\tilde B}(e^*_{\tilde B})}$, and the same holds for $e'$. Therefore, there are at most $O(\log n)$ pseudo-blocks $B\in \bset''$ with $(e,e')\in \chi(B)$.
\end{proof}


In order to construct the sets $\set{E^*(B)}_{B\in \bset''}$, we process the pseudo-blocks in $\bset''$ one by one, using the following lemma.
\begin{lemma}\label{lem: process a block}
	There is an efficient algorithm, that, given a pseudo-block $B\in \bset''$, computes a subset $E^*(B)\subseteq E(\tilde B')$ of edges, such that, if $\rho'$ is the drawing of the graph $\tilde B'\setminus E^*(B)$ induced by the unique planar drawing $\rho_{\tilde B}$ of graph $\tilde B$, then for every bridge $R\in \rset_G(\tilde B')$, all vertices of $L(R)$ lie on the boundary of a single face in $\rho'$. Moreover, $|E^*(B)|\leq O((|\chi(B)|+|\Gamma'(B)|)\cdot \poly(\Delta \log n ))$.
\end{lemma}
Notice that Lemma~\ref{lem: process a block} only considers bridges that are defined with respect to the original block $B$, namely bridges in $\rset_G(\tilde B')$. Graph $\tilde B'\setminus E^*(B)$ is probably not even connected, and its bridges in $G$ can be completely different. However, this weaker property turns out to be sufficient for us. % in order to establish the bridge consistency property for the final type-2 acceptable clusters in our decomposition (for each such cluster, all its real edges and the embeddings of all its fake edges will be contained in a single graph $\tilde B$ with $B\in \bset''$).
We defer the proof of Lemma~\ref{lem: process a block} to Section~\ref{sec:proof_of_process_a_block}.
Now we complete the proof of Theorem~\ref{thm: getting good pseudoblocks} using it.

\iffalse
%----------------------
%----------------------
Let $\tilde E$ be a set of edges that contains, for every block $B\in \bset(H)$, the edge connecting the endpoints of $B$, if such an edge is present in $H$. We need the following observation.

\begin{observation}\label{obs: few edges connecting endpoints}
$|\tilde E|\leq O(|E'|)$.	
\end{observation}
\begin{proof}
	Let $C$ be any connected component of $H$, and let $Z$ be any super-block in $\zset(C)$. Consider the block decomposition $\lset=\lset(Z)$ of $Z$, and let $\tau=\tau(\lset)$ be its corresponding block decomposition. 
\end{proof}
%------------------------
%-----------------------
\fi
%
%
We let $\tilde E_4=\bigcup_{B\in \bset''}E^*(B)$. From Observations~\ref{obs: bound gamma for marked blocks} and~\ref{claim: chi is small for each B},
\[
\begin{split}
|\tilde E_4|&=\sum_{B\in \bset''}|E^*(B)|  
\leq \sum_{B\in \bset''} O\left ((|\chi(B)|+|\Gamma'(B)|)\cdot\poly(\Delta\log n)\right )\\ 
&\leq O((|\Gamma|+\optcro(G))\cdot\poly(\Delta\log n))\leq O((|E'|+\optcro(G))\cdot\poly(\Delta\log n)).\end{split}\]



Lastly, we define the edge set $E_1$ to be the union of edge sets $E'$, $\tilde E_1$, $\tilde E_2$, $\tilde E_3$ and $\tilde E_4$. From the above discussion, $|E_1|\leq O((|E'|+\optcro(G))\cdot\poly(\Delta\log n))$. 

Recall that, in graph $G\setminus (E'\cup \tilde E_1\cup \tilde E_2\cup \tilde E_3)$, all vertices in the set $\eta\cup U$ are isolated. From the definition of $\cset'_1$, it is immediate that for any cluster $C\in \cset_1'$, if a vertex of $C$ is incident to an edge in $\tilde E_4$, then this vertex must lie in $\eta$,
% this is because $\cset'_1$ contains not-marked blocks, while the edge set $\tilde E_4$ only contains edges incident to nodes in marked blocks
and therefore $C$ contains a single vertex. Therefore, every cluster $C\in \cset_1'$ remains a connected component of $G\setminus E_1$, and it contains at most $\mu$ vertices that are endpoints of edges in $E_1$. 
\iffalse
\paragraph{Summary of Stage 1:}
To summarize, in this stage we have defined a set $E_1$ of $O((|E'|+\optcro(G))\poly(\Delta\cdot \log n))$ edges, with $E'\subseteq E_1$. Let $\Gamma_1\subseteq V(G)$ be the set of all vertices that serve as endpoints of the edges of $E_1$. We have also defined a collection $\cset_1'$ of connected components of $G\setminus E_1$, such that for each $C\in \cset_1'$, $|C\cap \Gamma_1|\leq \mu$. The components in $\cset_1'$ will become type-1 acceptable clusters in the final decomposition, though we may introduce additional type-1 acceptable clusters. We have also defined a collection $\bset''\subseteq \bset(H)$ of blocks in the block decomposition of the graph $H=G\setminus E'$. For every block $B\in \bset''$, no vertex of $\tilde B$ lies in the components of $\cset_1$. Additionally, for every fake edge $e\in \tilde B$, all edges of $G$ that are incident to the endpoints of $e$ belong to $E_1$. Lastly, we ensured that for every bridge $R\in \rset_{\tilde B'}(G)$, there is a face $F$ in the unique drawing of $\tilde B'\setminus E_1$ whose boundary contains all vertices of $L(R)$ (we have achieved this property for the set $E^*(B)$ of edges, but augmenting the set $E^*(B)$ of edges to $E_1$ cannot destroy this property).
\fi
Denote $H_1=G\setminus E_1$. It is now enough to prove the following claim.
\begin{claim}\label{claim: every block is good}
	For every connected component $C$ of $H_1$ with $C\not\in\cset_1'$, every pseudo-block in the block decomposition $\bset(C)$ of $C$ is good.
\end{claim}
%\vspace{-2mm}
\begin{proof}
Assume for contradiction that the claim is false. Let $B_1\in \bset(C)$ be a bad pseudo-block, and
%, so there must be some pseudo-block $B_1\in \bset_{H_1}$ that is bad. 
let $R\in \rset_G(\tilde B_1')$ be a bridge that is a witness for $B_1$. Note that $|V(B_1)|>3$.
Let $B_2\in \bset(H)$ be the pseudo-block corresponding to $B_1$, given by Lemma \ref{lem: block containment}. 
Recall that $V(\tilde B_1)\subseteq V(\tilde B_2)$;
every real edge of $\tilde B_1$ belongs to $\tilde B_2$ as a real edge, except (possibly) for the edge connecting the endpoints of $B_2$; 
for every fake edge $e=(u,v)$ in $\tilde B_1$, there is a path $P(e)$ in $\tilde B_2$ (that may contain fake edges of $\tilde B_2$) that connects $u$ to $v$, and is internally disjoint from $V(\tilde B_1)$. Moreover, if $e$ and $e'$ are distinct fake edges of $\tilde B_1$, then their corresponding paths $P(e)$ and $P(e')$ are internally disjoint. 
Since $C\not\in\cset_1'$ and $|V(B_1)|>3$, $B_2\in \bset''$.
Since all edges incident to endpoints of fake edges of graph $\tilde B_2$ were added to $\tilde E_1\subseteq E_1$, and since graph $\tilde B_2$ contains a fake edge connecting its endpoints, graph $\tilde B_1$ may not contain a real edge connecting the endpoints of $B_2$.

%We denote the endpoints of $B_2$ by $(x,y)$. Notice that edge $(x,y)$ may not belong to $\tilde B_1'$, since .... then we denote this edge by $e^*$; otherwise, edge $e^*$ is undefined. Note that in either case, graph $\tilde B_2$ must contain a fake edge $(x,y)$.

Note that the unique planar drawing $\rho_{\tilde B_2}$ of $\tilde B_2$ naturally induces a drawing of $\tilde B_1'$,
% (if edge $e^*$ is present in $\tilde B_1'$, we draw it along the image of the fake edge $(x,y)$). 
that we denote by $\rho'$. We also denote by $\rho''=\rho'_{\tilde B_1'}$ the drawing of $\tilde B_1'$ induced by $\rho_{\tilde B_1}$. 
We prove the following claim.
\begin{claim}\label{claim: identical drawings}
	The drawings $\rho'$ and $\rho''$ of $\tilde B_1'$ are identical. %\snote{$\rho''$ is not defined}
\end{claim}
%\vspace{-2mm}
\begin{proof}
Let $A$ be the set of fake edges of $\tilde B_1$, so $\tilde B_1'=\tilde B_1\setminus A$.
Consider the drawing $\rho'$ of $\tilde B_1'$. We will show that we can augment this drawing by adding drawings of the edges in $A$, so that the resulting drawing remains planar. Note that, if this is true, then it follows that $\rho'=\rho''$. To see this, note that $\tilde B_1$ is $3$-connected, so it has a unique planar drawing, and therefore the resulting drawing of $\tilde B_1$ is identical to $\rho_{\tilde B_1}$. Since both $\rho'$ and $\rho''$ are obtained from the drawing $\rho_{\tilde B_1}$ of $\tilde B_1$ by deleting the images of the fake edges from it, $\rho'=\rho''$.

We now show that we can augment the drawing $\rho'$ by adding the images of edges in $A$ to it, while preserving the planarity. Recall that Lemma \ref{lem: block containment} defines, for every fake edge $e=(u,v)\in A$, a path $P(e)$ in $\tilde B_2$ that connects $u$ to $v$, and is internally disjoint from $V(\tilde B_1)$, such that, if $e$ and $e'$ are distinct fake edges in $A$, then their corresponding paths $P(e)$ and $P(e')$ are internally disjoint from each other.  %(Recall that the paths in $\pset$ are allowed to contain fake edges of $\tilde B_2$.) %Moreover, if edge $e^*$ is present in $\tilde B_1'$, then no path in $\pset=\set{P(e)\mid e\in A}$ may contain the fake edge $(x,y)$ of $\tilde B_2$. 
We simply draw every fake edge $e\in A$ along the curve $\gamma(e)$ corresponding to the drawing of the path $P(e)$, that is obtained by concatenating the images of the edges of $P(e)$ in $\rho_{\tilde B_2}$. Since the drawing $\rho_{\tilde B_2}$ of $\tilde B_2$ is planar, we obtain a planar drawing of $\tilde B_1$.
\end{proof}

Let $\fset$ be the set of faces in the drawing $\rho'$ of $\tilde B_1'$. From Lemma~\ref{lem: process a block}, for every bridge $R'\in \rset_G(\tilde B_2')$, if $L(R')\cap V(\tilde B_1')\ne \emptyset$, then there is some face $F\in \fset$, such that all vertices of $L(R')\cap V(\tilde B_1')$ lie on the boundary of $F$ in the drawing $\rho'$.
On the other hand,
for every vertex $v\in V(\tilde B_2)\setminus V(\tilde B_1)$, there is a unique face $F(v)\in \fset$, such that the image of vertex $v$ in $\rho_{\tilde B_2}$ lies in the interior of the face $F(v)$.

Now consider the witness bridge $R$ for $B_1$.
Recall that $T_R\subseteq R$ is a tree whose leaves are precisely the vertices of $L(R)$. 
Assume first that $V(T_R)\cap V(\tilde B_2)=L(R)$. In this case, there is some bridge $R'\in \rset_G(\tilde B_2')$ that contains the tree $T_R$, so $L(R)\subseteq L(R')$. However, from Lemma~\ref{lem: process a block}, all vertices of $L(R')$ lie on the boundary of the same face in the drawing $\rho''$. This leads to a contradiction to $R$ being a witness bridge for $B_1$. %Since $B_2$ is a good block, there must be a face in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B'_2$ whose boundary contains all vertices of $L(R)$.

Assume now that there is some vertex $v\in V(T_R)\cap  V(\tilde B_2)$ that does not lie in $L(R)$. %Let $F=F(v)$ be the face of $\fset$ in whose interior the image of $v$ in $\rho_{\tilde B_2}$ lies. 
We will show that all vertices of $L(R)$ must lie on the boundary of $F(v)$, again leading to a contradiction. Let $u$ be an arbitrary vertex of $L(R)$. %It suffices to show that $u$ must lie on the boundary of the face $F(v)$.
Let $P\subseteq T_R$ be the unique path connecting $v$ to $u$ in $T_R$. Since the leaves of tree $T_R$ are precisely the vertices of $L(R)$, except for $v$, every vertex $x$ of $P$ lies outside $V(\tilde B_1)$, and the image of $x$ in $\rho_{\tilde B_2}$ lies in the interior of some face in $\fset$. Let $v=v_1,v_2,\ldots,v_r=u$ be all vertices of $P$ that belong to $V(\tilde B_2)$, and assume that they appear on $P$ in this order. 
It remains to prove the following observation.

\begin{observation}
	For $1\leq i<r-1$, $F(v_i)=F(v_{i+1})$. Moreover, $v_r$ lies on the boundary of $F(v_{r-1})$.
\end{observation}
\begin{proof}
Fix some index $1\leq i\leq r-1$. Assume for contradiction that the observation is false.
Then there is some face $F'\in \fset$, such that $v_i$ lies in the interior of $F'$, but $v_{i+1}$ does not lie in the interior or on the boundary of $F'$ (the latter case is only relevant for $i=r-1$). Since the boundary of $F'$ separates $v_i$ from $v_{i+1}$, they  cannot lie on the boundary of the same face in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B_2'$. 
Let $\sigma_i$ be the subpath of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge $(v_i,v_{i+1})$, then it is either a bridge in $\rset_G(\tilde B_2')$, or it is an edge of $\tilde B_2'$. In the former case, Lemma \ref{lem: process a block} ensures that the endpoints of $\sigma_i$  may not be separated by the boundary of a face of drawing $\rho'$. In the latter case, the same holds since the drawing $\rho'_{\tilde B_2'}$ is planar. In either case, we reach a contradiction. Otherwise, there exists a bridge $R'\in \rset_G(\tilde B_2')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. However, from Lemma \ref{lem: process a block}, it is impossible that the boundary of a face in the drawing $\rho'$ separates the two vertices, a contradiction. 
	%	We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B_2'}$ of $\tilde B_2'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B_1'\subseteq \tilde B_2'$, and from the way the drawing $\rho'_{\tilde B_1'}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B_1'}$ that contains $F_i$.	
\end{proof}	
\end{proof}

%In order to complete the proof of Theorem \ref{thm: getting good pseudoblocks} it suffices to prove Lemma \ref{lem: process a block}, which we do next.


%-------------------------------------------------------
%-------------------------------------------------------
%-------------------------------------------------------
\subsection{Proof of Lemma \ref{lem: process a block}}
\label{sec:proof_of_process_a_block}
%-------------------------------------------------------
%-------------------------------------------------------
%-------------------------------------------------------
%-------------------------------------------------------
In this section we provide the proof of Lemma~\ref{lem: process a block}. 
We fix a pseudo-block $B\in \bset''$ throughout the proof. For brevity, we denote $\Gamma'=\Gamma'(B)$ and denote $\rho=\rho_{\tilde B}$, the unique planar drawing of $\tilde B$.
%, and $\rho'$ is the drawing of $\tilde B'$ that is induced by $\rho$. 
Recall that $\Gamma'$ contains all terminals of $\Gamma$ (endpoints of edges of $E'$), all endpoints of fake edges of $\tilde B$, and all separator vertices $U\cap V(\tilde B)$. The set $\Gamma'$ of vertices remains fixed throughout the algorithm. Abusing the notation, we call the vertices of $\Gamma'$ \emph{terminals} throughout the proof.
	
Throughout the algorithm, we maintain a subgraph $J$ of $\tilde B$ and gradually construct the set $E^*(B)$. Initially, we set $E^*(B)=\emptyset$ and $J=\tilde B'$, the graph obtained from $\tilde B$ by deleting all its fake edges. Over the course of the algorithm, we will move some edges from $J$ to the set $E^*(B)$. We will always use $\rho'$ to denote the drawing of the current graph $J$ induced by the drawing $\rho$ of $\tilde B$. 
%We note that graph $J$ may become disconnected over the course of the algorithm, but its drawing $\rho'$ is always fixed to be the drawing of $J$ induced by $\rho$.

Notice that a terminal of $\Gamma'$ may belong to the boundaries of several faces in the drawing $\rho'$, which is somewhat inconvenient for us. As our first step, we move all edges that are incident to the terminals in $\Gamma'$ from $J$ to $E^*(B)$. Notice that now each terminal of $\Gamma'$ becomes an isolated vertex
%but its drawing in $\rho'$ is fixed, as $\rho'$ is the unique drawing of the current graph $J$ induced by the drawing $\rho$ of $\tilde B$ (throughout this proof, we only refer to the vertices in the original set $\Gamma'$ as terminals). 
and lies on the (inner) boundary of exactly one face of the current drawing $\rho'$. Clearly, $|E^*(B)|\leq \Delta\cdot |\Gamma'|$.


%--------------------
%--------------------
%--------------------
%--------------------
%--------------------
%--------------------

\iffalse
%--------------------
%--------------------
%--------------------

In our first step, we slightly modify the graph $\tilde B'$ to ensure that every terminal that lies in this graph has degree $1$. This will ensure that every terminal lies on an \emph{inner} boundary of some face of the drawing, and in particular there is a unique face of the drawing on whose boundary the terminal lies. As our algorithm progresses, we may add new edges to the set $E'$, and delete them from $\tilde B'$, creating new terminals. We will ensure that all such new terminals have degrees at most $1$ as well.

In order to achieve this, we construct a new graph $J$ from $\tilde B'$, as follows. We start with $J=\tilde B'$. Next, for every edge $e=(u,v)\in E(J)$, we subdivide the edge by two new vertices, replacing it with a path $(u,u_e,v_e,v)$. We denote the edges $(u,u_e),(u_e,v_e)$ and $(v_e,v)$ by $e_1,e_2$ and $e_3$, respectively. Each of these edges is referred to as a \emph{segment} of $e$, and edge $e_2$ is called the \emph{middle segment} of $e$. We will maintain a set $\hat E$ of edges that we gradually delete from $J$. Eventually, set $E^*(B)$ will contain every edge whose segment belongs to $\hat E$. At the beginning, $\hat E$ contains all edges (incident to the terminals of $\Gamma'$) that we have removed so far. Throughout the algorithm, the set $\Gamma'$ of terminals contains all vertices that are endpoints of edges in $E'\cup \hat E$.

Next, we consider the terminals $t\in \Gamma'$ one-by-one. We would like to ensure that the degree of each such terminal in $J$ is $1$. Consider any such terminal $t$, and assume that its degree in the current graph $J$ is greater than $1$. Let $(t,v)\in E(J)$ be any edge that is incident to $t$. We add this edge to $\hat E$ and delete it from $J$. Vertex $v$ now becomes a terminal, and its degree in $J$ is $1$, since $(e,z)$ must be a segment of some edge $e\in E(\tilde B')$ that was incident to $t$. Once we process all terminals that belonged to the original set $\Gamma'$, the cardinality of $\Gamma'$ increases by at most factor $\Delta$, and we are now guaranteed that every terminal in $\Gamma'$ has degree $1$ in $J$. In the remainder of the algorithm, whenever an edge $e\in E(J)$ is added to the set $\hat E$ of deleted edges, if $e$ is a segment of some edge $e'\in E(\tilde B')$, then we will ensure that $e$ is the middle segment of $e'$. This will ensure that all terminals that are added to $\Gamma'$ over the course of the algorithm have degree at most $1$. As the algorithm progresses, we denote by $\phi$ the drawing of $J$  that is induced by the drawing $\rho'$ of $\tilde B'$, and we denote by $\fset$ the set of its faces.
\fi


From now on, we denote by $\fset$ the set of all faces in the drawing $\rho'$ of the current graph $J$.
For every terminal $t\in \Gamma'$, there is a unique face $F(t)\in \fset$, such that $t$ lies on the (inner) boundary of $F(t)$. For a face $F\in \fset$, we denote by $\Gamma(F)\subseteq \Gamma'$ the set of all terminals $t$ with $F(t)=F$.

\paragraph{Bad Faces.} 
We denote by $\rset=\rset_{G}(\tilde B')$ the set of bridges for the graph $\tilde B'$ in $G$.
For each bridge $R\in \rset$, it is not hard to see that all vertices in $L(R)$ are terminals. Let $\fset(R)=\set{F\in \fset\mid L(R)\cap \Gamma(F)\neq \emptyset}$ be the set of all faces in the drawing $\rho'$ of the current graph $J$, whose inner boundaries contain terminals of $L(R)$. We say that a bridge $R\in \rset$ is \emph{bad} for $J$ iff $|\fset(R)|>1$, namely, not all vertices of $L(R)$ lie on the boundary of the same face of $\fset$. In such a case, we say that every face in $\fset(R)$ is a \emph{bad face}, and for each face $F\in \fset(R)$, we say that bridge $R$ is \emph{responsible for $F$ being bad}. As the algorithm progresses and the graph $J$ changes, so does the set $\fset$. The set $\rset$ of bridges does not change over the course of the algorithm, and the definitions of the sets $\fset(R)$ of faces for $R\in \rset$ and of bad faces are always with respect to the current graph $J$ and its drawing. 
The main subroutine that we use in our algorithm is summarized in the following lemma.
\begin{lemma}\label{lem: one step for bad faces}
	There is an efficient algorithm, that, given the current graph $J$ and its drawing $\rho'$, computes a subset $\hat E$ of at most $O\left((|\chi(B)|+|\Gamma'|)\cdot \poly(\Delta\log n)\right)$ edges, such that, if $n_1$ is the number of bad faces in the drawing $\rho'$ of $J$, and $n_2$ is the number of bad faces in the drawing of $J\setminus \hat E$ induced by $\rho'$, then $n_2\leq n_1/2$.
\end{lemma}
It is easy to complete the proof of Lemma \ref{lem: process a block} using Lemma \ref{lem: one step for bad faces}. As long as the  drawing $\rho'$ of the current graph $J$ contains bad faces (note that the number of bad faces is always either $0$ or at least $2$), we apply the algorithm from Lemma \ref{lem: one step for bad faces} to graph $J$ to compute a set $\hat E$ of edges, then move the edges of $\hat E$ from $J$ to $E^*(B)$, and continue to the next iteration. Once the drawing $\rho'$ of the current graph $J$ contains no bad faces, the algorithm terminates. It is easy to see that the number of iterations in the algorithm is $O(\log n)$. Therefore, at the end, $|E^*(B)|\leq O\left ((|\chi(B)|+|\Gamma'|)\cdot \poly(\Delta\log n)\right )$.
Consider now the graph $J$ obtained at the end of the algorithm. Since the drawing $\rho'$ of $J$ contains no bad faces, for every bridge $R\in \rset$, there is a single face of $\rho'$ whose boundary contains all vertices of $L(R)$ (we emphasize that the graph $J$ is not connected, and the vertices of $L(R)$ are isolated since they are terminals; but the drawing of each such vertex and the face to whose boundary it belongs are fixed by the original drawing of $\tilde B'$ induced by $\rho$). In order to complete the proof of Lemma \ref{lem: process a block}, it suffices to prove Lemma \ref{lem: one step for bad faces}.

From now on we focus on the proof of Lemma \ref{lem: one step for bad faces}.
Throughout the proof, we fix the drawing $\rho'$ of the current graph $J$.
Consider a pair $F,F'$ of faces in $\fset$. Let $P$ be the shortest path connecting $F$ to $F'$ in the dual graph of $J$ with respect to $\rho'$. This path defines a curve $\gamma(F,F')$, that starts at the interior of $F$, terminates at the interior of $F'$, and intersects the image of $J$ only at edges. Let $E(\gamma(F,F'))$ be the set of all edges whose image intersects $\gamma(F,F')$. Equivalently, $\gamma(F,F')$ can viewed as the curve that, among all curves $\gamma$ connecting a point in the interior of $F$ to a point in the interior of $F'$ that only intersects the image of $J$ at its edges, minimizes $|E(\gamma)|$. We define the distance between $F$ and $F'$ to be $\dist(F,F')=|E(\gamma(F,F'))|$. Equivalently, $\dist(F,F')$ is the minimum cardinality of a set $\tilde E\subseteq E(J)$ of edges, such that, in the drawing of $J\setminus \tilde E$ induced by $\rho'$, the faces $F$ and $F'$ are merged into a single face.

Let $\fset'\subseteq \fset$ be the set of bad faces. For each $F\in \fset'$, denote $\hat F=\arg\min_{F'\in \fset'}\set{\dist(F, F')}$. We also denote $\Pi=\set{(F,\hat F)\mid F\in \fset'}$. 
%Note that a bad face may participate in several such pairs. 
We define $\hat E=\bigcup_{F\in \fset'}E(\gamma(F,\hat F))$. In other words, set $\hat E$ contains, for every pair $(F,\hat F)\in \Pi$, the set $E(\gamma(F,\hat F))$ of edges.
% -- the minimum-cardinality set of edges whose removal from $J$ results in a merge of these faces. 
Notice that, since a bad face may participate in several pairs in $\Pi$, it is possible that more than two faces may be merged into a single face. We remove the edges of $\hat E$ from $J$. Note that no new bad faces may be created, since the bad faces are only defined with respect to the original set $\rset_{G}(\tilde B')$ of bridges. Therefore,  the number of bad faces decreases by at least a factor of $2$. It now remains to show that $|\hat E|\leq O\left ((|\Gamma'|+|\chi(B)|)\cdot \poly(\Delta\log n)\right )$. 
This is done in the next claim, whose proof completes the proof of Lemma \ref{lem: one step for bad faces}.
\begin{claim}
\label{claim:bound on hatE}
$|\hat E|\leq O\left((|\Gamma'|+|\chi(B)|)\cdot \Delta\log n\right)$. 
\end{claim}
\begin{proof}
For each $F\in \fset'$, we denote $c(F)=\dist(F,\hat F)$. To prove Claim~\ref{claim:bound on hatE}, it is sufficient to show that 
$\sum_{F\in \fset'}c(F)\leq O\left((|\Gamma'|+|\chi(B)|)\cdot \Delta\log n\right)$.
%Consider now some bad face $F\in \fset'$, and let $R\in \rset_{\tilde B'}(G)$ be the bad bridge that is responsible for $F$ being bad.
%We denote by $F'\in \fset'$ any face with a vertex of $L(R)$ lying on the boundary of $F'$, such that $F'\neq F$. We call $F'$ the \emph{twin face} of $F$.
\iffalse

Our proof uses the notion of $G$-normal curves:

\begin{definition} 
Suppose we are given a planar graph $\hat J$ together with its plane drawing, and any simple curve $\gamma$ in this drawing (that is, $\gamma$ does not intersect itself). We say that $\gamma$ is an \emph{$\hat J$-normal curve} iff it intersects the drawing of $\hat J$ in its vertices only. The \emph{length} of $\gamma$ is the number of vertices of $\hat J$ that lie on $\gamma$.
\end{definition}

We also use the following easy observation.

\begin{observation}\label{obs: long normal curve between bad vertices}
	Let $F\in \fset'$ be a bad face, and let $F'$ be its twin face. Consider the drawing $\rho'$ of $J$, and let $\gamma$ be a $J$-normal curve connecting a vertex that lies on the boundary of $F$ to a vertex that lies on the boundary of $F'$. Then the length of $\gamma$ is at least $c(F)/\Delta$.
\end{observation}
\begin{proof}
	Assume for contradiction that the claim is false. Let $U\subseteq V(J)$ be the set of all vertices of $J$ whose images lie on the curve $\gamma$.
	We can slightly modify the curve $\gamma$, obtaining a new curve $\gamma'$, that starts at a point in the interior of $F$, terminates at a point in the interior of $F'$, does not intersect images of vertices of $J$, and only intersects images of those edges of $J$ that are incident to the vertices of $U$. Therefore, curve $\gamma'$ intersects images of fewer than $c(F)$ edges of $J$, and so $\dist(F,F')<c(F)$, contradicting the definition of $c(F)$.
\end{proof}
\fi
We partition the set $\fset'$ of bad faces into $O(\log n)$ classes $\fset'_1,\ldots,\fset'_z$, for $z\leq O(\log n)$ as follows. For each $1\leq i\leq z$, face $F\in \fset'$ lies in class $\fset'_i$ iff $2^i\leq c(F)<2^{i+1}$. Clearly, there must be an index $i^*$, such that $\sum_{F\in \fset'_i}c(F)\geq \sum_{F'\in \fset'}c(F')/O(\log n)$. We denote $\fset'_{i^*}=\fset^*$ and $c^*=2^{i^*}$. Therefore, for every face $F\in \fset^*$, $c^*\leq c(F)<2c^*$. 
%Notice that we can assume that $c^*$ is greater than a large enough constant. 
Since each bad face contains at least one terminal of $\Gamma'$ on its inner boundary, $|F^*|\geq |\Gamma'|$. Therefore, if $c^*$ is upper bounded by a constant, then $\sum_{F'\in \fset'}c(F')\leq O(c^*\cdot |\fset^*|\cdot \log n)\leq O(|\Gamma'|\log n)$. We will assume from now on that $c^*$ is greater than some large constant. We use the following claim.
\begin{claim}\label{claim: Fstar is large enough}
 $|\fset^*|\leq O(|\chi(B)|\cdot \Delta/c^*)$. 
\end{claim}
Note that Claim~\ref{claim: Fstar is large enough} completes the proof of Claim~\ref{claim:bound on hatE}, since
\[\sum_{F'\in \fset'}c(F')\leq O(\log n)\cdot \sum_{F\in \fset^*}c(F)\leq O(|\fset^*|\cdot c^*\cdot \log n)\leq O(|\chi(B)|\Delta\log n).
\]
From now on we focus on the proof of Claim \ref{claim: Fstar is large enough}. 
The main idea of the proof is to associate, with each face $F\in \fset^*$, a collection $\chi^F\subseteq \chi(B)$ of $\Omega(c^*/\Delta)$ crossings of $\chi(B)$, such that each crossing in $\chi(B)$ appears in at most $O(1)$ sets of $\set{\chi_F}_{F\in \fset^*}$. Clearly, this implies that $|\fset^*|\leq O(|\chi(B)|\Delta/c^*)$. In order to define the sets $\chi^F$ of crossings, we carefully construct a witness graph $W(F)\subseteq \tilde B$ for each face $F\in \fset^*$, such that, for every pair $F,F'\in \fset^*$ of distinct faces, graphs $W(F)$ and $W(F')$ are disjoint. We define the set $\chi^F$ of crossings for the face $F$ by carefully considering the crossings in which the edges of $W(F)$ participate in the optimal drawing $\phi^*$ of $G$. %The witness graph $W(F)$ are defined in three steps. First, we compute a ``shell'' around the face $F$, which is a collection of disjoint subgraphs of $J$. The shell is used in order to compute a collection $\yset(F)$ of $\Omega(c^*/\Delta)$ disjoint cycles, which are then in turn used to define the graph $W(F)$.
The remainder of the proof consists of three steps. In the first step, we define a ``shell'' around each face $F$. In the second step, we use the shells in order to define the witness graphs $\set{W(F)}_{F\in \fset^*}$. In the third and the last step, we use the witness graphs in order to define the collections $\chi^F\subseteq \chi(B)$ of crossings associated with each face $F\in \fset^*$.
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%\vspace{-3mm}
\paragraph{Step 1: Computing the Shells.}
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
We denote $z=\floor{c^*/(16\Delta)}$. In this step we compute, for every face $F\in \fset^*$, a shell $\hset(F)$, which is a collection $\hset(F)=\set{L_1(F),\ldots,L_z(F)}$ of $z$ disjoint sub-graphs of $J$, that we refer to as \emph{layers}. 

We now fix a face $F\in \fset^*$ and  define its shell $\hset(F)$ inductively, as follows. We consider the drawing $\rho'$ of the graph $J$, and we view the face $F$ as the outer face of the drawing. We let $L_1(F)$ be the boundary of the face $F$ (note that this boundary may not be connected). 
%If we let $p^*$ be any point in the interior of $F$, then a vertex $v$ belongs to $L_1(F)$ iff there is a curve $\gamma$ connecting $p^*$ to the image of $v$, such that $\gamma$ only intersects $J$ at its endpoint $v$. Similarly, an edge $e$ belongs to $L_1(F)$ iff there is a curve $\gamma$ connecting $p^*$ to a point on the image of $e$,  such that $\gamma$ only intersects $J$ at its endpoint.
Assume now that we have defined layers $L_1(F),\ldots,L_{i-1}(F)$. In order to define $L_i(F)$, we again consider the drawing $\rho'$ of $J$, with $F$ being its outer face, and we delete from this drawing the images of all vertices  of $L_1(F),\ldots,L_{i-1}(F)$, and of all edges that are incident to these vertices. We then let $L_i(F)$ be the boundary of the outer face in the resulting plane graph.
This completes the definition of the shell $\hset(F)=\set{L_1(F),\ldots,L_z(F)}$.
 We denote $\Lambda(F)=\bigcup_{i=1}^zL_i(F)$. 
 
In order to analyze the properties of the shells, we need the following notion of $J$-normal curves.
\begin{definition}
Given a plane graph $\hat J$ and a curve $\gamma$, we say that $\gamma$ is a $\hat J$-normal curve iff it intersects the image of $\hat J$ only at the image of its vertices.
\end{definition}
We state some simple properties of the shells in the next observation and its two corollaries. 
\begin{observation}\label{obs: J-normal curve for shell}
Let	$\hset(F)=\set{L_1(F),\ldots,L_z(F)}$ be a shell for some face $F\in \fset^*$. Then for each $1\leq i\leq z$, for every vertex $v\in L_i(F)$, there is a $J$-normal curve $\gamma$ connecting $v$ to a point in the interior of $F$, such that $\gamma$ intersects exactly $i$ vertices of $J$ -- one vertex from each graph $L_1(F),\ldots,L_i(F)$.
\end{observation}
\begin{proof}
It suffices to show that, for each $1< j\leq z$ and for every vertex $v'\in L_j(F)$, there is a vertex $v''\in L_{j-1}(F)$ and a curve $\gamma_j$ connecting $v'$ to $v''$, intersecting $J$ only at its endpoints. The existence of the curve $\gamma_j$ follows immediately from the definition of $L_j(F)$. 
Indeed, consider the drawing obtained from $\rho'$ after we delete the images all vertices of $L_1(F),\ldots,L_{j-2}(F)$ together with all incident edges from it. Then there must be a face $F'$ in the resulting drawing, that contains $v'$ on its boundary, as well as another vertex $v''\in L_{j-1}(F)$. This is because $v'$ does not lie on the boundary of the outer face in the current drawing, but it lies on the boundary of the outer face in the drawing obtained from the current one by deleting all vertices of $L_{j-1}(F)$ and all incident edges from it. Therefore, there must be a curve $\gamma_j$ connecting $v'$ to $v''$, that is contained in $F'$ and intersects $J$ only at its endpoints.
\end{proof}
\begin{corollary}\label{cor: no faces captured by shell}
Let $F\in \fset^*$ and let $F'\neq F$ be any other bad face in $\fset'$. Then graph $\Lambda(F)$ contains no vertex that lies on the boundary of $F'$.
\end{corollary}
\begin{proof}
Assume for contradiction that the claim is false, and let $v\in \Lambda(F)$ be a vertex that lies on the boundary of $F'$. Then from Observation \ref{obs: J-normal curve for shell}, there is a $J$-normal curve $\gamma$ in the drawing $\rho'$ of $J$, connecting $v$ to a point in the interior of $F$, such that $\gamma$ intersects at most $z\leq c^*/(16\Delta)$ vertices of $J$. Let $U\subseteq V(J)$ be the set of these vertices. By slightly adjusting $\gamma$ we can ensure that it originates at the interior of $F'$, terminates at the interior of $F$, does not intersect any vertices of $J$, and only intersects those edges of $J$ that are incident to the vertices of $U$. But then $\dist(F,F')\leq |U|\cdot \Delta<c^*\leq c(F)$, a contradiction to the definition of $c(F)$.
\end{proof}

Notice that, since $|\fset'|\geq 2$, Corollary \ref{cor: no faces captured by shell} implies, that for every face $F\in \fset^*$, $L_z(F)$ is non-empty.
\begin{corollary}\label{cor:every pair of shells disjoint}
	Let $F,F'\in \fset^*$ be two distinct faces. Then $\Lambda(F)\cap \Lambda(F')=\emptyset$.
\end{corollary}
\begin{proof}
	Assume for contradiction that the claim is false, and let $v$ be a vertex that lies in both $\Lambda(F)$ and $\Lambda(F')$.  Then from Observation \ref{obs: J-normal curve for shell}, there is a $J$-normal curve $\gamma_1$ in the drawing $\rho'$ of $J$, connecting $v$ to a point in the interior of $F$, such that $\gamma_1$ contains images of at most $z\leq c^*/(16\Delta)$ vertices of $J$. 
	Similarly, there is a $J$-normal curve $\gamma_2$, connecting $v$ to a point in the interior of $F'$, such that $\gamma_2$ contains images of at most $c^*/(16\Delta)$ vertices of $J$. Let $U$ be the set of all vertices of $J$ whose images lie on either $\gamma_1$ or $\gamma_2$.
	By concatenating the two curves and slightly adjusting the resulting curve, we can obtain a curve that originates at the interior of $F$, terminates at the interior of $F'$, does not intersect any vertices of $J$, and only intersects those edges of $J$ that are incident to the vertices of $U$. But then $\dist(F,F')\leq |U|\cdot \Delta<c^*\leq c(F)$, a contradiction to the definition of $c(F)$.
\end{proof}
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%\vspace{-3mm}
\paragraph{Step 2: Computing the Witness Graphs.}
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
In this step we compute, for every face $F\in \fset^*$, its witness graph $W(F)$. The witness graph $W(F)$ consists of two parts. The first part is a collection $\yset(F)=\set{Y_1(F),\ldots,Y_{z-3}(F)}$ of $z-3$ vertex-disjoint cycles. We will ensure that $Y_i(F)\subseteq L_i(F)$ for all $1\leq i\leq z-3$. The second part is a collection $\qset(F)=\set{Q_1(F),Q_2(F),Q_3(F)}$ of three vertex-disjoint paths in graph $\tilde B$, each of which has a non-empty intersection with each cycle in $\yset(F)$. Graph $W(F)$ is defined to be the union of the cycles in $\yset(F)$ and the paths in $\qset(F)$. The main challenge in this part is to define the path sets $\set{\qset(F)}_{F\in \fset^*}$ so that the resulting witness graphs are disjoint.
	

We now fix a face $F\in \fset^*$, and we start by defining the collection $\yset(F)=\set{Y_1(F),\ldots,Y_{z-3}(F)}$ of cycles for it. Let $R\in \rset$ be the bad bridge that is responsible for $F$ being a bad face. Then there must be a bad face $\notF\in \fset'$, such that $F\neq \notF$, and at least one vertex of $L(R)$ lies on the (inner) boundary of $\notF$.
%(here we use the fact that all vertices of $L(R)$ are terminals and hence they are isolated vertices in $J$, and each such vertex lies on a boundary of a single face of $\rho'$). 
Let $P^*(F)$ be any path that is contained in $R$ and connects a vertex of $L(R)$ on the boundary of $F$ to a vertex of $L(R)$ on the boundary of $\notF$. Note that path $P^*(F)$ is internally disjoint from $\tilde B'$.

From Corollary \ref{cor: no faces captured by shell}, no vertex of $\notF$ may lie in $\Lambda(F)$. Therefore, for all $1\leq i\leq z$, there is a simple cycle $Y_i(F)\subseteq L_i(F)$ that separates $\notF$ from $F$. In other words, if we denote by $D(Y_i(F))$ the unique disc in the drawing $\rho'$ with $F$ as the outer face of the drawing, whose boundary is $Y_i(F)$, then $\notF\subseteq D(Y_i(F))$, and $F$ is disjoint from the interior of $D(Y_i(F))$. Clearly, the boundary of $\notF$ is contained in $D(Y_z(F))$, and $D(Y_z(F))\subsetneq D(Y_{z-1}(F))\subsetneq \cdots\subsetneq D(Y_1(F))$, while the boundary of $F$ is disjoint from the interior of $D(Y_1(F))$. We let $\yset(F)=\set{Y_1(F),\ldots,Y_{z-3}(F)}$ be the collection of disjoint cycles associated with $F$ (we note that we exclude that last three cycles $Y_{z-2}(F),\ldots,Y_z(F)$ on purpose).

It remains to define a collection $\qset(F)$ of three disjoint paths in graph $\tilde B$, each of which connects a vertex of $Y_1(F)$ to a vertex of $Y_{z-3}(F)$. We emphasize that, while the cycles in $\yset(F)$ are all contained in the current graph $J\subseteq \tilde B'$ that only contains real edges of $\tilde B$ that have not been deleted yet,
the paths in $\qset(F)$ are defined in graph $\tilde B$ and are allowed to contain fake edges. Since graph $\tilde B$ is $3$-connected, it is not hard to see that such a collection $\qset(F)$ of paths must exist. However, we would like to ensure that all paths in the set $\bigcup_{F'\in \fset^*}\qset(F')$ are mutually vertex-disjoint. In order to achieve this, we show in the next claim that there exist a desired set $\qset(F)$ of paths that only uses vertices in $\Lambda(F)$. Since all graphs in $\set{\Lambda(F')}_{F'\in \fset^*}$ are mutually vertex-disjoint, the path sets $\set{\qset(F')}_{F'\in \fset^*}$ are also mutually vertex-disjoint. The proof uses the fact that we have left the ``padding'' of three layers $L_{z-2}(F),L_{z-1}(F),L_z(F)$ between the cycles in $\yset(F)$ and $J\setminus \Lambda$.
\begin{claim}\label{claim: find the paths}
For every face $F\in \fset^*$, there is a collection $\qset(F)$ of three vertex-disjoint paths in graph $\tilde B$, where each path connects a vertex of $Y_1(F)$ to a vertex of $Y_{z-3}(F)$, and only contains vertices of $\Lambda(F)$.
\end{claim}
\begin{proof}
Fix some face $F\in \fset^*$. 
Since $\tilde B$ is $3$-connected, there must be a collection $\qset$ of three vertex-disjoint paths in graph $\tilde B$, each of which connects a vertex of $Y_1(F)$ to a vertex of $Y_{z-3}(F)$.
%(otherwise, we could disconnect $\tilde B$ by removing two vertices from it, contradicting the fact that it is $3$-connected). 
Among all such sets $\qset$ of paths we select the one that minimizes the number of vertices of $V(\tilde B)\setminus V(\Lambda(F))$ that belong to the paths in $\qset$. We now claim that no vertex of $V(\tilde B)\setminus V(\Lambda(F))$ may lie on a path in $\qset$. 
	
Assume that this is false, and let $v\in V(\tilde B)\setminus V(\Lambda(F))$ be any vertex that lies on some path in $\qset$. 
Let graph $K$ be the union of graph $\Lambda(F)$ and the paths in $\qset$. 
From the definition of the paths in $\qset$, graph $K\setminus \set{v}$ does not contain three vertex-disjoint paths that connect vertices of $Y_1(F)$ to vertices of $Y_{z-3}(F)$. 
In particular, there are two vertices $x,y\in V(K)\setminus\set{v}$, such that in graph $K\setminus\set{v,x,y}$, there is no path connecting a vertex of $Y_1(F)$ to a vertex of $Y_{z-3}(F)$. 
We will prove that this is false, reaching a contradiction. 	
Notice that each of the vertices $v,x,y$ must lie on a distinct path in $\qset$. We let $Q\in \qset$ be the path that contains $v$, so $Q$ does not contain $x$ or $y$. Notice that, from the definition of shells, for each $z-3<j\leq z$, graph $L_j(F)$ must contain a simple cycle $X_j$ that separates $v$ from every cycle in $\yset(F)$ in the drawing $\rho'$ of $J$. At least one of these three cycles $X\in \set{X_{z-2},X_{z-1},X_z}$ is disjoint from $x$ and $y$. Notice that path $Q$
% in order to reach vertex $v$, 
must intersect the cycle $X$ (this is since the drawing $\rho'$ of $J$ is the drawing induced by the unique planar drawing $\rho_{\tilde B}$ of $\tilde B$, and so $X$ separates the cycles of $\yset(F)$ from $v$ in $\rho_{\tilde B}$ as well). We view the path $Q$ as originating at some vertex $a\in V(Y_1(F))$ and terminating at some vertex $b\in V(Y_{z-3}(F))$. Let $v_1$ be the first vertex of $Q$ that lies on $X$, and let $v_2$ be the last vertex of $Q$ that lies on $X$. Then we can use the segment of $Q$ from $a$ to $v_1$, the cycle $X$, and the segment of $Q$ from $v_2$ to $b$ to construct a path connecting $a$ to $b$ in graph $K$. Moreover, neither of these three graphs may contain a vertex of $\set{x,y,v}$, and so $K\setminus\set{x,y,v}$ contains a path connecting a vertex of $Y_1(F)$ to a vertex of $Y_{z-3}(F)$, a contradiction.
\end{proof}

The witness graph $W(F)$ is defined to be the union of all cycles in $\yset(F)$ and the three paths in $\qset(F)$. Note that, from Corollary \ref{cor:every pair of shells disjoint}, all witness graphs in $\set{W(F)\mid F\in \fset^*}$ are mutually vertex-disjoint. We emphasize that the cycles of $\yset(F)$ only contain real edges of $\tilde B$ (that belong to $J$), while the paths in $\qset(F)$ may contain fake edges of $\tilde B$.
%---------------------------
%---------------------------
%---------------------------
%\vspace{-3mm}
\paragraph{Step 3: Defining the Sets of Crossings.}
%---------------------------
%---------------------------
%---------------------------
The goal of this step is to define, for each face $F\in \fset^*$, a set $\chi^F\subseteq \chi(B)$ of $\Omega(c^*/\Delta)$ crossings, such that each crossing in $\chi(B)$ appears in at most two sets of $\set{\chi_F}_{F\in \fset^*}$. This will imply that $|\fset^*|\leq O(|\chi(B)|\cdot\Delta/c^*)$, thus concluding the proof of Claim \ref{claim: Fstar is large enough}.

We now fix a face $F\in \fset^*$ and define the set $\chi^F$ of crossings. We will first partition the graph $W(F)$ into $z'=\floor{(z-3)/3}$ disjoint subgraphs $W_1(F),\ldots,W_{z'}(F)$, each of which consists of three consecutive cycles in $\yset(F)$, and a set of three paths connecting them. Each such new graph will contribute exactly one crossing to $\chi(F)$. Recall that $z=\Theta(c^*/\Delta)$, so $z'=\Theta(c^*/\Delta)$.

We now fix an index $1\leq i\leq z'$, and define the corresponding graph $W_i(F)$. We start with the set $\yset_i(F)=\set{Y_{3i-2}(F),Y_{3i-1}(F),Y_{3i}(F)}$ of three cycles. Additionally, we define a collection $\qset_i(F)$ of three disjoint paths, connecting vertices of $Y_{3i-2}(F)$ to vertices of $Y_{3i}(F)$, as follows.
Consider any of the three paths $Q\in \qset(F)$. We view $Q$ as originating at a vertex $a\in Y_1(F)$ and terminating at a vertex $b\in Y_{z-3}(F)$. From the definition of the cycles, path $Q$ must intersect every cycle in $\yset(F)$. We let $v$ be the last vertex of $Q$ that lies on $Y_{3i-2}(F)$, and we let $v'$ be the first vertex that appears on $Q$ after $v$ and lies on $Y_{3i}(F)$. We let $Q^i$ be the segment of $Q$ between $v$ and $v'$. Notice that $Q^i$ originates at a vertex of $Y_{3i-2}(F)$, terminates at a vertex of $Y_{3i}(F)$, and the inner vertices of $Q_i$ are disjoint from all cycles in $\yset(F)$ except for $Y_{3i-1}$ (that $Q^i$ must intersect). Moreover, in the drawing $\rho'$ of $J$ where $F$ is viewed as the outer face of the drawing, the interior of the image of $Q^i$ is contained in $D(Y_{3i-2}(F))\setminus D(Y_{3i}(F))$.
We let $\qset_i(F)=\set{Q^i\mid Q\in \qset(F)}$ be the resulting set of three paths, containing one segment from each path in $\qset(F)$.
Initially, we let the graph $W_i(F)$ be the union of the cycles in $\yset_i(F)$ and the paths in $\qset_i(F)$. 
Notice that for all $1\leq i<i'\leq z'$, $W_i(F)\cap W_{i'}(F)=\emptyset$. 
For convenience, we rename the three cycles $Y_{3i-2}(F),Y_{3i-1}(F),Y_{3i}(F)$ in $\yset_i$ by $Y^1_i(F),Y^2_i(F)$ and $Y^3_i(F)$, respectively.
Next, we slightly modify the graph $W_i(F)$, as follows. We let $\qset'_i(F)$ be a set of $3$ vertex-disjoint paths in $W_i(F)$
that connect vertices of $Y^1_i(F)$ to vertices of $Y^3_i(F)$ and are internally disjoint from $V(Y^1_i(F))\cup V(Y^3_i(F))$, and among all such paths, we choose those that contain fewest vertices of $V(W_i(F))\setminus \left (\bigcup_{j=1}^3V(Y^j_i(F))\right )$ in total. Clearly, set $\qset'_i(F)$ of paths is well defined, since we can use the set $\qset_i(F)$ of paths. We discard from $W_i(F)$ all vertices and edges except for those lying on the cycles in $\yset_i(F)$ and on the paths in $\qset_i(F)$. This finishes the definition of the graph $W_i(F)$.

To recap, graph $W_i(F)$ is the union of (i) three cycles $Y_i^1(F),Y_i^2(F)$ and $Y_i^3(F)$; each of the three cycles is contained in graph $J$ and only contains real edges of graph $\tilde B$, and (ii) a set $\qset'_i(F)$ of three disjoint paths, each of which connects a distinct vertex of $Y_i^1(F)$ to a distinct vertex of $Y_i^3(F)$, and is internally disjoint from $V(Y^1_i(F))\cup V(Y^3_i(F))$. Set $\qset'_i(F)$ of paths is chosen to minimize the number of vertices of $V(W_i(F))\setminus \left (\bigcup_{j=1}^3V(Y^j_i(F))\right )$ that lie on the paths.  The paths in $\qset'_i(F)$ are contained in graph $\tilde B$ and may contain fake edges. All resulting graphs $W_i(F)$ for all $F\in \fset^*$ and $1\leq i\leq z'$ are disjoint from each other. 
Note that each such graph $W_i(F)\subseteq \tilde B$ is a planar graph. 
We need the following claim.

\begin{claim}\label{claim: drawing the witness graph}
	For each $F\in \fset^*$ and $1\leq i\leq z'$, if $\psi$ is any planar drawing of $W_i(F)$ on the sphere, and $D,D'$ are the two discs whose boundary is the image of $Y_i^2(F)$, then the images of $Y^1_i(F),Y^3_i(F)$ cannot lie in the same disc in $\set{D,D'}$ (in other words, the image of $Y_i^2(F)$ separates the images of $Y^1_i(F)$ and $Y^3_i(F)$).
\end{claim}

\begin{proof}
%Observe that, from the definition of the cycles in $\yset(F)$, in the unique planar drawing $\rho_{\tilde B}$ of $\tilde B$ on the sphere, the image of $Y_i^2(F)$ separates the images of $Y^1_i(F)$ and $Y^2_i(F)$. Therefore, there exists a planar drawing of  $W_i(F)\subseteq \tilde B$ on the sphere, such that, if $D,D'$ are the two discs whose boundary is the image of $Y_i^2(F)$, then the images of $Y^1_i(F),Y^3_i(F)$ do not lie in the same disc in $\set{D,D'}$. %In order to prove the claim, it is now enough to show that graph $W_i(F)$ has a unique planar drawing.
Let $W$ be the graph obtained from $W_i(F)$ after all degree-$2$ vertices are suppressed. We denote by $Y^1,Y^2$ and $Y^3$ the cycles corresponding to $Y^1_i(F),Y^2_i(F)$ and $Y^3_i(F)$ in $W$ respectively, and we denote by $Q_1,Q_3$ and $Q_3$ the paths corresponding to the paths in $\qset'_i(F)$ in $W$. Notice that every vertex of $W$ must lie on one of the cycles $Y^1,Y^2,Y^3$, and on one of the paths $Q_1,Q_2,Q_3$. Moreover, graph $W$ may not have parallel edges (due to the minimality of the set $\qset'_i(F)$ of paths). 
%Drawing $\rho_{\tilde B}$ of $\tilde B$ induces a planar drawing of $W$ on the sphere, such that, if $D,D'$ are the two discs whose boundary is the image of $Y^2$, then the images of $Y^1,Y^3$ do not lie in the same disc in $\set{D,D'}$. Conversely, every planar drawing of $W$ on the sphere induces a corresponding planar drawing of $W_i(F)$ on the sphere.

Observe that, from the definition of the cycles in $\yset(F)$, in the unique planar drawing $\rho_{\tilde B}$ of $\tilde B$ on the sphere, the image of $Y^2$ separates the images of $Y^1$ and $Y^3$. Therefore, there exists a planar drawing of $W$ on the sphere, such that, if $D,D'$ are the two discs whose boundary is the image of $Y^2$, then the images of $Y^1$ and $Y^3$ do not lie in the same disc in $\set{D,D'}$.
Therefore, it suffices to show that $W$ is a $3$-connected graph.

Assume for contradiction that this is not the case, and let $\set{x,y}$ be a pair of vertices of $W$, such that there is a partition $(X,X')$ of $V(W)\setminus\set{x,y}$, with $X,X'\neq \emptyset$, and no edge of $W$ connects a vertex of $X$ to a vertex of $X'$. For brevity, we denote $\yset=\set{Y^1,Y^2,Y^3}$, $\qset=\set{Q_1,Q_2,Q_3}$, and we will sometimes say that a cycle $Y\in \yset$ is contained in $X$ (or in $X'$) if $V(Y)\subseteq X$ (or $V(Y)\subseteq X'$, respectively). We will use a similar convention for paths in $\qset$.
	
We first claim that both $x,y$ must belong to the same cycle of $\yset$. Indeed, assume for contradiction that they belong to different cycles. Then there must be a path $Q\in \qset$ that is disjoint from $x,y$, so all vertices of $Q$ lie in one of the two sets $X,X'$ (say $X$). But, since $Q$ intersects every cycle in $\yset$, for each cycle $Y\in \yset$, all vertices of $V(Y)\setminus\set{x,y}$ lie in $X$ (as $Y\setminus\set{x,y}$ is either a cycle or a connected path). Therefore, $X'=\emptyset$, an contradiction.
	
We denote by $Y$ the cycle in $\yset$ that contain vertices $x,y$.  Note that each of the remaining cycles must be contained in $X$ or contained in $X'$. We now consider two cases.
	
The first case is when there is some path $Q\in \qset$ that contains both vertices $x$ and $y$; assume w.l.o.g. that it is $Q_1$. Since $Q_1$ is a connected path, and exactly two vertices of $Q_1$ lie in the cut $\set{x,y}$, both endpoints of $Q_1$ must lie in the same set: $X$ or $X'$; we assume that it is $X$. Since the two endpoints of $Q_1$ lie on cycles $Y^1$ and $Y^3$ respectively, one of these cycles (say $Y^1$), that is distinct from $Y$, must be also contained in $X$. The paths $Q_2,Q_3$ are disjoint from the vertices $x,y$, and they both contain at least one vertex of $Y_1$, so both these paths are also contained in $X$. As these paths contain vertices from all three cycles, both cycles of $\yset\setminus\set{Y}$ must be contained in $X$.
	Therefore, $X'$ may only contain vertices of the cycle $Y$, and of the path $Q_1$. Since every vertex of $W$ lies on a cycle in $\yset$ and on a path in $\qset$, graph $W[X'\cup \set{x,y}]$ must be a path, that is a sub-path of the cycle $Y$ and of the path $Q_1$. But since we have suppressed all degree-$2$ vertices, $X'=\emptyset$ must hold, a contradiction.
	
	It remains to consider the case where $x$ and $y$ lie on two different paths of $\set{Q_1,Q_2,Q_3}$, say $Q_1$ and $Q_2$. Then path $Q_3$ is disjoint from $x,y$, and is contained in one of the sets $X,X'$; assume without loss of generality that it is $X$. Notice that path $Q_3$ contains vertices from all three cycles in $\yset$, therefore, each of the two cycles in $\yset\setminus \set{Y}$ is also contained in $X$. Set $X'$ then contains vertices of a single cycle in $\yset$ -- the cycle $Y$ (that contains the vertices $x$ and $y$). Since the paths $Q_1$ and $Q_2$ connect vertices of $Y^1$ to vertices of $Y^3$, 
	and each of them has one endpoint in $X$ and another in $X'$, $Y\neq Y^2$ must hold. We assume without loss of generality that $Y=Y^1$ (the case where $Y=Y^3$ is symmetric). Therefore, every vertex of $X'\cup \set{x,y}$ lies on cycle $Y^1$, and on either path $Q_1$ or path $Q_2$. However, from our construction of set $\qset'_i(F)$, each path of $\qset$ contains exactly one vertex of $Y_1$ (which serves as its endpoint). Since each of the paths $Q_1,Q_2$ contains one vertex of $\set{x,y}$ that lies on $Y_1$, it follows that $X'=\emptyset$, a contradiction.
	
	We conclude that graph $W$ is $3$-connected and therefore has a unique planar drawing -- the drawing induced by the drawing $\rho_{\tilde B}$ of $\tilde B$. In that drawing (on the sphere), the image of cycle $Y^2$ separates the images of cycles $Y^1$ and $Y^3$. Therefore, in every planar drawing of $W$ on the sphere, the image of $Y^2$ separates the images of $Y^1$ and $Y^3$. Since graph $W_i(F)$ is obtained from $W$ by subdividing some of its edges, in every planar drawing of $W_i(F)$ on the sphere, the image of $Y_i^2(F)$ separates the images of $Y^1_i(F)$ and $Y^3_i(F)$.
\end{proof}

Lastly, we use the following claim to associate a crossing of $\chi(B)$ with the graph $W_i(F)$.
\begin{claim}\label{claim: find one crossing}
Consider some face $F\in \fset^*$ and index $1\leq i\leq z'$. Let $\phi^*$ be the fixed optimal drawing of the graph $G$. Then there is a crossing $(e,e')$ in this drawing, such that:
\begin{itemize}
\item either at least one of the edges $e,e'$ is a real edge of $\tilde B$ that lies in $W_i(F)$; or
\item there are two distinct fake edges $e_1,e_2\in E(\tilde B)$, that belong to $W_i(F)$, such that $e\in P(e_1)$ and $e'\in P(e_2)$, where $P(e_1),P(e_2)\in \pset_{\tilde B}$ are the embeddings of the fake edges $e_1,e_2$, respectively.
\end{itemize}
\end{claim}

Assuming that the claim is correct, the crossing $(e,e')$ must lie in $\chi(B)$. We denote by $\chi_i^F$ the crossing $(e,e')$ obtained by applying Claim \ref{claim: find one crossing} to graph $W_i(F)$. We then set $\chi^F=\set{\chi_i^F\mid 1\leq i\leq z'}$. It is easy to verify that $\chi^F\subseteq \chi(B)$, and that it contains $z'=\Omega(c^*/\Delta)$ distinct crossings. Moreover, since all witness graphs in $\set{W(F)\mid F\in \fset^*}$ are disjoint from each other, 
%for all distinct faces $F,F'\in \fset^*$, $\chi^F\cap \chi^{F'}=\emptyset$. 
each crossing in $\chi(B)$ appears in at most two sets of $\set{\chi_F}_{F\in \fset^*}$.
It remains to prove Claim \ref{claim: find one crossing}.

\begin{proofof}{Claim \ref{claim: find one crossing}}
	We fix a face $F\in \fset^*$ and an index $1\leq i\leq z'$. 
	Consider the fixed optimal drawing $\phi^*$ of graph $G$ on the sphere. If this drawing contains a crossing $(e,e')$, where at least one of the edges $e,e'$ is a real edge of $\tilde B$ that lies in $W_i(F)$, then we are done. Therefore, we assume from now on that this is not the case. In particular, we can assume that the edges of the cycles $\yset_i(F)$ do not participate in any crossings in $\phi^*$ (recall that all edges of these cycles are real edges of $\tilde B$.)
	
	Therefore, the image of cycle $Y^2_i(F)$ in $\phi^*$ is a simple closed curve. Let $D,D'$ be the two discs whose boundaries are $Y^2_i(F)$. We claim that the images of both remaining cycles, $Y^1_i(F),Y^3_i(F)$ must lie inside a single disc in $\set{D,D'}$.
	
	
	Recall that we have defined a path $P^*(F)$, that is contained in some bridge $R\in \rset$, and connects some vertex $v$ on the boundary of $F$ to some vertex $v'$ on the boundary of $\notF$. Since both $v,v'$ lie in $\tilde B$, and since graph $\tilde B$ is connected, there is a path $P$ in $\tilde B$ that connects $v$ to $v'$; we view path $P$ as originating from $v$ and terminating at $v'$. Since each cycle $Y\in \yset_i(F)$ separates the boundary of $F$ from the boundary of $F'$ in the drawing $\rho'$ of $J$, and since $J\subseteq \tilde B$ and $\rho'$ is the drawing of $J$ induced by the planar drawing $\rho_{\tilde B}$ of $\tilde B$, path $P$ must intersect every cycle in $\yset_i(F)$. We let $x$ be the first vertex of $P$ that lies on cycle $Y^1_i(F)$, and $y$ the last vertex on $P$ that lies on cycle $Y^3_i(F)$. Let $P'$ be the sub-path of $P$ connecting $v$ to $x$, and let $P''$ be the sub-path of $P$ connecting $y$ to $v'$. Notice that both paths are internally disjoint from the cycles in $\yset_i(F)$. Next, we denote by $\hat P$ the path that is obtained by concatenating the paths $P',P^*$ and $P''$. Therefore, path $\hat P$ connects a vertex $x\in Y^1_i(F)$ to a vertex $y\in Y^3_i(F)$, and it is internally disjoint from the cycles in $\yset_i(F)$. Note however that path $\hat P$ may contain fake edges of $\tilde B$. For every fake edge $e\in A_{\tilde B}$ that lies on $\hat P$, we replace $e$ with its embedding $P(e)\in \pset_{\tilde B}$ given by using Lemma \ref{lem:block_endpoints_routing}. Recall that the lemma guarantees that the path $P(e)$ is internally disjoint from the vertices of $\tilde B$, and that all paths in $\pset_{\tilde B}=\set{P_{\tilde B}(e')\mid e'\in A_{\tilde B}}$ are mutually internally disjoint. Let $\hat P'$ be the path obtained from $\hat P$ after we replace every fake edge on $\hat P$ with its corresponding embedding path. Notice that $\hat P'$ still connects $x$ to $y$ and it is still internally disjoint from all cycles in $\yset_i(F)$ (that are also present in $G$, as they only contain real edges). If the images of the cycles $Y^1_i(F),Y^3_i(F)$ are contained in distinct discs in $\set{D,D'}$, then the endpoints of the path $\hat P'$ lie on opposite sides of the image of $Y^2_i(F)$. Since path $\hat P'$ is disjoint from cycle $Y^2_i(F)$, at least one edge of $Y^2_i(F)$ must participate in a crossing in $\phi^*$, a contradiction. Therefore, we can assume from now on that the images of both cycles $Y^1_i(F),Y^3_i(F)$ lie inside a single disc in $\set{D,D'}$ (say $D$).

Next, we use the drawing $\phi^*$ of $G$ on the sphere in order to define a corresponding drawing $\phi$ of graph $W_i(F)$, as follows. Recall that every vertex and every real edge of $W_i(F)$ belong to $G$, so their images remain unchanged. Consider now some fake edge $e\in E(W_i(F))$. Let $P(e)$ be the path in $G$ into which this edge was embedded, and let $\gamma(e)$	be the image of this path in $\phi^*$ (obtained by concatenating the images of its edges). If curve $\gamma(e)$ crosses itself then we delete loops from it, until it becomes a simple open curve, and we draw the edge $e$ along the resulting curve. 
Recall that all paths that are used to embed the fake edges of $\tilde B$ are internally disjoint from $V(\tilde B)$ and internally disjoint from each other.

Consider now the resulting drawing $\phi$ of $W_i(F)$. As before, the edges of the cycles in $\yset_i(F)$ do not participate in crossings in $\phi$, and, if we define the discs $D,D'$ as before (the discs whose boundary is $Y^2_i(F)$), then the images of $Y^1_i(F),Y^2_i(F)$ lie in the same disc $D$. From Claim \ref{claim: drawing the witness graph}, the drawing $\phi$ of $W_i(F)$ is not planar. Let $(e_1,e_2)$ be any crossing in this drawing. It is impossible that $e_1$ or $e_2$ are real edges of $W_i(F)$, since we have assumed that no real edges of $W_i(F)$ participate in crossings in $\phi^*$. Therefore, $e_1,e_2$ must be two distinct fake edges of $W_i(F)$, such that there are edges $e\in P(e_1),e'\in P(e_2)$ whose images in $\phi^*$ cross.
\end{proofof}	
	%
	\iffalse`
	Consider now the optimal drawing $\phi^*$ of the graph $G$, that we view as being drawn on the sphere. For convenience, we denote the cycles $Y_{3i-2}$, $Y_{3i-1}$, and $Y_{3i}$ by $Y$, $Y'$ and $Y''$, respectively. We now consider two cases. First, if any edge of $Y\cup Y'\cup Y''$ participates in a crossing in $\phi^*$, then we obtain the desired crossing $(e,e')$, where $e$ is a real edge of $\tilde B$, that lies in $W_i(F)$.
	
	In the second case, no edge of $Y\cup Y'\cup Y''$ participates in crossings in $\phi^*$. Therefore, the images of each of the cycles $Y,Y',Y''$ is not self-crossing, and the image of path $\hat P'$ does not intersect the image of path $Y'$ (we use the fact that path $\hat P'$ is disjoint from cycle $Y'$). In particular, the image of the cycle $Y'$ partitions the sphere into two discs, $D,D'$, whose boundaries are precisely the image of $Y'$, and the image of path $\hat P'$ is completely contained in one of these discs, say $D$. In particular, both $x$ and $y$ lie in the interior of $D$, and so do the images of both cycles $Y',Y''$.
	

	Next, we consider the paths $Q\in \qset(F)$. Recall that each such path may contain fake edges of $\tilde B$. As before, we replace every fake edge $e\in A_{\tilde B}\cap E(Q)$ with its embedding $P(e)\in \pset(\tilde B)$ that we computed before, obtaining a new path $\hat Q\subseteq G$. Recall  the embeddings of all fake edges in $A_{\tilde B}$ are mutually internally disjoint. Therefore, if we denote by $\hat \qset=\set{\hat Q_1,\hat Q_2,\hat Q_3}$ the three paths that are obtained from the paths in $\qset$ by replacing their fake edges with their embeddings, then the paths in $\hat \qset$ remain disjoint from each other, and each of them connects a vertex of $Y$ to a vertex of $Y''$, and contains at least one vertex of $Y'$. 
	Assume now that there are two distinct paths $\hat Q_j,\hat Q_{j'}\in \hat \qset$, and a crossing $(e,e')$ in the drawing $\phi^*$, such that $e\in E(\hat Q_j')$ and $e'\in E(\hat Q_{j'}')$. If either of the edges $e,e'$ is a real edge of $W_{i}(F)$, then we obtain the desired crossing in which a real edge of $W_i(F)$ participates. Otherwise, there must be two distinct fake edges, $e_1\in E(\hat Q_j)$, $e_2\in E(\hat Q_{j'})$, with $e\in P(e_1)$, $e'\in P(e_2)$, as desired.
	Lastly, it remains to consider the case where no edge of $Y\cup Y'\cup Y''$ participates in crossings in $\phi^*$, and there is no crossing $(e,e')$ in $\phi^*$, where $e\in E(\hat Q_j)$ and $e'\in E(\hat Q_{j'})$ for $j\neq j'$; in other words, the images of the paths in $\hat \qset'$ do not cross each other (but the image of a single path in $\hat \qset'$ may cross itself).
	
	
		\mynote{Ignore the remainder. Enough to show that in every planar drawing of graph $W_i(F)$, image of $Y'$ must separate $Y$ and $Y''$.}
	
	For each path $\hat Q_j\in \hat\qset$, we let $\hat Q_j'$ be a segment of $\hat Q_j$ that originates at a vertex of $Y$, terminates at a vertex of $Y'$, and does not contain any vertices of $Y\cup Y'\cup Y''$ as inner vertices.
	
	Consider now the drawing $\phi^*$ of $G$ in the sphere, and delete from it all vertices and edges, except for those lying in $Y\cup Y'\cup Y''\cup \hat Q_1'\cup \hat Q_2'\cup \hat Q_3'$. If the image of any path $\hat Q_j$ crosses itself, we remove the resulting loop, so that each path $\hat Q_j'$ is now represented by a simple open curve, connecting a point on the image of $Y$ to a point on the image of $Y'$. Let $\hat \fset$ be the set of faces in the resulting drawing. Then there must be two faces $F,F'\in \hat \fset$, whose boundaries are $Y$ and $Y'$, respectively, and three additional faces, denoted by $F_1,F_2,F_3$. Each of these faces has two paths of $\set{\hat Q_j'}_{j=1}^3$ as part of its boundary, but its boundary is disjoint from the third path.
	
\fi	
\iffalse
	From the construction of the paths $P',P''$, it is also easy to see that they are internally disjoint from the paths in $\qset_i(F)$. Let $e^*$ be a new artificial edge for graph $W_i(F)$, connecting the pair $x,y$ of vertices (we will think of $P^{**}$ as the embedding of this edge. We use the following observation.
	
	\begin{observation}\label{obs: getting the right crossings}
		In any drawing of $W_i(F)\cup e^*$, there must be a crossing $(e,e')$, such that:
		\begin{itemize}
			\item either at least one of the edges $e,e'$ lies on a cycle in $\yset_i(F)$; or
			\item the two edges lie on two distinct paths in $\qset_i(F)$.
		\end{itemize}
	\end{observation}
	
	We prove the observation below, after we show that Claim \ref{claim: find one crossing} follows from it. Consider the optimal drawing $\phi^*$ of the graph $G$. We delete from this drawing all vertices and edges, except for: (i) all vertices and all \emph{real} edges of $W_i(F)$; (ii) all vertices and edges of path $P^{**}$; and (iii) for every fake edges $e\in E(W_i(F))$, all vertices and edges on the path $P(e)$ 
\fi	
%
%
%
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
\iffalse
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
In the remainder of the proof, we will compute a large subset $\hat \fset\subseteq \fset'$ of bad faces, and associate, with each face $F\in \hat \fset$, a subset $\chi^F$ of $\Omega(c(F)/\Delta)$ crossings $\chi(B)$, such that for $F\neq F'$, $\chi^F\cap \chi^{F'}=\emptyset$. This will be used in order to show that $\sum_{F\in \fset'}c(F) \leq O((|\Gamma'|+|\chi(B)|)\cdot \Delta\log n)$.

More precisely, we start by constructing, for each  (but one) bad face $F\in \fset'$, a collection $\yset(F)$ of $\Omega(c(F)/\Delta)$ disjoint cycles in graph $J$. We will ensure that all cycles in $\bigcup_{F\in \fset'}\yset(F)$ are completely disjoint from each other. Moreover, the collections of cycles will have a nice structure that will allow us to organize all faces in $\fset'$ into a forest-like structure, which will in turn allow us to select a subset $\hat \fset\subseteq \fset'$ of faces with $\sum_{F\in \hat \fset}c(F)\geq \Omega(\sum_{F\in \fset'}c(F)/\log n)$, such that the faces in $\hat \fset$ correspond to vertices of degree $1$ and $2$ in the forest, and all values $c(F)$ of such faces are close to each other. For each face $F\in \hat \fset$, we will use the cycles in $\yset(F)$ in order to define a subgraph of graph $B^*$, that will in turn allow us to define the subset $\chi^F\subseteq \chi(B)$ of $\Omega(c(F)/\Delta)$ crossings in $\chi(B)$.

The remainder of the proof consists of three parts. In the first part, we define the collections $\yset(F)$ of cycles for the bad faces $F\in \fset'$. In the second part, we prove that the resulting collections of cycles are disjoint, and use their structure in order to organize the faces of $\fset'$ into a forest, selecting a large subset $\hat \fset\subseteq \fset'$ of faces. Lastly, in the third part, we associate a subgraph of $B^*$ with each face $F\in \hat \fset$, and use this subgraph in order to define the set $\chi^F\subseteq \chi(B)$ of crossings.


\paragraph{Part 1: Defining the families of cycles.}
Let $F^*\in \fset'$ be a face with minimum value $c(F^*)$, breaking ties arbitrarily. Note that $c(F^*)\leq \half \sum_{F\in \fset'}c(F)$. In the remainder of the proof, view $F^*$ as the outer face of the current drawing $\rho'$ of the graph $J$. We now define, for each face $F\in \fset'\setminus\set{F^*}$, a set $\yset(F)$ of cycles, in graph $J$, using the notion of \emph{tight concentric cycles}, that was used in \cite{chuzhoy2016improved}, and is defined next.
%For the remainder of the proof it may be convenient to think of $\rho'$ as a drawing of $J$ on the sphere instead of the plane.

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------
%\paragraph{Tight Concentric Cycles.}

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------

%---------------------------------------------
%---------------------------------------------
%---------------------------------------------



Suppose we are given a planar graph $\hat H$ and its drawing $\psi$ in the plane.
 Consider any simple cycle $Y$ in $\hat H$. We denote by $\gamma(Y)$ the curve that is the drawing of $Y$ in $\psi$ (so $\gamma(Y)$ is the concatenation of the images of the edges of $Y$ in $\phi$). We denote by $D(Y)$ the unique disc in the plane whose boundary is $\gamma(Y)$.


Assume now that we are given any vertex $v$ of $\hat H$. We define a cycle $\mincycle(\hat H,v)$ as follows. We let $\mincycle(\hat H,v)$ be the simple cycle $Y\subseteq \hat H$ with $v$ lying in the interior of the disc $D(Y)$ (so $v\not\in V(Y)$), for which $D(Y)$ is smallest inclusion-wise. 

\iffalse
\begin{definition}
	Given a planar graph $H$ drawn in the plane and a vertex $v \in V(H)$ that is not incident to the infinite face, $\mincycle(H, v)$ is the cycle $C$ in $H$, such that: (i) $v\in\dnot(C)$; and (ii) among all cycles satisfying (i), $C$ is the one for which $D(C)$ is minimal inclusion-wise. 
\end{definition}
\fi

It is easy to verify that, if graph $\hat H$ contains a cycle $Y$ with $v$ lying in the interior of $D(Y)$, then $\mincycle(\hat H,v)$ is uniquely defined. Indeed, consider the graph $\hat H \setminus v$, and the face $F$ in the drawing of $\hat H \setminus v$ where $v$ used to reside. Then the outer boundary of $F$ is a simple cycle $Y$, and $Y=\mincycle(\hat H, v)$.
 



\begin{definition}
	Suppose we are given a planar graph $\hat H$, an embedding $\psi$ of $\hat H$ in the plane, a simple cycle $Y$ in $\hat H$, and an integral parameter $r\geq 1$. A \emph{family of $r$ tight concentric cycles around $Y$} is a sequence $Z_1,Z_2,\ldots,Z_r$ of disjoint simple cycles in $\hat H$, with the following properties:
	
	\begin{itemize}
		\item $Y=Z_1$;
		
		\item $D(Z_1)\subsetneq D(Z_2)\subsetneq\cdots\subsetneq D(Z_r)$;  and \label{prop: disc}
		
		%\item if $\hat H'$ is the graph obtained from $\hat H$ by contracting all vertices lying in $D(C)$ into a super-node $a$, then $Z_1=\mincycle(\hat H',a)$; and
		
		\item for every $1< h\leq r$, if $\hat H'$ is the graph obtained from $\hat H$ by contracting all vertices lying in $D(Z_{h-1})$ into a super-node $a$, then $Z_h = \mincycle(\hat H', a)$.
	\end{itemize}
\end{definition}

Next, we need the notion of $\hat H$-normal curves.

\begin{definition} 
	Suppose we are given a planar graph $\hat H$ together with its plane drawing, and any simple curve $\gamma$ in this drawing (that is, $\gamma$ does not intersect itself). We say that $\gamma$ is a \emph{$\hat H$-normal curve} iff it intersects the drawing of $\hat H$ in its vertices only. The \emph{length} of $\gamma$ is the number of vertices of $\hat J$ that lie on $\gamma$.
\end{definition}

We need the following observation about tight concentric cycles, that was shown in \cite{chuzhoy2016improved}.

\begin{observation}\label{obs: curve for concentric cycles}
	Let $Z_1,Z_2,\ldots,Z_r$ be a sequence of tight concentric cycles around $Z_1$ in a plane graph $\hat H$. Then for every vertex $v_r\in V(Z_r)$, there is a vertex $v_1\in V(Z_1)$, and an $\hat H$-normal curve $\gamma(v_r,v_1)$ in $\psi$, connecting $v_r$ to $v_1$, such that for all $1\leq i\leq r$, $\gamma(v_r,v_1)$ intersects the image of cycle $Z_i$ on exactly one vertex, and $\gamma$ does not intersect the images of any other vertices of $\hat H$.
\end{observation}

\begin{proof}
	In order to prove the observation, it is enough to show that for all $1\leq i<r$, for any vertex $v_{i+1}\in V(Z_{i+1})$, there is a vertex $v_{i}\in V(Z_{i})$, and a curve $\gamma_{i+1}$ connecting $v_{i+1}$ to $v_{i}$, that intersects the image of $\hat H$ on its endpoints only.
	%Assume for contradiction that such a curve does not exist.
	
	Let $\hat H'$ be the graph obtained from $\hat H$, by deleting all vertices that lie in the interior of $D(Z_i)$, and all vertices that lie outside of $D(Z_{i+1})$. Let $\psi'$ be the drawing of $\hat H'$ induced by $\psi$. Let $\hat H''$ be the graph obtained from $\hat H'$ by contracting all vertices of $Z_i$ into a single super-node $a$, and let $\psi''$ be the resulting drawing. Recall that, if we consider the drawing of $\hat H''\setminus\set{a}$ induced by $\psi''$, then $Z_{i+1}$ is precisely the outer boundary of the face where $a$ used to reside. Therefore, there is a curve $\gamma$ in the drawing $\psi'$ of $\hat H'$, connecting $v_{i+1}$ to $a$, that only intersects the image of $\hat H'$ on its endpoints. It is now immediate to see that there must be a curve  $\gamma_{i+1}$ in the drawing $\psi'$ of $\hat H'$ (and hence in the drawing $\psi$ of $\hat H$), connecting $v_{i+1}$ to some vertex of $Z_i$, that intersects the image of $\hat H$ on its endpoints only.	
	% Let $F$ be a face in this drawing, such that $v_{i+1}$ lies on the boundary of $F$, and $F\subseteq D(Z_{i+1})$. Note that the boundary of $F$ may not contain a vertex of $Z_i$, since otherwise there must be a curve connecting $v_{i+1}$ to a vertex of $Z_i$ that intersects the image of $\hat H$ on its endpoint only. Since $v_{i+1}$ lies on the boundary of $F$, the outer boundary of $F$ intersects $Z_{i+1}$. Moreover, it is impossible that the outer 	
\end{proof}




We now consider any bad face $F\in \fset'\setminus\set{F^*}$, and define the family $\yset(F)$ of cycles for it. Let $Y$ be the cycle that serves as the boundary of $F$. We then let $\yset(F)=\set{Z_1(F),Z_2(F),\ldots,Z_{r_F}(F)}$ be a maximal collection of tight concentric cycles around $Y$ in the drawing $\rho'$ of graph $J$  (that is, $r$ is the maximum integer for which such a collection of cycles exists).
 
%Recall that we have defined a face $F'$ in the drawing $\rho'$ of $J$, that we called the twin face of $F$. We let $Y$ be the simple cycle that forms the outer boundary of $F$ and $Y'$ the simple cycle that forms the outer boundary of $F'$. \mynote{need to be careful that neither of them is the outer face.}


%We consider the graph $\tilde B'$ and the drawing $\psi$ of this graph that is induced by the unique drawing $\rho_{\tilde B}$ of $\tilde B$. Let $v$ be any vertex of $Y'$, and let $F^*$ be any face of $\psi$ that has $v$ on its boundary, such that cycle $Y'$ separates the interior of $F^*$ from all vertices of $Y$; it is easy to verify that such a face must exist. We will view the face $F^*$ as the outer face of the drawing $\psi$ of $\tilde B$. Next, we construct a maximal collection $Z_1,Z_2,\ldots,Z_r$ of tight concentric cycles around $Y$ such that $V(Y')\cap V(Z_r)=\emptyset$ (that is, $r$ is the maximum integer for which such a collection of cycles exists).

\begin{claim}\label{claim: many cycles}
	$r\geq c(F)/\Delta$.
\end{claim}
\begin{proof}
	Assume otherwise. 
		Consider the graph $J'$ that is obtained from $J$, after we contract all vertices whose image lies in $D(Z_r(F))$ into a super-node $a$. Since we could not further augment the collection of tight concentric cycles, $\mincycle(J',a)$ does not exist.
		
		Let $Y^*$ be the boundary of the outer face $F^*$. Assume first that some vertex $v\in V(Y^*)$ lies on the cycle $Z_r(F)$. Then, from Observation \ref{obs: curve for concentric cycles}, there is a curve $\gamma$ in the drawing $\rho'$ of $J$, that connects $v$ to some vertex $v'\in V(Y)$, that intersects graph $J$ at exactly $r< c(F)/\Delta$ vertices and no edges. Let $U$ be the set of all vertices of $J$ that $\gamma$ intersects. By slightly adjusting the curve $\gamma$, we can ensure that it originates at a point in the interior of face $F$, terminates at a point in the interior of face $F^*$, does not intersect any vertices of $J$, and only intersects edges of $J$ that are incident to the vertices of $U$. But then $\dist(F,F^*)<c(F)$, a contradiction.
		
		Therefore, we can now assume that no vertex of  $v\in V(Y^*)$ lies on the cycle $Z_r(F)$. But then, since $Y^*$ is a connected graph, and it serves as the boundary of the outer face in the drawing $\rho^*$, no vertex of $V(Y^*)$ may lie in the disc $D(Z_r(F))$, and the cycle $Y^*$ must be present in the graph $J'$, contradicting the fact that $\mincycle(J',a)$ does not exist.
\end{proof}

We discard from $\yset(F)$ all but the first $\floor {c(F)/(10\Delta)}$ cycles, so now $\yset(F)=\set{Z_1(F),Z_2(F),\ldots,Z_{q_F}(F)}$, where $q_F(F)=\floor{c(F)/(10\Delta)}$. For convenience, we denote the disc $D(Z_{q_F}(F))$ by $\dout(F)$.
	
\paragraph{Part 2: Selecting the Set $\hat \fset$ of Bad Faces.}
We start with the following claim, that was also shown in \cite{chuzhoy2016improved}:

\begin{claim}
	All cycles in $\bigcup_{F\in \fset'\setminus\set{F^*}}\yset(F)$ are mutually disjoint.
\end{claim}
\begin{proof}
	Assume otherwise. Then there are faces $F_1,F_2\in \fset'$, with $F_1\neq F_2$, and cycles $Y'\in \yset(F_1)$, $Y''\in \yset(F_2)$, such that $Y'\cap Y''\neq \emptyset$. We let $v$ be any vertex in $V(Y)\cap V(Y'')$. Assume that $Y'$ is the $i$th cycle in $\yset(F_1)$, and that it is the $j$th vertex in $\yset(F_2)$. Assume without loss of generality that $c(F)\leq c(F')$, so $i+j\leq c(F)/(5\Delta)$. Then from Observation \ref{obs: curve for concentric cycles}, there is a curve $\gamma_1$ in the drawing $\psi$ of $\tilde B'$ that connects $v'$ to some vertex of $Y(F_1)$, that intersects at most $i$ vertices of $\tilde B'$ and no edges, and similarly, there is a curve $\gamma_2$ in $\psi$, connecting $v'$ to some vertex of $Y(F_2)$, that intersects at most $j$ vertices of $\tilde B'$ and no edges. By letting $\gamma$ be a concatenation of $\gamma_1$ and $\gamma_2$, we conclude that there is a $J$-normal curve $\gamma$ in $\rho'$, of length at most $c(F)/(5\Delta)$ connecting the interior of face $F_1$ to the interior of face $F_2$. Let $U$ be the set of all vertices of $J$ that $\gamma$ intersects. We can then slightly adjust $\gamma$ so it still connects the interior of face $F_1$ to the interior of face $F_2$, but now it does not intersect any vertices of $J$, and only intersects edges of $J$ that are incident to the vertices of $U$. We get that $\dist(F_1,F_2)<c(F)$, contradicting the definition of $c(F)$.
\end{proof}


Consider now a pair $F_1,F_2\in \fset'\setminus \set{F^*}$ of bad faces. We say that $F_1$ \emph{captures $F_2$} iff the face $F_2$ is contained in the disc $\dout(F_1)$.

The following observation is immediate:

\begin{observation}
	For any bad faces $F_1,F_2,F_3\in \fset'\setminus F^*$:
	\begin{itemize}
\item If $F_1$ captures $F_2$ and $F_2$ captures $F_3$ then $F_1$ captures $F_2$.
\item If $F_1$ captures $F_2$, then $F_2$ does not capture $F_1$.
\item If $F_1$ captures $F_2$, then either $\dout(F_2)\subseteq D(Z_1(F_1))$, or there is some index $1\leq i<q_{F_1}$, such that $\dout(F_2)\subseteq D(Z_{i+1}(F_1))\setminus D(Z_i(F_1))$.
\end{itemize}
\end{observation}

(the last statement follows from the fact that the cycles in $\yset(F_1)$ and $\yset(F_2)$ may not intersect).


Consider now some face $F\in \fset'\setminus \set{F^*}$. We say that $F$ is an \emph{eligible face} iff there is another face $F'\neq F$ with $F'\in \fset'$, such that $F$ does not capture $F'$, and there is some bridge $R\in \rset_{\tilde B'}(G)$ with legs $t,t'\in L(R)$, such that $t$ lies in $F$ and $t'$ lies in $F'$. Let $F^*\subseteq  \fset'\setminus \set{F^*}$ be the set of all eligible faces.





We can now construct a directed graph $\hat G$, whose vertex set is $\fset{v(F)\mid F\in \fset'\setminus \set{F^*}}$, and there is an edge $(v(F),v(F'))$ iff $F'$ interferes with $F$, and there is no face $F''\in \fset'\setminus\set{F^*}$, such that $F''$ interferes with $F$ and $F'$ interferes with $F''$. It is immediate to verify that the resulting graph $\hat G$ is a forest.

Consider now any vertex $v(F)$ of $\hat G$. We say that $v(F)$ is an 


We now proceed to gradually define the set $\hat \fset$ of faces. In order to do so, we start by defining a subset  $\fset^*\subseteq \fset'\setminus \set{F^*}$ of faces, that we will later refine. 

\paragraph{Part 3: Bounding $c(F)$}
Consider again some bad face $F\in \fset'$. We denote $\yset(F)=\set{Z_1,Z_2,\ldots,Z_q}$, where $q=\Omega(c(F)/\Delta)$. We will prove that for all $1\leq i\leq \floor{q/3}$, at least one edge of $C_{3i}\cup C_{3i+1}\cup C_{3i+2}$ must participate in a crossing in any drawing of the graph $G$. This will prove that $\chi(\tilde B')\geq \Omega(\sum_{F\in \fset'}c(F)/\Delta)$ and will thus complete the proof of Lemma \ref{lem: one step for bad faces}. We use the following claim in order to show this.


\mynote{next claim is false. This whole argument is to be fixed}
\begin{claim}\label{claim: crossins in a 3-cycle graph}
	Let $H$ be any  graph, such that there are three disjoint simple cycles $Y_1,Y_2,Y_3$ in $H$, an edge $e^*$ connecting a vertex of $Y_1$ to a vertex of $Y_3$, and three disjoint paths $P_1,P_2,P_3$, such that each path $P_i$ originates at a vertex of $Y_1$, terminates at a vertex of $Y_3$, and contains at least one vertex of $Y_2$. 
	Assume further that $H\setminus\set{e^*}$ is planar.
	Then in any drawing of $H$ in the plane, at least one edge of $Y_1\cup Y_2\cup Y_3$ must participate in a crossing.
\end{claim}
\begin{proof}
	Assume otherwise, that is, we have a planar drawing $\phi$ of $H$, in which on edge of $Y_1\cup Y_2\cup Y_3$ participates in crossings. It will be convenient for us to view $\phi$ as a drawing of $H$ on the sphere.
	Consider the curve $\gamma(Y_2)$ corresponding to the drawing of $Y_2$ in $\phi$. This curve partitions the sphere into two discs $D_1,D_2$.
	 Since the image of $e^*$ does not cross images of edges of $Y_2$, both endpoints of $e^*$ lie in the interior of the same disc - assume w.l.o.g. that it is $D_1$. Since $Y_1$ is a connected graph, and the images of its edges do not cross the edges of $Y_2$, all vertices and edges of $Y_1$ must be drawn in the interior of $D_1$, and the same is true for $Y_3$.
\end{proof}
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
\fi
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%---------------------------
%
%
\end{proof}




%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
\iffalse
--------------------------------------

Old stuff

-------------------------------------



We use the following Lemma, whose proof is deferred to Appendix~\ref{apd:crossing_charged_to_consecutive_cycles}.
\begin{lemma}
	\label{lem:crossing_charged_to_consecutive_cycles}
	Let $H$ be a $3$-connected graph and $C_1,\ldots,C_{\ell}$ ($\ell>30$) be vertex-disjoint cycles in $G$, such that, for any $1\le x<y<z\le \ell$, there is no path in $H\setminus C_y$ connecting any vertex of $C_x$ to any vertex of $C_z$. Let $P$ be a path (which does not belong to $H$) that connects a vertex of $C_1$ to a vertex of $C_{\ell}$, then in any drawing of the graph $H\cup P$ on the plane, for each $1\le i\le \ell-2$, at least one cycle of $C_{i}, C_{i+1}, C_{i+2}$ is crossed.
\end{lemma}

\begin{corollary}
	\label{cor:local_crossing}
	Let $H$ be a graph and $C_1,\ldots,C_{\ell}$ ($\ell>30$) be vertex-disjoint cycles in $G$, such that, for any $1\le x<y<z\le \ell$, there is no path of $H\setminus C_y$ connecting any vertex of $C_x$ to any vertex of $C_z$. Let $P$ be a path (which does not belong to $H$) that connects a vertex of $C_1$ to a vertex of $C_{\ell}$, then in any drawing of the graph $H\cup P$ on the plane, the number of crossings that the cycles $C_1,\ldots,C_{\ell}$ participate in is at least $\ell/3$.
\end{corollary}


Let $\cset=\set{C_1,\ldots,C_r}$ be the connected components of $G\setminus \hat E$.
%It is clear that the sets $V(C_1),\ldots,V(C_r)$ is a partition of $V(G)$.
So the each of graphs $C_1,\ldots, C_r$ is a subgraph of $H$. 
Fix a planar drawing $\psi$ of $H$. 
For any cluster $S$ of $H$, we denote by $\psi_{S}$ the induced drawing of $\psi$ on $S$.
%let $\fset_i$ be the collection of faces in the drawing $\psi_{C_i}$. 
We say that a vertex $v\in T\cap V(C_i)$ is a \emph{bad terminal} if there exist another vertex $v'$, a pair of distinct faces $F, F'$ in the drawing $\psi_{C_i}$ and a path $P$, such that (i) $v\in V(F)\setminus V(F')$ and $v'\in V(F')\setminus V(F)$; (ii) the path $P$ consists of edges in $\hat{E}$ {\color{red}(is this what we want to say or we want to say the path consists of edges in $G\setminus C_i$?)}; and (iii) the path $P$ connects $v$ to $v'$.

For each component $C\in \cset$, we run a separate process on $C$ that gradually adds some edges of $E(C)$ into $\hat{E}$. Let $E_C\subseteq E(C)$ be the subset of edges that are added into $E$ {\color{red}($\hat{E}$?)}.
The goal is to ensure that the induced planar drawing of $\psi_{C}$ on $C\setminus E_C$ contains no bad terminals, and $\sum_{C\in \cset}|E_C|=\tilde{O}(|E'|+\optcro(G))$.
%Then, for each $C\in \cset$, we add edges of $E_C$ into $\hat{E}$.

Now we fix a component $C\in \cset$. We denote $T(C)=T\cap V(C)$.
%and denote $\psi_C$ to be the induced drawing of $\psi$ on $C$.
We have $\sum_{C\in \cset}|T_C|=O(|E'|)$. 
Let $T^b\subseteq T(C)$ be the set of bad terminals of $C$.
For any sub-cluster $S$ of $C$, we denote by $T^b(S)$ the set of bad terminals in $T^b(S)$ {\color{red}($S$?)}.
Notice that, as the set $T$ changes, $T^b(S)$ also evolves.
Let $\fset_C$ be the set of faces in the drawing $\psi_C$ that contains some bad terminals. It is clear that $|\fset_C|=O(|T(C)|)$. 
%since each vertex lies on the boundary of at most $\Delta=O(1)$ faces.

We now describe the separate process on $C$ that gradually adds edges of $E(C)$ into $\hat{E}$.
The process proceeds in iterations. In the $i$th iteration, it takes as input a tuple $(S,T^b(S), \fset_S)$, where $S$ is a sub-cluster of $C$, $T^b(S)$ is the set of its bad terminals, and $\fset_S$ is a face cover of the vertices of $T^b(S)$ in the drawing $\psi_S$, computes a set $\tilde{E}_i$ of the edges of $S$, and outputs another tuple $(S',T^b(S'), \fset_{S'})$, where $S'=S\setminus \tilde{E}_i$ is a sub-cluster of $S$, $T^b(S')$ is the set of its bad terminals, and $\fset_{S'}$ is a face cover of vertices $T^b(S')$ in the drawing $\psi_{S'}$, such that $|\fset_{S'}|\le |\fset_{S}|/2$.  
The input of the first iteration is $(C,T^b, \fset_C)$.
Whenever in the output tuple $(S',T^b(S'), \fset_{S'})$ of some iteration, the set $T^b(S')=\emptyset$, we terminate the algorithm on $C$.
At the end, let $E_C$ be the union of the sets $\tilde E_i$ in all iterations of the process on $C$.

We now describe the $i$th iteration of the process on $C$.
Let $S^*$ be the dual graph of $S$ with respect to the planar drawing $\psi_S$. From the definition of a dual graph, for each face $F$ in the drawing $\psi_S$, there is a vertex $v_F\in V(S^*)$ in the dual graph $S^*$.
Define $\tilde V=\set{v_F\in V(S^*)\mid F\in\fset_S}$, so $\tilde{V}$ is a subset of $V(S^*)$.
For each $F\in \fset_S$, we perform a BFS in $S^*$ to compute a vertex 
$v^*\in \arg\min_{v\in \tilde{V}}\set{\dist_{S^*}(v,v_{F})}$, with tie breaking arbitrarily.
Let $N(F)\in \fset_S$ be the face of $\psi_S$ that $v^*$ corresponds to, and we also denote $d(F)=\dist_{S^*}(v^*,v_{F})$. We consider two cases.

\textbf{Case 1.} $d(F)\le 30$.
Let $\tilde{E}_i(F)$ be the set that we obtain by applying Lemma~\ref{lem:separating} to the cluster $S$ and its faces $F$ and $N(F)$. 
From Lemma~\ref{lem:separating}, $|\tilde{E}_i(F)|\le 30$.

\textbf{Case 2.} $d(F)> 30$.
Let $\tilde{E}_i(F)$ be the set that we obtain by applying Lemma~\ref{lem:separating} to the cluster $S$ and its faces $F$ and $N(F)$.
From Lemma~\ref{lem:separating}, $|\tilde{E}_i(F)|\le d(F)$.



We let the set $\tilde{E}_i$ be the union of $\tilde{E}_i(F)$ for all $F\in \fset_S$, namely $\tilde{E}_i=\cup_{F\in \fset_S}\tilde{E}_i(F)$. Then we add the edges of $\tilde{E}_i$ into $\hat{E}$ and update $T^b$ accordingly.
From Lemma~\ref{lem:separating}, each face $F$ of $\fset_S$ is merged with the face $N(F)$ after we take out the edges of $\tilde{E}_i$ from $S$. Therefore, we set $S'=S\setminus \tilde{E}_i$, set $T^b(S')=T^b\cap V(S')$, and let $\fset_{S'}$ be the faces in $\psi_{S'}$ that is formed by merging faces of $\fset_{S}$ in $\psi_{S}$. It is easy to see that $|\fset_{S'}|\le |\fset_{S}|/2$. The tuple $(S',T^b(S'), \fset_{S'})$ is our output.
This finishes the description of an iteration of the separate process on $C$, and also finishes the description of the separate process on $C$.

\begin{observation}
	\label{obs:number_of_iterations}
	The separate process on $C$ runs at most $O(\log |T_C|)=O(\log n)$ iterations.
\end{observation}

At the end of the process on $C$, we define $E_C$ to be the union of the sets $\tilde{E}_i$ from all iterations, namely the set of edges that are added into $\hat{E}$ in this process. From the process, it is easy to verify that the induced planar drawing of $\psi_{C}$ on $C\setminus E_C$ contains no bad terminals. It remains to show $\sum_{C\in \cset}|E_C|=\tilde{O}(|E'|+\optcro(G))$.

\begin{proposition}
	\label{pro:C_share}
	For each $C\in \cset$, $|E_C|=O(\log n\cdot (|T_C|+\cro_{\phi}(C)))$.
\end{proposition}
\begin{proof}
	Recall that $|\fset_C|=O(|T_C|)$. For each $i>1$, let $(S,T^b(S),\fset_S)$ be the tuple output by the $(i-1)$th iteration of the process on $C$. From the process, 
	$|\fset_S|\le |\fset_C|=O(|T_C|)$.
	Therefore,
	$$\sum_{F\in \fset_S, d(F)\le 30}|\tilde{E}_i(F)|\le O(|T_C|).$$
	For each face $F\in\fset_S$ such that $d(F)>30$, let $L_1,\ldots, L_{d(F)/3}$ be tight concentric cycles \explain around $F$, and let $E_F$ be the set of edges in these cycles. On one hand, it is not hard to see that, for every pair $F, F'$ of faces in $\fset_S$, the edge sets $E_F$ and $E_{F'}$ are disjoint. Therefore, $\sum_{F\in \fset_S}\cro_{\phi}(E_F)\le O(\cro_\phi(S))=O(\cro_\phi(C))$.
	On the other hand, from Corollary~\ref{cor:local_crossing}, 
	$\cro_{\phi}(E_F)= \Omega(d(F))$. Combined together, we have
	\[\sum_{F\in \fset, d(F)>30}|\tilde{E}_i(F)|\le \sum_{F\in \fset, d(F)>30}d(F)=O(\cro_{\phi}(C)).\]
	From Observation~\ref{obs:number_of_iterations}, $|E_C|=\sum_{1\le i\le \log n}|\tilde{E}_i|=O(\log n\cdot (|T_C|+\cro_{\phi}(C)))$. This finishes the proof of Proposition~\ref{pro:C_share}.
\end{proof}

Since the clusters in $\cset$ are mutually vertex-disjoint, we have $\sum_{C\in \cset}\cro_{\phi}(C)=O(\cro(\phi))$. Recall that $\sum_{C\in \cset}|T_C|=O(|E'|)$. As a result,
$\sum_{C\in \cset}|E_C|=O(\log n\cdot(|E'|+\cro(\phi)))$.

For each $C\in\cset$, we denote $C'=C\setminus \hat{E}$.
So far, we have computed a set $\hat{E}$ of edges (and a subset $T\subseteq V(H)$ accordingly), such that, for each component $C'$ of $H\setminus \hat{E}$, in the planar drawing $\psi_{C'}$, there is no path consisting of only edges of $\hat{E}$ that connects two vertices from $T\cap V(C)$ that do not lie on the same face of $\psi_{C'}$. However, we are not yet guaranteed that, for each $C'$, $T\cap V(C')$ is $(1/\poly\log n)$-well-linked in $C'$. Therefore, we still need to perform, for each $C'$, another well-linked decomposition in $C'$ with respect to $T\cap V(C')$ using Lemma~\ref{lem:well_linked-decomposition}. We add into $\hat{E}$ all inter-cluster edges, update $T$ accordingly, and denote by $\cset''=\set{C''_1,C''_2\ldots,C''_t}$ the set of clusters we get. It suffices to show that each $C''\in\cset''$ contains no bad terminals. {\color{red}TODO~}

{\color{red}Comment: we are not yet guaranteed that each connected component is $3$-connected.}



\fi

%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------
%--------------------------------------



%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
\subsection{Stage 2: Obtaining a Decomposition into Acceptable Clusters}

%-------------------------------------------
%-------------------------------------------
%-------------------------------------------
%-------------------------------------------

In this subsection we complete the proof of Theorem \ref{thm: can find edge set w acceptable clusters}. We start with a $3$-connected graph $G$ with maximum vertex degree $\Delta$, and a planarizing set $E'$ of edges of $G$. We then use Theorem \ref{thm: getting good pseudoblocks} to compute a subset $E_1$ of edges of $G$, with $E'\subseteq E_1$, such that $|E_1|\leq O\left((|E'|+\optcro(G))\cdot\poly(\Delta\log n)\right )$, and a set $\cset_1'$ of connected components of $G\setminus E_1$, each of which contains at most $\mu$ vertices that are incident to edges of $E_1$.

The remainder of the algorithm is iterative.
We use a parameter $\alpha'=8\Delta\alpha=\frac{1}{16 \alphasc(n)\log_{3/2} n}$. Recall that $\alpha=\frac{1}{128\Delta \alphasc(n)\log_{3/2} n}$ is the well-linkedness parameter from the definition of type-2 acceptable clusters. Throughout the algorithm, we maintain a set $\hat E$ of edges of $G$ that will only grow throughout the algorithm, initializing $\hat E=E_1$, and a set $A$ of fake edges, initializing $A=\emptyset$. We denote $\hH=G\setminus \hat E$ with respect to the current set $\hat E$, and we let $\hcset$ be the set of connected components of $\hH\cup A$, that we refer to as \emph{clusters}. We call the endpoints of the edges of $\hat E$ \emph{terminals}, and denote by $\hGamma$ the set of terminals. We will ensure that edges of $A$ only connect pairs of terminals. We will also maintain an embedding $\pset=\set{P(e)\mid e\in A}$ of the fake edges, where for each edge $e=(u,v)\in A$, path $P(e)$ is contained in graph $G$ connecting $u$ to $v$.  We will ensure that all paths in $\pset$ are mutually internally disjoint.
We also maintain a partition of $\hcset$ into two subsets: set $\cset^A$ of \emph{active} clusters, and set $\cset^I$ of \emph{inactive} clusters.
Set $\cset^I$ of inactive clusters is in turn partitioned into two subsets, $\cset_1^I$ and $\cset_2^I$. We will ensure that every cluster $C\in \cset_1^I$ is a type-1 acceptable cluster. In particular, no edges of $A$ are incident to vertices of clusters in $\cset_1^I$. For every cluster $C\in \cset_2^I$, we denote by $A_C\subseteq A\cap E(C)$ the set of fake edges contained in $C$. We will maintain, together with cluster $C$, a planar drawing $\psi_C$ on the sphere, such that  $C$ is a type-2 acceptable cluster with respect to $\psi_C$. Additionally, for every fake edge $e=(x,y)\in A_C$, its embedding $P(e)$ is internally disjoint from $C$. Moreover, we will ensure that there is some cluster $C(e)\in \cset^I_1$ containing $P(e)\setminus \set{x,y}$, and for every pair $e,e'\in A$ of distinct edges, $C(e)\neq C(e')$.  Lastly, we ensure that no fake edges are contained in an active cluster of $\cset^A$.


\paragraph{Vertex Budgets.}
For the sake of accounting, we assign a budget $b(v)$ to every vertex $v$ in $G$.  The budgets are defined as follows. 
If $v\notin \hG$, then $b(v)=0$. 
Assume now that $v\in \hG$, and let $C\in \hcset$ be the unique cluster containing $v$. 
If $C\in \cset^I$, then $b(v)=1$. 
Otherwise, $b(v)=8\Delta\cdot \log_{3/2}(|\hGamma\cap V(C)|)$. 
At the beginning of the algorithm, the total budget of all vertices is $\sum_{t\in \hat\Gamma}b(t)\leq O(|\hat \Gamma|\cdot\Delta\log n)\leq O(|E_1|\cdot\Delta \log n)$. 
Note that, as the algorithm progresses, the sets $\cset^I$ and $\cset^A$ evolve, and the budgets may change. 
We will ensure that, over the course of the algorithm, the total budget of all vertices does not increase. 
Since the budget of every terminal in $\hG$ is always at least $1$, the total budget of all vertices is at least $|\hGamma|$ throughout the algorithm, and this will ensure that the total number of terminals at the end of the algorithm is bounded by $O(|E_1|\cdot\Delta\log n)\leq O\left((|E'|+\optcro(G))\cdot\poly(\Delta\log n)\right)$, and therefore $|\hat E|$ is also bounded by the same amount.

%\vspace{-4mm}
\paragraph{Initialization.}
At the beginning, we let $\hat E=E_1$, and we let $\hcset$ be the set of all connected components of the graph $\hH\cup A$, where $\hH=G\setminus \hat E$.  The set $\hG$ contains all endpoints of edges in $\hE$.
Recall that we have identified a subset $\cset_1'$ of clusters of $\hH$, each of which contains at most $\mu$ terminals. We set $\cset^I=\cset^I_1=\cset_1'$, $\cset^I_2=\emptyset$, and $\cset^A=\hcset\setminus \cset^I$. The algorithm proceeds in iterations, and will continue to execute as long as $\cset^A\neq \emptyset$. %We now describe the execution of an iteration.

\subsubsection*{Description of an Iteration}
We now describe a single iteration.
Let $C\in \cset^A$ be any active cluster. If $|\hGamma\cap V(C)|\leq \mu$, then we  move $C$ from $\cset^A$ to $\cset^I_1$ and continue to the next iteration. Clearly, in this case $C$ is a type-1 acceptable cluster, and the budgets of vertices may only decrease.

We assume from now on that $|\hGamma\cap V(C)|> \mu$ and denote $\tilde\Gamma=\hGamma\cap V(C)$. 
We then apply the algorithm $\algsc$ for computing the (approximate) sparsest cut to the graph $C$, with respect to the set $\tilde\Gamma$. 
Let $(X,Y)$ denote the cut that the algorithm returns, and assume w.l.o.g. that $|X\cap \tilde\Gamma|\leq |Y\cap \tilde\Gamma|$. Denote $E^*=E_C(X,Y)$. Assume first that $|E^*|<\alpha'\cdot \alphasc(n) |X\cap \tilde\Gamma|$. Then we delete the edges of $E^*$ from $\hH$ and add them to the set $\hat E$. We then replace the cluster $C$ in $\cset^A$ by all connected components of $C\setminus E^*$ and continue to the next iteration. Note that we may have added new terminals to $\hGamma$ in this iteration: the endpoints of the edges in $E^*$. Denote by $\Gamma^*$ the set of endpoints of these edges.
The changes in the budgets of vertices are as follows. On the one hand, for every new terminal $t\in \Gamma^*$, the budget $b(t)$ may have grown from $0$ to at most $8\Delta\cdot \log_{3/2}n$.
%(this is since the total number of terminals that lie in $X$ at the end of this iteration is at most $|\tilde\Gamma|$ -- the number of terminals that originally lied in $C$, and the same is true for $Y$).
Since $|\Gamma^*|\leq 2|E^*|\leq 2 \alpha'\cdot \alphasc(n) |X\cap \tilde\Gamma|$, the total increase in the budget of new terminals is at most $16 \alpha'\cdot \alphasc(n) |X\cap \tilde\Gamma|\cdot \Delta\log_{3/2} n$.
Note that for terminals in $\tilde\Gamma\cap Y$, their budgets can only decrease.
On the other hand, since $|\tilde\Gamma\cap X|\leq |\tilde\Gamma\cap Y|$ and the cut $(X,Y)$ is sufficiently sparse, the total number of terminals that lie in $X$ at the end of the current iteration is at most $2|\tilde\Gamma|/3$. 
Therefore, the budget of every terminal in $\tilde\Gamma\cap X$ decreases by at least $8\Delta$, and the total decrease in the budget is therefore at least $8\Delta\cdot|X\cap \tilde\Gamma|$. 
Since $\alpha'=\frac{1}{16\alphasc(n)\log_{3/2}n}$, the total budget of all terminals does not increase.

We assume from now on that algorithm $\algsc$ returned a cut of sparsity at least $\alpha'\cdot \alphasc(n)$. Then we are guaranteed that with high probability, the set $\tilde \Gamma$ of terminals is $\alpha'$-well-linked in $C$. 
%Since $\alpha'>\alpha$, they are also $\alpha$-well-linked in $C$, but we will need to use this stronger $\alpha'$-well-linkedness property. 
%We denote by $U$ the set of all separator vertices of $C$.
%that is, a vertex $v\in U$ iff graph $C\setminus v$ is  . 
%
We use the following standard definition of vertex cuts:
\begin{definition}
Given a graph $\hat G$, a \emph{vertex cut} in $\hat G$ is a partition $(W,X,Y)$ of $V(\hat G)$ into three disjoint subsets, with $W,Y\neq\emptyset$, such that no edge of $\hat G$ connects a vertex of $W$ to a vertex of $Y$. We say that the cut is a \emph{$1$-vertex cut} if $|X|=1$, and we say that it is a $2$-vertex cut if $|X|=2$.
\end{definition}
In the remainder of the proof we consider three cases. The first case is when graph $C$ has a $1$-vertex cut $(W,X,Y)$, with $W$ and $Y$ containing at least two terminals of $\tilde \Gamma$ each. In this case, we delete some edges from $C$, decomposing it into smaller clusters, and continue to the next iteration. The second case is when $C$ has a $2$-vertex cut $(W,X,Y)$, where both $W$ and $Y$ contain at least three terminals of $\tilde \Gamma$. In this case, we also delete some edges from $C$, decomposing it into smaller connected components, and continue to the next iteration. The third case is when neither of the first two cases happens. In this case, we decompose $C$ into a single type-$2$ acceptable cluster, and a collection of type-$1$ acceptable clusters. We now proceed to describe each of the cases in turn.

\paragraph{Case 1.} We say that Case 1 happens if there is a $1$-vertex cut $(W,X,Y)$, with $|W\cap \tilde \Gamma|,|Y\cap \tilde \Gamma|\geq 2$. Set $X$ contains a single vertex, that we denote by $v$. Assume w.l.o.g. that $|W\cap \tilde \Gamma|\leq |Y\cap \tilde \Gamma|$. We start with the following simple claim.
\begin{claim}\label{claim: few vertices on one side of 1-sep}
	$|W\cap \tilde \Gamma|<\mu/4$.
\end{claim}
\begin{proof}
Assume for contradiction that the claim is false.
Consider a bi-partition $(W',Y')$ of $V(C)$, where $W'=W\cup \set{v}$ and $Y'=Y$. We denote by $E^*$ the set of all edges of $C$ incident to the separator vertex $v$, so $|E^*|\leq \Delta$. Since $E_C(W',Y')\subseteq E^*$, $|E_C(W',Y')|\leq \Delta$. However, since vertices of $\tilde \Gamma$ are $\alpha'$-well-linked in $C$, we have $|E_C(W',Y')|\geq \alpha'\cdot |W'\cap \tilde \Gamma|\geq \alpha' \cdot \mu/4>\Delta$, (as $\mu=512\Delta \alphasc(n)\log_{3/2} n$, while $\alpha'=\frac{1}{16\alphasc(n)\log_{3/2} n}$), a contradiction. 
\end{proof}

Let $E_0$ be the set of all edges that connect the separator vertex $v$ to the vertices of $W$. 
We add to $\hat E$ the edges of $E_0$. 
Consider now the graph $C\setminus E_0$. Note that for every connected component of $C\setminus E_0$, either $V(C')\subseteq W$, or $V(C')=Y\cup\set{v}$. We let $\sset$ contain all components $C'$ with $V(C')\subseteq W$. Note that every component $C'\in \sset$ is a type-1 acceptable cluster. This is because $|\tilde \Gamma\cap V(C')|\leq |\tilde \Gamma\cap W|\leq \mu/4$, and we have created at most $\Delta$ new terminals in $C'$: the endpoints of the edges in $E_0$. As $\mu>4\Delta$, every component $C'\in \sset$ now contains at most $\mu$ terminals. We add all components in $\sset$ to the set $\cset^I_1$ of inactive components (and also to the set $\cset^I_1$). Additionally, we replace the cluster $C$ in $\cset^A$ by the subgraph of $C$ induced by vertices of $Y\cup\set{v}$.

It remains to prove that the total budget of all vertices does not grow. 
Note that $|\tilde \Gamma\cap W|\ge 2$, %The budget of each such terminal before the current iteration was $8\Delta \cdot \log_{3/2}(|\tilde \Gamma|)$, and at the end of the current iteration, their budgets became $1$ each. 
and the budget of each terminal $t\in \tilde \Gamma\cap W$ has decreased from $8\Delta \cdot \log_{3/2}(|\tilde \Gamma|)$ to $1$. Therefore, the total budget decrease of these terminals is at least $16\Delta \cdot \log_{3/2}(|\tilde \Gamma|)-2$. We have created at most $\Delta$ new terminals in set $W$. For each new terminal, its new budget is $1$ since at the end of this iteration it belongs to an inactive cluster. We have created at most one new terminal in set $X\cup Y$ -- the vertex $v$. Since $|\tilde \Gamma\cap W|\ge 2$, the total number of terminals in $X\cup Y$ at the end of the iteration is at most $|\tilde \Gamma|-1$. Therefore, the budgets of terminals in $\tilde\Gamma \cap Y$ do not increase, and the budget of $v$ is at most $8\Delta \cdot \log_{3/2}(|\tilde \Gamma|)$. 
Altogether, the total budget increase is at most $8\Delta \cdot \log_{3/2}(|\tilde \Gamma|)+\Delta$, which is less than $16\Delta \cdot \log_{3/2}(|\tilde \Gamma|)-2$, the total budget decrease of vertices of $\tilde \Gamma\cap W$.
Conclusively, the total budget of all vertices does not increase.

From now on we assume that Case 1 does not happen. We need the following simple observation.
\begin{observation}\label{obs: no case 1 small cuts}
Assume that Case 1 does not happen. Let $(W,X,Y)$ be any $1$-vertex cut in $C$, then either $|W|=1$, or $|Y|=1$.
\end{observation}
\begin{proof}
Assume for contradiction that $|W|,|Y|>1$. Since Case 1 does not happen, either $|W\cap \tilde \Gamma|\leq 1$, or $|Y\cap \tilde \Gamma|\leq 1$. Assume w.l.o.g. that $|W\cap \tilde \Gamma|\leq 1$. 
Let $t\in W\cap \tilde \Gamma$ be the unique terminal that lies in $W$ (if it exists; otherwise $t$ is undefined), and let $u$ be any vertex that lies in $W\setminus \tilde \Gamma$ (since $|W|>1\ge |W\setminus \tilde \Gamma|$, such a vertex always exists). Note that the removal of $v$ and $t$ (if it exists) from $G$ separates $u$ from vertices of $Y$ in $G$, causing a contradiction to the fact that $G$ is $3$-connected.
\end{proof}

Let $U$ be the set of separator vertices of $C$. From the above observation, for every separator vertex $u\in U$, there is another vertex $u'\in V(C)$ that is a neighbor of $u$, such that $u'$ has degree $1$ in $C$. %Moreover, vertex $u$ is not a separator vertex for $C\setminus\set{u'}$. 
Since graph $G$ is $3$-connected, $u'$ must belong to $\tilde \Gamma$. Let $U'$ be the set of all such vertices. It is easy to verify that graph $C\setminus U'$ is $2$-connected.

%Assume otherwise. Consider a partition $(X,Y)$ of $V(C)$, that is defined as follows. Set $X$ contains, for every super-node $v_{Z'}\in V(T')$, all vertices of $Z'$, while set $Y$ contains all remaining vertices of $C$. Since $w(T')\geq \mu/4$, $|X\cap \tilde\Gamma|\geq \mu/4$. Moreover, from the choice of $Z_0$, $w(Y)\geq \mu/16$ must hold. Let $u'$ be the parent vertex of $v_{Z_0}$ in the tree, that must be a separator vertex, and let $E^*$ be the set of all edges of $C$ that are incident to $u'$. Clearly, $E_C(X,Y)\subseteq E^*$, and so $|E_C(X,Y)|\leq \Delta$. On the other hand, since the set $\tilde\Gamma$ of terminals is $\alpha'$-well-linked in $C$, $|E_C(X,Y)|\geq \alpha'\cdot \min\set{|X\cap \tilde\Gamma|,|Y\cap \tilde\Gamma|}\geq \alpha'\mu/16>\Delta$ (as $\mu=512\Delta \alphasc(n)\log_{3/2} n$, while $\alpha'=\frac{1}{16\alphasc(n)\log_{3/2} n}$), a contradiction.
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------
\paragraph{Case 2.}
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------
We say that Case 2 happens if Case 1 does not happen, and there is a $2$-vertex cut $(W,X,Y)$, with $|W\cap \tilde \Gamma|,|Y\cap \tilde \Gamma|\geq 3$. Set $X$ contains exactly two vertices, that we denote by $x,y$. Assume w.l.o.g. that $|W\cap \tilde \Gamma|\leq |Y\cap \tilde \Gamma|$. 
The algorithm for Case 2 is very similar to the algorithm for Case 1.
We start with the following simple claim, that is similar to Claim \ref{claim: few vertices on one side of 1-sep}, and its proof is almost identical.
\begin{claim}\label{claim: few vertices on one side of 2-sep}
$|W\cap \tilde \Gamma|<\mu/4$.
\end{claim}
\begin{proof}
Assume for contradiction that the claim is false.
Consider a bi-partition $(W',Y')$ of $V(C)$, where $W'=W\cup \set{x,y}$ and $Y'=Y$. Let $E^*$ be the set of all edges of $C$ incident to vertices $x$ or $y$, so $|E^*|\leq 2\Delta$. Since $E_C(W',Y')\subseteq E^*$, $|E_C(W',Y')|\leq 2\Delta$. However, since vertices of $\tilde \Gamma$ are $\alpha'$-well-linked in $C$, we have $|E_C(W',Y')|\geq \alpha'\cdot |W'\cap \tilde \Gamma|\geq \alpha' \cdot \mu/4>2\Delta$, (as $\mu=512\Delta \alphasc(n)\log_{3/2} n$, while $\alpha'=\frac{1}{16\alphasc(n)\log_{3/2} n}$), a contradiction. 
\end{proof}

Let $E_0$ be the set of all edges that connect the vertices $x,y$ to the vertices of $W$. 
We add to $\hat E$ the edges of $E_0$. 
Consider now the graph $C\setminus E_0$ and let $\sset$ be the set of its connected components. Note that, for every component of $C'\in \sset$, either $V(C')\subseteq W$ or $V(C')\subseteq Y\cup\set{x,y}$. We let $\sset_1\subseteq \sset$ contain all components $C'$ with $V(C')\subseteq W$, and we let $\sset_2$ contain all remaining connected components. Note that every component $C'\in \sset_1$ is a type-1 acceptable cluster. This is because $|\tilde \Gamma\cap V(C')|\leq |\tilde \Gamma\cap W|\leq \mu/4$, and we have created at most $2\Delta$ new terminals in $C'$: the endpoints of edges in $E_0$. As $\mu>8\Delta$, every component in $\sset_1$ now contains at most $\mu$ terminals. We add all components in $\sset_1$ to the set $\cset^I_1$ (and also to $\cset^I_1$). Additionally, we replace the cluster $C$ in $\cset^A$ by all components in $\sset_2$.

It remains to prove that the total budget of all vertices does not grow. The proof again is very similar to the proof in Case 1.
Note that set $|\tilde \Gamma\cap W|\ge 3$, and the budget of each terminal in $\tilde \Gamma\cap W$ has decreased from $8\Delta \cdot \log_{3/2}(|\tilde \Gamma|)$ to $1$. Therefore, the decrease of their total budgets is at least $24\Delta \cdot \log_{3/2}(|\tilde \Gamma|)-3$. We have created at most $2\Delta$ new terminals in set $W$ -- the neighbors of $x$ and $y$, and each such new terminal has new budget $1$ since it belongs to an inactive cluster at the end of this iteration. We have created at most two new terminals in set $X\cup Y$ -- $x$ and $y$. Since $|\tilde \Gamma\cap W|\ge 3$, the total number of terminals that belong to set $X\cup Y$ at the end of the current iteration is at most $|\tilde \Gamma|-1$. Therefore, the budgets of terminals in $\tilde{\Gamma}\cap Y$ do not increase, and the budgets of the vertices $x$ and $y$ are at most $8\Delta \cdot \log_{3/2}(|\tilde \Gamma|)$. 
Altogether, the total budget increase is at most $16\Delta \cdot \log_{3/2}(|\tilde \Gamma|)+2\Delta$, which is less than $24\Delta \cdot \log_{3/2}(|\tilde \Gamma|)-3$, the todal budget decrease of vertices of $\tilde \Gamma\cap W$.
Conclusively, the total budget of all vertices does not increase.
From now on, we can assume that Case 1 and Case 2 did not happen.

\paragraph{Case 3.} The third case happens if neither Case 1 nor Case 2 happens. Recall that we have denoted by $U$ the set of all separator vertices of the cluster $C$. We have defined $U'$ to be the set of vertices that is the neighbor of some $u\in U$ and has degree $1$ in $C$, and shown that $U'\subseteq \tilde \Gamma$. Our first step is to add to the set $\hat E$ all edges in $C$ connecting a vertex of $U$ to a vertex of $U'$, and let $C'=C\setminus U'$. Every vertex $u'\in U'$ is now an isolated vertex of $G\setminus \hat E$. For each such vertex $u'\in U'$, we add the cluster $\set{u'}$ to the set $\cset^I_1$ of inactivate type-1 acceptable clusters (and also to $\cset^I$). Notice that every vertex $u\in U$ now becomes a terminal. We denote by $\tilde \Gamma'=(\tilde \Gamma\cup U)\setminus U'$ the set of terminals in the current cluster $C'$. From the above discussion, $|\tilde \Gamma'|\leq |\tilde \Gamma|$, and cluster $C'$ is $2$-vertex connected. If $|\tilde \Gamma'|\leq \mu$, then $C'$ is a type-1 acceptable cluster. We then add it to the sets $\cset^I_1$ (and also to $\cset^I$), and terminate the current iteration. Note that the total budget of all vertices does not increase. This is because, before the current iteration, $|\tilde \Gamma|\geq \mu$, and every vertex in $\tilde \Gamma$ had budget at least $8\Delta\log \mu$; while at the end of the current iteration, every terminal in $\tilde \Gamma'\cup U'$ has budget $1$, and $|\tilde \Gamma'\cup U'|\leq 2\mu$. Therefore, we assume from now on that $|\tilde \Gamma'|>\mu$, and we refer to the vertices of $\tilde \Gamma'$ as terminals. In the remainder of this iteration, we will split the cluster $C'$ into a single type-2 acceptable cluster, and a collection of type-1 acceptable clusters, and we will prove that the total budget of all vertices does not increase.
Before we proceed further, we first prove the the following observations on $C'$ that we will use later.
\begin{observation}
\label{obs:C'_terminal_wl}
The set $\tGamma'$ of terminals is $\alpha'$-well-linked in $C'$.
\end{observation}
\begin{proof}
Consider any partition $(X,Y)$ of $V(C')$. Then we can augment $(X,Y)$ to a partition $(X',Y')$ of $V(C)$ as follows. Start with $X'=X$ and $Y'=Y$. For every vertex $u\in U$, if $u\in X$, then we add all its neighbors in $U'$ to $X'$, otherwise we add them to $Y'$. Note that $|\tGamma\cap X'|\geq |\tGamma'\cap X|$. This is because $\tGamma'=(\tGamma\cup U)\setminus U'$, and for every vertex $u\in U\cap X$, while $u$ may or may not belong to $\tGamma$, it always has a neighbor in $U'\cap \tGamma$.
Similarly, $|\tGamma\cap Y'|\geq |\tGamma'\cap Y|$. Since the set $\tGamma$ of terminals is $\alpha'$-well-linked in $C$, we get that $|E_{C'}(X,Y)|=|E_C(X',Y')|\geq \alpha'\cdot\min\set{|\tGamma\cap X'|,|\tGamma\cap Y'|}\geq \alpha'\cdot\min\set{|\tGamma'\cap X|,|\tGamma'\cap Y|}$. Therefore,  the set $\tGamma'$ of terminals is $\alpha'$-well-linked in $C'$.
\end{proof}
\begin{observation}\label{obs: small 2-vertex cuts in smaller cluster}
For every $2$-vertex cut $(W,X,Y)$ of $C'$ with $|W\cap \tilde \Gamma'|\leq |Y\cap \tilde \Gamma'|$, $|W\cap \tilde \Gamma'| \leq 2$.
\end{observation}
\begin{proof}
Let $(W,X,Y)$ be a $2$-vertex cut of $C'$ with $|W\cap \tilde \Gamma'|\leq |Y\cap \tilde \Gamma'|$. We augment it to a $2$-vertex cut $(W',X,Y')$ of $C$ as follows. Start with $W'=W$ and $Y'=Y$. For every vertex $u\in U$, if $u\in W$, then we add all its neighbors in $U'$ to $W$, otherwise we add them to $Y'$. It is immediate to verify that $(W',X',Y')$ is indeed a $2$-vertex cut in $C$, and that $|W'\cap \tilde \Gamma|\geq |W\cap \tilde \Gamma'|$ and  $|Y'\cap \tilde \Gamma'|\geq |Y\cap \tilde \Gamma'|$. Since we assumed that Case 2 does not happen, $|W'\cap \tilde \Gamma|\leq 2$ must hold, and so $|W\cap \tilde \Gamma'|\leq 2$.
\end{proof}

The next observation gives us a planar drawing of $C'$. %Recall that $\bset'$
%(defined in Section~\ref{sec:stage1}) 
%is the set of marked pseudo-blocks in the block decomposition of $G\setminus E'$, where $E'$ is the initial input planarizing set of edges.
\begin{observation}\label{obs: block containing cluster}
There is a good pseudo-block $B_0$ in graph $G\setminus E_1$ that is not contained in a component of $\cset'_1$, such that $C'\subseteq \tilde B_0'$. In particular, the unique planar drawing $\rho_{\tilde B_0}$ of $\tilde B_0$ naturally induces a planar drawing $\psi_{C'}$ of the cluster $C'$.
\end{observation}
\begin{proof}
Let $H_1=G\setminus E_1$ and $H_2=G\setminus \hat E$. Clearly $E_1\subseteq \hat{E}$. 
Denote by $\bset(H_1)$ the block decomposition of the graph $H_1$. 
Note that $C'$ itself is a pseudo-block in the block decomposition of $H_2$ (since $C'$ is the inclusion-wise maximal $2$-connected component of $C$).
Let $B_0\in \bset(H_1)$ be the pseudo-block corresponding to $C'$ given by Lemma~\ref{lem: block containment}, so $V(C')\subseteq V(B_0)$.
From Claim \ref{claim: every block is good}, $B_0$ is a good pseudo-block.
From the algorithm, it is impossible that $V(B_0)\subseteq V(\hat C)$ for a component $\hat C\in \cset_1'$, since initially all clusters in $\cset_1'$ belong to $\cset^I_1$ and will not be processed. 
%Therefore, $B_0\in \bset'$. 
%Recall that set $E_1\subseteq \hat E$ of edges contains all edges incident to the endpoints of the fake edges of $\tilde B_0$. 
%Lastly, since $\hat B\subseteq C'$, $C'$ is a $2$-connected subgraph of $H_2$, and $H_2\subseteq H_1$, it follows that all edges and vertices of $C'$ lie in $\tilde B_0'$.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%




We now proceed to split the cluster $C'$ into one type-2 acceptable cluster and a collection of type-1 clusters.
Recall that $C'$ is $2$-connected. %We denote by $S_2$ the set of all vertices that participate in some $2$-separator of $C'$. Equivalently, a vertex $v\in V(C')$ belongs to $S_2$ iff there is a vertex $v'\in V(C')$, such that $C'\setminus\set{v,v'}$ is not connected.
Let $\lset$ be the block decomposition of $C'$ given by Theorem~\ref{thm: block decomposition},
%Recall that the theorem ensures that for every vertex $v\in S_2$, either $v$ is an endpoint of a block of $\lset$, or $v$ has exactly two  neighbors in $C'$, and there is an edge $(v',v)\in E$, such that $v'$ is an endpoint of a block $B\in \lset$.
and let $\tau=\tau(\lset)$ be the decomposition tree associated with the decomposition $\lset$. We let $B\in \lset$ be the pseudo-block that, among all pseudo-blocks that contain at least $\mu/4$ terminals of $\tilde \Gamma'$, maximizes the distance in $\tau$ between its corresponding vertex $v(B)$ and the root of $\tau$, breaking ties arbitrarily. Notice that such a pseudo-block always exists, since $C'$ belongs to $\lset$ as a pseudo-block and contains at least $\mu$ terminals of $\tGamma'$. Let $v(B_1),\ldots,v(B_q)$ denote the child vertices of $v(B)$ in $\tau$, and let $B^c$ denote the complement block of $B$.
%(that is, $V(B^c)$ has the same endpoints as $B$, and contains, in addition to these endpoints, all vertices that do not lie in $B$; graph $B^c$ is the sub-graph of $C'$ induced by $V(B^c)$. 
We denote the endpoints of $B$ by $(x,y)$, and, for all $1\leq i\leq q$, the endpoints of $B_i$ by $(x_i,y_i)$. Recall that $\nset(B)=\set{B^c, B_1,\ldots,B_q}$. We use the following simple observations and their corollaries on $B$.
\begin{observation}
\label{obs:leaf_contain_terminals}
Let $\hat B$ be a pseudo-block in $\lset$ such that $v(\hat B)$ is a leaf of the tree $\tau$, then $\hat B$ contains terminal of $\tGamma'$ that is not an endpoint of $\hat B$.
\end{observation}
\begin{proof}
Let $x,y$ be the endpoints of $\hat B$. Assume that $\hat B$ does not contain a terminal that does not belong to $\set{x,y}$, then the removal of $\set{x,y}$ separates $V(\hat B)\setminus \set{x,y}$ from $V(G)\setminus V(\hat B)$, causing a contradiction to the fact that $G$ is $3$-connected.
\end{proof}
\begin{corollary}
\label{obs:number_of_branch}
$|\nset(B)|\leq |\tilde \Gamma'|$.
\end{corollary}
%\begin{proof}
%Since graph $G$ is $3$-connected, for all $1\leq i\leq q$, at least one vertex of $V(B_i)\setminus\set{x_i,y_i}$ must belong to $\tGamma'$. Similarly, at least one vertex of $V(B^c)\setminus \set{x,y}$ belongs to $\tGamma'$. Clearly, these vertices are distinct. Therefore, $|\nset(B)|\leq |\tilde \Gamma'|$.
%\end{proof}
\begin{observation}\label{obs: few terminals in every other block}
For all $1\leq i\leq q$, at most two vertices of $V(B_i)\setminus\set{x_i,y_i}$ belong to $\tGamma'$. Similarly, at most two vertices of $V(B^c)\setminus\set{x,y}$ belong to $\tGamma'$.
\end{observation}
\begin{proof}
Fix some $1\leq i\leq q$, and consider a $2$-vertex cut $(W,X,Y)$ of $C'$, where $W=V(B_i)\setminus\set{x_i,y_i}$, $X=\set{x_i,y_i}$, and $Y=V(C')\setminus(X\cup W)$. From the definition of the block $B$, $|W\cap \tilde \Gamma'|<\mu/4$. Since $|\tilde \Gamma'|>\mu$, $|Y\cap \tilde \Gamma'|\geq 3\mu/4-2>\mu/4>|W\cap \tilde \Gamma'|$. From \ref{obs: small 2-vertex cuts in smaller cluster}, $|W\cap \tGamma'|\leq 2$. Therefore, $V(B_i)\setminus\set{x_i,y_i}$ contains at most two terminals of $\tGamma'$.
The proof that $V(B^c)\setminus\set{x,y}$ contains at most two terminals of $\tGamma'$ is similar. 
%We define a $2$-vertex cut $(W,X,Y)$ of $C'$, where $W=V(B^c)\setminus \set{x,y}$, $X=\set{x,y}$, and $W=V(C')\setminus(X\cup Y)$. From the definition of the block $B$, and since $V(B)\setminus\set{x,y}\subseteq Y$, we get that $|Y\cap \tilde \Gamma'|\geq \mu/4-2>4$. But then, from \ref{obs: small 2-vertex cuts in smaller cluster}, $|W\cap \tGamma'|\leq 2$. Therefore, $V(B^c)\setminus\set{x,y}$ contains at most two terminals of $\tGamma'$.
\end{proof}
%The proof follows immediately from the fact that $G$ is a $3$-connected graph. By combining the above observation with Observation \ref{obs: few terminals in every other block}, we obtain the following immediate corollary.
\begin{corollary}\label{cor: few leaves in each sub-block}
There are at most two leaves in tree $\tau$ that are not descendants of $v(B)$. Moreover, for all $1\leq i\leq q$, there are at most two leaves in the sub-tree of $\tau$ rooted at $v(B_i)$.
\end{corollary}


We now describe the next steps of further processing $C'$.
We start with a high-level overview for some intuition. 
From Observation~\ref{obs: block containing cluster}, the drawing $\rho_{\tilde B_0}$ of $\tilde B_0$ naturally induces a planar drawing $\psi_{C'}$ of $C'$. One can show that $C'$ is a type-2 acceptable cluster with respect to the drawing $\psi_{C'}$, except that we cannot ensure that the size of $S_2(C)$, the set of vertices of $C'$ that participate in some $2$-separators of $C'$, is sufficiently small (recall that the requirement in the definition of type-$2$ acceptable clusters is that $|S_2(C')|\leq O(\Delta|\tilde \Gamma'|)$. 
To see this, consider the situation where the sub-tree of $\tau$ rooted at the child vertex $v(B_i)$ of $v(B)$, that we denote by $\tau_i$, is a long path. The cardinality of set $S_2(C')$ may be large as the length of the path, while there are only at most two terminals in $B_i$.

In order to overcome this difficulty, we need to ``prune'' the sub-tree $\tau_i$.
%Let $v(\hat B)$ be a leaf $\tau_i$. From Observation~\ref{obs:leaf_contain_terminals}, $\hat B$ contains a terminal $t\in \tilde \Gamma'$ that is not one of its endpoints, so $t$ also belongs to $B_i$ and it is not an endpoint of $B_i$. 
From Observation~\ref{obs: few terminals in every other block}, tree $\tau_i$ may contain at most two leaves. 
Assume first for simplicity that $\tau_i$ contains exactly one leaf, so $\tau_i$ is a path. 
%Note that, for every vertex $v(\hat B)$ on this path, the endpoints of $\hat B$ belong to $S_2(C')$. 
If we denote by $v(B^1_i),v(B^2_i),\ldots,v(B^r_i)$ the vertices that appear on path $\tau_i$ in this order, with $B^1_i=B_i$, we simply add to $\hat{E}$ all edges of $B^2_i$ incident to the endpoints of $B^1_i$, and replace $B^1_i$ with an fake edge connecting its endpoints in $C'$. 
The block $B^2_i$ is then decomposed into a number of a type-1 acceptable clusters. Notice that now the total number of vertices of $S_2(C')$ that block $B_i$ contributes is $O(1)$. If tree $\tau_i$ has two leaves, then the prune process of $\tau_i$ is slightly more complicated. We treat the complement block $B^c$ similarly as blocks in $\set{B_1,\ldots,B_q}$. 

We now provide a formal proof. We start with the cluster $\hat C=C'$ and the set $A_{\hat C}=\emptyset$ of fake edges, and then we iterate. In every iteration, we process a distinct block of $\nset(B)$, and modify the cluster $\hat C$ by deleting some edges and vertices and adding some fake edges to $A_{\hat C}$ and to $\hat C$. Throughout the algorithm, we will maintain the following invariants:
\begin{properties}{I}
\item $\hat C$ is a simple graph;
\item each $2$-separator of $\hat C$ is also a $2$-separator of $C'$; and\label{inv: 2-cuts preserved}
\item graph $\hat C\setminus A_{\hat C}$ is $2$-connected. \label{inv: 2-connectivity}
\end{properties}
%Throughout the algorithm, we will maintain a collection $\lset'$ of pseudo-blocks (that we call ``eliminated blocks''), starting from $\lset'=\emptyset$.
We now describe an iteration.
%\paragraph{Processing Blocks $B_i$.}
Consider a child block $B_i$ of block $B$ (the block $B^c$ will be processed similarly), and let $\tau_i$ be the sub-tree of $\tau$ rooted at $v(B_i)$. As our first step, we construct a set $V_i$ of nodes in $\tau_i$ that we are going to ``prune'' the subtree $\tau_i$ at, using the following observation.
\begin{observation}
\label{obs:prune}
There is an efficient algorithm, that, for each child block $B_i$ of $B$, constructs a subset $V_i\subseteq V(B_i)$ of vertices, that satisfies the following properties:
\begin{itemize}
\item for each vertex $\hat v\in V_i$, $v'$ has degree exactly $2$ in $\tau_i$, it is not $v(B_i)$ or one of its children, and the parent of $\hat v$ in $\tau_i$ has degree exactly $2$; 
\item if $|V_i|=2$ then neither vertex is a descendant of the other in $\tau_i$; and
\item if we let $\tau_i'$ be the sub-tree obtained from $\tau_i$ after we delete, for every vertex $\hat v\in V_i$, the sub-tree rooted at the child vertex of $\hat v$, then $|V(\tau_i')|\leq 10$.
\end{itemize}
The algorithm also constructs a subset $V_c$ of vertices of $V(B^c)$ that satisfies the above properties.
\end{observation} 
\begin{proof}
We fix a child block $B_i$ of $B$ and show how to construct $V_i$. 
The sets $\set{V_{j}}_{1\le j\le q, j\ne i}$ and $V_c$ are constructed similarly.
From Corollary \ref{cor: few leaves in each sub-block}, $\tau_i$ contains at most two leaves.
Therefore, there is at most one node in $\tau_i$ that has degree $3$, and all other nodes has degree $1$ or $2$. We consider the collowing cases:
\begin{enumerate}
	\item if $\tau_i$ contains no degree-$3$ node, and $|V(\tau_i)|\le 3$, then we set $V_i=\emptyset$;
	\item if $\tau_i$ contains no degree-$3$ node, and $|V(\tau_i)|\ge 4$, let $v(B_i)=v_1, v_2, v_3, v_4$ be the first four nodes of $\tau_i$ from the root; then we set $V_i=\set{v_3}$;
	\item if $\tau_i$ contains a degree-$3$ node $v'$, and the distance between $v'$ and $v(B_i)$ is at least $4$ in $\tau_i$, then let $v(B_i)=v_1, v_2, v_3, v_4$ be the first four nodes of $\tau_i$ from the root (note that none of them is $v'$), and we set $V_i=\set{v_3}$;
	\item if $\tau_i$ contains a degree-$3$ node $v'$, and the distance between $v'$ and $v(B_i)$ is at most $3$ in $\tau_i$, then the subtree of $\tau_i$ rooted at $v'$ can be viewed as the union of two paths that share a common endpoint $v'$; we denote by $\tau^1_i$ and $\tau^2_i$ the two paths; and
	\begin{enumerate}
		\item if $|V(\tau^1_i)|\le 3$, we set $V^1_i=\emptyset$;
		\item if $|V(\tau^1_i)|\ge 4$, let $v'=v'_1, v'_2, v'_3, v'_4$ be the first four nodes of $\tau^1_i$ from the root; then we set $V^1_i=\set{v'_3}$;
	\end{enumerate}
	we construct $V^2_i$ similarly, and set $V_i=V^1_i\cup V^2_i$.
\end{enumerate}
It is easy to see that, $V_i$ contains most two vertices, and satisfy the properties in Observation \ref{obs:prune}.
\end{proof} 

%(the constant $16$ above is arbitrary, and can be replaced by any other large enough constant). Note that we allow $V_i$ to be empty.

We consider the vertices in $V_i$ one by one. Let $\hat v\in V_i$ be a vertex in $V_i$, and let $\hat B$ be its corresponding block, namely $\hat v=v(\hat B)$. Let $v(\hat B')$ be the unique child vertex of $v(\hat B)$ in $\tau_i$, and let $(x',y')$ be its endpoints. Note that block $\hat B'$ contains a path $P$ connecting $x'$ to $y'$, and there is a path $P'$ in $\hat B\setminus \hat B'$ connecting $x'$ to $y'$. Let $\tilde E$ be the set of all edges of $\hat B'$ incident to $x'$ and $y'$. We add the edges of $\tilde E$ to $\hat E$. Consider now the graph $\hat C\setminus \tilde E$. It is immediate that there is one component $\tilde C$ containing all vertices of $\hat C\setminus\hat B'$, and all the remaining components are a type-1 acceptable clusters and are contained in $\hat B'$. We add these components to $\cset^I_1$ (and also to $\cset^I$). If the edge $(x',y')$ does not lie in $\tilde C$, then we add the edge $e'=(x',y')$ to the set $A_{\hat C}$ of fake edges, and let $P(e')=P$ be its embedding. %For the sake of the analysis, we set $P'(e)=P'$ be the path connecting $x'$ to $y'$ in $\hat B\setminus (\hat B'\setminus\set{x',y'})$. 
It is immediate that there is some type-1 acceptable clusters of $\hat C\setminus \tilde E$ that contains the path $P(e')\setminus\set{x',y'}$. 
%We let $C(e)$ be that connected component. 
Finally, we update $\hat C$ to be $\tilde C\cup \set{(x',y')}$. Put in other words, the new cluster $\hat C$ is obtained from the original cluster $\hat C$ by deleting all vertices of $\hat B'\setminus\set{x',y'}$ from it, and adding the fake edge $(x',y')$. 
We say that the block $\hat B$ is \emph{eliminated} when processing $B_i$. 
%We add $B^{**}$ to the set $\lset'$ of eliminated blocks.
\begin{claim}
After each vertex $\hat v\in V_i$ is processed, the invariants continue to hold.
\end{claim}
\begin{proof}
We denote by $C_1$ and $C_2$ the cluster $\hat C$ before and after $\hat v$ was processed, respectively. Similarly, we denote by $A_1$ and $A_2$ the set $A_{\hat C}$ of vertices before and after $\hat v$ was processed, respectively. We assume that all invariants held before $\hat v$ was processed. Clearly, $C_2$ is a simple graph, since we add a fake edge to $\hat C$ only if $\hat C$ does not contain it.
	
We first show that $C_2\setminus A_2$ is $2$-connected. Assume for contradiction that this is not the case, and let $(W,X,Y)$ be a $1$-vertex cut of $C_2\setminus A_2$.  We claim that either (i) $x'\in W$, $y'\in Y$, or (ii) $x'\in Y$, $y'\in W$. In fact, if neither of these holds, we can assume w.l.o.g. that $x',y'\in W\cup X$. Then, by adding to $W$ all vertices of $\hat B'\setminus\set{x',y'}$, we obtain a $1$-vertex cut in $C_1\setminus A_1$, causing a contradiction to the assumption that $C_1\setminus A_1$ is $2$-connected.
We now assume without loss of generality that $x'\in W$ and $y'\in Y$. 
%Since $\tilde {\hat B}$ is $3$-connected, it must contain three internally disjoint paths connecting $x'$ to $y'$. Two of these paths, that we denote by $P_1,P_2$, do not contain the fake edge $(x',y')$. If we denote by $(x,y)$ the endpoints of the block $\hat B$, then one of $P_1,P_2$ (say $P_1$) is disjoint from the fake edge $(x,y)$. Path $P_2$ may contain the fake edge $(x,y)$. 
Note that there exists two paths $P_1$ and $P_2$ connecting $x'$ to $y'$, such that $P_1$ consists of only edges in $\hat B$, and $P_2$ may contain the fake edge $(x,y)$ (while all other edges of $P_2$ are real edges in $\hat B$).
%Since $v(B^*)\neq v(B_i)$ and it is not a child vertex of $v(B_i)$, no fake edges 
Let $v(B^p)$ be the parent vertex of $v(\hat B)$ in $\tau$. 
Since $v(B^p)$ has degree exactly $2$ in $\tau_i$, there are at most two fake edges in $\tilde B^p$. Since $\tilde B^p$ is $3$-connected, there is a path $P$ connecting $x$ to $y$ in $\tilde B^p$, that does not contain fake edges. By combining $P_2$ with $P$ (replacing the fake edge $(x,y)$ of $P_2$ by the path $P$, if $P_2$ contains $(x,y)$), we obtain a path $P_3$ connecting $x'$ to $y'$, that is disjoint from $P_1$, and contains no fake edges. But then both paths $P_1,P_3$ must contain the separator vertex that lies in $X$, a contradiction. Therefore, Invariant~\ref{inv: 2-connectivity} continues to hold.
	
To show that Invariant \ref{inv: 2-cuts preserved} continues to hold, it suffices to show that any $2$-separator in $C_2$ is also a $2$-separator in $C_1$. Consider any $2$-vertex cut $(W,X,Y)$ in $C_2$, and assume w.l.o.g. that $x',y'\in W\cup X$. By adding all vertices of 
$\hat B'\setminus\set{x',y'}$ to set $W$, we obtain a $2$-vertex cut in $C_1$. Therefore, $X$ is also a $2$-separator in $C_1$.
\end{proof}
%\paragraph{Processing the Block $B^c$.} The algorithm for processing the block $B^c$ is very similar to the algorithm for processing the blocks $B_i$. The details are omitted.
%\mynote{If you have time and energy please feel free to fill them in but this is not a priority right now, unless there is a doubt in correctness}

Let $\hat C$ be the cluster we obtain after all blocks in $\nset(B)$ are processed. 
Recall that from Observation \ref{obs: block containing cluster}, there is a good pseudo-block $B_0$ in the block decomposition of $H_1$ with $C'\subseteq \tilde B_0'$.
The unique planar drawing $\rho_{\tilde B_0}$ of $\tilde B_0$ induces a planar drawing $\rho'_{\tilde B_0'}$ of $\tilde B_0'$, which in turn induces a planar drawing $\psi_{\hat C}$ of $\hat C$, where for each fake edge $e\in A_{\hat C}$, the edge $e$ is drawn along the drawing of the path $P(e)$ in $\rho'_{\tilde B_0'}$. We prove the following Lemma in Section~\ref{subsec:type-2-acceptable}.
\begin{lemma}\label{lemma: acceptable}
Cluster $\hat C$ is a type-2 acceptable cluster with respect to the drawing $\psi_{\hat C}$.
\end{lemma}
To complete the proof of \ref{thm: can find edge set w acceptable clusters}, it remains to show that if Case 3 happens, then the total budget of all vertices does not increase once after the cluster $C$ is processed.
Recall that $\tilde \Gamma$ is the set of terminals in $C$ before $C$ was processed, and $|\tilde \Gamma|\geq \mu$. Let $\tGamma_n$ be the set of all new terminals that were added to $\tGamma$ over the course of processing $C$. 
Notice that every vertex in $\tilde \Gamma$ had a budget of at least $8\Delta$ before $C$ was processed. After $C$ was processed, the budget of every terminal in $\tilde \Gamma\cup\tGamma_n$ is $1$. Therefore, in order to show that the total budget of all vertices did not grow, it is sufficient to show that $|\tGamma_n|\leq 7\Delta |\tGamma|$. Recall that we have created a set $U$ of at most $|\tilde \Gamma|$ terminals, and whenever a block $\hat B'$ was eliminated, we created at most $2\Delta$ new terminals (neighbors of endpoints of $\hat B'$. Since each such block $\hat B'$ contained at least one terminal of $\tGamma'=(\tilde \Gamma\cup U)\setminus U'$, the total number of new terminals that we have created is bounded by $|\tilde \Gamma|\cdot 4\Delta$. Therefore, the total budget of all vertices does not grow.






\subsection{Proof of Lemma \ref{lemma: acceptable}}
\label{subsec:type-2-acceptable}
From the invariants, $\hat C$ is a simple graph, and $\hat C\setminus A_{\hat C}$ is $2$-connected.

We first bound the cardinality of the set $S_2(\hat C)$. Recall that the invariants ensure that a $2$-separator in $\hat C$ is also a $2$-separator in $C'$, so $S_2(\hat C)\subseteq S_2(C')$. Moreover, Theorem \ref{thm: block decomposition} ensures that for every vertex $x\in S_2(C')$, either $x$ is an endpoint of a block of $\lset$, or there is a vertex $x'$ that is a neighbor of $x$ in $C'$, and it is an endpoint of a block of $\lset$. In the former case, we denote by $B(x)$ the largest (cardinality-wise) block of $\lset$ such that $x$ is an endpoint of $B(x)$, and in the latter case, we denote by $B(x)$ the largest block of $\lset$, such that $x'$ is an endpoint of $B(x)$. Notice that, if $\hat B$ is a block that was eliminated, and $x$ lies in $\hat B$ but is not an endpoint of $\hat B$, then $x$ is not a vertex of $\hat C$, and it does not belong to $S_2(\hat C)$. Notice that, from our algorithm, for every child block $B_i$ of $B$, there are at most $O(1)$ vertices $x$, such that $x\in V(\hat C)$, and $x$ serves as an endpoint of a block that is a descendant of $B_i$ in $\tau_i$. Therefore, at most $O(\Delta)$ vertices of $S_2(\hat C)$ may lie in $B_i\cap \hat C$. Similarly, at most $O(\Delta)$ vertices of $S_2(\hat C)$ may lie in $B^c\cap \hat C$. From Corollary~\ref{obs:number_of_branch}, $|\nset(B)|\leq |\tilde \Gamma'|$. It follows that $|S_2(\hat C)|\leq O(\Delta\cdot |\tilde \Gamma'|)$.
By definition, $\tilde \Gamma'\subseteq \hat \Gamma\cap V(\hat C)$. Therefore, $|S_2(\hat C)|\leq O(\Delta\cdot |\hat \Gamma\cap V(\hat C)|)$.

We then show that cluster $\hat C$ has the well-linkedness property.
\begin{claim}\label{claim: well linkedness}
The set $\tilde \Gamma\cap V(\hat C)$ of terminals is $\alpha$-well-linked in $\hat C\setminus A_{\hat C}$.
\end{claim}
\begin{proof}
%\mynote{needs to be completed. The idea. First, prove that $\hat \Gamma\cap V(C^*)$ is $4\alpha$-well-linked in $C^*$. In order to see this, take any cut $(X,Y)$ of $C^*$. Then augment it to a cut $(X',Y')$ of $C'$ by inserting back the eliminated blocks, like we did in the previous proof. Once you show it for $C^*$, we take the fake edges out. But for each fake edge $e=(x',y')$, we have defined a path $P'(e)$ that stays in $C^*\setminus A_{C^*}$. So the deletion of the fake edges only decreases the number of edges going across the cut by factor at most $2$.}
%Note that $\tilde \Gamma'=\hat \Gamma\cap V(\hat C)$.
We first show that the terminals in $\hat\Gamma\cap V(\hat C)$ are $2\alpha$-well-linked in $\hat C$. Let  $(X,Y)$ be any partition of $V(\hat C)$. Denote $\Gamma_X=(\hat\Gamma\cap V(\hat C))\cap X$ and $\Gamma_Y=(\hat\Gamma\cap V(\hat C))\cap Y$. It suffices to show that $|E_{\hat C}(X,Y)|\ge 2\alpha\cdot \min\set{|\Gamma_X|,|\Gamma_Y|}$.

Recall that, in addition to the terminals of $\tilde\Gamma'$, the sets $\Gamma_X,\Gamma_Y$ of terminals may also contain endpoints of blocks in $\nset(B)$. We call such terminals \emph{new terminals}.
%(a new terminal cannot belong to $\Gamma'$)
%We further partition sets $\Gamma_X$ and $\Gamma_Y$ as follows.
We let $\Gamma^1_X\subseteq \Gamma_X$ contain all terminals $t$, such that there is some block $B'\in \nset(B)$ with $t$ being one of its endpoints, and the other endpoint $t'$ of $B'$ lies in a different set in $\set{X,Y}$ than $t$. We let $\Gamma^2_X=\Gamma_X\setminus \Gamma^1_X$.
The partition $(\Gamma^1_Y,\Gamma^2_Y)$ of $\Gamma_Y$ is defined similarly. Observe that a new terminal may be an endpoint of more than one block in $\nset(B)$. Since the endpoints of every block in $\nset(B)$ are connected by a fake edge in $C$, it is immediate to verify that
\begin{equation}
|E_{\hat C}(X,Y)|\geq |\Gamma^1_X|\mbox{  and  } |E_{\hat C}(X,Y)|\geq |\Gamma^1_Y|. 
\label{eq: cut comparable to type 1 terminals}
\end{equation}
Next, we construct a cut $(X',Y')$ in graph $C'$ based on the cut $(X,Y)$ of $\hat C$, and then use the well-linkedness of the terminals in $\tilde\Gamma'$ in graph $C'$ (from Observation~\ref{obs:C'_terminal_wl}) to obtain a better lower bound of $|E_{\hat C}(X,Y)|$. We start with $X'=X$ and $Y'=Y$. Take any block $B'\in \nset(B)$ with endpoints $(x',y')$. 
%We define the set $S(B')$ of vertices to be the union of (i) $V(B')\setminus \set{x',y'}$; and (ii) all sets $X_i$ whose corresponding separator vertex $u_i\in U^*$ lies in $V(B')\setminus\set{x',y'}$. 
Note that $x',y'$ may not belong to $\tilde\Gamma'$. However, since we have assumed that graph $G$ is $3$-connected, set $V(B')\setminus \set{x',y'}$ must contain a terminal of $\tilde\Gamma'$. We denote this terminal by $t_{B'}$, and we will view this terminal as ``paying'' for $x'$ and $y'$ (if $x,y\in \Gamma^2_X\cup \Gamma^2_Y$).
If both $x',y'\in X$, then we add all vertices of $V(B')\setminus \set{x',y'}$ to $X$, otherwise we add them to $Y$. Notice that, if both $x',y'$ lie in the same set in $\set{X,Y}$, then we do not increase the number of edges in the cut $(X,Y)$. 
%Moreover, we can think of replacing the new terminals $x',y'$ with a terminal $t_{B'}\in \Gamma'\setminus \Gamma''$. 
Assume now that $x'\in X$ and $y'\in Y$ (the other case is symmetric). 
In this case, we have increased the number of edges in the cut $(X,Y)$ by at most $\Delta$, by adding all edges that are incident to $x'$ to this cut. Note however that the edge $(x',y')$ already belonged to this cut (possibly as a fake edge), so we charge this increase in the cut size to this fake edge. 
Once all blocks $B'\in \nset(B)$ are processed in this way, we obtain a cut $(X',Y')$ in graph $C'$. From the above discussion:
\begin{equation}
|E_{C'}(X',Y')|\leq \Delta\cdot |E_{\hat C}(X,Y)|.\label{eq: few new edges in cut}
\end{equation}
Consider now the terminals of $\Gamma_X$. Clearly $\Gamma_X\cap \tilde\Gamma'\subseteq X'$. For each terminal in $\Gamma^2_X$, we have added a terminal of $\tilde\Gamma'$ to $X'$ that pays for it, while each newly added terminal of $X'\cap \tilde\Gamma'$ pays for at most two terminals in $\Gamma^2_X$. Therefore, $|\Gamma^2_X|\leq 2|\tilde\Gamma'\cap X'|$, and similarly $|\Gamma^2_Y|\leq 2|\tilde\Gamma'\cap Y'|$. Since the set $\tilde\Gamma'$ of terminals was $\alpha'$-well-linked in $C'$,
$|E_{C'}(X',Y')|\geq \alpha'\cdot\min\set{|\tilde\Gamma'\cap X'|,|\tilde\Gamma'\cap Y'|}\geq (\alpha'/2) \min\set{|\Gamma^2_X|,|\Gamma^2_Y|}$.
Combining this with Equation \ref{eq: few new edges in cut}, we have $|E_{\hat C}(X,Y)| \geq \frac{\alpha'}{2\Delta}\cdot \min\set{|\Gamma^2_X|,|\Gamma^2_Y|}$.
Combining this with Equation \ref{eq: cut comparable to type 1 terminals}, and using $\alpha'=8\Delta\alpha$, we have $|E_{\hat C}(X,Y)| \geq \frac{\alpha'}{4\Delta}\cdot\min\set{|\Gamma_X|,|\Gamma_Y|}\geq 2\alpha \cdot\min\set{|\Gamma_X|,|\Gamma_Y|}$.
This completes the proof of Claim~\ref{claim: well linkedness}.

Now we consider the graph $\hat C\setminus A_{\hat{C}}$. Recall that, for each fake edge $e=(x',y')$, we have associated a path $P'(e)$ that is contained in $\hat C\setminus A_{\hat C}$, such that all associated paths for all fake edges are mutually edge-disjoint. Therefore, for each partition $(X,Y)$ of $V(\hat{C})$, the number of fake edges in $E_{\hat C\setminus A_{\hat C}}(X,Y)$ is at most $|E_{\hat C}(X,Y)|/2$. It follows that the terminals in $\hat{\Gamma}\cap V(\hat C)$ is $\alpha$-well-linked in $\hat C\setminus A_{\hat C}$.
\end{proof}

Lastly, the next claim will complete the proof of  Lemma \ref{lemma: acceptable}.
\begin{claim}
Cluster $\hat C$ has the bridge property.
\end{claim}
\begin{proof}
%\mynote{this needs to be completed. But because we already use a drawing of $C^*\setminus A_{C^*}$ that is induced by the drawing $\rho_{\tilde B_0}$ of $\tilde B_0$, we only need to use the second part of the original proof which is included here. The notation needs to be updated.}
Recall that, from Observation \ref{obs: block containing cluster}, $C'$ is contained in some block $B_0$ in $G\setminus E_1$ that is not contained in a component of $\cset'_1$. Therefore, the unique planar drawing $\rho_{\tilde B_0}$ induces a planar drawing of $C'$, and in turn induces a planar drawing of $\hat C\setminus A_{\hat C}$, that we denote by $\rho$. We now show that, for each bridge $R\in \rset_{G}(\hat C\setminus A_{\hat C})$, there is a face in $\rho$, whose boundary contains all vertices of $L(R)$.

Assume for contradiction that this is false, and let $R\in \rset_{G}(\hat C\setminus A_{\hat C})$ be a witness bridge such that not all vertices of $L(R)$ lie on the boundary of a single face of the drawing $\rho$.
Let $\fset$ be the set of all faces of the drawing $\rho$. 
For every vertex $v\in V(\tilde B_0)\setminus V(\hat C)$, there is a unique face $F(v)\in \fset$, such that the image of vertex $v$ in $\rho_{\tilde B_0}$ lies in the interior of the face $F$.
%\mynote{should we define $T_R$ here? Do we need it to have smallest number of edges, or is it enough that it is some tree spanning $L(R)$? (note that $R$ is no longer a bridge of a block, it's a bridge of $C^*$).}
Recall that $T_R$ is a tree in $R$ whose leaves are vertices of $L(R)$. 
Assume first that $V(T_R)\cap V(\tilde B_0)=L(R)$. In this case, there is some bridge $R'\in \rset_G(\tilde B_0')$ of $\tilde B_0'$ that contains the tree $T_R$, and so $L(R)\subseteq L(R')$. Since $B_0$ is a good pseudo-block, there must be a face in the drawing $\rho'_{\tilde B_0'}$, the drawing of $\tilde B_0'$ induced by $\rho_{\tilde B_0}$, whose boundary contains all vertices of $L(R)$. Therefore, for some face $F\in \fset$, all vertices of $L(R)$ must lie on the boundary of $F$. 
Assume now that there is some vertex $v\in V(T_R)\cap  V(\tilde B_0)$ that does not lie in $L(R)$. Let $F(v)$ be the face of $\fset$ whose interior contain the image of $v$ in $\rho_{\tilde B_0}$ (recall that $v\not\in V(\hat C)$, so it may not lie on a boundary of a face in $\fset$). We will show that all vertices of $L(R)$ must lie on the boundary of $F(v)$, leading to a contradiction. Let $u$ be an arbitrary vertex of $L(R)$. It suffices to show that $u$ must lie on the boundary of the face $F(v)$.
Let $P\subseteq T_R$ be the unique path connecting $v$ to $u$ in $T_R$. 
%Since the leaves of tree $T_R$ are vertices of $L(R)$, except for $v$, every vertex $x$ of $P$ lies outside $V(C^*)$, and the image of $x$ in $\rho_{\tilde B_0}$ lies in the interior of some face in $\fset$. 
Let $v=v_1,v_2,\ldots,v_r=u$ be all vertices of $P$ that belong to $V(\tilde B_0)$, and assume that they appear on $P$ in this order. 
It remains to prove the following observation.
\begin{observation}
$F(v_1)=F(v_2)=\cdots=F(v_r)$. Moreover, $v_r$ lies on the boundary of $F(v_{r-1})$.
\end{observation}
\begin{proof}
Fix some $1\leq i\leq r-1$. Assume that the observation is false.
Then there is some face $F'\in \fset$, such that $v_i$ lies in the interior of $F'$, but $v_{i+1}$ does not lie in the interior or on the boundary of $F'$ (the latter case is only relevant for $i=r-1$). Since the boundary of $F'$ separates $v_i$ from $v_{i+1}$, these two vertices cannot lie on the boundary of the same face in the drawing $\rho'_{\tilde B_0'}$ of $\tilde B_0'$. 
		
Let $\sigma_i$ be the subpath of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge connecting $v_i$ and $v_{i+1}$, then either it is a bridge in $\rset_G(\tilde B_0')$, or it is an edge of $\tilde B_0'$. In either case, the endpoints of $\sigma_i$ must lie on the boundary of a single face of the drawing $\rho'_{\tilde B_0'}$, a contradiction (we have used the fact that $B_0$ is a good block and that $\tilde B_0'$ is a planar graph). Otherwise, let $\sigma'_i$ be obtained from $\sigma_i$ by deleting the two endpoints from it. Then there must be a bridge $R'\in \rset_G(\tilde B_0')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. But then, since $B_0$ is a good pseudo-block, there must be a face in the drawing $\rho_{\tilde B_0}$ of $\tilde B_0$, whose boundary contains $v_i$ and $v_{i+1}$, leading to a contradiction. 
%	We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B_0'}$ of $\tilde B_0'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B_0_z\subseteq \tilde B_0'$, and from the way the drawing $\rho'_{\tilde B_0_z}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B_0_z}$ that contains $F_i$.	
\end{proof}
\end{proof}

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%--------------End of New Proof. Old Stuff below

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------

%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------


%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
\iffalse
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
The high-level plan for the remainder of the algorithm is the following. We will remove a small set of edges from $C$ and then decompose $C$ into a collection of subgraphs, such that all but one of these subgraphs are type-1 acceptable clusters. 
For the only non-type-1 subgraph, that we denote by $\hat C$, we will define a set $A_{\hat C}$ of fake edges, such that $C^*=\hat C\cup A_{\hat C}$ is a type-2 acceptable cluster. The remainder of the algorithm consists of three steps. In the first step, we compute the decomposition $\zset(C)$ of the cluster $C$ into super-blocks, and we identify a super-block $Z_0\in \zset(C)$, such that, roughly speaking, every connected component of $C\setminus Z_0$ contains fewer than $\mu/4$ terminals of $\tilde\Gamma$. In the second step, we compute the block decomposition $\lset(Z_0)$ of $Z_0$, and identify a pseudo-block $B_0\in \lset(Z_0)$, such that every connected component of $C\setminus \tilde B'_0$ contains at most $\mu$ terminals. In the third and the final step, we select a subset of edges to delete from $C$, define the cluster $C^*$ and the set $A_{C^*}$ of fake edges together with their embedding $\pset(A_{C^*})$, and complete the iteration.
In fact we will ensure that $C^*=\tilde B_0$ and show that $C^*$ is a type-2 acceptable cluster.
We now describe each of the three steps in turn.

%\vspace{-4mm}
\paragraph{Step 1: Selecting a super-block.}
Let $\zset(C)$ be the decomposition of cluster $C$ into super-blocks. %(maximal $2$-connected components) 
We can associate a tree $T$ with this decomposition, as follows. The set $V(T)$ of vertices is the union of two sets: the set $U$ of separator vertices, and the set $U'=\set{v_Z\mid Z\in \zset(C)}$ of vertices, that we call \emph{super-nodes}. For every super-block $Z\in \zset(C)$, and every separator vertex $u\in U$, such that $u\in V(Z)$, we add the edge $(u,v_Z)$ to the graph. It is easy to verify that graph $T$ is indeed a tree. We then define weights on vertices of $T$. For a vertex $u\in U$, its weight $w(u)$ is $1$ if $u\in \hGamma$, and is $0$ otherwise. For a super-node $v_Z$, the weight is the total number of terminals of $\hat \Gamma$ that lie in $Z\setminus U$. For each subtree $T'\subseteq T$, the weight of $T'$ is $w(T')=\sum_{v\in V(T')}w(v)$. Clearly, $w(T)=|\tilde\Gamma|$.
The current step is summarized in the following lemma.
\begin{lemma}\label{lemma: finding good super-block}
There is a super-block $Z_0\in \zset(C)$, such that the weight of every connected component of $T\setminus \set{v_{Z_0}}$ is at most $\mu/4$.
\end{lemma}
\begin{proof}
We root the tree $T$ at an arbitrary super-node $v_{Z}$. Let $v_{Z_0}$ be the lowest (that is, furthest from the root) super-node in the tree $T$, such that the sub-tree of $T$ rooted at $v_{Z_0}$ has weight at least $\mu/16$. Consider now the connected components of $T\setminus \set{v_{Z_0}}$. Let $T'$ be the connected component containing the root vertex (if such a component exists), and let $T_1,\ldots,T_q$ denote the remaining components, where component $T_i$ is the sub-tree of $T$ rooted at a child vertex $u_i$ of $v_{Z_0}$ (that must be a separator vertex). 
We need the following two observations.
\begin{observation}\label{obs: few terminals in root component}
$w(T')<\mu/4$.
\end{observation}
\begin{proof}
Assume otherwise. Consider a partition $(X,Y)$ of $V(C)$, that is defined as follows. Set $X$ contains, for every super-node $v_{Z'}\in V(T')$, all vertices of $Z'$, while set $Y$ contains all remaining vertices of $C$. Since $w(T')\geq \mu/4$, $|X\cap \tilde\Gamma|\geq \mu/4$. Moreover, from the choice of $Z_0$, $w(Y)\geq \mu/16$ must hold. Let $u'$ be the parent vertex of $v_{Z_0}$ in the tree, that must be a separator vertex, and let $E^*$ be the set of all edges of $C$ that are incident to $u'$. Clearly, $E_C(X,Y)\subseteq E^*$, and so $|E_C(X,Y)|\leq \Delta$. On the other hand, since the set $\tilde\Gamma$ of terminals is $\alpha'$-well-linked in $C$, $|E_C(X,Y)|\geq \alpha'\cdot \min\set{|X\cap \tilde\Gamma|,|Y\cap \tilde\Gamma|}\geq \alpha'\mu/16>\Delta$ (as $\mu=512\Delta \alphasc(n)\log_{3/2} n$, while $\alpha'=\frac{1}{16\alphasc(n)\log_{3/2} n}$), a contradiction.
\end{proof}
\begin{observation}\label{obs: few terminals in child components}
For all $1\leq i\leq q$, $w(T_i)\leq \mu/4$.
\end{observation}
\begin{proof}
Fix some $1\leq i\leq q$, and assume for contradiction that $w(T_i)>\mu/4$. Let $u$ be the child vertex of $v_{Z_0}$ in $T$, that serves as the root of the tree $T_i$, and let $T'_1,\ldots,T'_z$ be the trees that are rooted at the child vertices of $u$. From the choice of $v_{Z_0}$, for all $1\leq j\leq z$, $w(T'_j)<\mu/16$. Let $j'$ be the smallest index, such that $\sum_{j''=1}^{j'}w(T'_{j''})>\mu/16$. Then $\sum_{j''=1}^{j'}w(T'_{j''})<\mu/8$ must hold. We define a cut $(X,Y)$ in $C$ as follows. We let $X$ contain, for every super-node $v_{Z'}\in \bigcup_{j''=1}^{j'}V(T_{j''})$, all vertices of $Z'$, and we let $Y=V(C)\setminus X$. From the above discussion, $|X\cap \tilde\Gamma|,|Y\cap \tilde\Gamma|>\mu/16$. Let $E^*$ be the set of all edges that are incident to the vertex $u$. Then $E_C(X,Y)\subseteq E^*$, and we reach a contradiction exactly like in Observation \ref{obs: few terminals in root component}.
\end{proof}
\end{proof}

\paragraph{Step 2: Selecting a pseudo-block.}
We root the tree $T$ at the vertex $v_{Z_0}$, given by Lemma \ref{lemma: finding good super-block}, and we let $U^*=\set{u_1,\ldots,u_q}$ be set of the children of $v_{Z_0}$ in $T$. For each $1\leq i\leq q$, let $T_i$ be the sub-tree of $T$ rooted at $u_i$. 
Let set $X_i\subseteq V(C)$ contain (i) every separator vertex $u\in U\cap V(T_i)$, and (ii) for every super-node $v_Z\in V(T_i)$, all vertices of $Z$.
Let $\Gamma_i\subseteq \tilde\Gamma$ be the set of all terminals that contribute to $w(T_i)$, namely $\Gamma_i=X_i\cap \tilde\Gamma$. % that is, terminal $t$ belongs to $\Gamma_i$, if either $t$ is a separator vertex and belongs to $T_i$, or if there is a super-node $v_{Z'}\in V(T_i)$ with $t\in Z'$. 
Recall that, from Lemma \ref{lemma: finding good super-block}, $|\Gamma_i|\leq \mu/4$.

For a block $B\subseteq Z_0$, we say that $B$ \emph{owns} a terminal $t\in \tilde\Gamma$ iff either $t\in V(B)$, or $t\in T_i$ for some $1\leq i\leq q$ and $u_i\in V(B)$. 
We compute the block decomposition $\lset(Z_0)$ of the super-block $Z_0$. We use the following lemma in order to select the pseudo-block $B_0$.
\begin{lemma}\label{lemma: find the right block}
There is a pseudo-block $B_0\in \lset(Z_0)$ that owns at least $\mu/2$ terminals, such that every pseudo-block $B'\in \nset(B_0)$ owns at most $\mu/2$ terminals.
\end{lemma}
\begin{proof}
We let $B_0$ be the lowest pseudo-block in the decomposition tree $\tau=\tau(\lset(Z_0))$, that owns at least $\mu/2$ terminals. Since the super-block $Z_0$ owns at least $\mu$ terminals, such a pseudo-block exists. We now claim that every pseudo-block $B'\in \nset(B_0)$ owns at most $\mu/2$ terminals. This is clearly true for every child block $B'$ of $B_0$, from the choice of $B_0$. It now remains to prove that block $B^c$ owns at most $\mu/2$ terminals. Assume otherwise. 
Let $x,y$ be the endpoints of $B_0$, and let $E^*$ be the set of all edges of $C$ that are incident to $x$ or $y$. We define a partition $(X,Y)$ of $C$ as follows. Set $X$ contains all vertices of $B\setminus\set{x}$. Additionally, for each $1\leq i\leq q$ with $u_i\in V(B)\setminus\set{x}$, we add all vertices of $X_i$ to $X$. We then set $Y=V(C)\setminus X$. Note that $X$ contains all terminals that $B$ owns (with the only exception being $x$, if it is a terminal, or all terminals of $X_i$ if $x=u_i$ for some vertex $u_i\in U^*$), and $Y$ contains all terminals that $B^c$ owns (with the only exception being $y$, if it is a terminal, or all terminals of $X_i$ if $y=u_i$ for some vertex $u_i\in U^*$). Therefore $|X\cap \tilde\Gamma|,|Y\cap \tilde\Gamma|\geq \mu/4$. However, $E_C(X,Y)\subseteq E^*$, so $|E_C(X,Y)|\leq 2\Delta<\alpha' \mu/4\leq \alpha'\cdot \min\set{|X\cap \tilde\Gamma|,|Y\cap \tilde\Gamma|}$, a contradiction (we have used the fact that $\mu=512\Delta \alphasc(n)\log_{3/2} n$ and $\alpha'=\frac{1}{16\alphasc(n)\log_{3/2} n}$).
\end{proof}

\paragraph{Step 3: Constructing the type-$2$ acceptable cluster.}
Consider the block $B_0\in \lset(Z_0)$ given by Lemma \ref{lemma: find the right block}. We will gradually construct a cluster $C^*$ and a set $A_{C^*}$ of fake edges, such that eventually $C^*$ will become $\tilde B_0$ and $A_{C^*}$ will be precisely the set of all fake edges of $B_0$.
We will also compute an embedding of edges in $A_{C^*}$ into type-1 acceptable clusters in $\cset_1^I$. Additionally, we will also add some additional edges to $\hat E$, while ensuring that, once these edges are deleted from $C$, we obtain a collection of connected components, where all components other than $C^*$ are type-1 acceptable clusters.
%We denote $\nset(B)=\set{B^C,\ldots,B_1,\ldots,B_r}$, where $B_1,\ldots,B_r$ are child blocks of $B$. For each $1\leq i\leq r$, we denote by $x_i,y_i$ the endpoints of the block $B_i$, and we denote the endpoints of $B$ by $(x,y)$. We process the blocks in 

We start by processing the blocks in $\nset(B_0)$ one-by-one. We now describe a round in which a block $B'\in \nset(B_0)$ is processed.
Denote by $x',y'$ the endpoints of $B'$. First, we add to $\hat E$ all edges of $B'$ that are incident to $x'$ or $y'$. 
%Denote by $E^*$ the set of such edges.
Consider now the connected components of $C$ we remove these edges from it. Let $C'$ be the unique component containing the vertices of $\tilde B_0$, and let $\cset'$ be the set of remaining components. Observe that every component of $\cset'$ only contains terminals that were owned by $B'$, and the number of such terminals is at most $\mu/2$. Additionally, we have created at most $2\Delta$ new terminals by removing these $\set{x',y'}$-incident edges. Since $\mu\geq 8\Delta$, every connected component of $\cset'$ contains at most $\mu$ terminals. We then add all connected components of $\cset'$ to the set $\cset^I_1$ of type-1 acceptable clusters. Additionally, if the edge $(x',y')$ does not belong to $C'$, then we add a fake edge $e=(x',y')$ to the set $A$, and we let its embedding $P(e)$ be any path connecting $x'$ to $y'$ in $B'$. Notice that some connected component of $\cset'$ must contain the sub-path $P(e)\setminus\set{x',y'}$; we designate that component as $C(e)$.
We update $C$ to be $C'\cup e$ if the edge $(x',y')$ does not belong to $C'$, otherwise we update it to be $C'$.

Once every pseudo-block $B'\in \nset(B)$ is processed in this way, we consider every vertex $u_i\in U^*$ that lies in $B_0$ one-by-one. For each such vertex $u_i$, we add to $\hat E$ all edges that are incident to $u_i$, whose other endpoint lies in $X_i$. Consider the connected components of $C$ after these edges are removed from it. As before, we denote by $C'$ the unique component containing the vertices of $\tilde B_0$, and by $\cset'$ the set of remaining components. For every component $\hat C\in \cset'$, $V(\hat C)\subseteq X_i$, and so $\hat C$ originally contained at most $\mu/2$ terminals. We may have created at most $\Delta$ new terminals by removing these $u_i$-incident edges, so the total number of terminals in each such component $\hat C$ is at most $\mu/2+\Delta\leq \mu$. We add every cluster $\hat C\in \cset'$ to $\cset^I_1$.

Consider now the final cluster $C^*$ that we obtained after processing each block $B'\in \nset(B_0)$ and every vertex $u_i\in U^*\cap V(B_0)$. It is clear that $C^*=\tilde B_0$, so $C^*$ is either a simple $3$-connected graph or isomorphic to $K_3$. We have also defined a set $A_{C^*}=E(C^*)\cap A$ of fake edges for $C^*$, and for every edge $e=(x,y)\in A_{C^*}$, an embedding $P(e)$ of $e$, and a distinct type-$1$ acceptable cluster $C^*(e)$ that was just added to $\cset^I_1$, such that $P(e)\setminus\set{x,y}\subseteq C^*(e)$.
% We need to do one last step to ensure that $C$ is a type-2 acceptable cluster. Let $\bset$ be the block decomposition of the graph $H=G\setminus E_1$. Let $B\in \bset$ be the block with $V(\tilde B_0) \subseteq V(\tilde B)$ given by Lemma \ref{lem: block containment}. Recall that Theorem \ref{thm: getting good pseudoblocks} guarantees that $B$ is a good block. Let $(x,y)$ be the endpoints of block $B$. If the edge $(x,y)$ belongs to $E(C)\setminus A_C$, then we add this edge to the set $\hat E$ of deleted edges, and to the set $A$ of fake edges (in other words, this edge becomes a fake edge).  The embedding of the new fake edge $e$ is $P(e)=(x,y)$.
We prove the following claim.
\begin{claim}\label{lemma: resulting cluster is acceptable} Cluster $C^*$ is a type-2 acceptable cluster.
\end{claim}
We provide the proof of Claim~\ref{lemma: resulting cluster is acceptable} in the following subsection, 
after we complete the proof of Theorem~\ref{thm: can find edge set w acceptable clusters} using it in the remainder of this subsection. Note that it suffices to show that the total budget of all vertices does not increase after cluster $C$ is processed.

%\vspace{-4mm}
\paragraph{Accounting.}
%It now remains to show that the total budget of all vertices does not increase. 
%We can assume that algorithm $\algsc$ returns a cut of sparsity at least $\alpha'\cdot \alphasc(n)$ when it is applied to cluster $C$.
Let $\Gamma_{o}$ be the set of all old terminals that belonged to the cluster $C$ before we process it, and let $\Gamma_{n}$ be the set of all new terminals that emerged over the course of processing $C$. We further partition $\Gamma_{n}$ into two sets: set $\Gamma_{n}'$ contains all terminals lying in $V(C^*)$, and set $\Gamma_{n}''$ contains all remaining new terminals. Note that each terminal in $\Gamma_{n}''$ must be connected to a terminal in $\Gamma_{n}'\cup \Gamma_{o}$ by an edge, so $|\Gamma_{n}''|\leq \Delta\cdot (|\Gamma_{n}'|+|\Gamma_{o}|)$.
For any new terminal $t\in \Gamma_{n}'$, either $t\in U^*\cap V(B_0)$, or there is some block $B'\in \nset(B_0)$ that contains $t$ as an endpoint. Therefore, $|\Gamma_{n}'|\le |U^*\cap V(B_0)|+2|\nset(B_0)|$. However, since graph $G$ is $3$-connected, for every vertex $u_i\in U^*$, at least one vertex of $X_i\setminus\set{u_i}$ must be a terminal of $\Gamma'$ (since vertex $u_i$ is a $1$-separator for $X_i\setminus\set{u_i}$). Similarly, for every block $B'\in \nset(B_0)$ with endpoints $x'$ and $y'$, if no vertex of $U^*$ lies in $B'\setminus \set{x',y'}$, then some vertex of $V(B')\setminus \set{x',y'}$ must lie in $\Gamma_{o}$. Otherwise, there must be some vertex $u_i\in U^*\cap  (V(B')\setminus \set{x',y'})$, such that some vertex of $X_i\setminus \set{u_i}$ belongs to $\Gamma_{o}$. Therefore, $|\Gamma_{n}'|\leq 2|\Gamma_{o}|$, and $|\Gamma_{n}|\leq (\Delta+1)\cdot (|\Gamma_{n}'|+|\Gamma_{o}'|)\leq 4\Delta|\Gamma_{o}|$.

After we finish processing $C$, every vertex of $C^*$ lies in an inactive cluster, so every terminal in $\Gamma_{n}\cup  \Gamma_{o}$ has budget $1$, and the total budget of these vertices is therefore at most $5\Delta|\Gamma_{o}|$. On the other hand, before we process $C$, each terminal of $\Gamma_{o}$ had budget $8\Delta\cdot \log_{3/2}|\Gamma_{o}|\geq 8\Delta$. Therefore, the total budget of all vertices does not increase.
We can therefore conclude that the total budget of all vertices does not increase over the course of the algorithm, and so the number of terminals is always bounded by $O(|E_1|\Delta\log n)=O((|E'|+\optcro(G))\cdot \poly(\Delta\log n))$. The algorithm terminates when there are no more active clusters. We are then guaranteed that every cluster $C\in \cset^I_1$ is a type-1 acceptable cluster. For every fake edge $e=(x,y)\in A$, we have defined an embedding $P(e)$ of $e$, and a type-1 acceptable cluster $C(e)\in \cset^I_1$ with $P(e)\setminus\set{x,y}\subseteq C(e)$. Moreover, for every pair $e,e'\in A$ of edges, $C(e)\neq C(e')$.  Therefore, in order to complete the proof of Theorem \ref{thm: can find edge set w acceptable clusters}, it is now sufficient to prove Claim~\ref{lemma: resulting cluster is acceptable}.


%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
\fi

%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
\iffalse
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
\subsection{Proof of Claim~\ref{lemma: resulting cluster is acceptable}}
In this subsection we provide the proof of Claim~\ref{lemma: resulting cluster is acceptable}.
First, it is immediate that $C^*=\tilde B_0$. Therefore, $C^*$ is either a simple $3$-connected graph or is isomorphic to $K_3$. We then prove the following claim.
%-------------------------------
%-------------------------------
%-------------------------------		
\begin{claim}\label{claim: well linkedness of new terminals}
The set $\hGamma \cap V(C^*)$ of terminals is $\alpha$-well-linked in $C^*$.
\end{claim}
%-------------------------------
%-------------------------------
%-------------------------------
%-------------------------------
%-------------------------------
%-------------------------------	
\begin{proof}
We denote by $\Gamma'$ the original set of terminals in $C$ before it is processed, and denote by $\Gamma''$ the set of all terminals that belong to $V(C^*)$ after cluster $C$ is processed. %For convenience, we also denote $G'=C^*\cup A$.
Consider any partition $(X,Y)$ of $V(C^*)$. Denote $\Gamma_X=\Gamma''\cap X$ and $\Gamma_Y=\Gamma''\cap Y$. %, and assume w.l.o.g. that $|\Gamma_X|\leq |\Gamma_Y|$. 
We will show that $|E_{C}(X,Y)|\geq \alpha\cdot \min\set{|\Gamma_X|,|\Gamma_Y|}$.

Recall that, in addition to the terminals of $\Gamma'\cap V(C^*)$, the new set $\Gamma''$ of terminals also contains endpoints of all blocks in $\nset(B_0)$ and vertices of $U^*\cap V(C^*)$. We call such terminals \emph{new terminals}.
%(a new terminal cannot belong to $\Gamma'$)
We further partition sets $\Gamma_X$ and $\Gamma_Y$ as follows.
We let $\Gamma^1_X\subseteq \Gamma_X$ contains all terminals $t$, such that there is some block $B'\in \nset(B_0)$ with $t$ being one of its endpoints, and the other endpoint $t'$ of $B'$ lies in a different set in $\set{X,Y}$ than $t$ (so if $t\in X$, $t'\in Y$ and vice versa). And we let $\Gamma^2_X=\Gamma_X\setminus \Gamma^1_X$.
The partition $(\Gamma^1_Y,\Gamma^2_Y)$ is defined similarly. Observe that a new terminal may be an endpoint of more than one block in $\nset(B_0)$, and it may be also a vertex of $U^*$ (or both). Since the endpoints of every block in $\nset(B_0)$ are connected by a fake edge in $C$, it is immediate to verify that
\begin{equation}
|E_{C}(X,Y)|\geq |\Gamma^1_X|\mbox{  and  } |E_{C}(X,Y)|\geq |\Gamma^1_Y|. 
\label{eq: cut comparable to type 1 terminals}
\end{equation}
Next, we construct a cut $(X',Y')$ in graph $C$ based on the cut $(X,Y)$ of $C^*$, and then use the well-linkedness of the terminals in $\Gamma'$ in graph $C$ to obtain a better lower bound of $|E_{C}(X,Y)|$. We start with $X'=X$ and $Y'=Y$. Take any block $B'\in \nset(B_0)$ with endpoints $(x',y')$. We define the set $S(B')$ of vertices to be the union of (i) $V(B')\setminus \set{x',y'}$; and (ii) all sets $X_i$ whose corresponding separator vertex $u_i\in U^*$ lies in $V(B')\setminus\set{x',y'}$. Note that the endpoints $x',y'$ of $B'$ are terminals in $\Gamma''$ but they may not have been terminals in $\Gamma'$. However, since we have assumed that graph $G$ is $3$-connected, set $S(B')\setminus \set{x',y'}$ must contain a terminal that belongs to $\Gamma'$. We denote this terminal by $t_{B'}$, and we will view this terminal as ``paying'' for $x'$ and $y'$ (if $x,y\in \Gamma^2_X\cup \Gamma^2_X$).
If both $x',y'\in X$, then we add all vertices of $S(B')$ to $X$, otherwise we add them to $Y$. Notice that, if both $x',y'$ lie in the same set in $\set{X,Y}$, then we do not increase the number of edges in the cut $(X,Y)$. 
%Moreover, we can think of replacing the new terminals $x',y'$ with a terminal $t_{B'}\in \Gamma'\setminus \Gamma''$. 
Assume now that $x'\in X$ and $y'\in Y$ (the other case is symmetric). Note also that $x',y'$ must be type-1 new terminals. In this case, we have increased the number of edges in the cut $(X,Y)$ by at most $\Delta$, by adding all edges that are incident to $x'$ to this cut. \znote{what do we do specifically in this case?} Note however that the edge $(x',y')$ already belonged to this cut (possibly as a fake edge), so we charge this increase in the cut size to this fake edge. 

Once every block $B'\in \nset(B_0)$ is processed, we perform one last modification to the cut: for every vertex $u_i\in V(C^*)$, if $u_i\in X$, then we add all vertices of $X_i$ to $X$, otherwise we add them to $Y$. This step does not increase the number of edges in the cut $(X,Y)$. Observe that $u_i$ may be a new terminal. However, since graph $G$ is $3$-connected, set $X_i$ must contain a terminal, that we denote by $t_i$, and we view this terminal as ``paying'' for the terminal $u_i$.
We now obtain a cut $(X',Y')$ in graph $C$. From the above discussion:
\begin{equation}
|E_{C}(X',Y')|\leq \Delta\cdot |E_{C^*}(X,Y)|.\label{eq: few new edges in cut}
\end{equation}
Consider now the terminals of $\Gamma_X$. Clearly $\Gamma_X\cap \Gamma'\subseteq X'$. For each terminal in $\Gamma^2_X$, we have added a terminal of $\Gamma'$ to $X'$ that pays for it, while each newly added terminal of $X'\cap \Gamma'$ pays for at most two terminals in $\Gamma^2_X$. Therefore, $|\Gamma^2_X|\leq 2|\Gamma'\cap X'|$, and similarly $|\Gamma^2_Y|\leq 2|\Gamma'\cap Y'|$. Since the set $\Gamma'$ of terminals was $\alpha'$-well-linked in $C$,
$|E_{C}(X',Y')|\geq \alpha'\cdot\min\set{|\Gamma'\cap X'|,|\Gamma'\cap Y'|}\geq (\alpha'/2) \min\set{|\Gamma^2_X|,|\Gamma^2_Y|}$.
Combining this with Equation \ref{eq: few new edges in cut}, we have $|E_{C^*}(X,Y)| \geq \frac{\alpha'}{2\Delta}\cdot \min\set{|\Gamma^2_X|,|\Gamma^2_Y|}$.
Combining this with Equation \ref{eq: cut comparable to type 1 terminals}, and using $\alpha'=8\Delta\alpha$, we have $|E_{C^*}(X,Y)| \geq \frac{\alpha'}{4\Delta}\cdot\min\set{|\Gamma_X|,|\Gamma_Y|}\geq \alpha \cdot\min\set{|\Gamma_X|,|\Gamma_Y|}$.
This completes the proof of Claim~\ref{claim: well linkedness of new terminals}.
\end{proof}
%-------------------------------
%-------------------------------
%-------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
\fi
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------

\iffalse
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
---------Old Stuff------------------

Recall that graph $C^*$ is either a simple $3$-connected graph, or it is a $K_3$. Therefore, $C^*$ has a unique planar drawing, that we denote by $\rho$. This drawing induces a planar drawing of $C^*\setminus A$, that we denote by $\rho'$. 
It now remains to prove the following claim, that will conclude the proof of Lemma \ref{lemma: resulting cluster is acceptable}.
\begin{claim}\label{claim: good cluster}
For every bridge $R\in \rset_G(C^*\setminus A)$, there is a face $F$ in the drawing $\rho'$, such that the set $L(R)$ of vertices lie on the boundary of $F$.
\end{claim}
\begin{proof}
The proof of the claim is almost identical to the proof of Claim \ref{claim: every block is good}. \znote{so do we keep them both?}
Throughout the proof, we denote by $E_2$ the set $\hat E$ of edges obtained after cluster $C$ is processed. 
Denote $H_1=G\setminus E_1$ and $H_2=G\setminus E_2$, so $H_2\subseteq H_1$.
Recall that $\bset(H_1)$ is block decomposition of the graph $H_1$. 
Let $B\in \bset(H_1)$ be the pseudo-block corresponding to $B_0$, given by Lemma \ref{lem: block containment}, and let $(x,y)$ its endpoints. Therefore, $V(\tilde B_0)\subseteq V(\tilde B)$, every real edge of $\tilde B_0$ (except for possibly $(x,y)$) belongs to $\tilde B$ as a real edge, and for every fake edge $e\in E(\tilde B_0)$, there is a path $P(e)$ in $\tilde B$ connecting its endpoints, that is internally disjoint from $\tilde B_0$. Moreover, the paths in $\pset=\set{P(e)\mid e\in A_{B_0}}$ are mutually internally disjoint. Recall that $\tilde B_0=C^*$ and $A_{B_0}= A_{C^*}$. Therefore, $V(C^*)\subseteq V(\tilde B)$, every real edge of $C^*$ is a real edge of $\tilde B$ (except for possibly $(x,y)$), and set $\pset$ contains an embedding of every edge of $A_{C^*}$. Notice that $B\in \bset'$ must hold, since otherwise all vertices of $B$ lie in the clusters of $\cset'_1$, which is impossible since these clusters were inactive throughout the algorithm.

	
Assume for contradiction that the claim is false, and let $R\in \rset_G(C^*\setminus A)$ be a bridge such that not all vertices of $L(R)$ lie on the boundary of a single face of the drawing $\rho'$ of $C^*\setminus A$.
%	Let $R\in \rset_G(\tilde B_0)$ be a witness for $B_0$.
%Let $B\in \bset_H$ be the corresponding block given by Lemma \ref{lem: block containment}.
Consider the unique planar drawing $\rho_{\tilde B}$ of $\tilde B$. Since every vertex and every real edge of $C^*$ (except for possibly $(x,y)$) lie in $\tilde B$, and $\tilde B$ contains a fake edge $(x,y)$, this drawing naturally induces a drawing of $C^*\setminus A_{C^*}$.
%(we map the real edge $(x,y)$ of $C^*$ to the image of the fake edge $(x,y)$ in $\tilde B$)
For convenience, we denote by $\rho''$ the drawing of $C^*\setminus A_{C^*}$ induced by $\rho_{\tilde B}$. We prove the following claim.

\begin{claim}\label{claim: identical drawings}
	The drawings $\rho'$ and $\rho''$ of $C^*$ are identical. %\snote{$\rho''$ is not defined}
\end{claim}
\begin{proof}
%	Let $A$ be the set of all fake edges of $\tilde B_0$, so that $\tilde B_0_z=\tilde B_0\setminus A$.
Consider the drawing $\rho''$ of $C^*\setminus A_{C^*}$. We will show that we can augment this drawing by adding drawings of the edges in $A_{C^*}$, so that the resulting drawing remains planar. Note that, if this is true, then it follows that $\rho'=\rho''$. Indeed, recall that $C^*=\tilde B_0$ has a unique planar drawing. Therefore the resulting planar drawing of $\tilde B_0$ that we obtain from $\rho''$ is identical to $\rho_{\tilde B_0}$. Therefore, both $\rho'$ and $\rho''$ are obtained from the drawing $\rho_{\tilde B_0}$ of $\tilde B_0$ by deleting the images of the fake edges from $A_{C^*}$ from it. It follows that $\rho'=\rho''$.

It suffices to show that we can augment the drawing $\rho''$ by adding the images of edges in $A_{C^*}$ to it, while preserving the planarity. Recall that Lemma \ref{lem: block containment} defines, for every fake edge $e=(u,v)\in  A_{C^*}$, a path $Q(e)$ in $\tilde B$ that connects $u$ to $v$, and is internally disjoint from $V(\tilde B_0)$. Moreover, if $e$ and $e'$ are distinct fake edges in $A_{C^*}$, then their corresponding paths $Q(e)$ and $Q(e')$ are internally disjoint.  Recall that these paths are allowed to contain fake edges of $\tilde B$, and that, if graph $\tilde B_0$ contains a real edge $(x,y)$, then the resulting paths in $\set{Q(e)\mid e\in A_{C^*}}$ do not contain an edge $(x,y)$. Therefore, we can simply map every fake edge $e\in A_{C^*}$ to the curve $\gamma(Q(e))$ that represents the drawing of the path $Q(e)$ in $\rho_{\tilde B}$. Curve $\gamma(Q(e))$ is obtained by concatenating the images of the edges of $Q(e)$ in $\rho_{\tilde B}$. Since the drawing $\rho_{\tilde B}$ of $\tilde B$ is planar, we obtain a planar drawing of $\tilde B_0$. %\mynote{It may be good to replace these $P(e)$s with $Q(e)$ so they don't clash with the embeddings that we defined before}
	%
	%Lastly, if edge $e^*(x,y)$ belongs to $\tilde B_0$ as a real edge, then it does not belong to $C^*$, but it lies in the set $A$ of fake edges. We need to add the image of this edge to our drawing. Recall that $(x,y)$ are the endpoints of the block $B$, and so the edge $e^*$ belongs to $B$ either as a real or a fake edge. Recall that in this case, Lemma \ref{lem: block containment} guarantees that the paths in $\set{P(e)\mid e\in A\setminus\set{e^*}}$ do not contain the edge $(x,y)$. Therefore, we can let $P(e^*)=(x,y)$, embedding the edge $e^*$ into the edge $(x,y)$ in $\tilde B$. We then draw the edge $e^*$ along the image of the edge $(x,y)$ in drawing $\rho_{\tilde B}$ of $\tilde B$.
\end{proof}


Let $\fset$ be the set of all faces of the drawing $\rho'=\rho''$. 
For every vertex $v\in V(\tilde B)\setminus V(C^*)$, there is a unique face $F(v)\in \fset$, such that the image of vertex $v$ in $\rho_{\tilde B}$ lies in the interior of the face $F$.
%\mynote{should we define $T_R$ here? Do we need it to have smallest number of edges, or is it enough that it is some tree spanning $L(R)$? (note that $R$ is no longer a bridge of a block, it's a bridge of $C^*$).}
Recall that $T_R$ is a tree in $R$ whose leaves are vertices of $L(R)$. 
Assume first that $V(T_R)\cap V(\tilde B)=L(R)$. In this case, there is some bridge $R'\in \rset_G(\tilde B')$ of $\tilde B'$ that contains the tree $T_R$, and so $L(R)\subseteq L(R')$. Since $B$ is a good pseudo-block, there must be a face in the drawing $\rho'_{\tilde B'}$ whose boundary contains all vertices of $L(R)$. Therefore, for some face $F\in \fset$, all vertices of $L(R)$ must lie on the boundary of $F$. 
Assume now that there is some vertex $v\in V(T_R)\cap  V(\tilde B)$ that does not lie in $L(R)$. Let $F(v)$ be the face of $\fset$ whose interior contain the image of $v$ in $\rho_{\tilde B}$ (recall that $v\not\in V(C^*)$, so it may not lie on a boundary of a face in $\fset$). We will show that all vertices of $L(R)$ must lie on the boundary of $F(v)$, leading to a contradiction. Let $u$ be an arbitrary vertex of $L(R)$. It suffices to show that $u$ must lie on the boundary of the face $F(v)$.
Let $P\subseteq T_R$ be the unique path connecting $v$ to $u$ in $T_R$. 
%Since the leaves of tree $T_R$ are vertices of $L(R)$, except for $v$, every vertex $x$ of $P$ lies outside $V(C^*)$, and the image of $x$ in $\rho_{\tilde B}$ lies in the interior of some face in $\fset$. 
Let $v=v_1,v_2,\ldots,v_r=u$ be all vertices of $P$ that belong to $V(\tilde B)$, and assume that they appear on $P$ in this order. 
It remains to prove the following observation.

\begin{observation}
$F(v_1)=F(v_2)=\cdots=F(v_r)$. Moreover, $v_r$ lies on the boundary of $F(v_{r-1})$.
\end{observation}
\begin{proof}
Fix some $1\leq i\leq r-1$. Assume that the observation is false.
Then there is some face $F'\in \fset$, such that $v_i$ lies in the interior of $F'$, but $v_{i+1}$ does not lie in the interior or on the boundary of $F'$ (the latter case is only relevant for $i=r-1$). Since the boundary of $F'$ separates $v_i$ from $v_{i+1}$, these two vertices cannot lie on the boundary of the same face in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$. 
	
Let $\sigma_i$ be the subpath of $P$ between $v_i$ and $v_{i+1}$. If $\sigma_i$ consists of a single edge connecting $v_i$ and $v_{i+1}$, then either it is a bridge in $\rset_G(\tilde B')$, or it is an edge of $\tilde B'$. In either case, the endpoints of $\sigma_i$ must lie on the boundary of a single face of the drawing $\rho'_{\tilde B'}$, a contradiction (we have used the fact that $B$ is a good block and that $\tilde B'$ is a planar graph). Otherwise, let $\sigma'_i$ be obtained from $\sigma_i$ by deleting the two endpoints from it. Then there must be a bridge $R'\in \rset_G(\tilde B')$ containing $\sigma'_i$, with $v_{i},v_{i+1}\in L(R')$. But then, since $B$ is a good pseudo-block, there must be a face in the drawing $\rho_{\tilde B}$ of $\tilde B$, whose boundary contains $v_i$ and $v_{i+1}$, leading to a contradiction. 
	%	We conclude that for all $1\leq i<r$, there must be a face $F_i$ in the drawing $\rho'_{\tilde B'}$ of $\tilde B'$ such that $v_i,v_{i+1}$ lie on the boundary of $F_i$. Notice that, since $\tilde B_0_z\subseteq \tilde B'$, and from the way the drawing $\rho'_{\tilde B_0_z}$ was defined, there must be a face $F'_i$ of $\rho'_{\tilde B_0_z}$ that contains $F_i$.	
\end{proof}
\end{proof}

%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------
\fi
%---------------------------------
%---------------------------------
%---------------------------------\\
%---------------------------------
%---------------------------------



\iffalse

Finally, we are ready to define acceptable clusters.


\begin{definition}
	A cluster $C\in \cset$ is called \emph{acceptable} iff it is good, and additionally one of the following two properties hold:
	
	\begin{itemize}
		\item either $C$ is $3$-connected, and the vertices of $T\cap V(C)$ are $\alpha$-well-linked in $C$, for $\alpha=1/\poly\log n$ (in which case $C$ is a type-1 acceptable cluster); or
		
		\item $C$ contains at most $O(\Delta \poly\log n)$ terminals, where $\Delta$ is maximum vertex degree in $G$ (in which case $C$ is a type-2 acceptable cluster).
	\end{itemize}
\end{definition}


\fi





==> crossing_number_with_rotation_system.tex <==
\section{Crossing Number with Rotation System}
\label{sec:cr_rotation_system}

In this section we provide the proof of Theorem~\ref{thm: main_rot}.
We denote by $\tG$ the input graph and by $\tSigma$ the input rotation system on $\tG$. We let $\tphi$ be some fixed optimal drawing of $\tG$ that respects $\tSigma$. 
%We are guaranteed that $|E(\tG)|\le o(\cro(\tphi)^{1+\eps/2})$. 
%We will compute a drawing of $\tG$ respecting $\tSigma$ with relatively few crossings. 
Throughout this section, we denote $\cro=\cro(\tphi)$ and fix $\eps=1/22$.


We start with a high-level overview of the algorithm. 
The algorithm is recursive, and the idea is to recursively decompose the graph $\tG$ into smaller subgraphs by removing a set of vertices and edges, compute a drawing of each subgraph, combine the drawings of the subgraphs and then add back the deleted edges to the drawing. 
Specifically, if the maximum vertex degree of $\tG$ is at most $\cro^{1-\eps}$, then we can use the algorithm in~\cite{shahrokhi1994book} to compute a drawing of $\tG$ with $\tilde O(\cro+\cro^{1-\eps}\cdot|E(\tG)|)$ crossings. 
Now we assume the maximum vertex degree of $\tG$ is greater than $\cro^{1-\eps}$, and our goal is to decompose $\tG$ into subgraphs with maximum degree bounded by $\cro^{1-\eps}$, and then use the algorithm in~\cite{shahrokhi1994book} to compute a drawing of each of the subgraphs.
Let $v\in V(\tG)$ be a vertex of $\tG$ with degree at least $\cro^{1-\eps}$.
We denote by $e_1,\ldots,e_r$ the edges incident to $v$ that are ordered according to the rotation system $\tSigma$.
Denote $E_1=\set{e_1,\ldots,e_{\floor{r/2}}}$ and $E_2=\set{e_{\floor{r/2}+1},\ldots,e_{r}}$. 
We first split the vertex $v$ by replacing $v$ with two vertices, $v',v''$, where $v'$ is incident to all edges in $E_1$, and $v''$ is incident to all edges in $E_2$. Then we compute the minimum edge-cut in $\tG$ separating $v'$ from $v''$.
If the size of this min-cut is small, then we delete all edges in the cut and recurse on both sides. If the size of this min-cut is large, from Menger's Theorem, we obtain a set of edge-disjoint paths connecting the edges of $E_1$ to the edges of $E_2$.
We show that, we can efficiently find a constant number of these paths, that we call a \emph{skeleton}, such that (i) the drawing of these paths induced by $\tphi$ does not cross each other; (ii) each of the paths participate in few crossings in $\tphi$; and (iii) the ``region'' in $\tphi$ surrounded by these paths are ``touched'' by few other edges.
We then use the skeleton to compute a decomposition of $\tG$ into subgraphs, and recurse on each of them.

We start with some notations and definitions, and then we will describe the algorithm in detail in the following sections.


\subsection{Rotation Systems}

\input{RS_prelim}

\iffalse
\subsection{A Subroutine}

\input{RS_decomposition}
\fi


%\input{RS_non_interfering}

%\input{RS_flipstatus}

\subsection{The Algorithm}
Recall that we are given an input graph $\tG$ and a rotation system $\tSigma$ on $\tG$, and we will compute a drawing in $\Phi(\tG,\tSigma)$ with $\tilde O(\cro+\cro^{1-\eps}\cdot|E(\tG)|)$ crossings. 
%In this section, for a graph $G$ and an integer $k>0$, we denote by $V_{k}(G)$ the set of all vertices of $G$ with degree at least $k$ in $G$.


The algorithm is recursive and the depth of the recursion will be bounded by $O(\cro^{2\eps})$. 
%Throughout the algorithm, we maintain a set $E^*$ of \emph{discarded edges}, that is initialized to be $\emptyset$. As the algorithm proceeds, we will gradually add edges to $E^*$. Let $\hat{E}^*$ be the final status of $E^*$. We will compute a drawing of $\tG'\setminus \hat E^*$, and add the edges in $\hat E^*$ back to the drawing, to eventually obtain a drawing of $\tG'$.
Over the course of the algorithm, we will define some new sub-instances.
Each sub-instance $G'$ that we construct can be obtained by taking some subgraph of $\tG$, and then contracting some of its edges. Therefore, each edge of $G'$ corresponds to some edge of $\tG$. %Instances that lie in the same recursive level will be disjoint in their edges. 
For each instance $G'$, we will define a set $\hat E(G')\subseteq E(G')$ of \emph{difficult edges}.
%We ensure that, for each instance $G'$ that we construct, $|\hat{E}(G')|=\tilde O(\cro^{7\eps})$.
%If $G'$ is in the $i$th recursive level, then we will ensure that $|\hat E(G')|\leq i\cro^{1/3+\eps}$.
We will also associate, for each instance $G'$, with a drawing $\phi'_{G'}\in \Phi(G',\Sigma)$ that satisfies the following property: if a pair $e,e'$ of edges in $E(G')$ cross in $\phi'_{G'}$, then either $e,e'$ cross in the optimal drawing $\tphi$, or at least one of $\set{e,e'}$ belongs to $\hat{E}(G')$. Note that, the set of difficult edges and the associated drawing are not known to the algorithm and are only for the sake of analysis. 

We now begin to describe the algorithm.
The algorithm starts with a single graph $\tG$, with the set $\hat E(\tG)$ of difficult edges set to be $\emptyset$, and the associated drawing $\phi'_{\tG}$ set to be $\tphi$.
We will first describe the recursion base and the way to process it, and then describe a step in the recursion, in the following subsections.
%
%
%
%
%
\subsubsection{Recursion base: subgraphs with no vertices of degree above $\cro^{1-\eps}$}
Suppose that the current graph $G'$ contains no vertices of degree greater than $\cro^{1-\eps}$. We will show that we can efficiently find a drawing of $G'$ with relatively few crossings.
We use the following theorem from~\cite{shahrokhi1994book} and its corollary.
\begin{lemma}[Theorem 4.2 in \cite{shahrokhi1994book}]
\label{lem:cr_potential}
There is an efficient algorithm, that, given a simple graph $G$, finds a drawing of $G$ with $\tilde{O}(\optcro(G)+\sum_{v\in V}\deg^2_G(v))$ crossings. %Moreover, in the drawing, all vertices of $G$ are drawn on a line and all edges are drawn in the same halfspace with respect to the line.
\end{lemma}
\begin{corollary}
\label{cor:base}
There is an efficient algorithm, that, given a simple graph $G$ and a rotation system $\Sigma$ on $G$, finds a drawing of $G$ in $\Phi(G,\Sigma)$ with $\tilde O(\optcro(G)+\Delta\cdot |E(G)|)$ crossings.
\end{corollary}
\vspace{-4mm}
\begin{proof} 
Let $\psi$ be the drawing obtained by applying Lemma~\ref{lem:cr_potential} to $G$, so $\cro(\psi)=\tilde{O}(\optcro(G)+\sum_{v\in V}\deg^2_{G}(v))$.
Note that $\sum_{v\in V}\deg^2_{G}(v)\le \Delta\cdot\sum_{v\in V}\deg_{G}(v)\le O(\Delta|E(G)|)$. Therefore, we have $\cro(\psi)=\tilde O(\optcro(G)+\Delta|E(G)|)$.
We apply Lemma~\ref{lem:drawing_local_reodering} to graph $G$, drawing $\psi$, and rotation system $\Sigma$.
Let $\psi'$ be the drawing we get, so $\psi'\in \Phi(G,\Sigma)$.
Moreover, from Lemma~\ref{lem:drawing_local_reodering},
$\cro(\psi')\le\cro(\psi)+\sum_{v\in V}\deg^2_G(v)=\tilde O(\optcro(G)+\Delta|E(G)|)$.
Therefore, we efficiently find a drawing in $\Phi(G,\Sigma)$ with $\tilde O(\optcro(G)+\Delta |E(G)|)$ crossings.
\end{proof}

It follows from Corollary~\ref{cor:base} that we can efficiently find a drawing of $G'$ in $\Phi(G',\Sigma)$ with at most $\tilde O(\optcro(G')+\cro^{1-\eps}\cdot |E(G')|)$ crossings.



\input{RS_recursion}

\input{accounting}

























































%In previous steps, we have decomposed the input graph $\tG$ into a set $\gset=\set{G_1,\ldots,G_k}$ of instances, where each of them is in base case, and computed a drawing for each instance in $\gset$. In this step we first combine all the drawings together, and then add back the discarded edges in $E^*$. We use the following lemma.

%\begin{lemma}
%\label{lem:add_back_discarded_edges}
%Let $G=(V,E)$ be a graph, let $E'\subseteq E$ be a subset of its edges, let $\Sigma$ be a rotation system on $G$, and let $\phi'$ be any drawing of the subgraph $G\setminus E'$ in the plane such that $\phi'$ respects the rotation system $\Sigma$, and every pair of edges in $E\setminus E'$ crosses at most once in $\phi'$. Then we can efficiently find a drawing $\phi$ of $G$ in the plane, such that (i) $\phi(G\setminus E')=\phi'$; (ii) $\phi$ respects the rotation system $\Sigma$; and (iii) $\cro(\phi)\le \cro(\phi')+|E'|\cdot|E(G)|$.
%\end{lemma}

\iffalse
Note that, if an instance constructed in our algorithm contains at most $\cro^{1-\eps}$ edges, then it has to be a base-case instance. Also note that, the instances constructed in the algorithm is disjoint in their edges.
Therefore, the number of base-case instances is at most $O(\cro^{\eps})$, and the number of levels in our recursion is also at most $O(\cro^{\eps})$.
Since in each round of recursion, the number of new bad edges is at most $O(\cro^{6\eps})$, the total of bad edges in all instances of $\gset$ is at most $O(\cro^{7\eps})$.
We use the following observations.
\begin{observation}
$|E^*|=\tilde{O}(|E(\tG)|/\cro^{\eps})=\tilde{O}(\cro^{1-\eps})$.
\end{observation}
\begin{observation}
$\sum_{1\le i\le k}\optcro(G_i)=\tilde O(\cro^{7\eps}\cdot |E(\tG)|)$.
\end{observation}
\begin{proof}
\end{proof}
\begin{observation}
$\sum_{1\le i\le k}\cro(\psi_{G_i})=\tilde O(\cro^{7\eps}\cdot |E(\tG)|)+\tilde O(\cro^{1-\eps}\cdot |E(\tG)|)\le \tilde{O}(\cro^{2-\eps})$.
\end{observation}
\begin{proof}
\end{proof}
\fi


\iffalse
Assume in some round of the recursion, the instance $G$ is decomposed into two sub-instances $G_1$ and $G_2$. 
We now describe how to compose their drawings $\psi_{G_1}$ and $\psi_{G_2}$ to obtain the drawing $\psi_G$. We distinguish between the following $3$ cases of how the sub-instances $G_1$ and $G_2$ are obtained from $G$.


\textbf{Case 1. Removing a small cut.} In this case $G_1$ and $G_2$ are not only disjoint in their edges, but also disjoint in their vertices. We simply place $\psi_{G_1}$ and $\psi_{G_2}$ together in the plane without crossing each other. Let $\psi_{G}$ be the resulting drawing. It is clear that $\cro(\phi_G)\le \cro(\psi_{G_1})+\cro(\psi_{G_2})$.


\textbf{Case 2. Splitting a high-degree vertex and removing a small cut.} In this case $G_1$ and $G_2$ are disjoint in their edges, but $V(G_1)\cap V(G_2)=\set{v}$. 
We first perform a stereographic projection from $v$ and obtain new drawings $\psi'_{G_1}$ and $\psi'_{G_2}$, where $v$ lies on the outer face, and the corresponding rotation systems are still respected. 
We simply place $\psi'_{G_1}$ and $\psi'_{G_2}$ together in the plane by sticking the image of $v$ in both drawings, without creating new crossings. 
Let $\psi_{G}$ be the resulting drawing.
It is clear that $\cro(\psi_G)\le \cro(\psi_{G_1})+\cro(\psi_{G_2})$.



\textbf{Case 3. Removing a small cut and contracting a cycle.} 
Denote by $\hat v_1$ ($\hat v_2$, resp.) the vertex in $G_1$ ($G_2$, resp.) representing the contracted node. 
We first perform a stereographic projection from $\hat v_1$ in $\psi_{G_1}$ and a obtain new drawing $\psi'_{G_1}$ where $\hat v_1$ lies on the outer face, and the corresponding rotation systems are still respected. Then we uncontract $\hat{v}_1$ back to $Q$, to obtain a drawing $\psi''_{G_1}$ where the image of $Q$ is the boundary of the outer face.
We obtain a new drawing $\psi''_{G_2}$ from $\psi_{G_2}$ similarly.
We simply place $\psi''_{G_1}$ and $\psi''_{G_2}$ together in the plane by identify the image of $Q$ in both drawings, without creating new crossings. 
Let $\psi_{G}$ be the resulting drawing.
It is clear that $\cro(\psi_G)\le \cro(\psi_{G_1})+\cro(\psi_{G_2})$.

Therefore, we obtain a drawing of $\tG\setminus E^*$ with $\tilde{O}(\cro^{2-\eps})$ drawings. Using Lemma~\ref{lem:add_back_discarded_edges}, we can eventually add back the edges of $E^*$ to obtain a drawing of $\tG$ with 
$\tilde{O}(\cro^{2-\eps})+\tilde{O}(\cro^{1-\eps})\tilde{O}(\cro)=\tilde{O}(\cro^{2-\eps})$ crossings. This completes the proof of Theorem~\ref{thm: main_rot}.
\fi


















%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \iffalse
 
 \paragraph{Bounding the number of instances in the recursion.}
 The total number of edges in all the graphs participating in the same recursive level only decreases. When we consider graph $G'$ at the current recursive level, if $G_F$ is a sub-instance that we define, then there are at least $\cro^{1-2\eps}$ edges that lie in $G'$ but not in $G_F$: these are the edges that were initially incident to the vertex $v$ (we cannot use $\cro^{1-\eps}$ because it is possible that almost all edges incident to $v$ lie between two consecutive original paths, say $P_1$ and $P_2$. But because there are $\cro^{1-2\eps}$ such paths, we know that at least $\cro^{1-2\eps}$ edges incident to $v$ do not lie inside a fixed face). In fact every recursive sub-instance except for the leaf ones must have at least $\cro^{1-\eps}$ edges, and there must be at least $\cro^{1-2\eps}$ edges that belong to its parent but do not belong to it. From this, the total number of non-leaf recursive instances is at most $\cro^{2\eps}$. 
 
 
 
 \paragraph{Careful probabilistic argument.} Because there can be up to $\cro^{2\eps}$ non-leaf subinstances, we need to make sure that when we sample, the success probability in a single sub-instance is at least $(1-1/\cro^{2\eps})$, because at the end we will need all these samplings to be successful simultaneously. Suppose we say that a path is bad iff it crosses $x$ non-bad edges. Then we will get $\cro/x$ bad paths. We need to make sure that the probability that any bad path is sampled is no more than $1/\cro^{2\eps}$. So we need to sample with probability $x/\cro^{1+2\eps}$. Because the total number of paths may be as small as $\cro^{1-2\eps}$, and we have to ensure that some paths are sampled, we will need $x\geq \cro^{4\eps}$ to hold. This seems to be the lowest value of $x$ that we can afford, even if we are willing to settle for just two sampled paths. From a quick calculation, going with this value of $x$, we will end up with $\cro^{6\eps}$ bad edges, and the final number of crossings will be $\cro^{1+6\eps}+\cro^{2-\eps}$. To balance them, we take $\eps=1/7$, and get $\cro^{2-1/7}=\cro^{13/7}$.
 If $\cro<n^{7/13}$, then the approximation factor is $\cro^{6/7}=n^{6/13}$. If $\cro>n^{7/13}$, then the approximation factor is $n/\cro=n^{6/13}$. So from these rough calculations we are getting $n^{6/13}$. This is the best-case scenario; we may be losing additional factors.
 
 
 \fi
 
 
 
 
 \iffalse \textbf{An Alternative way to compute the drawing}
 Then we replace every vertex $v\in V(G)$ by a $(d_v\times d_v)$ grid $H_v$. An edge $(u,v)\in E(G')$ is replaced by an edge connecting a vertex on the first row of $H_v$ to a vertex on the first row of $H_u$, such that every vertex of a grid is used by at most one such edge. We obtain a new graph $G''$, whose maximum vertex degree is $5$, and $|V(G'')|=O(|V(G')|\cdot \cro^{1-\eps})$. We then use the algorithm with additive $|V(G)|$-approximation to compute a drawing of $G'$ with $O(|V(G')|\cdot \cro^{1-\eps})+\cro(G')$ crossings. Then we need to transform this drawing into a drawing of $G'$ by using the well-linkedness of the vertices on the first row of every grid. We need to bound the total sum of values $\cro(G')$ using the drawings $\phi'(G')$ and the fact that there are few difficult edges overall.
 \fi
 
 \iffalse
 \paragraph{Graph decomposition via small cuts or bounding boxes.}
 We now assume that the current graph $G'$ has at least one high-degree vertex, that we denote by $v$.
 \znote{first use Lemma 7.4 and 7.5}
 We let $e_1,\ldots,e_r$ be the edges incident to $v$ that are ordered according to the input ordering of these edges. Let $E_1=\set{e_1,\ldots,e_{\floor{r/2}}}$, and let $E_2$ contain the remaining edges. We first modify the graph $G'$, by replacing $v$ with two vertices, $v',v''$, where $v'$ is incident to all edges in $E_1$, and $v''$ is incident to all edges in $E_2$. Next, we consider the minimum edge-cut in $G'$ separating $v'$ from $v''$. We distinguish between two cases, based on whether the value of the cut (that we denote by $E'$) is large or small.
 
 \textbf{Case 1.} $|E'|< \cro^{1-2\eps}$.
 In this case, we let $G_1,G_2$ be the two subgraphs of $G'$ obtained by deleting the edges of $E'$ from it. We solve the problem on $G_1$ and $G_2$ separately and recursively. The sets of difficult edges and the associated drawings are defined in a natural way: for each $i\in \set{1,2}$, $\hat E(G_i)$ contains all edges of $\hat E(G)$ that lie in $G_i$, and the associated drawing $\phi'_{G_i}$ are simply the drawing of $G_i$ induced by $\tphi$. 
 %Once we obtain the drawings of $G_1$ and $G_2$ by solving the problem recursively, we first glue them by identifying the vertices $v'$ and $v''$ (so that edges incident to $v$ are drawn in the right order). After that, we add the drawings of the edges of $E'$. The number of crossings that this adds is bounded by $|E'|\cdot |E(G')|\leq \cro^{1-2\eps}|E(G')|$. While the total number of the recursive levels may be as high as $\cro^{2\eps}$, we may have at most $\cro^{\eps}$ sub-instances in which this cut step is applied (because every time we do this, we separate two sets of $\cro^{1-\eps}$ edges from each other). Therefore, overall, all such edge sets $E'$ will contribute at most $\cro^{2-\eps}$ crossings to the final drawing.
 
 \textbf{Case 2.} $|E'|\geq \cro^{1-2\eps}$.
 In this case, we first compute a set of $\cro^{1-2\eps}$ edge-disjoint paths, that connect edges of $E_1$ to edges to $E_2$. %We now go back to viewing $v$ as a single vertex.
 We apply Corollary~\ref{cor:finding_local_non_inf} to these of paths, and let $\pset$ be the set of locally non-interfering paths that we obtain. %Assume $\pset=\set{P_1,P_2,\ldots,P_k}$, and the order that first edges of these paths enter $v$ respect $\sigma_v$.
 %Consider a planar drawing of $v$ and $P_1,\ldots,P_k$, together with all edges incident to $v$ that are drawn in the right order. We can designate, as an outer face of this drawing, the face containing the area between $e_1$ and $e_r$. Once the outer face is selected, the resulting drawing is unique, where every path $P_i$ is a simple closed curve, and these curves are nested. We assume that the paths are indexed $P_1,\ldots,P_k$ in the natural order of their drawing, where $P_1$ defines the largest cycle, and $P_k$ is the innermost cycle.
 We say that a path $P\in \pset$ is \emph{$\beta$-bad} iff it participates in at least $\beta$ crossings with non-difficult edges in the drawing $\tphi(G')$, %\mynote{may need to adjust this threshold depending on how many faces we need; the fewer faces the lower threshold we can use.},
 or $P$ contains a difficult edge.
 So the number of $\beta$-bad paths in $\pset$ is at most $\tilde O(\cro/\beta)$.
 We say that a path in $\pset$ is \emph{long} if it contains at least $\cro^{3\eps}$ edges. Therefore, the number of long paths in $\pset$ is at most $\cro^{1-3\eps}$. We discard all long paths from $\pset$ and let $\pset'\subseteq\pset$ be the resulting set of paths, so $|\pset'|=\Omega(\cro^{1-2\eps})$.
 %We partition the paths in $\pset'$ into \emph{blocks} $B_1,B_2,\ldots,B_z$ of $100\cro^{1/2}$ consecutive paths each.
 We sample each path in $\pset'$ with probability $1/\cro^{1/2}$, and denote by $\qset\subseteq \pset'$ the set of sampled paths.
 %For odd indices $i$, we discard all paths of $B_i$ from $\qset$, and for even indices $i$, we discard all but one path of $B_i$ in $\qset$. Let $\qset'$ be the final set of paths. 
 
 \begin{observation}
 	With probability $1-O(n^{-100})$, the following is true:
 	\begin{enumerate}
 		\item none of the paths in $\qset$ is $100\cro^{1/2+\eps}$-bad;
 		%\item for each block $B_i$, at most $O(\log n)$ paths of $B_i$ lie in $\qset$; 
 		\item $|\qset|\geq \Omega(\cro^{1/2})$;
 		\item for two paths $Q',Q''$ that are cyclically adjacent in $\qset$, $|\sigma_v[Q',Q'']|, |\sigma_v[Q'',Q']|\geq \Omega(\cro^{1/2})$;  and
 		\item the paths in $\qset$ do not cross each other in the drawing  $\tphi(G)$.
 	\end{enumerate}
 \end{observation}
 \begin{proof}
 \end{proof}                                                                                                                                                                                                                                                                                                          
 
 %Consider some component $C\in \cset$. We will assign $C$ to some faces $F_1,\ldots, F_z$.
 %Before we do so, let $e\in E(G')$ be any edge that connects a vertex of $K$ to a vertex in some connected component $C\in \cset$. For example, assume that $e$ is incident to some vertex $u$ that lies on some path $P_i$. Since we are given a circular ordering of the edges incident to $u$, we get a unique face (that is either $F_i$ or $F_{i-1}$) on which $e$ must lie (more precisely, the drawing of $e$ must start inside that face, as it leaves the vertex $u$, but may then cross the boundaries of that face; it is only that first face that counts). Let $\Gamma$ denote the set of all edges that are incident to the vertices of $K$. In this way, for every edge $e\in \Gamma$, we have defined a unique face $F(e)\in \set{F_1,\ldots,F_z}$ to which $e$ belongs.
 %If the other endpoint of $e$ belongs to some component $C\in \cset$, then we assign $C$ to the face $F(e)$. Note that, as the result, each connected component $C\in \cset$ may be assigned to several faces. We first make a simplifying assumption that each component $C\in \cset$ is assigned to a single face, that we denote by $F(C)$, and show how to solve the problem. We will remove this assumption later.
 \iffalse
 For a recursion step, we consider some subgraph $G'$ of the current graph, and we let $v$ be any high-degree vertex in $G'$. Following is a central theorem for this algorithm.
 
 \begin{theorem}\label{thm: main for recursion}
 	One of the following two has to happen:
 	
 	\begin{itemize}
 		\item either there are two disjoint consecutive sets $E',E''$ of edges incident to $v$ with $|E'|,|E''|\geq \cro^{1-\eps}/2$, that can be disconnected from each other by removing at most $\cro^{1-3\eps}$ edges (the cut edges include all edges incident to $v$ that do not lie in $E'$ or $E''$); or
 		
 		\item there are two disjoint consecutive sets $E',E''$ of edges incident to $v$ with $|E'|,|E''|\geq \Omega(\cro^{1-3\eps})$, that can be disconnected from each other by removing at most $\cro^{1-5\eps}$ edges (the cut edges include all edges incident to $v$ that do not lie in $E'$ or $E''$); 
 	\end{itemize}
 \end{theorem}
 
 If the former happens, we say that the current iteration is a type-1 iteration, otherwise it is a type-2 iteration. In either case, we remove the cut edges, split the vertex $v$ according to the resulting two connected components, and then solve the problem recursively on both sides. 
 Once the two sub-problems are solved recursively, we glue the two copies of $v$, and then insert the cut edges.
 
 The total number of type-1 iterations over the course of the recursion can be bounded by $\cro^{\eps}$, and they contribute at most $\cro^{1-2\eps}$ total cut edges. The total number of type-2 iterations over the course of the recursion is bounded by $\cro^{3\eps}$, and they contribute $\cro^{1-2\eps}$ edges in total.  At the end, we will get a drawing with at most $\cro^{2-2\eps}$ crossings.
 
 From now on it only remains to prove the theorem.
 
 
 
 \begin{proofof}{Theorem \ref{thm: main for recursion}}
 	We assume that both claims are false, and reach a contradiction. Note that the theorem's claim is existential, so we don't need an algorithm. 
 	
 	We let $e_1,\ldots,e_r$ be the edges incident to $v$ that are indexed according to the input ordering of these edges. Let $E_1=\set{e_1,\ldots,e_{\floor{r/2}}}$, and let $E_2$ contain the remaining edges. 
 	Since the first claim is false, there is a collection $\pset$ of $\cro^{1-3\eps}$ edge-disjoint paths connecting edges of $E_1$ to edges of $E_2$. We denote the paths by $\pset=\set{P_1,\ldots,P_q}$, where the paths are indexed according to the ordering of the first edge of the path in $E_1$. 
 	
 	We say that a path $P_i$ is bad if participates in more than $\sqrt{\cro}$ crossings in the optimal drawing of $G$. Notice that at most $\sqrt{\cro}$ paths in $\pset$ are bad. Let $\pset'$ be obtained from $\pset$ by discarding the bad paths. Next, we partition $\pset'$ into blocks $B_1,\ldots,B_z$, each of which contains $\sqrt{\cro}$ consecutive paths, so the number of blocks is $z\geq \cro^{1/2-3\eps}/4$. We then let $\qset=\set{Q_1,\ldots,Q_z}$ be a set of paths, where $Q_i$ is the first path in block $B_i$. Since all paths in $\pset'$ are good, the paths in $\qset$ cannot cross each other in the optimal drawing.
 	
 	\fi
 	We call the union of the paths in $\qset'$ a \emph{skeleton}, and denote it by $K$. Let $\cset$ be the set of all connected components of $G'\setminus K$. 
 	Note that the optimal drawing $\tphi$ of $G$ induces a drawing of $K$, that we denote by $\phi_K$. Since we know the rotation system $\Sigma$, we can efficiently compute $\phi_K$. See Figure~\ref{fig:skeleton} for an example of $\phi_K$.
 	\begin{figure}[h]
 		\label{fig:skeleton}
 		\subfigure[]{\scalebox{0.33}{\includegraphics{skeleton}}}
 		\subfigure[]{\scalebox{0.33}{\includegraphics{ske_region}}}
 		\caption{An illustration of skeleton $K$  and its drawing $\phi_K$. Paths of in $\qset'$ are shown in different colors. A path of $\qset$ can cross itself in $\phi_K$ but cannot cross other paths in $\qset$. The right figure shows the region surrounded by good adjacent paths.}
 	\end{figure}
 	
 	
 	For $1\leq i\leq z$, let $E^i$ be the subset of the edges incident to $v$, that contains the first edge on every path in block $B_i$, so $|E^i|=\cro^{1/2}$.
 	We let $R_i$ be the region in the drawing $\phi_K$ of $K$ that contains the drawing of the first segment of the edges of $E^i$), and we say that the edges of $E^i$ are \emph{trapped} inside $R_i$. We call the path $Q_i$ and $Q_{i+1}$ the \emph{boundary paths} of the region $R_i$.
 	Notice that, even though the image of $Q_i$ and $Q_{i+1}$ do not cross in $\phi_K$, the image of $Q_i$ can cross itself (and same for the image of $Q_{i+1}$). Also, $Q_i$ and $Q_j$ can share nodes other than $v'$ and $v''$.
 	We denote by $\Gamma_i$ the set of edges in $G'$ 
 	that are incident to vertices in $(V(Q_{i+1})\setminus V(Q_{i}))\cup (V(Q_i)\setminus V(Q_{i+1}))$.
 	We say that the region $R_i$ is \emph{good} iff $|\Gamma_i|\le \cro^{1/2+4\eps}$. 
 	Since the total number of edges is $\tilde{O}(\cro)$, and each edge appears in at most two sets of $\set{\Gamma_1,\ldots,\Gamma_z}$, the number of non-good faces is at most $O(\cro^{1/2-4\eps})$.
 	Therefore, the total number of edges in $\bigcup_{1\le i\le z}E^i$ that are trapped in the good faces is then at least $\Omega(\cro^{1-3\eps})$.
 	
 	
 	We now randomly sample two faces from $\set{F_1,\ldots,F_z}$. Let $F_i$ and $F_j$ be the face that we obtain. We prove the following observation.
 	\begin{observation}
 		With probability $1-O(n^{-100})$, the following is true:
 		\begin{enumerate}
 			\item both $F_i$ and $F_j$ are good;
 			\item if we take the set of all edges that are incident to $v$, and delete from them the edges of $E^i$ and $E^j$, we obtain two disjoint consecutive sets of edges, $E',E''$, then $|E'|,|E''|\geq \cro^{1-3\eps}/32$; and
 			\item denote $T_i=V(Q_i)\cap V(Q_{i+1})$, then either $T_i$ is empty, or the vertices in $T_i\cap V_{\cro^{1-6\eps}}(G)$ appears in the same order on the paths $Q_i$ and $Q_{i+1}$, and the same holds for $j$.
 		\end{enumerate}	
 	\end{observation}
 	\begin{proof}
 	\end{proof}
 	
 	%If we take the set of all edges that are incident to $v$, and delete from them the edges of $E^i$ and $E^j$, we obtain two disjoint consecutive sets of edges, that we denote by $E',E''$. We can choose $E^i,E^j$ such that $|E'|,|E''|\geq \cro^{1-3\eps}/32$ (by letting $F_i,F_j$ be good faces that are furthest from each other in both clock-wise and counter-clock-wise direction). If we delete all edges that lie in $E^i,E^j$, and all edges whose drawings in $\phi'$ intersect the interiors of $F_i$ or $F_j$, then we will disconnect the edges of $E'$ from the edges of $E''$ (this is true even if, in the drawing $\phi_K$, the paths that form the boundaries of $F_i,F_j$ cross themselves; we only need the fact that they don't cross each other). Since $F_i,F_j$ are good faces, the size of this cut is at most $64\cro^{1/2+3\eps}$. We need to choose $\eps$ so that this is less than $\cro^{1-5\eps}$ to finish the proof (e.g., $\eps=1/16$ should work).
 	We add all edges of $\Gamma_i\cup \Gamma_j$ into $E^*$, the set of discarded edges.
 	We define the edge set $S'$ to be the union of (i) $E'$; and (ii) the set of edges incident to $T_i\cap V_{4}(G)$ or $T_j\cap V_{4}(G)$ and assigned to the region of $E'$. We define $S''$ similarly. Now we compute the min edge-cut separating $S'$ from $S''$ in $G'\setminus (V(F_i)\cup V(F_j))$. Let $\tilde E$ be the set of edges that we obtain. We add the edges of $\tilde E$ into the set of discarded edges. Let $G_1$ ($G_2$, resp.) be the graph by contracting the boundary of $E'$ ($E''$, resp.) into a single vertex $v_F$. The ordering of the edges incident to $v_F$ is fixed by using the orderings of the vertices along the boundary of $F$, and the orderings of their incident edges. We recursively solve the problem on $G_1$ and $G_2$.
 	
 	
 	
 	%We assume that each component $C\in \cset$ is assigned to a single face $F(C)$. We now consider each face $F\in \set{F_1,\ldots,F_z}$ separately. For each such face $F$, we will define a separate problem, which will be solved recursively.
 	
 	%Consider now some face $F\in \set{F_1,\ldots,F_z}$. Let $\cset_F\subseteq \cset$ be the set of all connected components that were assigned to $F$. We define a new graph $G_F$, that consists of the boundary of $F$, all components of $\cset_F$, and all edges connecting the boundary of $F$ to these components. Then we take the boundary of $F$ and contract it into a single vertex $v_F$. The ordering of the edges incident to $v_F$ is fixed by using the orderings of the vertices along the boundary of $F$, and the orderings of their incident edges.
 	
 	%We solve the problem recursively on $G_F$, and then combine the solutions together in a straightforward manner.
 	
 	We will also define the sets of difficult edges for each graph $G_F$, and the drawing $\phi(G_F)$ with the desired properties.
 	Consider again the graph $G_F$, before we contracted the boundary into a single vertex. Consider the drawing $\phi(G')$ of the current graph $G'$, and delete from it everything except for the boundary of $F$, and the components in $\cset_F$. If, for every component $C\in \cset_F$, all vertices and edges of $C$ are drawn inside $F$, then contracting the boundary of $F$ into a single vertex won't increase the number of crossings. So our problem is that for some component $C$, some subset $X_C$ of vertices of $C$ is drawn outside of $F$. Let $Y_C=V(C)\setminus X_C$. Notice that, if $e$ is an edge connecting a vertex $u$ on the boundary of $F$ to a vertex of $C$, then as $e$ leaves $u$, it is drawn inside $F$, but later it may cross the boundary of $F$. Therefore, if we delete all edges in $E_C(X_C,Y_C)$, then $X_C$ becomes disconnected from both $C$ and the boundary of $F$. Moreover, every edge in $E_C(X_C,Y_C)$ must cross the boundary of $F$. Therefore, the number of non-difficult edges in $E_C(X_C,Y_C)$ is at most $\cro^{1/3+\eps}$ (because the paths in $\qset$ are good). Even if we take the union of all such edges over all $C\in \cset_F$, their number is still at most $\cro^{1/3+\eps}$. So we simply move the drawing of $X_C$ to lie inside $F$, and then add the edges of $E_C(X_C,Y_C)$ to the current drawing arbitrarily. The edges of $E_C(X_C,Y_C)$ become difficult edges for $G_F$. Additionally, every edge $e\in E(G_F)$ that was difficult to $G'$ remains difficult for $G_F$.  This gives us the desired drawing $\phi(G_F)$ of $G_F$; note that the number of difficult edges remains suitably bounded. Moreover, if $e,e'$ is a pair of edges that cross in the drawing $\phi(G_F)$, the either $e,e'$ cross in the original drawing $\phi$ of $G$, or at least one of these edges is a difficult edge.
 	\fi
 
 \iffalse
 \paragraph{Without the Simplifying Assumption}
 Let us assume that some component $C\in \cset$ was assigned to faces $F_{i_1},F_{i_2},\ldots,F_{i_q}$. The idea now is to compute a cut in $C$ to disconnect these faces, so that each resulting connected component is only assigned to one face. The cut edges will need to be added back. The claim is that there are relatively few of them because they will need to intersect every path $Q_j$ that lies between the corresponding two faces, so the total new number of crossings should be small.
 
 
 
 \paragraph{Finishing the Multicut Question}
 It looks like we don't need the skeleton $K$ to contain that many paths and faces. It looks like it is enough to keep just two paths and faces (or some constant number). In order for the number of the recursive levels to be small, we want to ensure that for every face there are at least $\cro^{1-2\eps}$ edges that are incident to $v$ and lie outside of the face. This seems easy to ensure even if we use just two paths and faces. The question of multicut then reduces to a simple cut question (or multicut with a constant number of terminals if there are more than two faces). The total number of edges deleted in all these multicuts must be at most $O(\cro^{1/3+\eps})$, because each such edge represents a path connecting two different faces, that has to cross at least one of the paths of the skeleton. The total number of such paths is bounded by the number of the bad edges plus $O(\cro^{1/3+\eps})$. Altogether, we get at most $O(\cro^{1/3+3\eps})$ multicut edges over all connected components in $\cset$ (we take into account that there could be up to $\cro^{1/3+3\eps}$ bad edges). Even if we look at all recursive levels and all subinstances, we will get at most  $\cro^{1/3+5\eps}$ multicut edges overall, so inserting them will not create many crossings.
 
 \fi
 \iffalse
 
 \subsection{The Multicut Argument}
 Our starting point is the skeleton $K$, that consists of paths $Q_1,\ldots,Q_q$ connecting $u$ to $v$, and the faces $F_1,\ldots,F_q$ defined by the drawing of $K$, where the boundaries of $F_i$ are $Q_i$ and $Q_{i+1}$. Each edge that has an endpoint in $V(K)$ is assigned to one of these faces, as described above. We denote by $\Gamma$ the set of all such edges. Let $\cset$ be the set of all connected components of $G\setminus K$. For every connected component $C\in \cset$, we have assigned $C$ to a number of faces: if a vertex of $C$ is incident to an edge $e\in \Gamma$, and $e$ is assigned to $F_i$, then we assign $C$ to $F_i$ as well.
 
 In this step, for each connected component $C\in \cset$, we will select a subset $E'\subseteq E(C)$ of edges to delete. If we consider the set $\rset(C)$ of connected components of $C\setminus E'$, then we will ensure that each such resulting component is only assigned to a single face. In other words, for each $R\in \rset(C)$, there is a single face $F\in \set{F_1,\ldots,F_q}$, such that vertices of $R$ are incident to edges of $\Gamma$ that are assigned to $F$. We will solve the problem recursively on each face as described above, and then insert the deleted edges back, as follows. (we will refer to the edges in $E'$ as $E'_C$, since we will need to argue about edges deleted from different components.)
 
 
 Assume that we have two components $R,R'\in \rset(C)$, with $R$ assigned to $F_i$ and $R'$ assigned to $F_j$, where $i<j$. If $e\in E'_C$ is any edge connecting a vertex of $R$ to a vertex of $R'$, then, after we solve the problems defined by each face recursively, we will insert this edge back. 
 We can insert it in one of two ways: so that it goes in clock-wise direction from $F_i$ to $F_j$, or in counter-clock wise direction from $F_j$ to $F_i$. In the former case, it will be allowed to cross any edges that belong to the sub-problems associated with the faces $F_i,F_{i+1},\ldots,F_j$; we will say that $e$ conflicts with these faces. In the latter case it will be allowed to cross all edges that belong to the sub-problems of faces $F_j,F_{j+1},\ldots,F_q,F_1,\ldots,F_i$, and we will say that $e$ has conflicts with these faces. The crux in the algorithm and its analysis is to ensure that for every face $F$, the total number of edges (in $\bigcup_{C\in \cset}E'_C$ that have conflict with $F$ is small. This will ensure that the number of crossings that we obtain by adding these edges back is also small.
 
 In order to ensure this, we will associate, to each edge $e$ as above, a path $P(e)$ (that we call a \emph{witness path}), connecting a vertex on the boundary of $F_i$ to a vertex on the boundary of $F_j$ (we assume that $e$ connects component $R$ assigned to $F_i$ to component $R'$ assigned to $F_j$), and we will ensure that for $e\neq e'$, the paths $P(e),P(e')$ are edge-disjoint. Note that the drawing $P_e$ must either cross the boundaries of all faces $F_i,F_{i+1},\ldots,F_j$, or it must cross the boundaries of all faces $F_j,F_{j+1},\ldots,F_q,F_1,\ldots,F_i$. So if we choose the direction (clock-wise or counter-clock-wise) of the drawing of $e$ correctly, then for every face $F$ that $e$ conflicts with, the path $P(e)$ must cross the boundaries of this face. Since each path $Q_i$ only participates in a small number of crossings, this will ensure that the total number of edges that conflict with each face is small. 
 
 \paragraph{Orientation of Edges}
 Even though we do not know what is the right orientation of the drawing of each edge $e\in \bigcup_{C\in \cset}E'_C$, this problem is easy to resolve. Recall that path $Q_1$ only participates in at most $\sqrt{cr}$ crossings in the optimal solution. So there are at most $\sqrt{cr}$ edges $e\in \bigcup_{C\in \cset}E'_C$, whose witness path $P(e)$ crosses $Q_1$ in the optimal drawing. We can choose the orientation of the drawing of each such edge in the opposite direction, so it does not cross $Q_1$. This will only add a small overhead in the number of crossings. So in the end, when we insert the edges if $\bigcup_{C\in \cset}E'_C$ into the drawing, we draw each edge so that it does not cross $Q_1$.
 
 To complete the whole algorithm it is now enough to prove the following lemma.
 
 \begin{lemma}
 	There is an efficient algorithm, that, given a component $C\in \cset$, computes a subset $E'\in E(C)$ of edges, and for each edge $e\in E(C)$, a witness path $P(e)$ in $C$, such that the following hold:
 	\begin{itemize}
 		\item If $\rset$ is the set of all connected components of $C\setminus E'$, then for each component $R\in \rset$, there is a unique face $F\in \set{F_1,\ldots,F_q}$, such that an edge of $\Gamma$ that is assigned to $F$ is incident to a vertex of $R$;
 		
 		\item If $e\in E'$ connects a vertex of $R\in \rset$ to a vertex of $R'\in \rset$, such that $R$ is assigned to $F_i$ while $R'$ is assigned to $F_j$, then $P(e)$ connects a vertex on the boundary of $F_i$ to a vertex on the boundary of $F_j$; and
 		
 		\item The paths in $\set{P(e)\mid e\in E'}$ are edge-disjoint.
 	\end{itemize}
 \end{lemma}
 
 \begin{proof}
 	Throughout the proof, we fix a single component $C\in \cset$, and we assume that $C$ is assigned to faces $F_{i_1},ldots,F_{i_z}$, where $i_1<i_2<\cdots<i_z$. We first slightly modify the component $C$, as follows. For each $1\leq j\leq z$, for every edge $e=(x,y)\in \Gamma$ that is assigned to $F_{i_j}$, such that $x\in V(C)$ and $y$ lies on the boundary of $F_{i_j}$, we introduce a new vertex $y'$, and a new edge $(x,y')$, that is added to $C$ (notice that $C$ does not contain $y$). We say that $y'$ is a terminal that belongs to $F_{i_j}$. We let $T_j$ be the set of all such terminals that belong to $F_{i_j}$, and we denote the resulting graph by $H$.
 	
 	Next, we perform $z-1$ iterations. We start with $E'=\emptyset$, and in every iteration, we add some new edges to $E'$. We will ensure that, at the end of the $j$th iteration, graph $H\setminus E'$ contains no path from a terminal in $\bigcup_{j'=1}^jT_{j'}$ to a terminal in $\bigcup_{j'=j+1}^zT_{j'}$. Consider the set $E'$ of edges that is obtained at the end of iteration $j$. We define a sub-graph $H'_j\subseteq H\setminus E'$, to contain all connected components containing terminals of $T_j\cup\cdots\cup T_z$. 
 	Additionally, if $e=(x,y)\in E'$ has an endpoint (say $x$) that lies in $H'_j$, with $y\not\in H'_j$, then we add a new edge $(x,t_e)$ to $H'_j$, and we say that $t_e$ is an \emph{extra terminal for iteration $j+1$}. We denote by $X_j$ the set of all extra terminals for iteration $j+1$. An edge $e\in E'$ (at the end of iteration $j$) is called \emph{active} iff one of its endpoints lies in $H'_j$, and it is called inactive otherwise.
 	Lastly, we ensure that the following invariants hold: 	Consider the set $E'$ of edges at the end of iteration $j$, and the corresponding graph $H'_j$
 	
 	\begin{properties}{I}
 		\item If a connected component of $H_j$ contains terminals from two different sets $T_r,T_{r'}$ for $r\neq r'$, then $r,r'>j$ (in other words, every connected component of $H_j$ except those containing terminals of $T_{j+1},\ldots,T_z$ is assigned to a single face);
 		
 		\item	 For every edge $e\in E'$, we maintain a path $P(e)$, such that all paths in set $\set{P(e)\mid e\in E'}$ are edge-disjoint, and they are internally disjoint from graph $H'_j$. If $e\in E'$ is inactive, then $P(e)$ is a valid witness path for it; otherwise, $P(e)$ connects a terminal in $T_1\cup \cdots\cup T_j$ to the extra terminal $t_e$.
 	\end{properties}
 	
 	We now describe the execution of the $(j+1)$th iteration, for $0\leq j<z$. We start with the graph $H'_j$, and compute a minimum cut separating the terminals of $T_{j+1}\cup X_j$ from the terminals of $T_{j+2}\cup\cdots\cup T_z$. Let $E'_j$ be the resulting set of edges, and let $(A,B)$ denote the resulting cut, with $T_{j+1}\cup X_j\subseteq S$. We add the edges of $E'_j$ to $E'$. From the max-flow/min-cut theorem, there is a collection $\pset'$ of edge-disjoint paths, contained in $H'_j[A]$, connecting every edge of $E'_j$ to a distinct vertex of $T_{j+1}\cup X_j$. For each edge $e\in E'_j$, we let $P'(e)$ denote the corresponding path. If path $P'(e)$ originates from a vertex of $T_{j+1}$, then we set $P(e)=P'(e)$. Otherwise, path $P'(e)$ must originate from some extra terminal $t_{e'}$. We then let $P(e)$ be the concatenation of $P(e')$ and $P'(e)$. If the endpoint of $e$ that lies in $B$ is a terminal, then $e$ becomes an inactive edge, and $P(e)$ is its witness path. Otherwise, in the next iteration, we will introduce a new extra terminal $t_e$ representing $e$, and then $P(e)$ is the corresponding path that has the required properties.	
 \end{proof}
 \fi
 
 
 
 \iffalse
 \subsubsection*{Step 1: Graph Decomposition with respect to High-Degree nodes.}
 
 In this step, we construct an algorithm that efficiently computes a subset $\hat{E}\subseteq E(\tG')$ of at most $\tilde O(|E(\tG')|\cdot n^{-\eps})$ edges, such that, in each connected component of the remaining graph $\tG'\setminus \hat{E}$, for every pair of high-degree nodes, there are $d/n^{\eps}$ edge-disjoint paths connecting them. 
 
 We now describe the algorithm.
 Throughout the algorithm, we maintain (i) a set $\tilde{E}$ of edges in $E(\tG')$, that is initialized to be $\emptyset$; and (ii) a set $\cset$ of mutually node-disjoint subgraphs of $\tG'$, that is initialized to be $\set{\tG'}$. The algorithm proceeds in iterations.
 %and continues to be executed iff there exists a subgraph $C\in \cset$ and a pair $v,v'$ of H-node in $C$, such that the min-cut of $C$ separating $v$ and $v'$ contains no more than  $d/n^{\eps}$ edges.
 In an iteration, the algorithm computes, for each cluster $C\in \cset$, and for each pair of H-node in $C$, the min-cut of $C$ separating them.
 If for each cluster $C\in \cset$ and for each pair of H-node in $C$, the min-cut of $C$ separating them contains at least $d/n^{\eps}$ edges, then the algorithm is terminated. Otherwise, we arbitrarily pick such a cluster $C\in \cset$ together with a pair $v,v'$ of H-node in $C$, such that the min-cut $(S,S')$ of $C$ separating $v$ and $v'$ contains no more than  $d/n^{\eps}$ edges. We add all edges in this min-cut into $\tilde{E}$ and replace the cluster $C\in \cset$ by the clusters $C[S]$ and $C[S']$. This completes the description of an iteration, and also completes the description of the algorithm.
 
 Denote by $\hat{E}$ the set $\tilde E$ at the end of the algorithm, and let $\hat\cset$ be the set of connected components of $\tG'\setminus \hat{E}$. From the algorithm, it is clear that, for each $C\in \hat\cset$, and for every pair of high-degree nodes in $C$, there are $d/n^{\eps}$ edge-disjoint paths connecting them in $C$. Since $|V_H|=O(n^{4\eps})$, and in each iteration we add at least one edge into $\tilde E$, the algorithm runs in polynomial time. 
 
 It remains to bound the size of $\hat{E}$, which we do by a charging scheme, as follows.
 When in an iteration, we find a cut $(S,S')$ (assuming $|E(S)|\le |E(S')|$) in $C$ separating a pair $v,v'$ of H-node in $C$, such that $v\in S$ and $v'\in S'$, we charge the edges in $E(S,S')$, the edges that is added into $\tilde E$ in this iteration, uniformly to the edges in $E(S)$.
 Observe that each time an edge is charged, the size (the number of edges) of the cluster in $\cset$ that contains it shrinks by a constant factor. Therefore, each edge is charged at most $O(\log n)$ times. 
 As a corollary, for each high-node, the size of the cluster in $\hat{\cset}$ that contains it is at least $d-O(\log n)\cdot d/n^{\eps}=d(1-o(1))$.
 Therefore, at any time in the algorithm, the size of the cluster in $\hat{\cset}$ that contains some H-node is at least $d-O(\log n)\cdot d/n^{\eps}=d(1-o(1))$. As a result, each time an edge is charged, it is charged at most $O((d/n^\eps)/d)=O(n^{-\eps})$. Therefore, the total charge throughout the algorithm is bounded by $|E(\tG')|\cdot O(\log n/n^{\eps})$, so the number of edges in $\hat{E}$ is $\tilde O(|E(\tG')|\cdot n^{-\eps})$.
 \fi
 
 
 
 
 
 \iffalse
 \subsubsection*{Step 3: Extending the skeleton to span all high-degree nodes.}
 
 Denote by $S$ the skeleton produced in the last step. Sketch in this step (\znote{informal}):
 \begin{itemize}
 	\item Let $\hat V_H$ be the set of any high-degree nodes that does not lie in the skeleton, we can find, for each node $u\in\hat{V}_H$, a set $\pset_u$ of $\Omega(d'/n^{\eps})$ paths, such that each path in $\pset_u$ connects $u$ to some node in $S$, and the paths in $\bigcup_{u\in \hat{V}_H}\pset_u$ are edge-disjoint.
 	\item Assume without loss of generality that each path in $\pset_u$ only contains one node in $S$. Prove that, for each $u\in \hat{V}_H$, there exists $1\le i\le |\hat\qset|$, such that almost all ``other endpoints'' of the paths in $\pset_u$ lie in $\hat{Q}_i\cup \hat{Q}_{i+1}$.
 	\item 
 	Denote $\tilde Q_i\subseteq \qset$ to be the subset of paths of $\qset$ that lie between (with respect to the circular ordering $\sigma$) $\hat Q_i$ and $\hat{Q}_{i+1}$, namely $\tilde Q_i=\sigma[\hat Q_i,\hat Q_{i+1}]$.
 	We call a path in $\pset_u$ bad if it contains at least $n^{0.25}$ vertices from $V(\tilde Q_{i-1})$ or $V(\tilde Q_{i+1})$. Prove that the number of bad paths is small (at most $n^{0.25}$) compared with $d'/n^{\eps}$.
 	\item For each $u\in \hat{V}_H$, delete from $\pset_u$ all bad paths, so the number of remaining paths is still $d'/n^{\eps}$. Sample each path with probability $n^{-0.25}$ to get $\hat{\pset}_u$. We call $\bigcup_{u\in \hat{V}_H}\hat\pset_u$ the extension of the skeleton produced in Step 2.
 	\item Prove that with high probability, the image of the paths in $\hat{\pset}_u$ in $\tphi'$ do not cross, and they all lie in the cell surrounded by $\hat{Q}_i$ and $\hat{Q}_{i+1}$ in the skeleton $S$.
 \end{itemize}
 
 \subsubsection*{Step 4: Handling the remaining pieces.}
 
 Let $\tilde S$ be the extended skeleton produced in Step 3.
 Since the degree of each node in $C\setminus \tilde{S}$ is at most $d$, $\sum_{v}\deg(v)^2\le d\cdot \sum_{v}\deg(v)=O(n^{1-\eps})$.
 Ideally we can use Lemma~\ref{lem:cro} to compute a drawing of all remaining pieces with $O(n^{1-\eps})$ crossings.
 \fi
 
 

==> ideal_partition.tex <==
\section{Proof of Theorem~\ref{thm: ideal partition}}

In this section we provide the proof of Theorem~\ref{thm: ideal partition}.



\subsection{Auxiliary Lemmas}

\iffalse
\begin{lemma}
\label{lemma:face_distance}
For any two faces $F,F'$ of the plane graph $H$, the depth of the largest shell \explain around $F$ that does not intersect $F'$ equals $\dist_{H^*}(F,F')-1$. 
\end{lemma}
\fi

\begin{lemma}
\label{lem:separating}
There exists an algorithm, that, given any 3-connected graph $H$ drawn in the plane and two faces $F,F'$ of its plane drawing $\phi$, computes a set $\tilde E\subseteq E(H)$ of $\dist_{H^*}(F,F')$ edges, such that in the induced drawing of $\phi$ on $H\setminus \tilde{E}$, the faces $F$ and $F'$ are merged \explain.
\end{lemma}

We use the following Lemma, whose proof is deferred to Appendix~\ref{apd:crossing_charged_to_consecutive_cycles}.
\begin{lemma}
\label{lem:crossing_charged_to_consecutive_cycles}
Let $H$ be a $3$-connected graph and $C_1,\ldots,C_{\ell}$ ($\ell>30$) be vertex-disjoint cycles in $G$, such that, for any $1\le x<y<z\le \ell$, there is no path in $H\setminus C_y$ connecting any vertex of $C_x$ to any vertex of $C_z$. Let $P$ be a path (which does not belong to $H$) that connects a vertex of $C_1$ to a vertex of $C_{\ell}$, then in any drawing of the graph $H\cup P$ on the plane, for each $1\le i\le \ell-2$, at least one cycle of $C_{i}, C_{i+1}, C_{i+2}$ is crossed.
\end{lemma}

\begin{corollary}
\label{cor:local_crossing}
Let $H$ be a graph and $C_1,\ldots,C_{\ell}$ ($\ell>30$) be vertex-disjoint cycles in $G$, such that, for any $1\le x<y<z\le \ell$, there is no path of $H\setminus C_y$ connecting any vertex of $C_x$ to any vertex of $C_z$. Let $P$ be a path (which does not belong to $H$) that connects a vertex of $C_1$ to a vertex of $C_{\ell}$, then in any drawing of the graph $H\cup P$ on the plane, the number of crossings that the cycles $C_1,\ldots,C_{\ell}$ participate in is at least $\ell/3$.
\end{corollary}


\subsection{Terminal Well-Linked Decomposition}

\begin{lemma}[Terminal Well-Linked Decomposition]
\label{lem:well_linked-decomposition}
There is an efficient algorithm, that, given any connected graph $G$ and a subset $T\subseteq V(G)$ of its vertices with $|T|=k$, computes a collection $(G_1,\ldots,G_r)$ of connected subgraphs of $G$, such that:
\begin{enumerate}
\item for each $1\le i\le r$, denote $V_i=V(G_i)$, then $(V_1,\ldots,V_r)$ forms a partition of $V(G)$;
\item for each $1\le i\le r$, the subset $T_i\cup \Gamma(V_i)$ {\color{red} (need to define both $T_i$ and $\Gamma(V_i)$)}of vertices is $\Omega(\frac{1}{\log^{3/2} k})$-well-linked in $G_i$; and
\item $\sum_{1\le i\le r}|\out(V_i)|\le 0.01 k$ {\color{red}(need to define $\out(V_i)$)}, as a corollary, $\sum_{1\le i\le r}|T_i\cup \Gamma(V_i)|\le 1.01 k$.
\end{enumerate}
\end{lemma}
We call the algorithm in the above lemma the \emph{well-linked decomposition of $H$ with respect to $T$}.
We call an edge $(u,u')$ of $G$ an \emph{inter-cluster} edge if $u$ and $u'$ belong to different parts of the partition $(V_1,\ldots,V_r)$.

\subsection{Proof of Theorem~\ref{thm: ideal partition}}

Throughout, we maintain (i) a set of edges $\hat{E}$, that is initialized to be $E'$, and (ii) a set of vertices $T$, that initially contains all vertices that has an edge in $E'$ incident to it. The invariant is that, at any time, the set $T$ contains all vertices that has an edge in $\hat E$ incident to it.
We will gradually add some edges of $G\setminus E'$ into $\hat{E}$, and update $T$ accordingly so that the invariant always holds.
The final set $\hat E$ will be the output edge set $E''$.

For each connected component $R$ of $H$ {\color{red}(we need to say what $H$ is with respect to $G$)}, we first perform a well-linked decomposition with respect to $T\cap V(R)$ using Lemma~\ref{lem:well_linked-decomposition} and obtain a collection of subgraphs of the component. We add all inter-cluster edges into $\hat E$ and update $T$ accordingly. 
From Lemma~\ref{lem:well_linked-decomposition}, the number of edges that we added into $\hat E$ is $O(|E'|)$.

Let $\cset=\set{C_1,\ldots,C_r}$ be the connected components of $G\setminus \hat E$.
%It is clear that the sets $V(C_1),\ldots,V(C_r)$ is a partition of $V(G)$.
So the each of graphs $C_1,\ldots, C_r$ is a subgraph of $H$. 
Fix a planar drawing $\psi$ of $H$. 
For any cluster $S$ of $H$, we denote by $\psi_{S}$ the induced drawing of $\psi$ on $S$.
%let $\fset_i$ be the collection of faces in the drawing $\psi_{C_i}$. 
We say that a vertex $v\in T\cap V(C_i)$ is a \emph{bad terminal} if there exist another vertex $v'$, a pair of distinct faces $F, F'$ in the drawing $\psi_{C_i}$ and a path $P$, such that (i) $v\in V(F)\setminus V(F')$ and $v'\in V(F')\setminus V(F)$; (ii) the path $P$ consists of edges in $\hat{E}$ {\color{red}(is this what we want to say or we want to say the path consists of edges in $G\setminus C_i$?)}; and (iii) the path $P$ connects $v$ to $v'$.

For each component $C\in \cset$, we run a separate process on $C$ that gradually adds some edges of $E(C)$ into $\hat{E}$. Let $E_C\subseteq E(C)$ be the subset of edges that are added into $E$ {\color{red}($\hat{E}$?)}.
The goal is to ensure that the induced planar drawing of $\psi_{C}$ on $C\setminus E_C$ contains no bad terminals, and $\sum_{C\in \cset}|E_C|=\tilde{O}(|E'|+\cro(G))$.
%Then, for each $C\in \cset$, we add edges of $E_C$ into $\hat{E}$.

Now we fix a component $C\in \cset$. We denote $T(C)=T\cap V(C)$.
%and denote $\psi_C$ to be the induced drawing of $\psi$ on $C$.
We have $\sum_{C\in \cset}|T_C|=O(|E'|)$. 
Let $T^b\subseteq T(C)$ be the set of bad terminals of $C$.
For any sub-cluster $S$ of $C$, we denote by $T^b(S)$ the set of bad terminals in $T^b(S)$ {\color{red}($S$?)}.
Notice that, as the set $T$ changes, $T^b(S)$ also evolves.
Let $\fset_C$ be the set of faces in the drawing $\psi_C$ that contains some bad terminals. It is clear that $|\fset_C|=O(|T(C)|)$. 
%since each vertex lies on the boundary of at most $\Delta=O(1)$ faces.

We now describe the separate process on $C$ that gradually adds edges of $E(C)$ into $\hat{E}$.
The process proceeds in iterations. In the $i$th iteration, it takes as input a tuple $(S,T^b(S), \fset_S)$, where $S$ is a sub-cluster of $C$, $T^b(S)$ is the set of its bad terminals, and $\fset_S$ is a face cover of the vertices of $T^b(S)$ in the drawing $\psi_S$, computes a set $\tilde{E}_i$ of the edges of $S$, and outputs another tuple $(S',T^b(S'), \fset_{S'})$, where $S'=S\setminus \tilde{E}_i$ is a sub-cluster of $S$, $T^b(S')$ is the set of its bad terminals, and $\fset_{S'}$ is a face cover of vertices $T^b(S')$ in the drawing $\psi_{S'}$, such that $|\fset_{S'}|\le |\fset_{S}|/2$.  
The input of the first iteration is $(C,T^b, \fset_C)$.
Whenever in the output tuple $(S',T^b(S'), \fset_{S'})$ of some iteration, the set $T^b(S')=\emptyset$, we terminate the algorithm on $C$.
At the end, let $E_C$ be the union of the sets $\tilde E_i$ in all iterations of the process on $C$.

We now describe the $i$th iteration of the process on $C$.
Let $S^*$ be the dual graph of $S$ with respect to the planar drawing $\psi_S$. From the definition of a dual graph, for each face $F$ in the drawing $\psi_S$, there is a vertex $v_F\in V(S^*)$ in the dual graph $S^*$.
Define $\tilde V=\set{v_F\in V(S^*)\mid F\in\fset_S}$, so $\tilde{V}$ is a subset of $V(S^*)$.
For each $F\in \fset_S$, we perform a BFS in $S^*$ to compute a vertex 
$v^*\in \arg\min_{v\in \tilde{V}}\set{\dist_{S^*}(v,v_{F})}$, with tie breaking arbitrarily.
Let $N(F)\in \fset_S$ be the face of $\psi_S$ that $v^*$ corresponds to, and we also denote $d(F)=\dist_{S^*}(v^*,v_{F})$. We consider two cases.

\textbf{Case 1.} $d(F)\le 30$.
Let $\tilde{E}_i(F)$ be the set that we obtain by applying Lemma~\ref{lem:separating} to the cluster $S$ and its faces $F$ and $N(F)$. 
From Lemma~\ref{lem:separating}, $|\tilde{E}_i(F)|\le 30$.

\textbf{Case 2.} $d(F)> 30$.
Let $\tilde{E}_i(F)$ be the set that we obtain by applying Lemma~\ref{lem:separating} to the cluster $S$ and its faces $F$ and $N(F)$.
From Lemma~\ref{lem:separating}, $|\tilde{E}_i(F)|\le d(F)$.



We let the set $\tilde{E}_i$ be the union of $\tilde{E}_i(F)$ for all $F\in \fset_S$, namely $\tilde{E}_i=\cup_{F\in \fset_S}\tilde{E}_i(F)$. Then we add the edges of $\tilde{E}_i$ into $\hat{E}$ and update $T^b$ accordingly.
From Lemma~\ref{lem:separating}, each face $F$ of $\fset_S$ is merged with the face $N(F)$ after we take out the edges of $\tilde{E}_i$ from $S$. Therefore, we set $S'=S\setminus \tilde{E}_i$, set $T^b(S')=T^b\cap V(S')$, and let $\fset_{S'}$ be the faces in $\psi_{S'}$ that is formed by merging faces of $\fset_{S}$ in $\psi_{S}$. It is easy to see that $|\fset_{S'}|\le |\fset_{S}|/2$. The tuple $(S',T^b(S'), \fset_{S'})$ is our output.
This finishes the description of an iteration of the separate process on $C$, and also finishes the description of the separate process on $C$.

\begin{observation}
\label{obs:number_of_iterations}
The separate process on $C$ runs at most $O(\log |T_C|)=O(\log n)$ iterations.
\end{observation}

At the end of the process on $C$, we define $E_C$ to be the union of the sets $\tilde{E}_i$ from all iterations, namely the set of edges that are added into $\hat{E}$ in this process. From the process, it is easy to verify that the induced planar drawing of $\psi_{C}$ on $C\setminus E_C$ contains no bad terminals. It remains to show $\sum_{C\in \cset}|E_C|=\tilde{O}(|E'|+\cro(G))$.

\begin{proposition}
\label{pro:C_share}
For each $C\in \cset$, $|E_C|=O(\log n\cdot (|T_C|+\cro_{\phi}(C)))$.
\end{proposition}
\begin{proof}
Recall that $|\fset_C|=O(|T_C|)$. For each $i>1$, let $(S,T^b(S),\fset_S)$ be the tuple output by the $(i-1)$th iteration of the process on $C$. From the process, 
$|\fset_S|\le |\fset_C|=O(|T_C|)$.
Therefore,
$$\sum_{F\in \fset_S, d(F)\le 30}|\tilde{E}_i(F)|\le O(|T_C|).$$
For each face $F\in\fset_S$ such that $d(F)>30$, let $L_1,\ldots, L_{d(F)/3}$ be tight concentric cycles \explain around $F$, and let $E_F$ be the set of edges in these cycles. On one hand, it is not hard to see that, for every pair $F, F'$ of faces in $\fset_S$, the edge sets $E_F$ and $E_{F'}$ are disjoint. Therefore, $\sum_{F\in \fset_S}\cro_{\phi}(E_F)\le O(\cro_\phi(S))=O(\cro_\phi(C))$.
On the other hand, from Corollary~\ref{cor:local_crossing}, 
$\cro_{\phi}(E_F)= \Omega(d(F))$. Combined together, we have
\[\sum_{F\in \fset, d(F)>30}|\tilde{E}_i(F)|\le \sum_{F\in \fset, d(F)>30}d(F)=O(\cro_{\phi}(C)).\]
From Observation~\ref{obs:number_of_iterations}, $|E_C|=\sum_{1\le i\le \log n}|\tilde{E}_i|=O(\log n\cdot (|T_C|+\cro_{\phi}(C)))$. This finishes the proof of Proposition~\ref{pro:C_share}.
\end{proof}

Since the clusters in $\cset$ are mutually vertex-disjoint, we have $\sum_{C\in \cset}\cro_{\phi}(C)=O(\cro(\phi))$. Recall that $\sum_{C\in \cset}|T_C|=O(|E'|)$. As a result,
$\sum_{C\in \cset}|E_C|=O(\log n\cdot(|E'|+\cro(\phi)))$.

For each $C\in\cset$, we denote $C'=C\setminus \hat{E}$.
So far, we have computed a set $\hat{E}$ of edges (and a subset $T\subseteq V(H)$ accordingly), such that, for each component $C'$ of $H\setminus \hat{E}$, in the planar drawing $\psi_{C'}$, there is no path consisting of only edges of $\hat{E}$ that connects two vertices from $T\cap V(C)$ that do not lie on the same face of $\psi_{C'}$. However, we are not yet guaranteed that, for each $C'$, $T\cap V(C')$ is $(1/\poly\log n)$-well-linked in $C'$. Therefore, we still need to perform, for each $C'$, another well-linked decomposition in $C'$ with respect to $T\cap V(C')$ using Lemma~\ref{lem:well_linked-decomposition}. We add into $\hat{E}$ all inter-cluster edges, update $T$ accordingly, and denote by $\cset''=\set{C''_1,C''_2\ldots,C''_t}$ the set of clusters we get. It suffices to show that each $C''\in\cset''$ contains no bad terminals. {\color{red}TODO~}

{\color{red}Comment: we are not yet guaranteed that each connected component is $3$-connected.}





==> leftover.tex <==
From now on we will only focus on group $\uset_1$. We denote $Q^1_L,Q^1_R,Q^1$ by $Q_L,Q_R,Q$, respectively, and we denote $\qset^1$ by $\qset^*$.
We also denote the sets $Z^1_1,Z^1_2$ of common and uncommon vertices for group $\uset^1$ by $Z_1$ and $Z_2$, respectively. To summarize, the facts that we will use in Step 3 are that: if event $\event$ does not happen, then the total number of interfering edges (edges whose image intersects the interior of the region $R^*$ associated with group $\uset^1$) that are non-difficult edges is $|\eint\setminus \hat E(G'')|\leq \chi^{1-7\eps}$, and the total number of edges that are incident to the vertices of $Z_2$ (the non-common vertices for $\uset_1$) is bounded by $\chi^{1-4\eps}$.


==> proof_of_find_confluent_paths.tex <==
\subsection{Proof of Lemma~\ref{lem:find_confluent_paths}}
\label{subsec:proof_of_find_confluent_paths}

In this section we provide the proof of Lemma~\ref{lem:find_confluent_paths}.
%Let $G$ be a graph. Given a set $\pset$ of paths in $G$ and a number $\beta>0$, we define the \emph{congestion} $c(\pset)$ of the set $\pset$ of paths to be the maximum number of paths that contain a same edge, namely $c(\pset)=\max_{e\in G}\set{c_{\pset}(e)}$.

%We use the following lemmas.

The following lemma is from~\cite{chuzhoy2011algorithm}. 
%(Claim D.11 in~\cite{chuzhoy2011algorithm}). We note that the claim in~\cite{chuzhoy2011algorithm} is somewhat weaker. In particular, the confluency of the path set is not guaranteed. But the proof in~\cite{chuzhoy2011algorithm} immediately implies the stronger result that we state below.
\begin{lemma}
\label{lem:confluent_paths_in_grid}
Let $H$ be a $k\times k$ grid, where $k$ is a power of $2$, and let $S$ be the set of vertices in the last row of $G$. Then there is a distribution $\dset$ on pairs $(u^*,\qset)$, where $u^*\in V(H)$, and $\qset$ is a collection of %{\bf confluent}
paths connecting every vertex in $S$ to $u^*$, such that for each edge $e\in E(H)$, $\mathbb{E}_{(u^*,\qset)\in \dset}[c^2_{\qset}(e)]=O(\log k)$.
\end{lemma}
\begin{corollary}
\label{cor:confluent_paths_in_grid}
There is an efficient deterministic algorithm, that, given (i) a $k\times k$ grid $R$; and (ii) for each edge $e$ of the grid, an integer $w(e)\ge 0$, finds a vertex $u^*$ and a set $\qset$ of paths connecting every vertex in $S$ to $u^*$, such that
$\sum_{e\in R}w(e)\cdot c^2_{\qset}(e)=O(\log k\cdot \sum_{e\in R}w(e)).$
\end{corollary}

The following lemma is implicit in~\cite{chekuri2004edge}.

\begin{lemma}\label{lem:route_to_grid}
There exists an efficient algorithm, that, given a planar graph $G$ and a set $T$ of $r$ vertices that is $\alpha$-well-linked in $G$ for some $0<\alpha<1$, finds an $\Omega(\alpha r)\times\Omega(\alpha r)$ grid in $G$, such that, there are $\Omega(\alpha r)$ edge-disjoint paths, each connecting a distinct vertex of $T$ to a distinct vertex of the last row of the grid.
\end{lemma}
\znote{Strictly speaking, in~\cite{chekuri2004edge}, they can find a ``grid minor'' rather than a grid.}

We now begin to prove Lemma~\ref{lem:find_confluent_paths}. We will construct three sets $\qset_1, \qset_2, \qset_3$ of paths in $G$, and then properly concatenate the paths in $\qset_1, \qset_2, \qset_3$ to obtain the final set $\qset$ of paths.

First, from Lemma~\ref{lem:route_to_grid}, we can efficiently find an $\Omega(\alpha r)\times\Omega(\alpha r)$ grid $R$ in $G$. Denote by $I$ the set of vertices of the last row of $R$. From Lemma~\ref{lem:route_to_grid}, we can also efficiently find a set $\qset_1$ of $\Omega(\alpha r)$ edge-disjoint paths in $G$, each connecting a distinct vertex of $S$ to a distinct vertex of $I$. For each $v\in I$ we denote the path in $\qset_1$ with one endpoint being $v$ by $Q^1_v$.
 
Let $S_1\subseteq S$ be the set of endpoints in $S$ of paths in $\qset_1$, so $|S_1|=|I|$ and therefore $|S_1|=\Omega(\alpha r)$. We arbitrarily partition the set $S\setminus S_1$ into groups $S_2,\ldots,S_t$ such that $|S_1|=|S_2|=\cdots=|S_{t-1}|\ge |S_t|$, so $t=O(1/\alpha)$. Since the set $S$ of vertices is $\alpha$-well-linked in $G$, for each $2\le i\le t$, there exists a set $\pset_i$ of paths in $G$, each connecting a distinct vertex of $S_i$ to a distinct vertex of $S_1$, such that $c(\pset_i)=O(1/\alpha)$. Additionally, let the set $\pset_1$ contain, for each vertex $v\in S$, a single-node path of $v$. Denote $\qset_2=\bigcup_{1\le i\le t}\pset_i$. So the set $\qset_2$ contains, for each vertex $v\in S$, a path connecting $v$ to a vertex in $S_1$, such that each vertex $u\in S_1$ serves as the endpoint of at most $O(1/\alpha)$ paths in $\qset_2$, and $c(\qset_2)=O(1/\alpha)$. For each path $Q\in \qset_2$, let $u(Q)\in S_1$ be the endpoint of $Q$ in $S_1$.

Then, from Corollary~\ref{cor:confluent_paths_in_grid}, in the grid $R$, we can efficiently find a vertex $u^*$ and a set $\qset_3$ of $|I|$ paths, each connecting a distinct vertex of $I$ to $u^*$, such that
$\sum_{e\in R}w(e)\cdot c^2_{\qset_3}(e)=O(\log k\cdot \sum_{e\in R}w(e)).$
%For each $v\in I$ we denote the path in $\qset_3$ with one endpoint being $v$ by $Q^3_v$. 

We now show how to concatenate the paths in $\qset_1, \qset_2, \qset_3$ to obtain the final set $\qset$ of paths. 
We let the set $\qset$ contains, for each path $Q\in \qset_2$, a path formed by the concatenation of (i) the path $Q\in \qset_2$; (ii) the path $Q^1_{u(Q)}\in \qset_1$, and (iii) the path in $\qset_3$ that connects the endpoint of $Q^1_{u(Q)}$ in $I$ to $u^*$. Therefore, the set $\qset$ contains, for each $v\in S$, a path that connects $v$ to $u^*$. 

On the other hand, from the definition of $\qset$, and the property that each vertex $u\in S_1$ serves as the endpoint of at most $O(\alpha)$ paths in $\qset_2$, we know that each path in $\qset_1$ serves as the subpath of at most $O(\alpha)$ paths in $\qset$, and the same holds for $\pset_3$.
Therefore, for each edge $e\in G$, $$c_\qset(e)=O(1/\alpha)\cdot c_{\qset_1}(e)+c_{\qset_2}(e)+O(1/\alpha)\cdot c_{\qset_3}(e)=O(1/\alpha)+O(1/\alpha)\cdot c_{\qset_3}(e).$$
We then have
\begin{equation}
\begin{split}
\sum_{e\in E(G)}w(e)\cdot c^2_{\qset}(e)= 
&\text{ }O\left(\sum_{e\in E(G)}w(e)\cdot \left(\frac{1+c_{\qset_3}(e)}{\alpha}\right)^2\right)\\
= &\text{ } O\left(\sum_{e\in E(G)}w(e)\cdot \left(\frac{1+2\cdot c_{\qset_3}(e)+c^2_{\qset_3}(e)}{\alpha^2}\right)\right)\\
\le &\text{ } O\left(\frac{1}{\alpha^2}\cdot\sum_{e\in E(G)}w(e)+\frac{3}{\alpha^2}\sum_{e\in E(G)}w(e)\cdot c^2_{\qset_3}(e)\right)\\
\le &\text{ } O\left(\frac{\log n}{\alpha^2}\cdot\sum_{e\in E(G)}w(e)\right).
\end{split}
\end{equation}
This completes the proof of Lemma~\ref{lem:find_confluent_paths}.








==> side.tex <==
%\section{Proof of Theorem~\ref{thm:ideal_drawing}}











\subsection{Rest of the proof -- needs to be incorporated into the previous parts of this section and broken into smaller pieces. I have commented out parts that were shown/defined already.}

\iffalse
\mynote{We need to remove the assumption that $G$ is 3-connected. Some of the notation below was defined already (as bridges). Also, in the definition of canonical drawing we need to remove the bit where the edges of $C$ don't participate in any crossings, because this will not happen in type-1 clusters. I would say though that the drawing of $C$ is the same as the drawing that we have defined before for both type-1 nd type-2 clusters, and hence planar, and that each bridge is drawn in the face on whose boundary its legs sit. I suggest to make a separate subsection that talks about these canonical drawings to make the proof more readable. It should probably appear after Sec 7.1.}

In this section we provide the proof of Theorem~\ref{thm:ideal_drawing}.
\znote{For now we are assuming that $G$ is 3-connected, and each connected component of $G\setminus E''$ is 2-connected.}

We first formally define what is a \emph{canonical} drawing. For this we need some notations. 
Given a graph $G$ and an \ok\text{ }edge-planarizing set $E''\subseteq E(G)$, let $C$ be a connected component of $G\setminus E''$. Recall that $\rho_C$ is the unique planar drawing of $C$, therefore, $\fset_C\subseteq \fset(\rho_C)$. \znote{$\fset_C$ is the set of bad faces in C, this definition needs to be coordinated with the ``ideal partition'' section. here we need the property that the faces are node-disjoint}
Let $\wset$ be the set of all connected components of $G\setminus C$.
For a face $F\in \fset_C$, and a component $W\in \wset$, we say that the component $W$ \emph{touches} the face $F$ iff there is an edge in $E''$ connecting a vertex of $W$ to a vertex of $F$. Let $\wset_F\subseteq \wset$ be the subset of components that touch the face $F$. Since $E''$ is acceptable, for distinct faces $F,F'\in \fset_C$, $\wset_F\cap \wset_{F'}=\emptyset$. Since $G$ is connected, $\set{\wset_{F}}_{F\in \fset_C}$ is a partition of $\wset$.
For each $F\in\fset_C$, the subgraph $G_{C,F}$ of $G$ is defined to be the union of (i) the cycle graph $F$; (ii) the edges in $E''$ that connect a pair of vertices of $F$; (iii) the components in $\wset_F$; and (iv) the edges in $E''$ that connect a vertex of $F$ to a vertex of some component in $\wset_{F}$. 
Intuitively, the subgraph $G_{C,F}$ is the cluster of $G$ that is connected to vertices of $V(F)$ after we delete the edges of $C$ from $G$. Denote $\gset_{C}=\set{G_{C,F}}_{F\in \fset_C}$. Since the vertex sets $\set{V(F)}_{F\in \fset_C}$ are mutually disjoint, the following observation is immediate from the definition.

\begin{observation}
\label{obs:separation_configuration}
The following properties hold for subgraphs in $\gset_{C}$:
\begin{enumerate}
\item each vertex of $V(G)\setminus V(C)$ belongs to exactly one subgraph in $\gset_{C}$;
\item each edge of $E(G)\setminus E(C)$ belongs to exactly one subgraph in $\gset_{C}$; and
\item each connected component $C'$ of $G\setminus E''$ ($C'\ne C$) is entirely contained in exactly one subgraph in $\gset_{C}$.
\end{enumerate}
\end{observation}

\begin{definition}[Canonical Drawing]
Given a graph $G=(V,E)$ and an \ok\text{ }edge-planarizing set $E''\subseteq E$, let $C$ be a connected component of $G\setminus E''$. We say that a drawing $\phi$ of $G$ in the plane is \emph{$E''$-canonical with respect to $C$}, if 
\begin{enumerate}
\item the drawing of $C$ induced by $\phi$ is $\rho_C$ (namely $\phi(C)=\rho_C$);
\item the edges of $C$ do not participate in any crossings in $\phi$;
\item for each face $F$ of $\rho_C$, the image of $G_{C,F}$ is entirely contained in the disc $D(\rho_C,F)$.
\end{enumerate}
If the drawing $\phi$ of $G$ is $E''$-canonical with respect to each connected component $C$ of $G\setminus E''$, then we say that $\phi$ is \emph{$E''$-canonical}.
\end{definition}

\begin{observation}\label{obs:canonical_is_in}
If a drawing $\phi$ is $E''$-canonical, then $\phi\in \Phi_{E''}(G)$.
\end{observation}
\begin{proof}
Since for each connected component $C$ of $G\setminus E''$, $\phi(C)$ is the unique planar drawing of $C$, and the edges of $\phi(C)$ do not participate in any crossing of $\phi$, we know that $\phi(G\setminus E'')$ is planar. From the definition of $\Phi_{E''}(G)$, $\phi\in \Phi_{E''}(G)$.
\end{proof}


Now we begin to prove Theorem~\ref{thm:ideal_drawing}.
We denote our input graph by $\tG$, and denote the input edge-planarizing set by $\tE'$. We denote by $\cset=\set{C_1,\ldots,C_t}$ the set of connected components of $\tG\setminus \tE'$. We denote by $\tphi$ the optimal drawing of $\tG$ in the plane, namely $\tphi=\arg\min_{\phi}\set{\cro_{\phi}(G)}$.

We start with the optimal drawing $\tphi$, and denote $\phi^0=\tphi$. We will gradually modify the drawing $\tphi$ so that at the end it becomes a canonical drawing.
Specifically, we will construct a sequence of drawings $\phi^1,\ldots,\phi^t$ of $\tG$ in the plane, such that, for each $1\le i\le t$, $\phi^i$ is canonical with respect to connected components $C_1,\ldots,C_i$. At the end, we obtain a drawing $\phi^t$ of $\tG$ that is canonical with respect to all connected components in $\cset$, and is therefore a canonical drawing by definition. We will then show that $\cro(\phi^t)=\tilde{O}(\cro(\tphi))$.

\fi



We now describe the way to construct, for each $1\le i\le t$, the drawing $\phi^i$, assuming that we are given the drawing $\phi^{i-1}$.

For brevity we rename $C_i$ by $C$.
We denote by $T\subseteq V(C)$ the set of vertices of $C$ that are incident to some edge in $\tE'$, and denote by $\fset$ the face cover of $T$. \znote{Define}
For each face $F\in \fset$,
let $\tilde G_{C,F}$ be the graph obtained from $G_{C,F}$ by replacing each edge $e=(v,v')$ that connects a pair of vertices of $F$ by a new vertex $y_e$ and two new edges $(v,y_e)$ and $(v',y_e)$.
We denote by $\tilde E_{C,F}$ the set of new edges.
We denote $\widetilde\out(C,F)=\tilde E_{C,F}\cup(\out_G(C)\cap E(\tilde G_{C,F}))$, namely the set of edges of $\tilde G_{C,F}$ with exactly one endpoint in $V(F)$.
We define $\widetilde\out(C)=\bigcup_{F\in\fset_C}\widetilde\out(C,F)$, so $\widetilde\out(C)=\out_G(C)\cup(\bigcup_{F\in \fset_C}\tilde E_{C,F})$.

We define the weights of the edges in $C$ as follows. We start by setting the
weight of every edge of $C$ to be $\cro_{\tphi}(e)$. Then, for every edge in $\ir_E(\tphi(C),\rho_{C})$, we increase its weight by $1$, and for every vertex in $\ir_V(\tphi(C),\rho_{C})$, we increase the weight of each of its
adjacent edges in $C$ by $1$. This completes defining the weights on the edges of $C$.
Since the maximum degree of a vertex in $G$ is $O(1)$, from Lemma~\ref{lem:irregular_bounded_by_crossing},
\[\sum_{e\in E(C)}w(e)=|\ir_E(\tphi(C),\rho_{C})|+O(|\ir_V(\tphi(C),\rho_{C})|)+\sum_{e\in E(C)}\cro_{\tphi}(e,G)=O(\cro_{\tphi}(C,G)).\]
We now apply Lemma~\ref{lem:find_confluent_paths} to compute a vertex $u^*\in V(C)$ and a set $\qset$ of confluent paths in $C$, each connecting a distinct vertex of $T$ to $u^*$, such that $\sum_{e\in E(C)}w(e)\cdot c^2_{\qset}(e)= O(\log n\cdot\cro_{\tphi}(C,G)/\alpha^2)$.
For each $e=(u_e,v_e)\in \widetilde\out(C)$ where $v_e$ is its endpoint in $C$ (so $v_e\in T$), we split the edge $e$ by creating a new node $x_e$ and replacing the edge $(u_e,v_e)$ by the new edges $(u_e,x_e)$ and $(v_e,x_e)$. We denote $X=\set{x_e\mid e\in \widetilde\out(C)}$, $\out'(C)=\set{(x_e,v_e)\mid e\in \widetilde\out(C)}$, and $\out'(C,F)=\set{(x_e,v_e)\mid e\in \widetilde\out(C,F)}$.
We define another set of paths $\qset'$ as follows. For each edge $e\in \widetilde\out(C)$, there is a path $Q_e$ in $\qset'$, where $Q_e$ is defined to be the concatenation of the edge $(x_e,v_e)$ and the path $Q$ in $\qset$ that connects $v_e$ to $u^*$. Therefore, the set $\qset'$ is a set of paths connecting vertices of $X$ to $u^*$. Since the maximum degree of the graph $G$ is $O(1)$, we are still guaranteed that
$\sum_{e\in E(C)}w(e)\cdot c^2_{\qset'}(e)= O(\log n\cdot\cro_{\tphi}(C,G)/\alpha^2).$

It is clear that the planar drawing $\rho_{C}$ of $C$ can be extended to a planar drawing $\psi$ of $C\cup \out'(C)$ such that, for each face $F\in\fset$, all edges in $\out'(C,F)$ are drawn in the face $F$ of $\rho_{C}$, where for each $v\in T$, the circular ordering of all edges in $\out'(C)$ that are incident to $v$ is chosen arbitrarily.
In particular, the drawing $\psi$ contains the image of all paths in $\qset'$.

Now we apply Lemma~\ref{lem:uncrossing} to $\qset'$ and $\psi$ and obtain another set $\pset$ of paths connecting vertices of $X$ to $u^*$, such that $\pset$ is non-interfering with respect to $\psi$, and, for each edge $e\in G$, $c_{\pset}(e)\le c_{\qset'}(e)$.
For each $e\in \widetilde\out(C)$, denote by $P_e$ the path in $\pset$ that connects $x_e$ to $u^*$.
Note that, we also obtain a non-interfering representation (a set of curves) of $\pset$ with respect to $\psi$. We denote the set of curves by $\Gamma=\set{\gamma_P}_{P\in \pset}$. According to the curves in $\Gamma$, for each $v\in C$, we obtain a circular ordering $\oset(v)$ in which the paths in $\pset$ containing $v$ enter $v$, and for each $e\in C$, we also obtain a circular ordering $\oset(e)$ in which the paths in $\pset$ containing $e$ traverse along $e$ (see Figure~\ref{fig:circular_ordering}). For each face $F\in \fset$, let $\pset_{F}\subseteq \pset$ be the subset of paths in $\pset$ whose endpoints in $C$ lie in $F$. Then the drawing $\psi$ also induces a circular ordering $\oset(F)$ in which the paths in $\pset_F$ touches the boundary of $F$.

\begin{figure}[h]
\centering
\includegraphics[scale=0.35]{circular_ordering.jpg}
\caption{An illustration of circular orderings. The circular ordering of $v$ is $\oset(v)=(P_1,P_2, P_3, P_4)$. The circular ordering of edge $(v,v'')$ is $\oset((v,v''))=(P_2,P_3)$. $\oset((v,v'))=(P_1,P_2, P_3, P_4)$. \label{fig:circular_ordering}}
\end{figure}

\textbf{Routing along Non-interfering Paths.}
We are now ready to transform the drawing $\phi^{i-1}$ into $\phi^i$. For brevity we rename $\phi^{i-1}$ by $\phi$.
%We denote by $D_{u^*}$ the small disc around the image $\phi(u^*)$ of the vertex $u^*$, whose boundary intersects with only the image of edges that are incident to $u^*$ in $\phi$.
The transformation consists of the following six steps. 

\textbf{Step 1.} Erase the drawing $\phi(C)$ of $C$ from $\phi$, but keep the image of the paths of $\qset$, namely the drawings $\set{\phi(Q)}_{Q\in \qset}$. 

\textbf{Step 2.} For each $e=(u_e,v_e)\in \widetilde\out(C)$, since we have split it into two edges $(u_e,x_e)$ and $(x_e,v_e)$, we can identify an arbitrary point (but not the endpoints) of the curve $\phi(e)$ as $\phi(x_e)$, the image of the vertex $x_e$, and then subdivide $\phi(e)$ into two curves representing $\phi((u_e,x_e))$ and $\phi((x_e,v_e))$ respectively.
Recall that there is a path $P_e$ in $\pset$ connecting $x_e$ to $u^*$. We draw a curve $\gamma'_{P_e}$ that connects $\phi(x_e)$ to $\phi(u^*)$ and lies entirely in the thin strip $S_{P_e}$ around the image of $P_e$.
We replace the drawing $\phi(e)$ of $e$ by the concatenation of the curve $\phi((u_e,x_e))$ and the curve $\gamma'_{P_e}$. 
Denote $\Gamma'=\set{\gamma'_{P_e}\mid e\in \widetilde\out(C)}$.
Note that, for now, for distinct $e,e'\in  \widetilde\out(C)$, the curves $\gamma'_{P_e},\gamma'_{P_{e'}}$ in $\Gamma'$ may intersect in some thin strip $S_{\tilde{e}}$ where $\tilde e$ is an edge of $C$ that is shared by paths $P_e$ and $P_{e'}$. We will arrange the curves in each such thin strip in the last step.

\textbf{Step 3.} Draw a small disc $D_{u^*}$ around the image $\phi(u^*)$ of the vertex $u^*$, whose boundary intersects (once) with only the image of each edge that is incident to $u^*$ in $\phi$. Place the drawing $\rho_C$ of $C$ inside $D_{u^*}$ %so that the vertices of the outer face of $\rho_{C}$ appear on the boundary of the disc $D$. 
and erase part of the curves in $\Gamma'$ that lie in $D_{u^*}$.
For each $e\in \widetilde\out(C)$, let $\tau_e$ be the intersection of the curve $\gamma'_{P_e}$ and the boundary of $D_{u^*}$, and we denote by $\gamma''_{P_e}$ the sub-curve of $\gamma'_{P_e}$ between $\phi(u_e)$ and $\tau_e$.

\textbf{Step 4.} For each $e\in \widetilde\out(C)$, we connect the point $\tau_e$ to the image of $v_e$ in $D_{u^*}$ by a curve $\zeta_e$ inside $D_{u^*}$, so that, if $v_e$ lies on the outer face of $\rho_C$, then the curve $\zeta_e$ does not intersect with $\rho_C$ except at its endpoint in $C$. We then denote by $\tilde \gamma_{P_e}$ the concatenation of the curves $\zeta_e$ and $\gamma''_{P_e}$. We then re-identify $\tilde \gamma_{P_e}$ as the drawing of $e$.
Note that, for now it is possible that curves $\set{\zeta_e}$ may intersect arbitrarily with each other. We will deal with this issue in the last step so that the number of crossings caused by them is properly bounded.

\textbf{Step 5.} \znote{To modify} For each face $F\in \fset$ that is not the outer face of $\rho_{C}$, we flip the induced drawing $\phi(G_{C,F})$ into the face $F$ of $\rho_{C}$.

Let $\tilde{\phi}$ be the drawing that we obtain after the above five steps are applied to the drawing $\phi$.
Please see Figure~\ref{fig:layout} and Figure~\ref{fig:transformation} for an illustration of the above five steps.

\begin{figure}
\centering
\subfigure[The planar drawing of $C\cup \out'(C)$. $T=\set{a,b,c,d}$. Edges of $\out'(C)$ are shown in red and green.]{\scalebox{0.25}{\includegraphics{layout_1.jpg}}}
\hspace{1cm}
\subfigure[The set $\qset$ of paths connecting distinct vertices of $T$ to $u^*$.]{
\scalebox{0.25}{\includegraphics{layout_2.jpg}}}
\caption{Layout of $C$.\label{fig:layout}}
%\end{figure}
%\begin{figure}
\centering
\subfigure[The drawing $\phi$ of $G$. The drawing $\phi(C)$ is shown in blue. The drawing $\phi(G_{C,F_1})$ is shown in green and the drawing $\phi(G_{C,F_2})$ is shown in red.]{\scalebox{0.25}{\includegraphics{step_0.jpg}}}
\hspace{1cm}
\subfigure[Step 1: Erase $\phi(C)$, but keep the image of paths in $\qset$, that are shown in bold green and red curves.]{
	\scalebox{0.25}{\includegraphics{step_1.jpg}}}
\subfigure[Step 2: Redraw the edges of $\widetilde\out(C)$ using the image of paths of $\pset$ in $\phi$. The new drawings are shown in dash red curves and dash blue curves.]{\scalebox{0.25}{\includegraphics{step_2.jpg}}}
\hspace{1cm}
\subfigure[Step 3: Draw a small disc $D_{u^*}$ around the image of $u^*$, and then place the drawing $\rho_C$ inside the disc.]{
	\scalebox{0.25}{\includegraphics{step_3.jpg}}}
\subfigure[Step 4: Rearrange the drawings of the edges of $\widetilde\out(C)$ by new curves in $D_{u^*}$.]{\scalebox{0.25}{\includegraphics{step_4.jpg}}}
\hspace{1cm}
\subfigure[Step 5: ``Flip'' the drawing of $G_{C,F_2}$ induced by $\phi$ into the face $F_2$ of $\rho_C$.]{
	\scalebox{0.25}{\includegraphics{step_5.jpg}}}
\caption{An illustration of the steps in the transformation from $\phi$ to $\tilde\phi$.\label{fig:transformation}}
\end{figure}

\textbf{Step 6.} \znote{To modify} In the last step, intuitively we would like to ensure that the images of the paths of $\pset$ hit the boundary of the disc $D_{u^*}$ in the right order. Specifically, we want to ensure that, for each face $F\in \fset$, the circular ordering in which the images of paths of $\pset_F$ touch the boundary of $F$ is $\oset(F)$. We call this step \emph{path adjusting}. In this step view the paths in $\pset$ as being directed towards the vertex $u^*$.

From Lemma~\ref{lem:uncrossing}, we can compute an ordering of the vertices of $C$, such that, for each pair of $v,v'\in C$, if some path $P_e\in \pset$ visits $v$ before visits $v'$, then $v$ must appear before $v'$ in this ordering. Let $v_1,v_2,\ldots,v_r$ be the vertices of $C$ according to the ordering.
For an edge $(v_i,v_j)\in E(\pset)$ such that $i<j$, we say that the edge $(v_i,v_j)$ is an \emph{out-edge} of $v_i$, and an \emph{in-edge} of $v_j$.
We process the vertices of $C$ one by one according to the ordering, and adjust the in-edges of each of them.
Specifically, consider an iteration when the vertex $v=v_j$ is processed. Let $e_1,\ldots,e_z$ be the set of in-edges of $v$. For each $1\leq z'\leq z$, let $\pset_{z'}\subseteq \pset$ be the set of paths containing the edge $e_{z'}$, and let $\pset(v)=\bigcup_{z'=1}^z\pset_{z'}$ be the set of all paths containing $v$.
If, for some $1\leq z'\leq z$, the paths in $\pset_{z'}$ traverse the edge $e_{z'}$ within the thin strip $S_{e_z}$ in an order different from $\oset(e_{z'})$, then we re-adjust their ordering by letting the curves of each bad pair of paths in $P_{z'}$ -- pairs of paths whose image traverse the edge $e$ in a relatively incorrect order -- cross once (see Figure~\ref{fig:ordering_adj}). If, at the end, the paths in $\pset(v)$ enter the small disc $D_v$ around the image of $v$ in an order different from $\oset(v)$, then we re-adjust their ordering similarly.
It is clear that once we process all vertices of $C$ this way, the paths will eventually enter the disc $D_{u^*}$ in the right order in Step 2. 
We let $\phi'$ be the drawing we obtain after this path adjusting step, and set $\phi^{i}=\phi'$.
This completes the description of the process of transforming the drawing $\phi^{i-1}$ into $\phi^{i}$.

\begin{figure}[h]
\centering
\subfigure[]{\scalebox{0.25}{\includegraphics{order_adj_edge.jpg}}}
\hspace{1cm}
\subfigure[]{
		\scalebox{0.25}{\includegraphics{order_adj_vertex.jpg}}}
\caption{Adjusting the circular ordering in a thin strip or a small disc.\label{fig:ordering_adj}}
\end{figure}

We now proceed to show that the drawing $\phi^t$ that we obtain from the algorithm above is $E''$-canonical, and $\cro(\phi^t)=\tilde O(\cro(\tphi))$. We begin with the following observation.

\begin{observation}
\label{obs:untouched_intra-cluster-edge_uninfluenced}
If an edge of $E(C')$ for some $C'\in \cset, C'\ne C$ does not participate in any crossing in $\phi$, then it will not participate in any crossing in $\tilde{\phi}$ and $\phi'$.
\end{observation}
\begin{proof}
Recall that $\tilde{\phi}$ is the drawing that we obtain after the first five steps are applied to the drawing $\phi$.
The only possibility of a new crossing being created in $\tilde{\phi}$ over the first five steps is when we re-draw the an edge $e\in\out(C)$ in the second step, we let its image be the concatenation of the curves $\phi((u_e,x_e))$ and $\gamma'_{P_e}$. 
Note that, if an edge of $E(C')$ for some $C'\in \cset$ is crossed by this curve, then it has to be crossed by either the curve $\phi((u_e,x_e))$ or the curve $\gamma'_{P_e}$. 
In either case, it is crossed in $\phi$.
On the other hand, it is clear that the path adjusting step only creates crossings between edge in $\tE'$ and does not create or eliminate other crossings in $\tilde{\phi}$. As a result, any edge of $E(C')$ for some $C'\in \cset, C'\ne C$ that is crossed in $\phi'$ or $\tilde{\phi}$ has to be also crossed in $\phi$.
\end{proof}
\begin{claim}
\label{cl:canonical}
For each $1\le i\le t$, the drawing $\phi^{i}$ of $G$ is $E''$-canonical with respect to $C_1,\ldots,C_i$.
\end{claim}
\begin{proof}
We prove the claim by induction on $i$. The base case is when $i=1$. From the third step of the algorithm, it is clear the induced drawing of $C_1$ is $\phi^1(C_1)=\rho_{C_1}$, which is planar. Additionally, from the fifth step of algorithm, the image of every subgraph $G_{C_1,F}$ of $\gset_{C_1}$ is entirely contained in the face $F$ of $\rho_{C_1}$, and is therefore contained in the disc $D(\rho_{C_1},F)$. Therefore, it is also true that the edges of $C_1$ do not participate in any crossings in $\phi^{1}$.

Assume the claim is true for $1,\ldots,i-1$, now we consider the drawing $\phi^i$. We first show that every edge in $\bigcup_{1\le j\le i}E(C_j)$ does not participate in any crossings in $\phi^{i}$. Similarly as the base case, it can be derived that the edges of $C_i$ do not participate in any crossings in $\phi^{i}$.
From the induction hypothesis, the edges in $\bigcup_{1\le j\le i-1}E(C_j)$ do not participate in any crossings in $\phi^{i-1}$. From Observation~\ref{obs:untouched_intra-cluster-edge_uninfluenced}, they do not participate in any crossings in $\phi^{i}$, either. Therefore, every edge in $\bigcup_{1\le j\le i}E(C_j)$ does not participate in any crossings in $\phi^{i}$.

We then show that, for each $1\le j\le i$, the induced drawing of $\phi^i$ on $C_j$ is $\rho_{C_j}$. It is clear from the algorithm that the induced drawing of $C_i$ is $\rho_{C_i}$. From the induction hypothesis, for each $1\le j\le i-1$, the induced drawing of $C_j$ in $\phi^{i-1}$ is $\rho_{C_j}$. In the transformation from $\phi^{i-1}$ to $\phi^{i}$, for each $1\le j\le i-1$, either $C_j$ is entirely contained in some subgraph $G_{C_i,F}$ (where $F$ is not the outer face of $\rho_C$) and is flipped into the face $F$ of $\rho_{C_i}$, or we do nothing to the induced drawing of $C_j$ in $\phi^{i-1}$. Either way, the induced drawing of $C_j$ in $\phi^{i}$ is still $\rho_{C_j}$.

Finally we show that, for each $1\le j\le i$ and each face $F$ of $\rho_{C_j}$, the induced drawing of the subgraph $G_{C_j,F}$ in $\phi^i$ is entirely contained in the disc $D(\rho_{C_j},F)$.
It is clear from the algorithm that the induced drawing of $C_i$ is $\rho_{C_i}$, and, for each face $F$ of $\rho_{C_j}$, the subgraph $G_{C_i,F}$ is drawn in the disc $D(\rho_{C_i},F)$.
From the induction hypothesis, for each $1\le j\le i-1$ and for each face $F$ of $\rho_{C_j}$, and the induced drawing of the subgraph $G_{C_j,F}$ in $\phi^{i-1}$ is entirely contained in the disc $D(\rho_{C_j},F)$. In the transformation from $\phi^{i-1}$ to $\phi^{i}$, each $1\le j\le i-1$ and each face $F$ of $\rho_{C_j}$, we consider the following cases.

\textbf{Case 1.} Both $C_j$ and $G_{C_j,F}$ are entirely contained in some subgraph $G_{C_i,F'}$, and is flipped into the face $F'$ of $\rho_{C_i}$ if $F'$ is not the outer face of $\rho_{C_i}$. In this case, it is clear that the subgraph $G_{C_j,F}$ is still drawn in $D(\rho_{C_j},F)$.

\textbf{Case 2.} $G_{C_j,F}$ contains $C_i$, so $C_i$ is entirely contained in the face $F$ of $\rho_{C_j}$ in $\phi^{i-1}$. Let $F'$ be the face of $\rho_{C_i}$ that contains $C_j$, then the subgraph $C_j\cup (G_{C_j,F}\setminus C_i)$ is flipped into the face $F'$ of $\rho_{C_i}$. It is clear that $C_i$, $G_{C_j,F}\setminus C_i$ and edges of $E(C_i,G_{C_j,F}\setminus C_i)$ is still drawn in $D(\rho_{C_j},F)$ in $\phi^{i}$, so $G_{C_j,F}$ is still drawn in $D(\rho_{C_j},F)$ in $\phi^{i}$.

This completes the induction, and therefore also completes the proof of claim~\ref{cl:canonical}.
\end{proof}

As a corollary, the final drawing $\phi^t$ is $E''$-canonical with respect to $C_1,\ldots,C_t$, and is therefore $E''$-canonical by definition.
For completing the proof of Theorem~\ref{thm:ideal_drawing}, it remains to bound the number of crossings in $\phi^t$. We first prove the following claims.

\begin{claim}
\label{cl:out_self_crossings}
For all $1\le i\le j\le t$, $\cro_{\phi^j}(\out(C_i))\le \sum_{e\in C_i}w(e)\cdot c^2_{\pset}(e)$.
\end{claim}
\begin{proof}
	\znote{To Modify}
The number of crossings we will introduce by doing so is at most $|\pset(v)|^2$. The main idea is that this re-adjustment is only needed when one of the incident edges $e_{z'}$ is an irregular edge (and then we pay $(c_{\pset}(e_{z'}))^2$; but then the weight of $e_{z'}$ is at least $1$), or vertex $v$ is an irregular edge. In the latter case, if $e$ is the edge through which the paths in $\pset(v)$ leave $v$, then its weight is at least $1$, and the number of crossings that we introduce is at most $(c_{\pset}(e))^2$.  The number of crossings that we introduce due to re-ordering is at most 
$\sum_{e\in E(C)}w(e)c^2_{\pset}(e)=O(\log n\cdot\cro_{\tphi}(C,G)/\alpha^2)$. Put in other words, $\cro_{\phi^i}(\out(C))=O(\log n\cdot\cro_{\tphi}(C,G)/\alpha^2)$.
\end{proof}

\begin{claim}
\label{cl:out_pair_crossings}
For all $1\le i< j\le k\le t$, 
$$\cro_{\phi^k}(\out(C_i),\out(C_j))\le \sum_{e\in\pset_i,e'\in \pset_j}\indicator[e\text{ and }e' \text{ cross in }\tphi]\cdot c_{\pset_i}(e)\cdot c_{\pset_j}(e').$$
\end{claim}
\begin{proof}
	\znote{To Prove}
\end{proof}

Combine claim~\ref{cl:out_self_crossings} and claim~\ref{cl:out_pair_crossings}, we have
\begin{equation}
\begin{split}
\cro(\phi^t)= &\text{ }\cro_{\phi^t}(\tE',\tG)\\
\le &\text{ } \sum_{C\in \cset}\cro_{\phi^t}(\out(C))+\sum_{1\le i< j\le t}\cro_{\phi^t}(\out(C_i),\out(C_j))\\
\le &\text{ } \sum_{C\in \cset}\sum_{e\in C}w(e)\cdot c^2_{\pset}(e)+\sum_{e\in\pset_i,e'\in \pset_j}\indicator[e\text{ and }e' \text{ cross in }\tphi]\cdot c_{\pset_i}(e)\cdot c_{\pset_j}(e')\\
\le &\text{ } \sum_{C\in \cset}\sum_{e\in C}w(e)\cdot c^2_{\pset}(e)+
\sum_{e\in\pset_i,e'\in \pset_j}\indicator[e\text{ and }e' \text{ cross in }\tphi]\cdot \frac{c^2_{\pset_i}(e)+ c^2_{\pset_j}(e')}{2}\\
\le &\text{ } \sum_{C\in \cset}\sum_{e\in C}w(e)\cdot c^2_{\pset}(e)+
\frac{1}{2}\cdot\sum_{C\in \cset}\sum_{e\in C}\cro_{\tphi}(e)\cdot c^2_{\pset}(e)\\
\le &\text{ } O\left(\frac{\log n}{\alpha^2}\cdot \sum_{C\in \cset}\cro_{\tphi}(C,G)\right)\le O\left(\frac{\log n}{\alpha^2}\cdot \cro(\tphi)\right).
\end{split}
\end{equation}
This completes the proof of Theorem~\ref{thm:ideal_drawing}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse (Do one-component flipping in an order)
For each connected component $C\in\cset$, we denote by $\fset_C$ the face cover of $T\cap V(C)$ {\color{red} (To Define)}.
We define a graph $L$ as follows. The vertex set of $L$ is defined to be $V(L)=\set{v_{C}\mid C\in \cset}$, and the edge set of $L$ is defined to be 
$E(L)=\set{(v_C,v_{C'})\mid \exists (u,u')\in \tE', u\in C, u'\in C'}$. Since $\tG$ is connected, $L$ is also connected. Throughout the algorithm, each node of $L$ is either marked \emph{processed} or \emph{unprocessed}. Initially, all nodes are unprocessed.

While there is at least one unprocessed node in $L$, we arbitrarily pick an unprocessed node that is adjacent to some processed node in $L$. As $L$ is connected, such a node always exists (at the very beginning, there is no processed node, so we simply pick an arbitrary node). Let $v_{C}$ be the node we pick, and let $\set{v_{C_1},\ldots,v_{C_t}}$ be the set of processed nodes that $v_{C}$ is adjacent to. We use the following observation.
\begin{observation}\label{obs:same_face}
	Let $\Gamma'(C)$ be the set of vertices of $C$ that is adjacent to some vertex of $\bigcup_{1\le i\le t}V(C_i)$ in $\tG$, then in the planar drawing $\rho_C$, all the vertices of $\Gamma'(C)$ are on the same face.
\end{observation}
\begin{proof}
\end{proof}

From Observation~\ref{obs:same_face}, let $F'$ be the face of $\psi(C')$ containing the nodes that are adjacent to some cluster in $\set{C_1,\ldots,C_t}$.
We apply Lemma~\ref{lem:one_component_canonicalize} to $\phi'$ with $C'$ and $F'$, and obtain another drawing $\phi''$. We mark the node $v_{C'}$ processed. We repeat this process until all the nodes in $L$ are processed. %Let $\hat{\phi}$ be the final drawing we get.
\fi

==> temp.tex <==

%------------------------
%------------------------
%------------------------
%------------------------
Fake edge embedded into C_i

%------------------------
%------------------------
%------------------------
%------------------------

Consider now some cluster $C_i\in \cset_1$. Let $e_i=(x_i,y_i)\in A$ be the unique fake edge that is embedded into $C_i$;
in other words, if $P(e_i)\in \pset(A)$ is the path into which edge $e_i$ is embedded, then $P(e_i)\setminus\set{x_i,y_i}\subseteq C_i$.
 If no such edge exists, $e_i$ is undefined. We set $C_i'=C_i\cup \set{e_i}$, and we let $x'_i,y'_i$ be the endpoints of the path $P(e_i)\setminus \set{x_i,y_i}$.
 
  Recall that edge $e_i$ belongs to some type-2 acceptable cluster $C$, which is a connected graph. Therefore, $C$ must also contain a path $P'_i$ connecting $x_i$ to $y_i$.
 Some edges on path $P'_i$ may be fake edges that lie in $A$. However, for each such fake edge $e\in P'_i$, its embedding $P(e)\in \pset(A)$ must be disjoint from $C_i$. By replacing each fake edge $e\in P'_i$ with its embedding $P(e)\in \pset(A)$, we obtain a path $P_i\subseteq G\setminus C_i$ connecting $x_i$ to $y_i$.
 % We can extend this path using the edges $(x_i,x'_i)$ and $(y_i,y'_i)$, to obtain a path that connects $x'_i$ to $y'_i$ and is internally disjoint from $C'_i$. 
 Therefore, there must be a bridge $R_i\in \rset_{G}(C_i)$ that contains the path $P_i$, with $x'_i,y'_i\in L(R_i)$. 

==> temp2.tex <==

\subsection{Proof of Lemma \ref{lem:add_back_discarded_edges new}}\label{subsec: proof of adding back edges}

%Note that it is sufficient to prove the lemma for the special case where $|E'|=1$, as we can then add the edges of $E'$ to the drawing one-by-one. We use the following claim.
The following claim is central to the proof of the lemma.

\begin{claim}\label{claim: add one edge}
	There is an efficient algorithm, that, given an instance $(H,\Sigma)$ of the \CNwRS problem, an edge $e\in E(H)$, and a drawing $\phi$ of graph $H\setminus \set{e}$ that respects $\Sigma$, computes one of the following:
	
	\begin{itemize}
		\item either a drawing $\hat \phi$ of $H\setminus \set{e}$ that respects $\Sigma$, with $\cro(\hat \phi)<\cro(\phi)$; or
		\item a drawing $\phi'$ of $H$ that respects $\Sigma$, with $\cro(\phi')\le \cro(\phi)+|E(H)|$.
	\end{itemize} a drawing $\phi'$ of $H$ that respects $\Sigma$, such that $\cro(\phi')\le \cro(\phi)+|E'|\cdot|E(H)|$.
\end{claim}

It is now easy to complete the proof of Lemma \ref{lem:add_back_discarded_edges new} using Claim \ref{claim: add one edge}. 
We denote $E'=\set{e_1,\ldots,e_r}$. The algorithm consists of $r$ phases, where in the $i$th phase we compute a drawing $\phi_i$ of graph $(H\setminus E')\cup \set{e_1,\ldots,e_i}$ that respects the rotation system $\Sigma$. We set $\phi_0=\emptyset$. We now describe the $i$th phase. 

Recall that, at the beginning of the $i$th phase, we are given a drawing $\phi_{i-1}$ of graph $(H\setminus E')\cup \set{e_1,\ldots,e_{i-1}}$.  We iteratively apply the algorithm from Claim \ref{claim: add one edge} to the current drawing $\phi_{i-1}$. If the outcome of the algorithm is another drawing  $\hat \phi_{i-1}$ of of graph $(H\setminus E')\cup \set{e_1,\ldots,e_{i-1}}$ that respects $\Sigma$ with $\cro(\hat \phi_{i-1})<\cro(\phi_{i-1})$, then we replace $\phi_{i-1}$ with $\hat \phi_{i-1}$ and continue to the next iteration. Otherwise, we obtain the desired drawing $\phi_i$ of graph $(H\setminus E')\cup \set{e_1,\ldots,e_{i}}$ that respects $\Sigma$, with $\cro(\phi_i)\le \cro(\phi_{i-1})+|E(H)|$ (recall that $E'\subseteq E(H)$). We then return this drawing as the outcome of the $i$th phase, and continue to the next phase.

Let $\phi'=\phi_r$ be the drawing of $H$ that is obtained after the $r$th phase. Then we are guaranteed that $\phi'$ respects the rotation system $\Sigma$, and moreover, from the above discussion, $\cro(\phi')\le \cro(\phi)+|E'|\cdot|E(H)|$.
 Therefore, in order to complete  the proof of Lemma \ref{lem:add_back_discarded_edges new}, it is now enough to prove Claim \ref{claim: add one edge}.

\begin{proofof}{Claim \ref{claim: add one edge}}
Let $e=(u,v)$. We compute a curve $\gamma$ in the current drawing $\phi$ of $H\setminus\set{e}$ connecting $u$ to $v$, such that $\gamma$ intersects the drawing of $H\setminus\set{e}$ at images of edges only, does not include any crossing points of the drawing $\phi$, and, moreover, if we add the edge $e$ to the drawing $\phi$ such that the image of $\phi$ is $\gamma$, then the resulting drawing of $H$ respects the rotation system $\Sigma$. Among all curves $\gamma$ with the above properties, we choose the one that has fewest crossings with the edges of $H\setminus \set{e}$, and does not cross itself. Such a curve $\gamma$ can be computed as follows.
Let $\fset$ be the set of all faces in the drawing $\phi$ of $H\setminus\set{e}$. Let $F$ be the face that is incident to $v$, such that, if edge $e$ is added to the drawing in a manner that respects the ordering $\oset(v)$ of all edges incident to $v$, then there must be a segment of the image of $e$ that contains $v$, does not contain any crossings, and is contained in $F$. We define the face $F'$ incident to $u$ similarly. We then compute a graph that is dual to the drawing $\phi$ of $H\setminus\set{e}$, and in that graph we compute a shortest path between the two vertices that represent faces $F$ and $F'$. The resulting path then naturally defines the desired curve $\gamma$.

We now consider two cases. First, if curve $\gamma$ has at most $|E(H)|$ crossings, then we add the edge $e$ to the drawing $\phi$ so that the image of $e$ is $\gamma$, and return the resulting drawing of $H$. Clearly, this drawing has at most $\cro(\phi)+|E'|\cdot|E(H)|$ crossings, and it respects $\Sigma$. Assume now that $\gamma$ has more than $|E(H)|$ crossings. Then there is some edge $e'\in E(H)\setminus\set{e}$, that crosses $\gamma$ at least twice. Let $x,y$ be two points where $\gamma$ and $e'$ cross. We denote by $\sigma$ the segment of $\gamma$ between $x$ and $y$, and we denote by $\sigma'$ the segment of the image of $e'$ between $x$ and $y$. Let $N$ be the number of crossings in which $\sigma$ participates (excluding the points $x$ and $y$), and let $N'$ be defined similarly for $\sigma'$. Observe that $N< N'$ must hold. Indeed, if $N\geq N'$, then we can modify the curve $\gamma$ as follows. Assume that $\gamma$ is directed so that point $x$ appears before point $y$ on $\gamma$. Let $t$ be a point on $\gamma$ that appears just before point $x$ on it, and let $t'$ be a point on $\gamma$ that appears just after point $y$ on it. Let $\sigma^*$ be a curve that connects $t$ to $t'$, and follows the segment $\sigma'$. By replacing the segment of curve $\gamma$ between $t$ and $t'$ with $\sigma^*$, we obtain a new curve $\gamma'$ that has all the required properties, but has fewer crossings than $\gamma$, a contradiction. We conclude that $N<N'$ must hold.

We then modify the drawing of edge $e'$ in $\phi$, by replacing the segment $\sigma'$ with $\sigma$. This produces a new drawing $\hat \phi$ of $H\setminus\set{e}$ with $\cro(\hat \phi)<\cro(\phi)$, that respects the rotation system $\Sigma$.
\end{proofof}
